The California-Kepler Survey. X. The Radius Gap as a Function of Stellar Mass, Metallicity, and Age

In 2017, the California-Kepler Survey (CKS) published its first data release (DR1) of high-resolution optical spectra of 1305 planet hosts. Refined CKS planet radii revealed that small planets are bifurcated into two distinct populations: super-Earths (smaller than 1.5 $R_E$) and sub-Neptunes (between 2.0 and 4.0 $R_E$), with few planets in between (the "Radius Gap.") Several theoretical models of the Radius Gap predict variation with stellar mass, but testing these predictions are challenging with CKS DR1 due to its limited $M_\star$ range of 0.8-1.4 $M_\odot$. Here, we present CKS DR2 with 411 additional spectra and derived properties focusing on stars of 0.5-0.8 $M_\odot$. We found the Radius Gap follows $R_p \propto P^m$ with $m = -0.10 \pm 0.03$, consistent with predictions of XUV- and core-powered mass-loss mechanisms. We found no evidence that $m$ varies with $M_\star$. We observed a correlation between the average sub-Neptune size and $M_\star$. Over 0.5 to 1.4 $M_\odot$, the average sub-Neptune grows from 2.1 to 2.6 $R_E$, following $R_p \propto M_\star^\alpha$ with $\alpha = 0.25 \pm 0.03$. In contrast, there is no detectable change for super-Earths. These $M_\star$-$R_p$ trends suggests that protoplanetary disks can efficiently produce cores up to a threshold mass of $M_c$, which grows linearly with stellar mass according to $M_c \approx 10 M_E~(M_\star / M_\odot)$. There is no significant correlation between sub-Neptune size and stellar metallicity (over $-$0.5 to $+$0.5 dex) suggesting a weak relationship between planet envelope opacity and stellar metallicity. Finally, there is no significant variation in sub-Neptune size with stellar age (over 1 to 10 Gyr), which suggests that the majority of envelope contraction concludes after $\sim$1 Gyr.

==> tab_planet.tex <==
%id_koicand & koi_period & dr25_ror & dr25_tau & gdir_prad & giso_tau0 & giso_sma & giso_sinc & in_curated
K00001.01 & 2.5 & 12.39 & 1.29 & 14.04 & 2.83 & 0.037 & 814.85 & 0 \\ 
K00002.01 & 2.2 & 7.52 & 3.55 & 16.42 & 4.58 & 0.039 & 3855.68 & 1 \\ 
K00003.01 & 4.9 & 5.80 & 2.23 & 4.92 & 2.84 & 0.053 & 80.94 & 1 \\ 
K00007.01 & 3.2 & 2.45 & 3.84 & 4.07 & 4.29 & 0.046 & 1082.71 & 1 \\ 
K00010.01 & 3.5 & 9.21 & 2.75 & 15.51 & 4.47 & 0.050 & 1262.15 & 1 \\ 
K00017.01 & 3.2 & 9.26 & 3.26 & 12.73 & 3.65 & 0.046 & 698.45 & 1 \\ 
K00018.01 & 3.5 & 7.82 & 4.19 & 14.88 & 4.85 & 0.052 & 1601.29 & 1 \\ 
K00020.01 & 4.4 & 11.68 & 4.16 & 19.15 & 4.76 & 0.057 & 765.95 & 1 \\ 
K00022.01 & 7.9 & 9.34 & 3.86 & 12.82 & 4.84 & 0.083 & 246.19 & 1 \\ 
K00041.01 & 12.8 & 1.36 & 6.17 & 2.27 & 6.80 & 0.115 & 182.81 & 1 \\ 
K00041.02 & 6.9 & 0.76 & 4.35 & 1.27 & 5.54 & 0.076 & 414.98 & 1 \\ 
K00041.03 & 35.3 & 0.92 & 5.79 & 1.53 & 9.50 & 0.224 & 47.93 & 1 \\ 
K00042.01 & 17.8 & 1.67 & 4.40 & 2.73 & 7.28 & 0.148 & 150.70 & 1 \\ 
K00046.01 & 3.5 & 3.25 & 3.68 & 5.90 & 4.74 & 0.049 & 999.41 & 1 \\ 
K00049.01 & 8.3 & 2.67 & 2.87 & 3.77 & 5.27 & 0.082 & 246.76 & 0 \\ 
K00063.01 & 9.4 & 5.79 & 2.58 & 5.64 & 3.90 & 0.089 & 93.05 & 1 \\ 
K00069.01 & 4.7 & 1.52 & 2.83 & 1.57 & 3.30 & 0.055 & 259.14 & 1 \\ 
K00070.01 & 10.9 & 2.92 & 3.62 & 2.81 & 4.04 & 0.096 & 69.44 & 1 \\ 
K00070.02 & 3.7 & 1.78 & 2.40 & 1.72 & 2.83 & 0.047 & 287.83 & 1 \\ 
K00070.04 & 6.1 & 0.84 & 2.92 & 0.81 & 3.34 & 0.066 & 148.62 & 1 \\ 
K00070.05 & 19.6 & 0.90 & 3.38 & 0.86 & 4.90 & 0.142 & 31.87 & 1 \\ 
K00072.02 & 45.3 & 2.00 & 6.61 & 2.36 & 7.99 & 0.243 & 17.52 & 1 \\ 
K00075.01 & 105.9 & 3.70 & 16.77 & 10.27 & 21.81 & 0.484 & 29.07 & 1 \\ 
K00082.01 & 16.1 & 2.75 & 3.49 & 2.23 & 4.18 & 0.117 & 18.69 & 1 \\ 
K00082.02 & 10.3 & 1.49 & 3.07 & 1.21 & 3.61 & 0.087 & 33.79 & 1 \\ 
K00082.03 & 27.5 & 1.06 & 3.63 & 0.85 & 4.98 & 0.166 & 9.28 & 1 \\ 
K00082.04 & 7.1 & 0.73 & 2.74 & 0.59 & 3.18 & 0.068 & 55.59 & 1 \\ 
K00082.05 & 5.3 & 0.58 & 2.53 & 0.47 & 2.89 & 0.056 & 81.60 & 1 \\ 
K00084.01 & 9.3 & 2.40 & 3.27 & 2.31 & 3.88 & 0.085 & 86.69 & 1 \\ 
K00085.01 & 5.9 & 1.65 & 3.92 & 2.61 & 4.83 & 0.071 & 551.38 & 1 \\ 
K00085.02 & 2.2 & 0.92 & 3.07 & 1.46 & 3.47 & 0.037 & 2065.10 & 1 \\ 
K00085.03 & 8.1 & 0.98 & 4.13 & 1.54 & 5.38 & 0.088 & 357.82 & 1 \\ 
K00087.01 & 289.9 & 2.10 & 6.90 & 1.94 & 11.79 & 0.814 & 0.91 & 0 \\ 
K00092.01 & 65.7 & 2.33 & 3.16 & 2.71 & 8.42 & 0.330 & 11.45 & 0 \\ 
K00094.01 & 22.3 & 6.87 & 6.17 & 10.44 & 7.40 & 0.168 & 87.91 & 1 \\ 
K00094.02 & 10.4 & 2.57 & 5.02 & 3.92 & 5.75 & 0.102 & 240.51 & 1 \\ 
K00094.03 & 54.3 & 4.08 & 8.02 & 6.21 & 9.92 & 0.302 & 27.21 & 1 \\ 
K00094.04 & 3.7 & 1.07 & 3.62 & 1.63 & 4.10 & 0.052 & 929.49 & 1 \\ 
K00097.01 & 4.9 & 7.99 & 4.67 & 17.39 & 6.10 & 0.065 & 1114.11 & 1 \\ 
K00103.01 & 14.9 & 2.68 & 3.22 & 2.56 & 4.46 & 0.118 & 47.25 & 1 \\ 
K00104.01 & 2.5 & 3.82 & 1.03 & 3.21 & 2.24 & 0.034 & 163.81 & 1 \\ 
K00105.01 & 9.0 & 2.99 & 1.80 & 3.55 & 4.85 & 0.080 & 150.83 & 0 \\ 
K00107.01 & 7.3 & 1.97 & 4.71 & 3.42 & 5.75 & 0.081 & 423.34 & 1 \\ 
K00108.01 & 16.0 & 2.01 & 4.38 & 3.30 & 7.18 & 0.134 & 134.90 & 1 \\ 
K00108.02 & 179.6 & 3.33 & 12.55 & 5.46 & 15.96 & 0.660 & 5.53 & 1 \\ 
K00110.01 & 9.9 & 2.10 & 3.80 & 2.83 & 5.17 & 0.096 & 222.38 & 1 \\ 
K00111.01 & 11.4 & 2.06 & 4.42 & 2.34 & 4.98 & 0.096 & 118.61 & 1 \\ 
K00111.02 & 23.7 & 1.96 & 5.53 & 2.23 & 6.34 & 0.155 & 45.36 & 1 \\ 
K00111.03 & 51.8 & 2.29 & 7.07 & 2.60 & 8.20 & 0.260 & 16.15 & 1 \\ 
K00115.01 & 5.4 & 2.24 & 2.77 & 2.52 & 3.62 & 0.062 & 301.60 & 1 \\ 
K00115.02 & 7.1 & 1.28 & 2.80 & 1.43 & 3.96 & 0.075 & 209.77 & 1 \\ 
K00116.01 & 13.6 & 2.08 & 3.08 & 2.36 & 4.99 & 0.113 & 87.90 & 1 \\ 
K00116.02 & 43.8 & 2.29 & 6.18 & 2.61 & 7.34 & 0.245 & 18.69 & 1 \\ 
K00116.03 & 6.2 & 0.69 & 3.13 & 0.78 & 3.84 & 0.067 & 249.08 & 1 \\ 
K00116.04 & 24.0 & 0.94 & 4.84 & 1.06 & 6.02 & 0.165 & 41.46 & 1 \\ 
K00117.01 & 14.7 & 1.90 & 5.91 & 3.02 & 6.72 & 0.128 & 133.26 & 1 \\ 
K00117.02 & 4.9 & 1.09 & 4.06 & 1.73 & 4.67 & 0.062 & 570.50 & 1 \\ 
K00117.03 & 3.2 & 1.01 & 3.50 & 1.60 & 4.05 & 0.047 & 1009.89 & 1 \\ 
K00117.04 & 8.0 & 0.65 & 4.32 & 1.02 & 5.48 & 0.085 & 300.89 & 1 \\ 
K00118.01 & 25.0 & 1.51 & 5.71 & 2.29 & 7.94 & 0.174 & 63.17 & 1 \\ 
K00122.01 & 11.5 & 2.04 & 3.77 & 3.16 & 6.18 & 0.105 & 161.71 & 1 \\ 
K00123.01 & 6.5 & 1.59 & 3.57 & 2.34 & 4.92 & 0.072 & 387.36 & 1 \\ 
K00123.02 & 21.2 & 1.76 & 6.32 & 2.60 & 7.28 & 0.157 & 80.94 & 1 \\ 
K00124.02 & 31.7 & 1.76 & 4.68 & 2.38 & 7.76 & 0.201 & 42.40 & 1 \\ 
K00125.01 & 38.5 & 13.81 & 4.40 & 12.28 & 5.84 & 0.219 & 11.38 & 1 \\ 
K00127.01 & 3.6 & 9.60 & 2.64 & 10.33 & 3.03 & 0.048 & 368.32 & 1 \\ 
K00128.01 & 4.9 & 9.94 & 2.82 & 13.17 & 4.09 & 0.059 & 374.33 & 1 \\ 
K00129.01 & 24.7 & 7.63 & 6.46 & 12.73 & 8.08 & 0.186 & 117.05 & 0 \\ 
K00131.01 & 5.0 & 7.45 & 4.23 & 13.34 & 5.02 & 0.066 & 960.40 & 0 \\ 
K00135.01 & 3.0 & 8.18 & 2.53 & 12.17 & 3.71 & 0.045 & 1012.57 & 1 \\ 
K00137.01 & 7.6 & 4.27 & 3.25 & 4.26 & 3.68 & 0.077 & 109.60 & 1 \\ 
K00137.02 & 14.9 & 5.14 & 3.32 & 5.13 & 4.59 & 0.120 & 45.56 & 1 \\ 
K00137.03 & 3.5 & 1.61 & 1.92 & 1.61 & 2.85 & 0.046 & 306.67 & 1 \\ 
K00139.01 & 224.8 & 5.68 & 10.01 & 6.82 & 12.91 & 0.755 & 2.35 & 1 \\ 
K00139.02 & 3.3 & 1.22 & 2.86 & 1.48 & 3.22 & 0.047 & 607.13 & 1 \\ 
K00144.01 & 4.2 & 3.32 & 3.41 & 2.91 & 2.74 & 0.048 & 113.70 & 1 \\ 
K00148.01 & 4.8 & 1.96 & 2.67 & 1.80 & 2.99 & 0.055 & 153.06 & 1 \\ 
K00148.02 & 9.7 & 2.77 & 3.16 & 2.55 & 3.77 & 0.088 & 60.32 & 1 \\ 
K00148.03 & 42.9 & 2.13 & 5.50 & 1.96 & 6.17 & 0.235 & 8.45 & 1 \\ 
K00149.01 & 14.6 & 2.82 & 7.44 & 5.77 & 8.75 & 0.124 & 212.99 & 1 \\ 
K00150.01 & 8.4 & 2.58 & 3.39 & 2.55 & 3.99 & 0.077 & 116.32 & 1 \\ 
K00150.02 & 28.6 & 2.64 & 4.77 & 2.61 & 5.98 & 0.172 & 23.14 & 1 \\ 
K00152.01 & 52.1 & 4.94 & 8.12 & 7.10 & 9.04 & 0.299 & 28.82 & 1 \\ 
K00152.02 & 27.4 & 2.52 & 6.60 & 3.63 & 7.31 & 0.196 & 67.28 & 1 \\ 
K00152.03 & 13.5 & 2.36 & 4.86 & 3.40 & 5.79 & 0.123 & 171.54 & 1 \\ 
K00152.04 & 81.1 & 2.03 & 2.90 & 2.91 & 10.46 & 0.401 & 16.07 & 0 \\ 
K00153.01 & 8.9 & 2.80 & 2.52 & 2.33 & 3.43 & 0.079 & 36.85 & 1 \\ 
K00153.02 & 4.8 & 2.45 & 2.43 & 2.04 & 2.79 & 0.052 & 84.63 & 1 \\ 
K00155.01 & 5.7 & 2.49 & 4.45 & 4.39 & 5.80 & 0.063 & 589.32 & 1 \\ 
K00156.02 & 5.2 & 1.72 & 2.31 & 1.37 & 2.79 & 0.054 & 63.38 & 1 \\ 
K00156.03 & 11.8 & 3.43 & 2.75 & 2.73 & 3.66 & 0.093 & 21.48 & 1 \\ 
K00157.01 & 13.0 & 2.54 & 4.42 & 3.02 & 5.10 & 0.111 & 93.16 & 1 \\ 
K00157.02 & 22.7 & 2.83 & 5.28 & 3.36 & 6.12 & 0.160 & 44.78 & 1 \\ 
K00157.03 & 32.0 & 3.39 & 3.99 & 4.03 & 6.86 & 0.201 & 28.45 & 0 \\ 
K00157.04 & 46.7 & 2.22 & 6.15 & 2.63 & 7.77 & 0.258 & 17.27 & 1 \\ 
K00157.05 & 118.4 & 3.00 & 9.14 & 3.55 & 10.56 & 0.477 & 5.06 & 1 \\ 
K00157.06 & 10.3 & 1.63 & 4.13 & 1.93 & 4.72 & 0.095 & 126.93 & 1 \\ 
K00159.01 & 9.0 & 1.98 & 4.01 & 2.45 & 4.59 & 0.089 & 189.28 & 1 \\ 
K00159.02 & 2.4 & 0.81 & 1.32 & 0.99 & 2.97 & 0.037 & 1079.85 & 1 \\ 
K00161.01 & 3.1 & 2.73 & 1.63 & 2.39 & 2.51 & 0.040 & 177.24 & 1 \\ 
K00166.01 & 12.5 & 2.42 & 2.18 & 2.01 & 3.93 & 0.099 & 37.92 & 0 \\ 
K00167.01 & 4.9 & 1.91 & 4.07 & 2.96 & 4.53 & 0.062 & 677.92 & 1 \\ 
K00168.01 & 10.7 & 1.86 & 5.88 & 3.06 & 6.62 & 0.098 & 234.08 & 1 \\ 
K00168.02 & 15.3 & 1.32 & 5.91 & 2.17 & 7.44 & 0.123 & 147.09 & 1 \\ 
K00168.03 & 7.1 & 1.05 & 5.02 & 1.73 & 5.78 & 0.074 & 403.83 & 1 \\ 
K00171.01 & 6.0 & 2.09 & 3.54 & 3.18 & 4.75 & 0.071 & 511.55 & 1 \\ 
K00171.02 & 13.1 & 1.47 & 2.97 & 2.23 & 6.15 & 0.119 & 181.76 & 0 \\ 
K00172.01 & 13.7 & 2.19 & 4.96 & 2.88 & 6.00 & 0.110 & 108.16 & 1 \\ 
K00173.01 & 10.1 & 1.97 & 4.37 & 2.69 & 5.44 & 0.092 & 163.95 & 1 \\ 
K00176.01 & 30.2 & 1.95 & 6.28 & 2.84 & 7.85 & 0.204 & 63.94 & 1 \\ 
K00179.01 & 20.7 & 2.95 & 9.85 & 7.06 & 10.49 & 0.172 & 200.19 & 1 \\ 
K00180.01 & 10.0 & 2.38 & 3.11 & 2.31 & 3.96 & 0.092 & 85.48 & 1 \\ 
K00189.01 & 30.4 & 13.15 & 5.18 & 11.12 & 5.24 & 0.178 & 8.28 & 1 \\ 
K00197.01 & 17.3 & 9.06 & 3.60 & 7.39 & 4.35 & 0.123 & 20.67 & 1 \\ 
K00201.01 & 4.2 & 7.82 & 2.61 & 8.42 & 3.20 & 0.053 & 294.48 & 1 \\ 
K00222.01 & 6.3 & 3.23 & 2.65 & 2.53 & 2.93 & 0.061 & 43.55 & 1 \\ 
K00222.02 & 12.8 & 2.58 & 3.32 & 2.02 & 3.70 & 0.098 & 17.14 & 1 \\ 
K00237.01 & 8.5 & 2.33 & 3.36 & 2.86 & 4.46 & 0.086 & 163.61 & 1 \\ 
K00238.01 & 17.2 & 2.09 & 4.41 & 3.03 & 6.66 & 0.138 & 115.51 & 1 \\ 
K00238.02 & 26.7 & 1.07 & 4.46 & 1.54 & 7.70 & 0.184 & 64.82 & 0 \\ 
K00238.03 & 363.0 & 1.49 & 14.23 & 2.15 & 18.21 & 1.031 & 2.07 & 1 \\ 
K00241.01 & 13.8 & 2.50 & 3.47 & 2.06 & 3.83 & 0.102 & 24.49 & 1 \\ 
K00241.02 & 31.0 & 1.58 & 4.41 & 1.29 & 4.99 & 0.173 & 8.45 & 1 \\ 
K00241.03 & 3.4 & 1.07 & 2.36 & 0.87 & 2.41 & 0.040 & 155.32 & 1 \\ 
K00244.01 & 12.7 & 3.23 & 2.51 & 4.73 & 5.90 & 0.115 & 183.43 & 0 \\ 
K00244.02 & 6.2 & 1.85 & 3.44 & 2.69 & 4.67 & 0.072 & 469.79 & 1 \\ 
K00245.01 & 39.8 & 2.25 & 4.33 & 1.93 & 5.83 & 0.215 & 9.90 & 1 \\ 
K00245.02 & 21.3 & 0.86 & 3.85 & 0.74 & 4.74 & 0.142 & 22.59 & 1 \\ 
K00246.01 & 5.4 & 1.70 & 3.35 & 2.34 & 4.35 & 0.063 & 388.51 & 1 \\ 
K00246.02 & 9.6 & 0.68 & 2.94 & 0.94 & 5.26 & 0.092 & 181.61 & 0 \\ 
K00247.01 & 13.8 & 2.94 & 2.06 & 1.88 & 3.40 & 0.095 & 7.08 & 1 \\ 
K00248.01 & 7.2 & 3.85 & 2.44 & 2.60 & 2.82 & 0.063 & 21.04 & 1 \\ 
K00248.02 & 10.9 & 3.43 & 2.04 & 2.32 & 3.24 & 0.083 & 12.16 & 1 \\ 
K00248.03 & 2.6 & 2.68 & 1.56 & 1.81 & 2.01 & 0.032 & 81.73 & 1 \\ 
K00248.04 & 18.6 & 2.63 & 2.24 & 1.77 & 3.86 & 0.118 & 6.02 & 0 \\ 
K00249.01 & 9.5 & 3.92 & 1.53 & 1.77 & 2.41 & 0.067 & 5.12 & 1 \\ 
K00250.01 & 12.3 & 4.85 & 2.58 & 3.19 & 3.31 & 0.089 & 10.47 & 1 \\ 
K00250.02 & 17.3 & 4.17 & 1.85 & 2.75 & 3.70 & 0.112 & 6.68 & 0 \\ 
K00250.03 & 3.5 & 2.08 & 1.80 & 1.37 & 2.19 & 0.039 & 53.99 & 1 \\ 
K00250.04 & 46.8 & 3.62 & 1.82 & 2.38 & 5.14 & 0.216 & 1.79 & 0 \\ 
K00251.01 & 4.2 & 4.42 & 1.73 & 2.64 & 2.19 & 0.042 & 29.78 & 1 \\ 
K00251.02 & 5.8 & 1.44 & 1.71 & 0.85 & 2.43 & 0.053 & 19.34 & 1 \\ 
K00252.01 & 17.6 & 4.37 & 3.38 & 3.01 & 3.85 & 0.114 & 5.93 & 1 \\ 
K00253.01 & 6.4 & 4.37 & 1.68 & 3.18 & 2.91 & 0.059 & 29.20 & 0 \\ 
K00253.02 & 20.6 & 2.53 & 3.15 & 1.83 & 4.28 & 0.129 & 6.21 & 1 \\ 
K00254.01 & 2.5 & 17.05 & 1.47 & 11.49 & 2.01 & 0.031 & 82.28 & 1 \\ 
K00257.01 & 6.9 & 2.05 & 2.02 & 2.65 & 4.31 & 0.077 & 316.68 & 0 \\ 
K00260.01 & 10.5 & 0.96 & 4.63 & 1.46 & 5.83 & 0.101 & 261.64 & 1 \\ 
K00260.02 & 100.3 & 1.74 & 10.42 & 2.65 & 12.29 & 0.449 & 13.30 & 1 \\ 
K00260.03 & 21.9 & 1.04 & 5.37 & 1.59 & 7.43 & 0.164 & 99.28 & 1 \\ 
K00261.01 & 16.2 & 2.32 & 3.73 & 2.40 & 4.84 & 0.128 & 53.23 & 1 \\ 
K00262.01 & 7.8 & 1.01 & 4.03 & 1.76 & 5.98 & 0.084 & 459.68 & 1 \\ 
K00262.02 & 9.4 & 1.01 & 2.01 & 1.77 & 6.36 & 0.095 & 361.29 & 0 \\ 
K00265.01 & 3.6 & 0.91 & 3.16 & 1.27 & 3.75 & 0.049 & 767.89 & 1 \\ 
K00266.01 & 25.3 & 1.14 & 5.53 & 1.48 & 6.68 & 0.180 & 58.20 & 1 \\ 
K00266.02 & 47.7 & 0.91 & 2.45 & 1.17 & 8.24 & 0.273 & 25.18 & 0 \\ 
K00269.01 & 18.0 & 0.96 & 6.24 & 1.51 & 7.01 & 0.147 & 134.46 & 1 \\ 
K00271.01 & 48.6 & 1.70 & 6.86 & 2.58 & 9.26 & 0.287 & 29.42 & 1 \\ 
K00271.02 & 29.4 & 1.66 & 6.80 & 2.52 & 7.85 & 0.206 & 57.19 & 1 \\ 
K00271.03 & 14.4 & 0.96 & 3.32 & 1.45 & 6.21 & 0.129 & 146.20 & 0 \\ 
K00273.01 & 10.6 & 1.58 & 1.67 & 1.84 & 4.64 & 0.098 & 108.60 & 0 \\ 
K00274.01 & 15.1 & 0.82 & 4.31 & 1.49 & 7.74 & 0.130 & 198.64 & 0 \\ 
K00275.01 & 15.8 & 1.30 & 7.08 & 2.33 & 7.62 & 0.135 & 148.11 & 1 \\ 
K00275.02 & 82.2 & 1.40 & 10.30 & 2.49 & 13.14 & 0.402 & 16.78 & 1 \\ 
K00276.01 & 41.7 & 1.89 & 4.48 & 2.46 & 8.03 & 0.244 & 26.64 & 0 \\ 
K00277.01 & 16.2 & 2.06 & 7.21 & 3.66 & 8.04 & 0.131 & 173.84 & 1 \\ 
K00280.01 & 11.9 & 1.69 & 2.31 & 1.92 & 4.81 & 0.104 & 122.69 & 0 \\ 
K00281.01 & 19.6 & 1.59 & 7.77 & 2.50 & 8.06 & 0.139 & 100.37 & 1 \\ 
K00282.01 & 27.5 & 2.32 & 5.66 & 2.89 & 6.95 & 0.179 & 42.91 & 1 \\ 
K00282.02 & 8.5 & 0.81 & 3.24 & 1.01 & 4.71 & 0.082 & 203.57 & 1 \\ 
K00282.03 & 87.5 & 1.07 & 1.91 & 1.32 & 10.18 & 0.385 & 9.31 & 0 \\ 
K00283.01 & 16.1 & 1.86 & 2.80 & 2.03 & 5.02 & 0.129 & 59.48 & 0 \\ 
K00283.02 & 25.5 & 0.75 & 4.57 & 0.82 & 5.84 & 0.175 & 32.37 & 1 \\ 
K00285.01 & 13.7 & 1.90 & 5.83 & 3.66 & 7.73 & 0.125 & 218.79 & 1 \\ 
K00285.02 & 26.7 & 1.28 & 8.27 & 2.47 & 9.63 & 0.194 & 91.00 & 1 \\ 
K00288.01 & 10.3 & 1.34 & 6.13 & 2.98 & 7.83 & 0.107 & 470.06 & 1 \\ 
K00289.01 & 26.6 & 2.04 & 7.60 & 3.81 & 10.18 & 0.176 & 95.60 & 1 \\ 
K00289.02 & 296.6 & 4.85 & 15.18 & 9.00 & 22.55 & 0.866 & 3.97 & 1 \\ 
K00292.01 & 2.6 & 1.36 & 2.21 & 1.46 & 2.80 & 0.037 & 691.62 & 1 \\ 
K00295.01 & 5.3 & 1.58 & 2.82 & 1.68 & 3.45 & 0.061 & 284.52 & 1 \\ 
K00295.02 & 10.1 & 1.00 & 1.97 & 1.06 & 4.26 & 0.093 & 121.90 & 0 \\ 
K00296.01 & 28.9 & 1.94 & 5.09 & 2.31 & 6.83 & 0.183 & 34.18 & 1 \\ 
K00299.01 & 1.5 & 1.57 & 1.87 & 1.57 & 2.17 & 0.027 & 972.78 & 1 \\ 
K00301.01 & 6.0 & 1.31 & 3.82 & 2.02 & 5.01 & 0.068 & 485.12 & 1 \\ 
K00301.02 & 11.4 & 0.80 & 4.79 & 1.23 & 6.20 & 0.104 & 206.87 & 1 \\ 
K00303.01 & 60.9 & 2.52 & 6.10 & 2.76 & 8.21 & 0.294 & 10.13 & 1 \\ 
K00304.01 & 8.5 & 2.25 & 2.14 & 2.26 & 3.87 & 0.082 & 126.96 & 0 \\ 
K00305.01 & 4.6 & 1.88 & 2.30 & 1.57 & 2.76 & 0.051 & 85.55 & 1 \\ 
K00306.01 & 24.3 & 2.37 & 2.52 & 2.13 & 5.04 & 0.162 & 19.28 & 0 \\ 
K00312.01 & 11.6 & 1.44 & 2.67 & 2.30 & 6.07 & 0.111 & 228.70 & 0 \\ 
K00312.02 & 16.4 & 1.38 & 3.34 & 2.19 & 6.81 & 0.139 & 144.46 & 0 \\ 
K00313.01 & 18.7 & 2.16 & 2.87 & 2.02 & 4.82 & 0.134 & 27.13 & 0 \\ 
K00313.02 & 8.4 & 1.68 & 3.15 & 1.57 & 3.70 & 0.079 & 77.77 & 1 \\ 
K00314.01 & 13.8 & 2.53 & 2.23 & 1.50 & 3.22 & 0.093 & 6.22 & 1 \\ 
K00314.02 & 23.1 & 2.26 & 1.67 & 1.33 & 3.81 & 0.131 & 3.15 & 0 \\ 
K00314.03 & 10.3 & 1.09 & 1.99 & 0.64 & 2.92 & 0.077 & 9.12 & 1 \\ 
K00315.01 & 35.6 & 2.76 & 3.85 & 2.07 & 5.11 & 0.190 & 5.90 & 1 \\ 
K00316.01 & 15.8 & 2.12 & 4.90 & 2.44 & 5.17 & 0.129 & 60.04 & 1 \\ 
K00316.02 & 157.1 & 2.14 & 7.83 & 2.45 & 11.04 & 0.586 & 2.89 & 1 \\ 
K00316.03 & 7.3 & 1.49 & 1.36 & 1.71 & 4.01 & 0.077 & 165.79 & 0 \\ 
K00317.01 & 22.2 & 1.98 & 7.10 & 3.60 & 8.40 & 0.174 & 143.40 & 1 \\ 
K00318.01 & 38.6 & 3.96 & 10.01 & 7.21 & 10.09 & 0.253 & 62.14 & 0 \\ 
K00319.01 & 46.2 & 4.67 & 5.05 & 10.66 & 13.48 & 0.279 & 61.06 & 0 \\ 
K00321.01 & 2.4 & 1.25 & 2.58 & 1.45 & 2.84 & 0.037 & 739.51 & 1 \\ 
K00321.02 & 4.6 & 0.72 & 2.95 & 0.84 & 3.51 & 0.057 & 315.74 & 1 \\ 
K00323.01 & 5.8 & 2.16 & 1.95 & 1.90 & 3.11 & 0.063 & 135.80 & 1 \\ 
K00327.01 & 3.3 & 1.17 & 2.91 & 1.49 & 3.42 & 0.045 & 778.41 & 1 \\ 
K00327.02 & 91.4 & 1.34 & 8.48 & 1.71 & 10.27 & 0.410 & 9.54 & 1 \\ 
K00330.01 & 8.0 & 1.58 & 5.21 & 2.75 & 6.10 & 0.083 & 377.43 & 1 \\ 
K00330.02 & 1.9 & 0.71 & 3.32 & 1.24 & 3.79 & 0.032 & 2526.05 & 1 \\ 
K00331.01 & 18.7 & 1.78 & 6.40 & 3.93 & 10.14 & 0.147 & 151.25 & 1 \\ 
K00332.01 & 5.5 & 1.47 & 3.90 & 2.45 & 5.03 & 0.067 & 517.99 & 1 \\ 
K00337.01 & 19.8 & 1.77 & 5.32 & 2.28 & 6.33 & 0.147 & 61.48 & 1 \\ 
K00338.01 & 7.0 & 1.63 & 2.96 & 1.39 & 3.35 & 0.070 & 75.84 & 1 \\ 
K00338.02 & 3.1 & 0.79 & 2.31 & 0.67 & 2.56 & 0.041 & 221.98 & 1 \\ 
K00341.01 & 7.2 & 2.68 & 2.83 & 2.60 & 3.53 & 0.074 & 123.83 & 1 \\ 
K00341.02 & 4.7 & 1.72 & 2.48 & 1.66 & 3.07 & 0.056 & 216.29 & 1 \\ 
K00343.01 & 4.8 & 2.04 & 3.21 & 2.48 & 3.77 & 0.057 & 367.45 & 1 \\ 
K00343.02 & 2.0 & 1.42 & 2.46 & 1.73 & 2.84 & 0.032 & 1136.59 & 1 \\ 
K00343.03 & 41.8 & 1.27 & 7.52 & 1.55 & 7.71 & 0.239 & 20.88 & 1 \\ 
K00344.01 & 39.3 & 3.07 & 5.54 & 2.97 & 6.31 & 0.219 & 14.22 & 1 \\ 
K00345.01 & 29.9 & 3.22 & 4.28 & 2.59 & 5.16 & 0.177 & 9.50 & 1 \\ 
K00346.01 & 12.9 & 2.81 & 2.50 & 2.31 & 4.00 & 0.103 & 34.56 & 1 \\ 
K00348.01 & 28.5 & 3.84 & 4.17 & 3.04 & 4.95 & 0.169 & 7.59 & 1 \\ 
K00350.01 & 13.0 & 1.83 & 2.32 & 1.97 & 4.66 & 0.111 & 78.52 & 0 \\ 
K00351.02 & 210.6 & 5.89 & 11.14 & 7.69 & 13.69 & 0.719 & 3.15 & 1 \\ 
K00351.03 & 59.7 & 2.19 & 7.73 & 2.87 & 9.03 & 0.313 & 16.60 & 1 \\ 
K00351.04 & 91.9 & 2.03 & 8.87 & 2.66 & 10.41 & 0.416 & 9.40 & 1 \\ 
K00351.05 & 8.7 & 1.17 & 3.64 & 1.53 & 4.79 & 0.088 & 210.57 & 1 \\ 
K00351.06 & 7.0 & 1.00 & 3.77 & 1.30 & 4.45 & 0.076 & 280.97 & 1 \\ 
K00351.07 & 124.9 & 2.05 & 9.96 & 2.68 & 11.52 & 0.509 & 6.27 & 1 \\ 
K00352.01 & 27.1 & 1.90 & 4.43 & 2.74 & 7.86 & 0.181 & 53.39 & 0 \\ 
K00352.02 & 16.0 & 1.56 & 0.93 & 2.24 & 6.61 & 0.128 & 106.87 & 0 \\ 
K00355.01 & 4.9 & 1.69 & 2.82 & 2.37 & 4.15 & 0.062 & 533.67 & 1 \\ 
K00361.01 & 3.2 & 1.32 & 2.46 & 1.38 & 2.87 & 0.044 & 436.26 & 1 \\ 
K00365.01 & 81.7 & 2.29 & 6.46 & 2.16 & 7.83 & 0.356 & 4.70 & 1 \\ 
K00366.01 & 75.1 & 6.34 & 4.07 & 12.42 & 13.49 & 0.394 & 32.20 & 0 \\ 
K00367.01 & 31.6 & 4.20 & 2.04 & 4.57 & 6.26 & 0.202 & 23.92 & 0 \\ 
K00369.01 & 5.9 & 0.99 & 1.90 & 1.27 & 4.13 & 0.068 & 397.40 & 0 \\ 
K00369.02 & 10.1 & 1.00 & 2.30 & 1.27 & 4.93 & 0.097 & 194.70 & 0 \\ 
K00370.01 & 42.9 & 1.87 & 9.38 & 3.83 & 11.90 & 0.267 & 60.71 & 1 \\ 
K00370.02 & 23.0 & 1.06 & 4.33 & 2.16 & 9.68 & 0.177 & 138.56 & 0 \\ 
K00373.01 & 135.2 & 2.36 & 8.49 & 2.40 & 9.96 & 0.496 & 3.49 & 1 \\ 
K00374.01 & 172.7 & 2.36 & 10.89 & 3.12 & 13.56 & 0.602 & 4.23 & 1 \\ 
K00384.01 & 5.1 & 1.38 & 5.01 & 3.22 & 6.74 & 0.064 & 1275.06 & 1 \\ 
K00385.01 & 13.1 & 1.58 & 3.53 & 1.55 & 4.36 & 0.109 & 53.86 & 1 \\ 
K00386.01 & 31.2 & 2.85 & 4.99 & 3.20 & 6.37 & 0.201 & 29.66 & 1 \\ 
K00386.02 & 76.7 & 2.42 & 5.98 & 2.71 & 8.57 & 0.364 & 9.03 & 1 \\ 
K00388.01 & 6.1 & 1.67 & 5.38 & 3.30 & 6.26 & 0.071 & 634.49 & 1 \\ 
K00392.01 & 33.4 & 1.53 & 7.28 & 2.59 & 9.39 & 0.217 & 53.69 & 1 \\ 
K00392.02 & 12.6 & 0.89 & 4.29 & 1.50 & 6.81 & 0.114 & 194.29 & 1 \\ 
K00393.01 & 21.4 & 1.64 & 6.85 & 2.64 & 7.76 & 0.162 & 112.45 & 1 \\ 
K00396.01 & 14.6 & 5452.69 & \nodata & 5644.01 & 4.70 & 0.119 & 60.90 & 0 \\ 
K00401.01 & 29.2 & 4.08 & 4.87 & 4.40 & 6.06 & 0.189 & 21.25 & 1 \\ 
K00401.02 & 160.0 & 3.61 & 4.75 & 3.89 & 10.63 & 0.581 & 2.25 & 0 \\ 
K00401.03 & 55.3 & 1.65 & 6.62 & 1.77 & 7.49 & 0.288 & 9.14 & 1 \\ 
K00409.01 & 13.2 & 2.33 & 4.29 & 2.68 & 4.89 & 0.115 & 87.67 & 1 \\ 
K00415.01 & 166.8 & 6.27 & 5.47 & 8.63 & 14.26 & 0.575 & 4.41 & 0 \\ 
K00430.01 & 12.4 & 3.75 & 2.57 & 2.63 & 3.42 & 0.092 & 12.63 & 1 \\ 
K00430.02 & 9.3 & 1.31 & 2.38 & 0.91 & 3.12 & 0.076 & 18.31 & 1 \\ 
K00440.01 & 15.9 & 2.75 & 3.85 & 2.42 & 4.33 & 0.120 & 26.77 & 1 \\ 
K00440.02 & 5.0 & 2.48 & 1.54 & 2.18 & 2.95 & 0.056 & 124.22 & 0 \\ 
K00442.01 & 13.5 & 1.98 & 4.33 & 2.33 & 5.15 & 0.113 & 90.39 & 1 \\ 
K00442.02 & 1.7 & 1.25 & 2.16 & 1.47 & 2.61 & 0.029 & 1364.17 & 1 \\ 
K00442.03 & 7.0 & 1.27 & 2.16 & 1.49 & 4.15 & 0.073 & 214.90 & 0 \\ 
K00444.01 & 11.7 & 2.03 & 4.09 & 2.03 & 4.30 & 0.101 & 74.25 & 1 \\ 
K00446.01 & 16.7 & 2.62 & 2.45 & 1.86 & 3.77 & 0.112 & 11.32 & 1 \\ 
K00446.02 & 28.6 & 2.56 & 3.95 & 1.81 & 4.50 & 0.160 & 5.58 & 1 \\ 
K00448.01 & 10.1 & 3.12 & 2.55 & 2.30 & 3.37 & 0.083 & 23.98 & 1 \\ 
K00457.01 & 4.9 & 2.49 & 1.83 & 2.04 & 2.95 & 0.056 & 129.91 & 1 \\ 
K00457.02 & 7.1 & 2.45 & 1.32 & 2.01 & 3.32 & 0.071 & 80.62 & 0 \\ 
K00458.01 & 53.7 & 6.69 & 2.83 & 6.80 & 7.23 & 0.273 & 10.63 & 0 \\ 
K00476.01 & 18.4 & 2.40 & 2.77 & 1.95 & 4.22 & 0.124 & 15.47 & 1 \\ 
K00478.01 & 11.0 & 3.83 & 1.37 & 2.30 & 3.04 & 0.081 & 7.52 & 0 \\ 
K00479.01 & 34.2 & 2.96 & 5.12 & 3.02 & 6.30 & 0.201 & 17.67 & 1 \\ 
K00486.01 & 22.2 & 2.49 & 4.96 & 2.88 & 6.29 & 0.148 & 45.30 & 1 \\ 
K00490.01 & 4.4 & 1.90 & 2.38 & 1.57 & 2.70 & 0.049 & 98.81 & 1 \\ 
K00490.03 & 7.4 & 1.84 & 2.82 & 1.52 & 3.21 & 0.069 & 49.59 & 1 \\ 
K00490.04 & 21.8 & 1.42 & 3.26 & 1.16 & 4.58 & 0.141 & 11.92 & 1 \\ 
K00494.01 & 25.7 & 3.11 & 3.76 & 2.43 & 4.55 & 0.152 & 8.78 & 1 \\ 
K00496.01 & 1.6 & 1.89 & 1.52 & 1.65 & 2.03 & 0.027 & 652.09 & 1 \\ 
K00500.01 & 7.1 & 3.50 & 2.31 & 2.71 & 3.03 & 0.066 & 37.88 & 1 \\ 
K00500.02 & 9.5 & 3.52 & 2.27 & 2.72 & 3.35 & 0.080 & 25.49 & 1 \\ 
K00500.03 & 3.1 & 2.13 & 1.80 & 1.64 & 2.30 & 0.038 & 113.47 & 1 \\ 
K00500.04 & 4.6 & 2.18 & 1.97 & 1.68 & 2.64 & 0.050 & 65.74 & 1 \\ 
K00500.05 & 1.0 & 1.92 & 1.22 & 1.48 & 1.58 & 0.018 & 508.06 & 1 \\ 
K00503.01 & 8.2 & 3.43 & 2.60 & 2.36 & 2.94 & 0.070 & 21.51 & 1 \\ 
K00505.01 & 13.8 & 2.37 & 2.72 & 1.88 & 4.05 & 0.108 & 29.97 & 1 \\ 
K00505.02 & 6.2 & 1.56 & 2.85 & 1.24 & 3.11 & 0.064 & 86.00 & 1 \\ 
K00505.03 & 3.3 & 1.34 & 2.20 & 1.06 & 2.52 & 0.042 & 201.48 & 1 \\ 
K00505.04 & 8.3 & 1.54 & 2.70 & 1.23 & 3.44 & 0.078 & 58.01 & 1 \\ 
K00505.05 & 87.1 & 3.04 & 6.23 & 2.42 & 7.45 & 0.365 & 2.63 & 1 \\ 
K00517.01 & 2.8 & 2.56 & 2.00 & 2.51 & 2.59 & 0.040 & 446.14 & 1 \\ 
K00518.01 & 14.0 & 2.89 & 2.84 & 2.30 & 3.64 & 0.100 & 17.62 & 1 \\ 
K00518.02 & 44.0 & 2.22 & 4.95 & 1.76 & 5.31 & 0.213 & 3.88 & 1 \\ 
K00518.03 & 247.4 & 3.28 & 8.27 & 2.61 & 9.38 & 0.666 & 0.40 & 1 \\ 
K00520.01 & 12.8 & 2.68 & 3.41 & 2.33 & 4.00 & 0.103 & 36.17 & 1 \\ 
K00520.02 & 5.4 & 1.64 & 2.31 & 1.43 & 3.01 & 0.059 & 111.64 & 1 \\ 
K00520.03 & 25.8 & 2.46 & 2.67 & 2.14 & 5.04 & 0.164 & 14.32 & 0 \\ 
K00520.04 & 51.2 & 1.46 & 4.38 & 1.27 & 6.32 & 0.259 & 5.78 & 1 \\ 
K00531.01 & 3.7 & 9.15 & 0.69 & 6.92 & 2.45 & 0.042 & 64.58 & 0 \\ 
K00548.01 & 21.3 & 2.36 & 3.96 & 3.35 & 7.02 & 0.157 & 77.40 & 0 \\ 
K00550.01 & 13.0 & 2.26 & 3.86 & 2.33 & 4.49 & 0.111 & 69.47 & 1 \\ 
K00561.01 & 5.4 & 1.99 & 2.60 & 1.66 & 2.98 & 0.057 & 105.06 & 1 \\ 
K00568.01 & 3.4 & 1.46 & 1.37 & 1.38 & 2.74 & 0.044 & 284.96 & 0 \\ 
K00568.02 & 2.4 & 0.88 & 1.61 & 0.83 & 2.43 & 0.035 & 458.74 & 1 \\ 
K00569.01 & 20.7 & 2.14 & 2.71 & 1.70 & 4.51 & 0.137 & 16.53 & 1 \\ 
K00569.02 & 1.6 & 1.31 & 1.55 & 1.04 & 1.95 & 0.026 & 473.27 & 1 \\ 
K00571.01 & 7.3 & 2.39 & 2.22 & 1.41 & 2.61 & 0.061 & 14.70 & 1 \\ 
K00571.02 & 13.3 & 2.63 & 2.63 & 1.56 & 3.19 & 0.091 & 6.59 & 1 \\ 
K00571.03 & 3.9 & 2.02 & 1.74 & 1.19 & 2.12 & 0.040 & 33.58 & 1 \\ 
K00571.04 & 22.4 & 2.40 & 3.20 & 1.42 & 3.78 & 0.129 & 3.32 & 1 \\ 
K00572.01 & 10.6 & 1.97 & 5.12 & 3.42 & 6.59 & 0.101 & 272.14 & 1 \\ 
K00572.02 & 4.9 & 1.03 & 4.27 & 1.78 & 5.11 & 0.061 & 749.52 & 1 \\ 
K00574.01 & 20.1 & 2.91 & 3.49 & 2.41 & 4.61 & 0.137 & 18.59 & 1 \\ 
K00574.02 & 10.4 & 1.50 & 3.25 & 1.24 & 3.71 & 0.088 & 44.46 & 1 \\ 
K00579.01 & 2.0 & 1.65 & 1.77 & 1.36 & 2.17 & 0.030 & 419.42 & 1 \\ 
K00579.02 & 3.8 & 1.71 & 1.54 & 1.40 & 2.67 & 0.046 & 184.50 & 0 \\ 
K00584.01 & 9.9 & 2.44 & 3.67 & 2.65 & 4.27 & 0.093 & 92.95 & 1 \\ 
K00584.02 & 21.2 & 2.21 & 4.62 & 2.39 & 5.48 & 0.153 & 34.09 & 1 \\ 
K00584.03 & 6.5 & 0.99 & 3.25 & 1.06 & 3.70 & 0.070 & 163.54 & 1 \\ 
K00596.01 & 1.7 & 2.42 & 1.36 & 1.44 & 1.62 & 0.023 & 89.67 & 1 \\ 
K00610.01 & 14.3 & 2.84 & 2.58 & 2.08 & 3.80 & 0.102 & 10.98 & 1 \\ 
K00611.01 & 3.3 & 8.37 & 0.96 & 11.85 & 3.57 & 0.048 & 1088.41 & 0 \\ 
K00612.01 & 20.7 & 2.25 & 2.97 & 1.95 & 4.68 & 0.141 & 19.44 & 1 \\ 
K00612.02 & 47.4 & 2.59 & 4.98 & 2.24 & 6.16 & 0.244 & 6.52 & 1 \\ 
K00612.03 & 122.1 & 2.54 & 3.07 & 2.19 & 8.41 & 0.456 & 1.87 & 0 \\ 
K00623.02 & 15.7 & 1.00 & 5.14 & 1.26 & 6.02 & 0.121 & 102.44 & 1 \\ 
K00623.03 & 5.6 & 0.85 & 3.68 & 1.08 & 4.28 & 0.061 & 398.73 & 1 \\ 
K00624.01 & 17.8 & 2.69 & 4.25 & 2.62 & 4.79 & 0.135 & 41.13 & 1 \\ 
K00624.02 & 49.6 & 2.47 & 3.62 & 2.40 & 6.72 & 0.265 & 10.64 & 0 \\ 
K00624.03 & 1.3 & 1.44 & 1.73 & 1.40 & 2.03 & 0.024 & 1284.72 & 1 \\ 
K00626.01 & 14.6 & 1.80 & 3.86 & 2.34 & 5.73 & 0.121 & 119.02 & 1 \\ 
K00627.01 & 7.8 & 1.84 & 3.43 & 2.84 & 5.26 & 0.084 & 334.21 & 1 \\ 
K00627.02 & 4.2 & 1.01 & 3.21 & 1.55 & 4.28 & 0.056 & 758.75 & 1 \\ 
K00628.01 & 14.5 & 1.96 & 2.71 & 2.08 & 4.96 & 0.113 & 70.80 & 0 \\ 
K00629.01 & 40.7 & 1.93 & 6.50 & 2.79 & 9.05 & 0.235 & 37.28 & 1 \\ 
K00631.01 & 15.5 & 5.93 & 8.18 & 12.49 & 9.08 & 0.131 & 221.38 & 1 \\ 
K00632.01 & 7.2 & 1.50 & 3.05 & 1.34 & 3.37 & 0.073 & 99.29 & 1 \\ 
K00633.01 & 161.5 & 2.64 & 9.79 & 3.90 & 14.78 & 0.572 & 5.30 & 1 \\ 
K00635.01 & 16.7 & 2.12 & 3.20 & 2.51 & 5.42 & 0.136 & 81.90 & 0 \\ 
K00638.01 & 23.6 & 3.04 & 4.82 & 3.02 & 5.34 & 0.162 & 30.57 & 1 \\ 
K00638.02 & 67.1 & 3.26 & 6.55 & 3.25 & 7.54 & 0.323 & 7.71 & 1 \\ 
K00639.01 & 18.0 & 1.98 & 5.41 & 2.64 & 6.09 & 0.144 & 92.14 & 1 \\ 
K00647.01 & 5.2 & 1.34 & 4.40 & 2.13 & 4.98 & 0.061 & 702.68 & 1 \\ 
K00649.01 & 23.4 & 1.64 & 8.38 & 3.69 & 10.30 & 0.186 & 163.47 & 1 \\ 
K00650.01 & 12.0 & 2.71 & 2.05 & 2.36 & 3.95 & 0.098 & 38.36 & 0 \\ 
K00654.01 & 8.6 & 1.69 & 3.14 & 1.82 & 4.06 & 0.084 & 138.46 & 1 \\ 
K00654.02 & 10.2 & 1.44 & 1.10 & 1.54 & 4.30 & 0.094 & 110.14 & 0 \\ 
K00655.01 & 25.7 & 1.81 & 5.48 & 2.47 & 7.08 & 0.181 & 60.73 & 1 \\ 
K00655.02 & 151.9 & 1.75 & 11.33 & 2.39 & 12.72 & 0.584 & 5.81 & 1 \\ 
K00657.01 & 4.1 & 2.10 & 2.00 & 1.60 & 2.52 & 0.046 & 96.81 & 1 \\ 
K00657.02 & 16.3 & 2.51 & 2.83 & 1.92 & 3.98 & 0.114 & 15.53 & 1 \\ 
K00658.01 & 3.2 & 2.07 & 1.87 & 2.34 & 3.02 & 0.044 & 588.44 & 1 \\ 
K00658.02 & 5.4 & 2.04 & 2.03 & 2.31 & 3.60 & 0.063 & 292.51 & 0 \\ 
K00658.03 & 11.3 & 1.18 & 3.71 & 1.34 & 4.60 & 0.103 & 109.19 & 1 \\ 
K00659.01 & 23.2 & 1.69 & 4.21 & 2.27 & 6.64 & 0.172 & 74.57 & 1 \\ 
K00661.01 & 14.4 & 1.80 & 3.83 & 1.93 & 4.78 & 0.120 & 73.17 & 1 \\ 
K00661.02 & 25.7 & 1.18 & 4.28 & 1.26 & 5.79 & 0.175 & 34.13 & 1 \\ 
K00662.01 & 10.2 & 1.60 & 5.65 & 2.82 & 6.83 & 0.096 & 276.80 & 1 \\ 
K00664.01 & 13.1 & 1.34 & 4.65 & 1.59 & 5.14 & 0.111 & 89.43 & 1 \\ 
K00664.02 & 7.8 & 0.95 & 3.82 & 1.12 & 4.32 & 0.079 & 178.51 & 1 \\ 
K00664.03 & 23.4 & 0.85 & 5.47 & 1.00 & 6.22 & 0.163 & 41.64 & 1 \\ 
K00665.01 & 5.9 & 1.91 & 3.88 & 3.54 & 5.58 & 0.072 & 620.97 & 1 \\ 
K00665.02 & 1.6 & 0.92 & 2.95 & 1.71 & 3.64 & 0.031 & 3418.24 & 1 \\ 
K00665.03 & 3.1 & 0.85 & 3.90 & 1.58 & 4.51 & 0.047 & 1459.39 & 1 \\ 
K00666.01 & 22.2 & 2.27 & 3.77 & 2.43 & 5.53 & 0.157 & 34.17 & 1 \\ 
K00670.01 & 9.5 & 1.48 & 3.42 & 2.62 & 6.62 & 0.092 & 265.24 & 0 \\ 
K00671.01 & 4.2 & 1.13 & 3.27 & 1.54 & 3.88 & 0.055 & 618.50 & 1 \\ 
K00671.02 & 7.5 & 1.02 & 3.79 & 1.38 & 4.68 & 0.080 & 292.01 & 1 \\ 
K00671.03 & 16.3 & 1.05 & 3.75 & 1.43 & 6.05 & 0.133 & 104.54 & 1 \\ 
K00671.04 & 11.1 & 0.90 & 3.96 & 1.22 & 5.34 & 0.104 & 172.37 & 1 \\ 
K00672.01 & 16.1 & 2.26 & 2.88 & 2.23 & 4.67 & 0.126 & 44.09 & 1 \\ 
K00672.02 & 41.7 & 2.96 & 5.38 & 2.93 & 6.40 & 0.236 & 12.52 & 1 \\ 
K00676.02 & 2.5 & 3.82 & 1.58 & 2.86 & 2.12 & 0.033 & 139.73 & 1 \\ 
K00678.01 & 6.0 & 1.42 & 1.93 & 1.18 & 3.19 & 0.064 & 107.84 & 1 \\ 
K00678.02 & 4.1 & 1.47 & 2.21 & 1.22 & 2.82 & 0.050 & 177.64 & 1 \\ 
K00679.01 & 31.8 & 1.73 & 8.00 & 2.77 & 8.78 & 0.211 & 50.39 & 1 \\ 
K00680.01 & 8.6 & 6.20 & 8.28 & 14.51 & 7.98 & 0.092 & 665.92 & 1 \\ 
K00683.01 & 278.1 & 4.38 & 3.34 & 5.20 & 13.63 & 0.862 & 1.71 & 0 \\ 
K00685.01 & 3.2 & 1.61 & 3.40 & 3.03 & 4.56 & 0.048 & 2073.01 & 1 \\ 
K00686.01 & 52.5 & 11.61 & 2.70 & 13.37 & 8.04 & 0.273 & 13.29 & 0 \\ 
K00689.01 & 15.9 & 1.89 & 3.42 & 1.72 & 4.60 & 0.114 & 37.54 & 1 \\ 
K00691.01 & 29.7 & 2.38 & 8.10 & 3.79 & 9.05 & 0.189 & 64.15 & 1 \\ 
K00691.02 & 16.2 & 1.01 & 6.35 & 1.61 & 7.41 & 0.127 & 142.27 & 1 \\ 
K00692.01 & 2.5 & 1.23 & 1.79 & 1.47 & 2.96 & 0.037 & 790.82 & 1 \\ 
K00692.02 & 4.8 & 1.71 & 0.80 & 2.04 & 3.69 & 0.058 & 325.60 & 0 \\ 
K00693.01 & 28.8 & 1.47 & 7.68 & 2.56 & 9.20 & 0.197 & 74.35 & 1 \\ 
K00693.02 & 15.7 & 1.81 & 6.78 & 3.15 & 7.53 & 0.132 & 166.01 & 1 \\ 
K00694.01 & 17.4 & 2.78 & 4.72 & 2.87 & 4.95 & 0.135 & 46.45 & 1 \\ 
K00695.01 & 29.9 & 2.23 & 4.70 & 2.25 & 6.14 & 0.180 & 25.04 & 1 \\ 
K00700.01 & 30.9 & 2.16 & 2.72 & 2.12 & 6.03 & 0.183 & 22.29 & 0 \\ 
K00700.02 & 9.4 & 1.42 & 3.08 & 1.39 & 4.07 & 0.083 & 107.68 & 1 \\ 
K00700.03 & 14.7 & 1.30 & 3.64 & 1.27 & 4.72 & 0.112 & 59.52 & 1 \\ 
K00700.04 & 68.2 & 1.59 & 5.45 & 1.55 & 7.83 & 0.309 & 7.83 & 1 \\ 
K00701.01 & 18.2 & 2.77 & 2.84 & 2.15 & 4.13 & 0.122 & 15.64 & 1 \\ 
K00701.02 & 5.7 & 1.88 & 2.28 & 1.46 & 2.82 & 0.057 & 71.96 & 1 \\ 
K00701.03 & 122.4 & 2.41 & 6.86 & 1.88 & 7.75 & 0.430 & 1.26 & 1 \\ 
K00704.01 & 18.4 & 2.37 & 2.52 & 1.96 & 4.51 & 0.131 & 25.25 & 0 \\ 
K00707.01 & 21.8 & 2.59 & 7.65 & 4.59 & 8.46 & 0.167 & 104.34 & 1 \\ 
K00707.02 & 41.0 & 2.14 & 9.44 & 3.80 & 10.43 & 0.253 & 45.22 & 1 \\ 
K00707.03 & 31.8 & 1.94 & 8.51 & 3.45 & 9.59 & 0.214 & 63.33 & 1 \\ 
K00707.04 & 13.2 & 1.54 & 6.49 & 2.73 & 7.17 & 0.120 & 202.52 & 1 \\ 
K00707.05 & 5.7 & 1.01 & 4.78 & 1.79 & 5.43 & 0.068 & 616.64 & 1 \\ 
K00708.01 & 17.4 & 2.24 & 6.63 & 3.82 & 7.66 & 0.141 & 147.59 & 1 \\ 
K00708.02 & 7.7 & 1.60 & 4.88 & 2.73 & 5.85 & 0.082 & 433.62 & 1 \\ 
K00709.01 & 21.4 & 2.35 & 3.92 & 2.18 & 5.04 & 0.145 & 25.58 & 1 \\ 
K00710.01 & 5.4 & 1.16 & 3.86 & 2.22 & 5.57 & 0.068 & 1061.00 & 1 \\ 
K00710.02 & 8.6 & 0.94 & 3.23 & 1.80 & 6.50 & 0.093 & 571.74 & 0 \\ 
K00710.03 & 3.9 & 0.71 & 3.64 & 1.36 & 5.01 & 0.055 & 1627.54 & 1 \\ 
K00711.02 & 3.6 & 1.31 & 2.97 & 1.49 & 3.16 & 0.049 & 405.24 & 1 \\ 
K00711.03 & 124.5 & 2.38 & 9.28 & 2.71 & 10.14 & 0.503 & 3.80 & 1 \\ 
K00714.01 & 4.2 & 2.63 & 2.16 & 2.42 & 2.85 & 0.051 & 206.57 & 1 \\ 
K00716.01 & 26.9 & 12.24 & \nodata & 22.70 & 9.40 & 0.194 & 91.86 & 0 \\ 
K00717.01 & 14.7 & 1.48 & 3.08 & 1.94 & 5.74 & 0.123 & 84.35 & 0 \\ 
K00717.02 & 0.9 & 0.58 & 1.34 & 0.76 & 2.28 & 0.019 & 3368.38 & 1 \\ 
K00718.01 & 4.6 & 1.79 & 3.24 & 2.28 & 3.71 & 0.059 & 425.03 & 1 \\ 
K00718.02 & 22.7 & 2.20 & 5.65 & 2.81 & 6.29 & 0.169 & 51.42 & 1 \\ 
K00718.03 & 47.9 & 1.79 & 5.51 & 2.28 & 8.04 & 0.276 & 19.20 & 1 \\ 
K00720.01 & 5.7 & 3.39 & 2.42 & 2.86 & 3.01 & 0.060 & 108.81 & 1 \\ 
K00720.02 & 10.0 & 3.04 & 2.46 & 2.57 & 3.63 & 0.088 & 51.42 & 1 \\ 
K00720.03 & 18.4 & 3.06 & 2.22 & 2.58 & 4.43 & 0.131 & 23.17 & 0 \\ 
K00720.04 & 2.8 & 1.80 & 1.96 & 1.51 & 2.38 & 0.038 & 278.01 & 1 \\ 
K00721.01 & 13.7 & 1.55 & 6.65 & 2.74 & 7.34 & 0.120 & 181.78 & 1 \\ 
K00722.01 & 46.4 & 2.00 & 6.80 & 2.60 & 8.31 & 0.264 & 26.24 & 1 \\ 
K00736.01 & 18.8 & 3.53 & 3.14 & 2.72 & 4.13 & 0.123 & 8.00 & 1 \\ 
K00736.02 & 6.7 & 2.22 & 2.74 & 1.71 & 2.94 & 0.063 & 30.98 & 1 \\ 
K00739.01 & 1.3 & 2.46 & 1.44 & 1.82 & 1.71 & 0.021 & 254.54 & 1 \\ 
K00740.01 & 17.7 & 2.73 & 3.08 & 2.37 & 4.35 & 0.124 & 15.81 & 1 \\ 
K00746.01 & 9.3 & 3.22 & 3.15 & 2.60 & 3.25 & 0.077 & 27.56 & 1 \\ 
K00747.01 & 6.0 & 3.90 & 1.52 & 2.85 & 2.74 & 0.058 & 37.92 & 0 \\ 
K00775.01 & 16.4 & 3.03 & 2.91 & 2.04 & 3.74 & 0.110 & 8.28 & 1 \\ 
K00775.02 & 7.9 & 3.26 & 2.01 & 2.19 & 2.94 & 0.068 & 21.78 & 1 \\ 
K00775.03 & 36.4 & 3.02 & 3.88 & 2.03 & 4.87 & 0.186 & 2.88 & 1 \\ 
K00778.01 & 2.2 & 2.64 & 0.97 & 1.87 & 1.94 & 0.030 & 114.42 & 1 \\ 
K00781.01 & 11.6 & 4.82 & 2.31 & 3.01 & 3.19 & 0.084 & 7.83 & 1 \\ 
K00784.01 & 19.3 & 3.20 & 2.66 & 1.79 & 3.70 & 0.121 & 7.63 & 0 \\ 
K00784.02 & 10.1 & 2.99 & 1.30 & 1.67 & 2.98 & 0.079 & 17.97 & 0 \\ 
K00811.01 & 20.5 & 4.12 & 3.86 & 3.30 & 4.53 & 0.137 & 13.94 & 1 \\ 
K00812.01 & 3.3 & 3.72 & 1.82 & 2.48 & 2.06 & 0.037 & 51.02 & 1 \\ 
K00812.02 & 20.1 & 3.56 & 3.13 & 2.36 & 3.72 & 0.122 & 4.79 & 1 \\ 
K00812.03 & 46.2 & 3.45 & 4.56 & 2.29 & 4.90 & 0.211 & 1.59 & 1 \\ 
K00812.04 & 7.8 & 2.11 & 2.05 & 1.40 & 2.73 & 0.065 & 16.58 & 1 \\ 
K00817.01 & 24.0 & 3.13 & 3.66 & 2.08 & 4.21 & 0.139 & 3.99 & 1 \\ 
K00817.02 & 8.3 & 2.65 & 1.17 & 1.76 & 2.96 & 0.069 & 16.18 & 0 \\ 
K00818.01 & 8.1 & 3.60 & 2.15 & 2.25 & 2.82 & 0.067 & 12.10 & 1 \\ 
K00825.01 & 8.1 & 2.69 & 3.05 & 2.30 & 3.38 & 0.074 & 46.34 & 1 \\ 
K00825.02 & 4.7 & 1.85 & 2.43 & 1.58 & 2.83 & 0.052 & 94.72 & 1 \\ 
K00835.01 & 11.8 & 2.90 & 2.80 & 2.46 & 3.85 & 0.095 & 30.21 & 1 \\ 
K00835.02 & 56.2 & 2.66 & 3.35 & 2.25 & 6.45 & 0.268 & 3.83 & 0 \\ 
K00837.01 & 8.0 & 2.66 & 2.54 & 2.26 & 3.35 & 0.073 & 45.24 & 1 \\ 
K00837.02 & 4.1 & 1.79 & 2.29 & 1.52 & 2.70 & 0.048 & 106.96 & 1 \\ 
K00854.01 & 56.1 & 3.67 & 4.47 & 2.23 & 5.25 & 0.237 & 0.90 & 1 \\ 
K00868.01 & 236.0 & 14.75 & 6.03 & 11.01 & 9.58 & 0.665 & 0.32 & 1 \\ 
K00870.01 & 5.9 & 2.80 & 2.25 & 2.00 & 2.82 & 0.059 & 51.73 & 1 \\ 
K00870.02 & 9.0 & 2.69 & 2.77 & 1.92 & 3.24 & 0.077 & 29.77 & 1 \\ 
K00874.01 & 4.6 & 2.48 & 2.18 & 2.05 & 2.88 & 0.053 & 138.56 & 1 \\ 
K00874.02 & 11.2 & 1.70 & 3.14 & 1.40 & 3.85 & 0.095 & 42.89 & 1 \\ 
K00875.01 & 4.2 & 4.46 & 2.81 & 3.63 & 2.60 & 0.047 & 72.33 & 1 \\ 
K00877.01 & 6.0 & 3.36 & 2.30 & 2.34 & 2.70 & 0.057 & 37.17 & 1 \\ 
K00877.02 & 12.0 & 3.17 & 2.63 & 2.21 & 3.40 & 0.091 & 14.67 & 1 \\ 
K00877.03 & 20.8 & 1.90 & 2.26 & 1.32 & 4.08 & 0.130 & 7.11 & 0 \\ 
K00878.01 & 23.6 & 3.18 & 4.10 & 2.76 & 4.74 & 0.148 & 11.06 & 1 \\ 
K00883.01 & 2.7 & 17.26 & 1.80 & 13.95 & 2.34 & 0.036 & 213.02 & 1 \\ 
K00886.01 & 8.0 & 3.36 & 2.23 & 1.91 & 2.62 & 0.064 & 11.11 & 1 \\ 
K00886.02 & 12.1 & 2.57 & 4.16 & 1.46 & 3.00 & 0.084 & 6.46 & 1 \\ 
K00886.03 & 21.0 & 2.57 & 2.52 & 1.46 & 3.61 & 0.122 & 3.11 & 1 \\ 
K00898.01 & 9.8 & 4.05 & 2.35 & 2.72 & 3.10 & 0.077 & 13.85 & 1 \\ 
K00898.02 & 5.2 & 3.00 & 2.08 & 2.01 & 2.51 & 0.051 & 32.08 & 1 \\ 
K00898.03 & 20.1 & 3.50 & 3.50 & 2.36 & 3.93 & 0.124 & 5.35 & 1 \\ 
K00899.01 & 7.1 & 2.59 & 2.10 & 1.45 & 2.51 & 0.059 & 12.17 & 1 \\ 
K00899.02 & 3.3 & 2.06 & 1.79 & 1.15 & 1.95 & 0.036 & 33.45 & 1 \\ 
K00899.03 & 15.4 & 2.51 & 2.40 & 1.40 & 3.23 & 0.098 & 4.40 & 1 \\ 
K00901.01 & 12.7 & 8.19 & 1.80 & 6.02 & 3.56 & 0.095 & 13.15 & 0 \\ 
K00902.01 & 83.9 & 8.57 & 5.84 & 6.50 & 6.78 & 0.335 & 1.34 & 1 \\ 
K00904.01 & 2.2 & 2.43 & 1.57 & 1.83 & 2.03 & 0.030 & 157.90 & 1 \\ 
K00904.02 & 28.0 & 2.76 & 3.78 & 2.08 & 4.69 & 0.162 & 5.55 & 1 \\ 
K00904.03 & 42.1 & 2.69 & 4.83 & 2.02 & 5.37 & 0.212 & 3.23 & 1 \\ 
K00904.04 & 4.6 & 2.17 & 2.17 & 1.63 & 2.59 & 0.049 & 59.74 & 1 \\ 
K00904.05 & 10.2 & 2.27 & 2.31 & 1.71 & 3.36 & 0.083 & 20.99 & 1 \\ 
K00912.01 & 10.8 & 3.66 & 2.87 & 2.67 & 3.39 & 0.086 & 19.23 & 1 \\ 
K00912.02 & 6.7 & 1.72 & 1.83 & 1.25 & 2.89 & 0.062 & 36.56 & 1 \\ 
K00936.01 & 9.5 & 4.30 & 2.33 & 2.46 & 2.80 & 0.072 & 8.24 & 1 \\ 
K00947.01 & 28.6 & 3.67 & 3.51 & 2.06 & 3.96 & 0.149 & 2.10 & 1 \\ 
K00950.01 & 31.2 & 17.13 & 1.85 & 10.17 & 4.24 & 0.160 & 2.17 & 0 \\ 
K00951.01 & 13.2 & 4.14 & 3.27 & 3.44 & 3.92 & 0.102 & 22.91 & 1 \\ 
K00951.02 & 33.7 & 3.04 & 3.75 & 2.52 & 5.33 & 0.189 & 6.66 & 1 \\ 
K00952.01 & 5.9 & 3.58 & 2.12 & 2.24 & 2.55 & 0.054 & 21.74 & 1 \\ 
K00952.02 & 8.8 & 3.40 & 2.29 & 2.13 & 2.90 & 0.070 & 12.92 & 1 \\ 
K00952.03 & 22.8 & 4.02 & 3.16 & 2.52 & 3.98 & 0.132 & 3.66 & 1 \\ 
K00952.04 & 2.9 & 2.29 & 1.62 & 1.43 & 2.01 & 0.034 & 55.64 & 1 \\ 
K00952.05 & 0.7 & 3.36 & 0.39 & 2.08 & 1.29 & 0.014 & 335.19 & 0 \\ 
K00956.01 & 8.4 & 4.04 & 2.57 & 3.12 & 3.22 & 0.074 & 32.13 & 1 \\ 
K00958.01 & 21.8 & 3.24 & 1.21 & 2.49 & 4.56 & 0.142 & 13.81 & 0 \\ 
K00974.01 & 53.5 & 1.30 & 10.20 & 2.73 & 13.13 & 0.310 & 52.94 & 1 \\ 
K00975.01 & 2.8 & 0.77 & 3.41 & 1.63 & 5.03 & 0.044 & 2534.89 & 1 \\ 
K00986.01 & 8.2 & 2.07 & 2.94 & 2.09 & 3.80 & 0.081 & 108.22 & 1 \\ 
K00986.02 & 76.0 & 1.92 & 7.00 & 1.93 & 7.92 & 0.354 & 5.71 & 1 \\ 
K00987.01 & 3.2 & 1.30 & 1.01 & 1.29 & 2.76 & 0.043 & 365.42 & 0 \\ 
K00988.01 & 10.4 & 2.56 & 2.63 & 2.09 & 3.72 & 0.090 & 46.54 & 1 \\ 
K00988.02 & 24.6 & 2.50 & 2.84 & 2.04 & 4.95 & 0.158 & 14.93 & 0 \\ 
K00999.01 & 16.6 & 3.30 & 4.08 & 2.61 & 4.24 & 0.120 & 24.22 & 1 \\ 
K00999.02 & 47.3 & 2.77 & 2.60 & 2.18 & 5.99 & 0.240 & 6.06 & 0 \\ 
K01001.01 & 40.8 & 1.64 & 12.67 & 3.53 & 11.99 & 0.265 & 76.45 & 1 \\ 
K01001.02 & 140.1 & 1.51 & 17.68 & 3.26 & 18.01 & 0.598 & 15.00 & 1 \\ 
K01014.01 & 17.3 & 3.55 & 2.93 & 2.82 & 4.07 & 0.118 & 18.12 & 1 \\ 
K01024.01 & 5.7 & 2.58 & 1.82 & 1.82 & 2.66 & 0.056 & 36.58 & 0 \\ 
K01050.01 & 1.3 & 1.67 & 1.44 & 1.50 & 1.93 & 0.022 & 783.49 & 1 \\ 
K01050.02 & 2.9 & 1.51 & 1.44 & 1.36 & 2.52 & 0.038 & 268.92 & 1 \\ 
K01078.01 & 3.4 & 3.31 & 1.42 & 1.95 & 2.02 & 0.037 & 41.20 & 1 \\ 
K01078.02 & 6.9 & 3.76 & 1.24 & 2.22 & 2.56 & 0.059 & 15.97 & 0 \\ 
K01078.03 & 28.5 & 3.76 & 2.57 & 2.22 & 4.08 & 0.151 & 2.45 & 1 \\ 
K01082.01 & 6.5 & 1.85 & 2.53 & 1.70 & 3.36 & 0.066 & 92.39 & 1 \\ 
K01082.03 & 1.2 & 1.37 & 1.21 & 1.26 & 1.92 & 0.021 & 863.20 & 1 \\ 
K01085.01 & 7.7 & 1.62 & 1.83 & 0.97 & 2.68 & 0.064 & 13.38 & 1 \\ 
K01101.01 & 11.4 & 1.92 & 2.15 & 1.64 & 3.86 & 0.094 & 37.70 & 0 \\ 
K01108.01 & 18.9 & 2.29 & 3.71 & 2.78 & 5.82 & 0.144 & 52.91 & 1 \\ 
K01108.02 & 1.5 & 1.13 & 2.23 & 1.37 & 2.51 & 0.027 & 1535.71 & 1 \\ 
K01108.03 & 4.2 & 1.35 & 2.50 & 1.63 & 3.53 & 0.053 & 391.81 & 1 \\ 
K01113.01 & 25.9 & 1.88 & 4.50 & 2.57 & 7.13 & 0.182 & 57.48 & 1 \\ 
K01113.02 & 83.4 & 2.07 & 6.36 & 2.83 & 10.48 & 0.393 & 12.29 & 1 \\ 
K01115.01 & 13.0 & 1.51 & 5.86 & 2.98 & 8.10 & 0.115 & 216.56 & 1 \\ 
K01116.01 & 3.7 & 1.24 & 1.79 & 1.43 & 3.29 & 0.049 & 449.33 & 0 \\ 
K01117.01 & 11.1 & 1.13 & 6.14 & 2.30 & 7.51 & 0.110 & 422.24 & 1 \\ 
K01128.01 & 1.0 & 1.29 & 1.56 & 1.18 & 1.77 & 0.019 & 1393.82 & 1 \\ 
K01141.01 & 5.7 & 2.33 & 2.00 & 1.63 & 2.64 & 0.055 & 31.00 & 1 \\ 
K01145.01 & 30.6 & 1.99 & 5.19 & 2.35 & 6.60 & 0.200 & 32.88 & 1 \\ 
K01146.01 & 7.1 & 1.77 & 2.05 & 1.06 & 2.62 & 0.060 & 14.79 & 1 \\ 
K01148.01 & 11.5 & 1.25 & 4.84 & 1.68 & 5.27 & 0.108 & 161.49 & 1 \\ 
K01148.02 & 25.3 & 1.03 & 6.11 & 1.38 & 6.83 & 0.182 & 56.99 & 1 \\ 
K01162.01 & 158.7 & 2.75 & 11.03 & 3.35 & 12.38 & 0.557 & 3.82 & 1 \\ 
K01165.01 & 7.1 & 2.06 & 1.56 & 1.92 & 3.44 & 0.071 & 108.44 & 0 \\ 
K01169.01 & 0.7 & 1.27 & 1.56 & 1.46 & 1.89 & 0.016 & 3915.12 & 1 \\ 
K01176.01 & 2.0 & 16.43 & 1.55 & 12.86 & 2.00 & 0.028 & 203.53 & 1 \\ 
K01194.01 & 8.7 & 3.39 & 2.40 & 2.29 & 2.94 & 0.072 & 21.02 & 1 \\ 
K01194.03 & 4.2 & 2.08 & 2.24 & 1.40 & 2.30 & 0.044 & 55.45 & 1 \\ 
K01199.01 & 53.5 & 2.95 & 5.41 & 2.31 & 6.09 & 0.256 & 3.40 & 1 \\ 
K01202.01 & 0.9 & 1.80 & 1.14 & 1.34 & 1.52 & 0.017 & 402.26 & 1 \\ 
K01215.01 & 17.3 & 1.43 & 7.66 & 2.75 & 8.32 & 0.145 & 170.62 & 1 \\ 
K01215.02 & 33.0 & 1.54 & 6.92 & 2.94 & 10.29 & 0.222 & 72.86 & 1 \\ 
K01216.01 & 11.1 & 1.33 & 4.14 & 2.41 & 7.11 & 0.103 & 276.99 & 0 \\ 
K01242.01 & 99.6 & 8.36 & \nodata & 11.65 & 11.25 & 0.443 & 10.44 & 0 \\ 
K01245.01 & 13.7 & 1.65 & 5.41 & 2.10 & 5.47 & 0.117 & 114.64 & 1 \\ 
K01266.01 & 11.4 & 2.76 & 3.85 & 2.03 & 3.43 & 0.089 & 17.13 & 1 \\ 
K01271.01 & 162.0 & 6.73 & 8.71 & 11.56 & 16.14 & 0.617 & 9.06 & 0 \\ 
K01275.01 & 50.3 & 3.07 & 6.07 & 3.98 & 8.58 & 0.274 & 19.45 & 1 \\ 
K01279.01 & 14.4 & 1.69 & 4.66 & 1.95 & 5.25 & 0.116 & 76.51 & 1 \\ 
K01279.02 & 9.7 & 0.94 & 4.20 & 1.08 & 4.61 & 0.089 & 129.44 & 1 \\ 
K01282.01 & 30.9 & 1.48 & 8.04 & 2.64 & 9.66 & 0.205 & 75.31 & 1 \\ 
K01283.01 & 8.1 & 0.75 & 5.28 & 1.28 & 6.38 & 0.080 & 376.90 & 1 \\ 
K01298.01 & 11.0 & 3.45 & 1.94 & 2.33 & 3.19 & 0.084 & 14.47 & 1 \\ 
K01308.01 & 23.6 & 1.90 & 5.29 & 2.98 & 8.21 & 0.164 & 68.45 & 1 \\ 
K01309.01 & 10.1 & 1.58 & 4.55 & 2.92 & 6.63 & 0.103 & 412.44 & 0 \\ 
K01311.01 & 83.6 & 2.32 & 6.92 & 2.68 & 9.43 & 0.369 & 8.82 & 1 \\ 
K01315.01 & 6.8 & 1.13 & 3.27 & 1.47 & 4.37 & 0.075 & 302.92 & 1 \\ 
K01316.01 & 7.6 & 0.69 & 6.31 & 1.40 & 6.68 & 0.086 & 485.14 & 1 \\ 
K01331.01 & 6.8 & 2.40 & 1.91 & 1.93 & 3.12 & 0.066 & 54.49 & 1 \\ 
K01344.01 & 4.5 & 0.98 & 2.80 & 1.47 & 4.51 & 0.055 & 747.60 & 1 \\ 
K01353.01 & 125.9 & 10.16 & 8.07 & 11.05 & 9.90 & 0.503 & 4.55 & 1 \\ 
K01353.02 & 34.5 & 1.92 & 3.20 & 2.09 & 6.46 & 0.214 & 25.07 & 0 \\ 
K01358.01 & 5.6 & 3.36 & 2.16 & 2.69 & 2.89 & 0.058 & 62.94 & 1 \\ 
K01358.02 & 8.7 & 2.51 & 2.54 & 2.00 & 3.34 & 0.077 & 35.33 & 1 \\ 
K01358.03 & 3.6 & 1.74 & 1.94 & 1.39 & 2.51 & 0.043 & 111.99 & 1 \\ 
K01358.04 & 2.3 & 1.61 & 1.64 & 1.28 & 2.17 & 0.032 & 200.60 & 1 \\ 
K01379.01 & 5.6 & 1.20 & 2.35 & 1.32 & 3.70 & 0.062 & 242.34 & 1 \\ 
K01393.01 & 1.7 & 3.45 & 1.59 & 2.41 & 1.80 & 0.024 & 138.27 & 1 \\ 
K01397.01 & 6.2 & 3.58 & 1.43 & 2.44 & 2.66 & 0.057 & 23.80 & 0 \\ 
K01399.01 & 8.8 & 2.67 & 2.72 & 2.22 & 3.41 & 0.078 & 38.08 & 1 \\ 
K01403.01 & 18.8 & 2.88 & 2.93 & 2.10 & 4.10 & 0.125 & 9.14 & 1 \\ 
K01404.01 & 13.3 & 2.59 & 3.12 & 1.94 & 3.64 & 0.098 & 14.51 & 1 \\ 
K01404.02 & 18.9 & 1.82 & 3.77 & 1.36 & 4.08 & 0.124 & 9.14 & 1 \\ 
K01408.01 & 14.5 & 2.07 & 3.12 & 1.53 & 3.69 & 0.102 & 9.85 & 1 \\ 
K01411.01 & 305.1 & 5.92 & 5.55 & 7.50 & 15.03 & 0.914 & 1.49 & 0 \\ 
K01412.01 & 37.8 & 1.86 & 8.41 & 3.03 & 9.45 & 0.236 & 43.23 & 1 \\ 
K01420.01 & 13.4 & 5.16 & 3.33 & 4.62 & 3.96 & 0.103 & 20.65 & 1 \\ 
K01424.01 & 1.2 & 2.01 & 1.52 & 1.60 & 1.74 & 0.021 & 471.09 & 1 \\ 
K01427.01 & 2.6 & 2.26 & 1.74 & 1.54 & 1.98 & 0.032 & 83.41 & 1 \\ 
K01428.01 & 0.9 & 2.07 & 1.34 & 1.58 & 1.56 & 0.017 & 715.67 & 1 \\ 
K01430.01 & 10.5 & 2.95 & 2.18 & 2.19 & 3.27 & 0.083 & 19.20 & 1 \\ 
K01430.02 & 22.9 & 2.73 & 1.93 & 2.02 & 4.23 & 0.139 & 6.83 & 0 \\ 
K01430.03 & 77.5 & 3.54 & 3.82 & 2.63 & 6.33 & 0.310 & 1.37 & 1 \\ 
K01431.01 & 345.2 & 7.65 & 5.78 & 7.91 & 13.32 & 0.963 & 0.81 & 0 \\ 
K01438.01 & 6.9 & 1.30 & 5.53 & 2.88 & 7.23 & 0.078 & 614.60 & 1 \\ 
K01439.01 & 394.6 & 4.11 & 22.48 & 8.09 & 24.03 & 1.144 & 2.76 & 1 \\ 
K01442.01 & 0.7 & 1.04 & 1.58 & 1.17 & 1.79 & 0.016 & 3514.49 & 1 \\ 
K01444.01 & 44.9 & 1.93 & 6.28 & 4.50 & 13.33 & 0.282 & 72.52 & 0 \\ 
K01445.01 & 7.2 & 0.98 & 4.55 & 1.55 & 5.12 & 0.081 & 449.09 & 1 \\ 
K01466.01 & 281.6 & 12.80 & 7.74 & 10.18 & 10.56 & 0.765 & 0.36 & 1 \\ 
K01474.01 & 69.7 & 6.18 & 3.48 & 12.30 & 13.26 & 0.377 & 34.65 & 0 \\ 
K01475.01 & 1.6 & 2.44 & 1.56 & 1.85 & 1.79 & 0.024 & 209.86 & 1 \\ 
K01475.02 & 9.5 & 3.08 & 2.83 & 2.34 & 3.22 & 0.078 & 20.11 & 1 \\ 
K01475.03 & 4.7 & 1.88 & 2.18 & 1.42 & 2.56 & 0.049 & 50.58 & 1 \\ 
K01478.01 & 76.1 & 4.93 & 7.47 & 5.00 & 8.08 & 0.347 & 6.02 & 1 \\ 
K01480.01 & 20.4 & 3.59 & 3.62 & 2.77 & 4.39 & 0.134 & 14.90 & 1 \\ 
K01494.01 & 8.2 & 2.54 & 2.70 & 2.19 & 3.21 & 0.072 & 29.75 & 1 \\ 
K01501.01 & 2.6 & 2.02 & 1.97 & 1.52 & 2.06 & 0.033 & 133.66 & 1 \\ 
K01510.01 & 0.8 & 2.02 & 1.25 & 1.45 & 1.49 & 0.016 & 766.20 & 1 \\ 
K01515.01 & 1.9 & 1.65 & 1.45 & 1.08 & 1.72 & 0.026 & 104.33 & 1 \\ 
K01515.02 & 7.1 & 2.05 & 0.97 & 1.34 & 2.63 & 0.061 & 18.92 & 0 \\ 
K01528.01 & 4.0 & 1.26 & 1.57 & 1.17 & 2.83 & 0.049 & 217.46 & 0 \\ 
K01530.01 & 13.0 & 1.48 & 3.38 & 2.02 & 6.04 & 0.108 & 154.53 & 0 \\ 
K01532.01 & 18.1 & 1.44 & 4.86 & 2.21 & 6.93 & 0.148 & 115.07 & 1 \\ 
K01533.01 & 6.2 & 1.18 & 3.06 & 1.26 & 3.72 & 0.067 & 227.97 & 1 \\ 
K01534.01 & 20.4 & 1.27 & 6.09 & 1.91 & 7.10 & 0.158 & 98.56 & 1 \\ 
K01534.02 & 7.6 & 0.78 & 3.87 & 1.17 & 5.14 & 0.083 & 360.95 & 1 \\ 
K01535.01 & 70.7 & 1.74 & 6.44 & 1.75 & 7.95 & 0.323 & 7.93 & 1 \\ 
K01536.01 & 3.7 & 0.79 & 2.86 & 1.25 & 4.29 & 0.052 & 850.23 & 1 \\ 
K01537.01 & 10.2 & 0.73 & 6.00 & 1.43 & 7.22 & 0.102 & 406.20 & 1 \\ 
K01552.01 & 77.6 & 11.43 & 3.65 & 9.32 & 7.01 & 0.329 & 2.27 & 0 \\ 
K01557.01 & 3.3 & 3.76 & 1.75 & 2.74 & 2.36 & 0.040 & 128.49 & 1 \\ 
K01557.02 & 9.7 & 3.24 & 2.79 & 2.36 & 3.36 & 0.082 & 31.10 & 1 \\ 
K01557.03 & 5.3 & 2.83 & 1.05 & 2.05 & 2.76 & 0.055 & 68.36 & 0 \\ 
K01557.04 & 1.5 & 1.46 & 1.37 & 1.06 & 1.82 & 0.024 & 363.45 & 1 \\ 
K01567.01 & 7.2 & 2.65 & 2.80 & 2.25 & 3.26 & 0.069 & 62.66 & 1 \\ 
K01567.02 & 4.6 & 1.92 & 2.31 & 1.63 & 2.82 & 0.051 & 112.54 & 1 \\ 
K01567.03 & 17.3 & 2.56 & 3.99 & 2.17 & 4.35 & 0.122 & 19.80 & 1 \\ 
K01567.04 & 44.8 & 2.93 & 5.23 & 2.49 & 5.96 & 0.228 & 5.65 & 1 \\ 
K01569.01 & 13.8 & 3.14 & 2.60 & 2.22 & 3.58 & 0.099 & 15.52 & 1 \\ 
K01576.01 & 10.4 & 2.62 & 2.63 & 2.64 & 4.09 & 0.095 & 81.05 & 1 \\ 
K01576.02 & 13.1 & 2.34 & 2.90 & 2.36 & 4.41 & 0.111 & 59.98 & 1 \\ 
K01577.01 & 2.8 & 2.24 & 1.61 & 1.56 & 2.11 & 0.035 & 90.33 & 1 \\ 
K01584.01 & 5.9 & 2.04 & 2.45 & 1.42 & 2.67 & 0.056 & 32.62 & 1 \\ 
K01586.01 & 7.0 & 2.11 & 2.07 & 1.69 & 3.12 & 0.067 & 48.22 & 1 \\ 
K01588.01 & 3.5 & 2.09 & 1.50 & 1.40 & 2.17 & 0.039 & 56.28 & 1 \\ 
K01596.01 & 5.9 & 1.85 & 2.57 & 1.54 & 2.97 & 0.060 & 55.89 & 1 \\ 
K01606.01 & 5.1 & 1.52 & 1.76 & 1.46 & 3.14 & 0.058 & 178.14 & 0 \\ 
K01608.01 & 9.2 & 1.33 & 4.20 & 1.66 & 4.77 & 0.089 & 179.14 & 1 \\ 
K01608.02 & 19.7 & 1.20 & 4.70 & 1.50 & 6.14 & 0.147 & 65.18 & 1 \\ 
K01608.03 & 232.0 & 1.61 & 10.98 & 2.00 & 13.86 & 0.747 & 2.52 & 1 \\ 
K01609.01 & 41.7 & 1.94 & 5.54 & 2.18 & 7.40 & 0.229 & 22.28 & 1 \\ 
K01612.01 & 2.5 & 0.52 & 1.22 & 0.71 & 3.35 & 0.038 & 1348.29 & 1 \\ 
K01615.01 & 1.3 & 0.96 & 1.59 & 1.36 & 2.73 & 0.026 & 2825.19 & 1 \\ 
K01616.01 & 13.9 & 1.07 & 2.48 & 1.40 & 5.52 & 0.122 & 116.76 & 0 \\ 
K01618.01 & 2.4 & 0.50 & 3.24 & 0.81 & 3.70 & 0.039 & 1909.57 & 1 \\ 
K01619.01 & 20.7 & 0.90 & 3.22 & 0.72 & 4.39 & 0.134 & 13.36 & 1 \\ 
K01621.01 & 20.3 & 1.19 & 5.22 & 2.54 & 9.72 & 0.162 & 174.76 & 0 \\ 
K01628.01 & 19.7 & 2.03 & 3.31 & 3.73 & 8.22 & 0.161 & 147.57 & 0 \\ 
K01628.02 & 1.8 & 0.83 & 2.40 & 1.52 & 3.71 & 0.033 & 3555.88 & 0 \\ 
K01629.01 & 4.4 & 1.06 & 2.08 & 1.46 & 4.05 & 0.056 & 508.55 & 0 \\ 
K01632.01 & 4.6 & 0.97 & 2.81 & 1.56 & 4.67 & 0.059 & 758.04 & 1 \\ 
K01649.01 & 4.0 & 1.83 & 1.40 & 1.20 & 2.33 & 0.043 & 39.04 & 1 \\ 
K01655.01 & 0.9 & 1.35 & 1.28 & 1.35 & 1.88 & 0.019 & 1952.77 & 1 \\ 
K01658.01 & 1.5 & 8.72 & 0.95 & 12.83 & 2.89 & 0.029 & 2844.87 & 0 \\ 
K01665.01 & 6.9 & 1.01 & 4.33 & 1.43 & 4.67 & 0.078 & 309.65 & 1 \\ 
K01669.01 & 61.0 & 1.94 & 8.08 & 2.76 & 9.81 & 0.319 & 20.61 & 1 \\ 
K01671.01 & 1.5 & 0.72 & 2.44 & 0.99 & 2.81 & 0.027 & 2379.44 & 1 \\ 
K01672.01 & 33.9 & 2.70 & 3.45 & 2.08 & 5.10 & 0.186 & 4.83 & 1 \\ 
K01687.01 & 3.9 & 1.92 & 2.13 & 1.44 & 2.47 & 0.044 & 91.09 & 1 \\ 
K01692.01 & 6.0 & 2.63 & 2.65 & 2.54 & 3.31 & 0.066 & 144.50 & 1 \\ 
K01692.02 & 2.5 & 0.84 & 2.13 & 0.80 & 2.47 & 0.037 & 464.45 & 1 \\ 
K01695.01 & 71.5 & 1.37 & 6.08 & 2.03 & 10.82 & 0.354 & 15.48 & 0 \\ 
K01706.01 & 1.9 & 1.52 & 1.73 & 1.39 & 2.24 & 0.029 & 480.59 & 1 \\ 
K01711.01 & 55.7 & 2.50 & 3.64 & 2.09 & 6.55 & 0.273 & 4.78 & 0 \\ 
K01713.01 & 6.8 & 2.15 & 2.29 & 1.56 & 2.86 & 0.063 & 29.63 & 1 \\ 
K01713.02 & 2.2 & 1.92 & 1.38 & 1.39 & 1.98 & 0.030 & 128.99 & 1 \\ 
K01715.01 & 105.0 & 1.58 & 6.28 & 1.98 & 11.15 & 0.425 & 7.35 & 0 \\ 
K01716.01 & 4.9 & 1.66 & 2.52 & 1.31 & 2.78 & 0.053 & 82.52 & 1 \\ 
K01738.01 & 4.2 & 1.17 & 2.21 & 1.09 & 2.88 & 0.051 & 201.48 & 1 \\ 
K01754.01 & 15.1 & 1.48 & 2.14 & 1.88 & 5.55 & 0.127 & 107.70 & 0 \\ 
K01779.01 & 4.7 & 3.70 & 2.62 & 3.97 & 3.30 & 0.058 & 316.81 & 1 \\ 
K01779.02 & 11.8 & 2.90 & 2.46 & 3.10 & 4.48 & 0.107 & 92.85 & 0 \\ 
K01783.01 & 134.5 & 7.23 & 4.09 & 9.04 & 11.37 & 0.532 & 5.07 & 0 \\ 
K01783.02 & 284.1 & 4.51 & 6.71 & 5.61 & 14.55 & 0.872 & 1.89 & 0 \\ 
K01788.01 & 71.5 & 6.85 & 5.48 & 5.20 & 6.65 & 0.309 & 2.34 & 1 \\ 
K01797.01 & 16.8 & 2.71 & 3.58 & 2.16 & 4.30 & 0.123 & 21.82 & 1 \\ 
K01800.01 & 7.8 & 34.38 & \nodata & 32.24 & 3.58 & 0.077 & 108.94 & 0 \\ 
K01802.01 & 5.2 & 2.26 & 1.77 & 2.45 & 3.46 & 0.061 & 282.45 & 0 \\ 
K01804.01 & 5.9 & 7.62 & \nodata & 6.90 & 3.21 & 0.062 & 95.33 & 0 \\ 
K01805.01 & 6.9 & 2.64 & 1.70 & 2.45 & 3.40 & 0.071 & 123.62 & 0 \\ 
K01805.02 & 31.8 & 2.19 & 3.74 & 2.03 & 5.62 & 0.194 & 16.59 & 1 \\ 
K01805.03 & 4.4 & 1.69 & 2.18 & 1.57 & 2.92 & 0.052 & 228.20 & 1 \\ 
K01806.02 & 17.9 & 1.10 & 5.22 & 1.48 & 6.29 & 0.142 & 96.02 & 1 \\ 
K01806.03 & 8.4 & 0.91 & 4.08 & 1.23 & 4.89 & 0.086 & 262.50 & 1 \\ 
K01813.01 & 9.8 & 2.21 & 1.90 & 2.01 & 3.74 & 0.088 & 68.69 & 0 \\ 
K01814.01 & 14.8 & 2.08 & 5.55 & 4.11 & 9.02 & 0.118 & 230.35 & 0 \\ 
K01815.01 & 3.1 & 2.54 & 1.15 & 1.96 & 2.36 & 0.039 & 138.94 & 0 \\ 
K01818.01 & 16.9 & 2.61 & 3.64 & 2.44 & 4.58 & 0.128 & 37.37 & 1 \\ 
K01819.01 & 12.1 & 2.09 & 2.26 & 1.83 & 3.93 & 0.101 & 51.01 & 0 \\ 
K01820.01 & 4.3 & 1.72 & 2.44 & 1.52 & 2.82 & 0.052 & 191.95 & 1 \\ 
K01820.02 & 1.7 & 1.03 & 1.66 & 0.90 & 2.05 & 0.027 & 685.31 & 1 \\ 
K01822.01 & 150.9 & 2.33 & 8.35 & 2.73 & 11.22 & 0.561 & 4.40 & 1 \\ 
K01824.01 & 3.6 & 1.28 & 2.99 & 1.52 & 3.35 & 0.047 & 604.82 & 1 \\ 
K01824.02 & 1.7 & 1.12 & 2.33 & 1.33 & 2.61 & 0.029 & 1628.20 & 1 \\ 
K01825.01 & 13.5 & 2.40 & 3.85 & 2.10 & 4.09 & 0.109 & 41.61 & 1 \\ 
K01826.01 & 134.3 & 2.65 & 8.69 & 3.16 & 11.05 & 0.519 & 4.75 & 1 \\ 
K01831.01 & 51.8 & 3.87 & 5.72 & 3.54 & 6.57 & 0.265 & 6.73 & 0 \\ 
K01831.02 & 4.4 & 1.28 & 2.46 & 1.18 & 2.91 & 0.052 & 175.23 & 1 \\ 
K01831.04 & 14.0 & 1.74 & 1.09 & 1.60 & 4.26 & 0.112 & 37.93 & 0 \\ 
K01833.01 & 3.7 & 2.54 & 1.66 & 1.85 & 2.40 & 0.043 & 83.08 & 1 \\ 
K01833.02 & 7.7 & 3.12 & 1.09 & 2.28 & 3.05 & 0.069 & 31.58 & 0 \\ 
K01833.03 & 5.7 & 2.23 & 1.53 & 1.63 & 2.77 & 0.057 & 46.75 & 0 \\ 
K01837.01 & 34.2 & 2.28 & 4.43 & 1.96 & 5.48 & 0.200 & 10.59 & 1 \\ 
K01837.02 & 1.7 & 1.09 & 1.85 & 0.93 & 2.03 & 0.027 & 563.77 & 1 \\ 
K01838.01 & 16.7 & 3.08 & 1.77 & 2.15 & 3.88 & 0.115 & 10.92 & 0 \\ 
K01843.01 & 4.2 & 2.34 & 1.63 & 1.39 & 2.19 & 0.042 & 25.99 & 1 \\ 
K01845.01 & 2.0 & 1.80 & 1.68 & 1.62 & 2.11 & 0.029 & 261.31 & 1 \\ 
K01845.02 & 5.1 & 2.49 & \nodata & 2.24 & 2.88 & 0.054 & 75.28 & 1 \\ 
K01850.01 & 11.6 & 1.85 & 3.26 & 2.54 & 5.62 & 0.103 & 150.95 & 0 \\ 
K01854.01 & 43.0 & 2.13 & 5.90 & 2.17 & 6.61 & 0.240 & 13.05 & 1 \\ 
K01856.01 & 46.3 & 2.66 & 5.06 & 2.25 & 6.00 & 0.242 & 7.08 & 1 \\ 
K01860.01 & 6.3 & 2.20 & 3.14 & 2.41 & 3.70 & 0.069 & 198.49 & 1 \\ 
K01860.02 & 12.2 & 2.13 & 3.93 & 2.32 & 4.59 & 0.107 & 83.21 & 1 \\ 
K01860.03 & 3.1 & 1.35 & 2.54 & 1.47 & 2.91 & 0.043 & 513.35 & 1 \\ 
K01861.01 & 17.5 & 2.48 & 4.12 & 2.77 & 5.26 & 0.138 & 65.89 & 1 \\ 
K01863.01 & 33.8 & 2.36 & 5.30 & 2.85 & 6.89 & 0.217 & 29.84 & 1 \\ 
K01864.01 & 3.2 & 1.15 & 3.80 & 2.25 & 5.12 & 0.046 & 1351.43 & 1 \\ 
K01867.01 & 2.5 & 2.04 & 1.66 & 1.34 & 1.99 & 0.032 & 74.24 & 1 \\ 
K01867.02 & 14.0 & 3.05 & 1.36 & 2.01 & 3.48 & 0.097 & 7.86 & 0 \\ 
K01867.03 & 5.2 & 1.90 & 2.05 & 1.25 & 2.51 & 0.051 & 28.89 & 1 \\ 
K01868.01 & 17.8 & 3.29 & 1.58 & 2.27 & 3.83 & 0.115 & 6.34 & 0 \\ 
K01871.01 & 92.7 & 3.18 & 6.03 & 2.55 & 7.23 & 0.365 & 1.33 & 1 \\ 
K01871.02 & 32.4 & 2.46 & 3.93 & 1.96 & 5.11 & 0.182 & 5.34 & 1 \\ 
K01874.01 & 18.7 & 3.23 & 3.63 & 2.57 & 4.01 & 0.121 & 8.70 & 1 \\ 
K01874.02 & 7.4 & 2.06 & 2.06 & 1.63 & 2.96 & 0.066 & 29.44 & 1 \\ 
K01876.01 & 82.5 & 3.92 & 4.62 & 2.73 & 6.29 & 0.320 & 1.15 & 1 \\ 
K01877.01 & 20.2 & 1.68 & 3.56 & 1.33 & 4.50 & 0.136 & 15.50 & 1 \\ 
K01878.01 & 40.8 & 1.92 & 2.63 & 2.86 & 8.61 & 0.254 & 37.31 & 0 \\ 
K01879.01 & 22.1 & 5.03 & 1.99 & 3.24 & 4.03 & 0.131 & 4.16 & 0 \\ 
K01880.01 & 1.2 & 2.21 & 1.07 & 1.43 & 1.51 & 0.019 & 200.64 & 1 \\ 
K01883.01 & 2.7 & 0.77 & 3.35 & 1.33 & 4.21 & 0.041 & 1605.22 & 1 \\ 
K01886.01 & 6.0 & 1.27 & 1.61 & 2.20 & 5.31 & 0.072 & 635.00 & 0 \\ 
K01888.01 & 120.0 & 2.76 & 10.96 & 5.44 & 15.86 & 0.534 & 16.66 & 1 \\ 
K01891.01 & 16.0 & 2.49 & 3.84 & 2.14 & 4.37 & 0.119 & 25.92 & 1 \\ 
K01891.02 & 8.3 & 1.56 & 2.84 & 1.34 & 3.52 & 0.077 & 61.82 & 1 \\ 
K01893.01 & 3.6 & 1.42 & 2.06 & 2.00 & 4.11 & 0.045 & 765.06 & 0 \\ 
K01895.01 & 8.5 & 3.33 & 2.19 & 2.41 & 3.15 & 0.074 & 28.73 & 1 \\ 
K01895.02 & 17.3 & 3.62 & 2.71 & 2.62 & 3.99 & 0.118 & 11.18 & 1 \\ 
K01897.01 & 59.8 & 2.22 & 4.28 & 2.82 & 9.07 & 0.302 & 15.64 & 0 \\ 
K01898.01 & 6.5 & 1.27 & 2.25 & 1.62 & 4.40 & 0.070 & 271.54 & 0 \\ 
K01904.01 & 12.4 & 1.45 & 3.07 & 1.16 & 3.90 & 0.100 & 34.49 & 1 \\ 
K01905.01 & 7.6 & 1.56 & 2.36 & 1.17 & 3.16 & 0.071 & 54.82 & 1 \\ 
K01905.02 & 16.0 & 1.35 & 3.37 & 1.02 & 4.04 & 0.115 & 20.62 & 1 \\ 
K01905.03 & 34.2 & 1.49 & 4.86 & 1.12 & 5.19 & 0.190 & 7.56 & 1 \\ 
K01908.01 & 12.6 & 2.00 & 3.02 & 1.46 & 3.52 & 0.094 & 14.29 & 1 \\ 
K01908.02 & 24.1 & 1.77 & 3.81 & 1.29 & 4.36 & 0.144 & 6.04 & 1 \\ 
K01909.01 & 12.8 & 1.26 & 4.10 & 1.38 & 4.67 & 0.110 & 88.95 & 1 \\ 
K01909.02 & 5.5 & 0.98 & 3.12 & 1.07 & 3.53 & 0.063 & 272.03 & 1 \\ 
K01909.03 & 25.1 & 1.20 & 2.65 & 1.31 & 5.84 & 0.173 & 36.41 & 0 \\ 
K01913.01 & 5.5 & 1.30 & 2.90 & 1.27 & 3.25 & 0.062 & 171.69 & 1 \\ 
K01915.01 & 6.6 & 1.48 & 3.88 & 2.89 & 6.07 & 0.078 & 579.40 & 1 \\ 
K01915.02 & 67.8 & 1.34 & 11.21 & 2.61 & 13.12 & 0.363 & 26.54 & 1 \\ 
K01917.01 & 35.0 & 1.92 & 2.50 & 2.29 & 7.10 & 0.214 & 28.57 & 0 \\ 
K01921.01 & 16.0 & 1.81 & 6.33 & 2.86 & 6.67 & 0.138 & 167.84 & 1 \\ 
K01923.01 & 7.2 & 1.95 & 2.09 & 1.85 & 3.50 & 0.074 & 108.08 & 0 \\ 
K01925.01 & 69.0 & 1.02 & 3.03 & 1.00 & 7.59 & 0.324 & 5.89 & 0 \\ 
K01928.01 & 63.0 & 2.35 & 7.11 & 2.78 & 8.34 & 0.325 & 11.78 & 1 \\ 
K01929.01 & 9.7 & 1.09 & 5.48 & 2.16 & 7.43 & 0.094 & 328.27 & 1 \\ 
K01929.02 & 3.3 & 0.82 & 4.65 & 1.63 & 5.20 & 0.046 & 1365.15 & 1 \\ 
K01930.01 & 13.7 & 1.31 & 7.13 & 2.54 & 8.15 & 0.119 & 228.37 & 1 \\ 
K01930.02 & 24.3 & 1.25 & 8.53 & 2.43 & 9.84 & 0.174 & 107.39 & 1 \\ 
K01930.03 & 44.4 & 1.43 & 9.97 & 2.77 & 12.01 & 0.258 & 48.45 & 1 \\ 
K01930.04 & 9.3 & 0.84 & 6.04 & 1.62 & 7.18 & 0.092 & 379.57 & 1 \\ 
K01934.01 & 28.8 & 2.65 & 3.30 & 2.01 & 4.83 & 0.168 & 6.48 & 1 \\ 
K01937.01 & 1.4 & 1.77 & 1.36 & 1.30 & 1.72 & 0.022 & 264.43 & 1 \\ 
K01938.01 & 96.9 & 2.65 & 5.78 & 2.18 & 7.64 & 0.380 & 2.37 & 1 \\ 
K01940.01 & 11.0 & 2.69 & 1.55 & 1.88 & 3.27 & 0.085 & 15.24 & 0 \\ 
K01944.01 & 12.2 & 2.06 & 2.38 & 1.99 & 4.22 & 0.105 & 71.12 & 0 \\ 
K01947.01 & 6.4 & 1.49 & 1.09 & 2.01 & 4.41 & 0.073 & 318.26 & 0 \\ 
K01955.01 & 15.2 & 1.38 & 3.96 & 2.07 & 6.36 & 0.131 & 146.67 & 1 \\ 
K01955.03 & 1.6 & 0.64 & 2.71 & 0.96 & 3.06 & 0.030 & 2755.38 & 1 \\ 
K01955.04 & 26.2 & 1.24 & 2.71 & 1.85 & 7.63 & 0.188 & 71.18 & 0 \\ 
K01959.01 & 36.5 & 2.64 & 3.40 & 1.96 & 5.25 & 0.197 & 6.52 & 1 \\ 
K01960.01 & 9.0 & 1.41 & 4.26 & 1.87 & 4.92 & 0.089 & 183.25 & 1 \\ 
K01960.02 & 23.2 & 1.34 & 2.52 & 1.76 & 6.74 & 0.166 & 52.20 & 0 \\ 
K01980.01 & 122.9 & 2.45 & 6.99 & 2.30 & 8.84 & 0.478 & 2.69 & 1 \\ 
K01984.01 & 22.1 & 1.82 & 3.47 & 2.30 & 6.22 & 0.163 & 57.29 & 0 \\ 
K01985.01 & 5.8 & 2.29 & 0.97 & 1.87 & 3.01 & 0.059 & 85.14 & 0 \\ 
K01988.01 & 0.9 & 1.48 & 1.36 & 1.16 & 1.59 & 0.018 & 638.83 & 1 \\ 
K01989.01 & 201.1 & 2.21 & 9.94 & 2.37 & 11.47 & 0.673 & 1.99 & 1 \\ 
K02001.01 & 8.3 & 1.28 & 2.61 & 1.07 & 3.50 & 0.078 & 66.93 & 1 \\ 
K02004.01 & 56.2 & 1.70 & 6.00 & 3.01 & 11.72 & 0.304 & 25.31 & 0 \\ 
K02004.02 & 3.2 & 0.75 & 2.67 & 1.32 & 4.55 & 0.046 & 1116.80 & 0 \\ 
K02006.01 & 3.3 & 1.48 & 1.68 & 0.94 & 2.10 & 0.037 & 49.89 & 1 \\ 
K02007.01 & 15.4 & 1.26 & 4.48 & 1.37 & 4.96 & 0.126 & 67.94 & 1 \\ 
K02007.02 & 21.1 & 1.22 & 3.76 & 1.33 & 5.50 & 0.155 & 44.67 & 1 \\ 
K02009.01 & 86.7 & 2.14 & 8.83 & 2.56 & 10.12 & 0.369 & 7.90 & 1 \\ 
K02010.01 & 26.0 & 1.74 & 6.10 & 2.68 & 7.71 & 0.189 & 82.95 & 1 \\ 
K02011.01 & 7.1 & 1.07 & 1.96 & 1.52 & 4.67 & 0.079 & 408.73 & 0 \\ 
K02011.02 & 17.3 & 0.77 & 4.85 & 1.10 & 6.28 & 0.143 & 125.47 & 1 \\ 
K02013.01 & 2.4 & 1.25 & 1.26 & 0.88 & 2.00 & 0.031 & 111.72 & 1 \\ 
K02016.01 & 4.3 & 1.48 & 3.79 & 2.26 & 4.30 & 0.057 & 635.87 & 1 \\ 
K02017.01 & 2.3 & 1.22 & 1.55 & 1.15 & 2.39 & 0.035 & 588.15 & 1 \\ 
K02025.01 & 17.8 & 1.83 & 5.44 & 2.75 & 6.54 & 0.149 & 129.87 & 0 \\ 
K02025.02 & 26.1 & 1.77 & 6.41 & 2.65 & 7.42 & 0.191 & 78.50 & 0 \\ 
K02025.03 & 11.2 & 1.11 & 5.15 & 1.66 & 5.61 & 0.109 & 240.53 & 0 \\ 
K02026.01 & 2.8 & 1.35 & 2.00 & 1.45 & 2.79 & 0.040 & 708.64 & 1 \\ 
K02029.01 & 16.3 & 1.59 & 2.00 & 1.25 & 4.23 & 0.119 & 26.72 & 0 \\ 
K02029.02 & 10.1 & 1.11 & 2.89 & 0.87 & 3.60 & 0.087 & 50.69 & 1 \\ 
K02029.03 & 6.9 & 0.84 & 2.13 & 0.66 & 3.18 & 0.067 & 83.54 & 1 \\ 
K02031.01 & 9.3 & 2.28 & 1.86 & 1.83 & 3.36 & 0.079 & 25.61 & 0 \\ 
K02035.01 & 1.9 & 2.05 & 1.47 & 1.96 & 2.28 & 0.031 & 676.60 & 1 \\ 
K02036.01 & 8.4 & 2.52 & 2.13 & 1.74 & 3.02 & 0.070 & 18.16 & 1 \\ 
K02036.02 & 5.8 & 1.69 & 2.13 & 1.16 & 2.67 & 0.055 & 29.70 & 1 \\ 
K02040.01 & 19.6 & 2.10 & 1.36 & 2.29 & 5.49 & 0.143 & 44.31 & 0 \\ 
K02042.01 & 63.1 & 2.39 & 5.06 & 5.84 & 17.95 & 0.307 & 49.94 & 0 \\ 
K02043.01 & 78.5 & 2.36 & 8.36 & 2.97 & 9.81 & 0.364 & 10.12 & 1 \\ 
K02045.01 & 5.5 & 2.29 & 2.40 & 1.74 & 2.73 & 0.055 & 50.81 & 1 \\ 
K02046.01 & 23.9 & 1.56 & 15.33 & 2.71 & 8.85 & 0.170 & 73.84 & 1 \\ 
K02047.01 & 6.2 & 1.19 & 3.26 & 1.55 & 4.24 & 0.071 & 361.63 & 1 \\ 
K02049.01 & 1.6 & 1.12 & 2.71 & 1.63 & 3.01 & 0.028 & 2443.79 & 1 \\ 
K02053.01 & 13.1 & 1.30 & 3.46 & 1.99 & 6.22 & 0.119 & 179.87 & 0 \\ 
K02053.02 & 4.6 & 1.07 & 2.97 & 1.63 & 4.41 & 0.060 & 714.96 & 1 \\ 
K02057.01 & 5.9 & 1.84 & 2.08 & 1.19 & 2.58 & 0.055 & 23.23 & 1 \\ 
K02060.01 & 2.8 & 2.44 & 0.95 & 1.92 & 2.31 & 0.037 & 172.85 & 1 \\ 
K02071.01 & 3.9 & 1.04 & 2.00 & 0.95 & 2.78 & 0.048 & 212.99 & 1 \\ 
K02072.01 & 1.5 & 0.88 & 2.57 & 1.30 & 3.19 & 0.027 & 2554.84 & 1 \\ 
K02073.01 & 49.5 & 2.80 & 5.55 & 2.20 & 6.06 & 0.247 & 4.94 & 1 \\ 
K02073.02 & 6.5 & 2.09 & 2.60 & 1.63 & 3.10 & 0.065 & 72.44 & 1 \\ 
K02073.03 & 16.9 & 2.50 & 1.95 & 1.96 & 4.25 & 0.121 & 20.49 & 0 \\ 
K02078.01 & 18.8 & 2.85 & 2.94 & 2.05 & 4.07 & 0.124 & 8.64 & 1 \\ 
K02078.02 & 161.5 & 4.24 & 6.18 & 3.06 & 8.27 & 0.511 & 0.50 & 1 \\ 
K02079.01 & 0.7 & 0.65 & 1.56 & 0.69 & 1.75 & 0.016 & 2926.81 & 1 \\ 
K02082.01 & 31.6 & 1.76 & 3.32 & 2.63 & 8.04 & 0.213 & 46.74 & 0 \\ 
K02086.01 & 7.1 & 1.11 & 4.25 & 1.75 & 5.51 & 0.075 & 370.69 & 1 \\ 
K02086.02 & 8.9 & 1.24 & 4.03 & 1.96 & 5.93 & 0.087 & 276.00 & 1 \\ 
K02086.03 & 11.9 & 1.12 & 2.30 & 1.76 & 6.52 & 0.105 & 188.66 & 0 \\ 
K02087.01 & 23.1 & 1.16 & 4.70 & 1.28 & 5.72 & 0.165 & 43.30 & 1 \\ 
K02090.01 & 5.1 & 2.71 & 1.42 & 1.67 & 2.41 & 0.049 & 22.43 & 0 \\ 
K02101.01 & 2.9 & 1.73 & 1.30 & 1.32 & 2.21 & 0.036 & 99.95 & 1 \\ 
K02105.01 & 6.4 & 1.17 & 2.60 & 1.29 & 3.76 & 0.070 & 226.42 & 1 \\ 
K02109.01 & 19.8 & 1.81 & 3.12 & 3.26 & 8.34 & 0.156 & 129.31 & 0 \\ 
K02110.01 & 5.0 & 0.81 & 1.86 & 1.28 & 4.53 & 0.065 & 727.32 & 0 \\ 
K02114.01 & 4.4 & 2.35 & 1.93 & 1.61 & 2.42 & 0.046 & 44.29 & 1 \\ 
K02119.01 & 0.6 & 1.41 & 1.07 & 1.19 & 1.46 & 0.013 & 2243.19 & 1 \\ 
K02120.01 & 8.8 & 1.41 & 2.05 & 1.10 & 3.41 & 0.079 & 51.50 & 1 \\ 
K02126.01 & 9.7 & 3.06 & 2.62 & 2.36 & 3.38 & 0.081 & 31.81 & 1 \\ 
K02130.01 & 16.9 & 2.69 & 2.24 & 1.90 & 3.83 & 0.112 & 7.60 & 0 \\ 
K02135.01 & 55.2 & 1.80 & 8.82 & 2.91 & 10.49 & 0.307 & 29.32 & 1 \\ 
K02135.02 & 20.2 & 0.98 & 6.01 & 1.58 & 7.53 & 0.158 & 110.55 & 1 \\ 
K02135.03 & 8.5 & 0.98 & 5.15 & 1.57 & 5.66 & 0.089 & 347.06 & 1 \\ 
K02137.01 & 15.0 & 1.48 & 2.43 & 1.32 & 4.34 & 0.114 & 35.81 & 0 \\ 
K02143.01 & 4.8 & 1.09 & 2.66 & 1.02 & 3.03 & 0.056 & 186.17 & 1 \\ 
K02146.01 & 2.9 & 1.71 & 1.97 & 1.37 & 2.37 & 0.038 & 170.09 & 1 \\ 
K02148.01 & 11.9 & 1.22 & 6.06 & 2.15 & 6.88 & 0.111 & 179.93 & 1 \\ 
K02148.02 & 7.5 & 1.05 & 4.62 & 1.84 & 5.91 & 0.082 & 329.65 & 1 \\ 
K02149.01 & 13.2 & 0.92 & 5.19 & 1.47 & 6.36 & 0.122 & 193.88 & 1 \\ 
K02153.01 & 60.0 & 1.56 & 6.78 & 2.22 & 9.97 & 0.311 & 20.50 & 1 \\ 
K02153.02 & 25.7 & 1.10 & 6.84 & 1.57 & 7.55 & 0.178 & 62.61 & 1 \\ 
K02158.01 & 4.6 & 0.83 & 2.68 & 0.84 & 3.27 & 0.053 & 225.37 & 1 \\ 
K02158.02 & 6.7 & 0.64 & 3.13 & 0.65 & 3.71 & 0.068 & 136.17 & 1 \\ 
K02159.01 & 7.6 & 1.04 & 3.55 & 1.12 & 3.88 & 0.078 & 155.58 & 1 \\ 
K02162.01 & 108.6 & 1.70 & 7.76 & 1.69 & 9.30 & 0.419 & 4.33 & 1 \\ 
K02162.02 & 199.7 & 1.47 & 8.65 & 1.45 & 11.38 & 0.626 & 1.94 & 1 \\ 
K02169.01 & 5.5 & 0.85 & 2.07 & 0.80 & 3.18 & 0.061 & 154.22 & 1 \\ 
K02169.02 & 3.3 & 0.71 & 2.03 & 0.67 & 2.68 & 0.043 & 303.30 & 1 \\ 
K02173.01 & 37.8 & 1.53 & 4.51 & 1.18 & 5.42 & 0.204 & 5.55 & 1 \\ 
K02191.01 & 8.8 & 1.94 & 2.01 & 1.27 & 3.01 & 0.072 & 14.10 & 1 \\ 
K02193.01 & 2.4 & 2.19 & 1.20 & 1.50 & 1.92 & 0.030 & 121.30 & 1 \\ 
K02194.01 & 34.8 & 1.58 & 4.15 & 2.17 & 8.41 & 0.206 & 36.01 & 0 \\ 
K02194.02 & 68.0 & 1.66 & 7.70 & 2.27 & 10.50 & 0.321 & 14.86 & 1 \\ 
K02202.01 & 0.8 & 1.20 & 1.36 & 1.06 & 1.63 & 0.017 & 1641.70 & 1 \\ 
K02204.01 & 10.9 & 1.29 & 2.25 & 2.41 & 7.06 & 0.106 & 359.57 & 0 \\ 
K02205.01 & 24.1 & 2.94 & 2.03 & 2.38 & 4.65 & 0.149 & 9.64 & 0 \\ 
K02208.01 & 2.3 & 0.72 & 1.36 & 0.88 & 2.99 & 0.036 & 999.50 & 1 \\ 
K02210.01 & 2.9 & 1.82 & 1.54 & 1.33 & 2.27 & 0.037 & 184.62 & 1 \\ 
K02210.02 & 210.6 & 3.67 & 7.80 & 2.69 & 9.35 & 0.627 & 0.64 & 1 \\ 
K02214.01 & 2.4 & 1.62 & 1.69 & 1.28 & 2.16 & 0.032 & 193.88 & 1 \\ 
K02225.01 & 2.8 & 1.26 & 1.98 & 0.96 & 2.26 & 0.036 & 154.87 & 1 \\ 
K02238.01 & 1.6 & 1.56 & 1.19 & 1.03 & 1.72 & 0.024 & 134.35 & 1 \\ 
K02246.01 & 11.9 & 1.25 & 3.34 & 1.26 & 4.39 & 0.101 & 80.00 & 1 \\ 
K02247.01 & 4.5 & 1.20 & 2.26 & 0.93 & 2.63 & 0.049 & 72.87 & 1 \\ 
K02250.01 & 2.9 & 2.94 & 1.35 & 2.44 & 2.45 & 0.039 & 219.95 & 1 \\ 
K02250.02 & 0.6 & 1.90 & 1.13 & 1.57 & 1.47 & 0.014 & 1690.07 & 1 \\ 
K02252.01 & 13.5 & 1.08 & 4.27 & 2.66 & 9.49 & 0.128 & 376.43 & 0 \\ 
K02256.01 & 10.7 & 3.14 & 2.53 & 2.37 & 3.50 & 0.087 & 25.63 & 1 \\ 
K02260.01 & 6.1 & 0.72 & 3.39 & 1.05 & 4.66 & 0.071 & 455.64 & 1 \\ 
K02261.01 & 4.0 & 1.31 & 2.16 & 1.08 & 2.75 & 0.048 & 178.62 & 1 \\ 
K02266.01 & 1.0 & 2.02 & 1.39 & 1.72 & 1.66 & 0.018 & 698.65 & 1 \\ 
K02273.01 & 6.1 & 0.71 & 2.31 & 0.93 & 4.19 & 0.071 & 335.08 & 0 \\ 
K02278.01 & 14.2 & 1.45 & 2.47 & 2.27 & 6.87 & 0.118 & 152.33 & 0 \\ 
K02278.02 & 4.9 & 0.83 & 3.98 & 1.29 & 4.85 & 0.058 & 615.54 & 1 \\ 
K02279.01 & 27.0 & 1.57 & 5.22 & 2.03 & 6.93 & 0.184 & 45.55 & 1 \\ 
K02279.02 & 12.5 & 1.15 & 3.34 & 1.49 & 5.37 & 0.110 & 125.83 & 1 \\ 
K02281.01 & 0.8 & 0.97 & 0.98 & 0.82 & 1.60 & 0.016 & 1450.62 & 1 \\ 
K02289.01 & 62.8 & 1.67 & 4.65 & 2.34 & 9.75 & 0.327 & 18.19 & 0 \\ 
K02289.02 & 20.1 & 1.16 & 5.07 & 1.63 & 6.70 & 0.154 & 81.79 & 1 \\ 
K02300.01 & 2.7 & 1.46 & 1.03 & 1.19 & 2.35 & 0.036 & 277.48 & 1 \\ 
K02311.03 & 104.4 & 1.44 & 3.58 & 2.10 & 12.44 & 0.441 & 8.15 & 0 \\ 
K02318.01 & 10.5 & 1.59 & 3.03 & 1.11 & 3.33 & 0.084 & 24.33 & 1 \\ 
K02319.01 & 21.1 & 1.29 & 2.00 & 1.72 & 6.51 & 0.158 & 73.40 & 0 \\ 
K02329.01 & 1.6 & 2.08 & 0.97 & 1.36 & 1.70 & 0.023 & 129.23 & 1 \\ 
K02331.01 & 2.8 & 0.98 & 2.32 & 1.49 & 3.81 & 0.042 & 1135.08 & 1 \\ 
K02339.01 & 2.0 & 1.59 & 1.03 & 1.20 & 2.03 & 0.029 & 227.58 & 1 \\ 
K02344.01 & 1.1 & 1.39 & 1.50 & 1.11 & 1.67 & 0.020 & 416.10 & 1 \\ 
K02352.01 & 13.4 & 0.65 & 3.32 & 1.03 & 6.47 & 0.120 & 212.92 & 0 \\ 
K02352.02 & 5.6 & 0.58 & 3.71 & 0.92 & 4.86 & 0.068 & 668.43 & 1 \\ 
K02352.03 & 8.3 & 0.57 & 1.98 & 0.90 & 5.51 & 0.087 & 403.16 & 0 \\ 
K02355.01 & 1.2 & 1.94 & 1.33 & 1.47 & 1.74 & 0.021 & 506.30 & 1 \\ 
K02358.01 & 56.5 & 1.88 & 8.26 & 3.32 & 11.15 & 0.322 & 34.43 & 1 \\ 
K02365.01 & 36.0 & 1.51 & 2.64 & 2.23 & 8.42 & 0.228 & 38.05 & 0 \\ 
K02365.02 & 111.0 & 1.12 & 11.47 & 1.64 & 12.21 & 0.480 & 8.60 & 1 \\ 
K02366.01 & 25.4 & 0.97 & 4.55 & 1.33 & 7.07 & 0.180 & 61.60 & 1 \\ 
K02367.01 & 6.9 & 0.85 & 1.65 & 1.34 & 5.18 & 0.078 & 411.26 & 0 \\ 
K02372.01 & 5.3 & 0.87 & 4.10 & 1.37 & 4.94 & 0.063 & 581.73 & 1 \\ 
K02389.01 & 22.9 & 1.10 & 7.81 & 1.67 & 7.85 & 0.162 & 75.23 & 1 \\ 
K02390.01 & 16.1 & 1.03 & 5.56 & 3.04 & 11.97 & 0.144 & 382.37 & 0 \\ 
K02393.01 & 4.6 & 1.57 & 2.60 & 1.25 & 2.71 & 0.050 & 94.00 & 1 \\ 
K02393.02 & 0.8 & 1.41 & 1.22 & 1.12 & 1.50 & 0.015 & 1001.44 & 1 \\ 
K02399.01 & 1.9 & 0.94 & 1.37 & 0.76 & 2.10 & 0.029 & 406.01 & 1 \\ 
K02401.01 & 38.2 & 2.26 & 3.61 & 2.36 & 6.26 & 0.210 & 6.10 & 0 \\ 
K02402.01 & 16.3 & 1.46 & 3.71 & 1.24 & 4.19 & 0.117 & 15.19 & 1 \\ 
K02403.01 & 13.3 & 1.00 & 3.80 & 1.29 & 5.32 & 0.119 & 126.89 & 1 \\ 
K02408.01 & 94.3 & 2.07 & 3.89 & 2.09 & 8.79 & 0.391 & 4.44 & 0 \\ 
K02414.01 & 22.6 & 1.10 & 6.05 & 1.93 & 9.42 & 0.154 & 93.44 & 1 \\ 
K02414.02 & 45.3 & 1.17 & 4.64 & 2.06 & 11.85 & 0.244 & 37.26 & 0 \\ 
K02426.01 & 4.2 & 0.80 & 2.54 & 0.81 & 3.13 & 0.050 & 245.64 & 1 \\ 
K02443.01 & 6.8 & 0.94 & 3.24 & 1.16 & 4.52 & 0.069 & 266.75 & 1 \\ 
K02443.02 & 11.8 & 0.90 & 3.20 & 1.11 & 5.43 & 0.099 & 128.12 & 0 \\ 
K02462.01 & 12.1 & 0.77 & 6.11 & 1.45 & 7.31 & 0.113 & 252.39 & 1 \\ 
K02480.01 & 0.7 & 2.11 & 0.72 & 1.51 & 1.34 & 0.013 & 615.01 & 1 \\ 
K02484.01 & 68.9 & 1.11 & 5.72 & 1.79 & 12.36 & 0.323 & 20.18 & 0 \\ 
K02485.01 & 10.0 & 1.79 & 2.56 & 1.33 & 3.43 & 0.084 & 38.06 & 1 \\ 
K02485.02 & 3.6 & 1.56 & 1.88 & 1.16 & 2.45 & 0.043 & 146.39 & 1 \\ 
K02485.03 & 5.7 & 1.60 & 2.15 & 1.18 & 2.86 & 0.058 & 79.34 & 1 \\ 
K02488.01 & 12.4 & 0.96 & 4.18 & 1.49 & 6.41 & 0.110 & 181.85 & 1 \\ 
K02490.01 & 11.6 & 2.52 & 2.08 & 1.90 & 3.61 & 0.092 & 26.15 & 0 \\ 
K02492.01 & 1.0 & 0.83 & 1.91 & 0.99 & 2.32 & 0.019 & 3023.14 & 1 \\ 
K02497.01 & 48.4 & 2.69 & 3.66 & 2.10 & 6.01 & 0.243 & 5.07 & 1 \\ 
K02498.01 & 6.7 & 0.88 & 2.52 & 0.78 & 3.34 & 0.067 & 91.79 & 1 \\ 
K02503.01 & 14.8 & 1.22 & 3.85 & 1.04 & 4.15 & 0.111 & 21.48 & 1 \\ 
K02519.01 & 4.8 & 2.13 & 0.37 & 1.61 & 2.66 & 0.051 & 60.76 & 0 \\ 
K02520.01 & 6.5 & 1.71 & 2.13 & 1.30 & 2.94 & 0.062 & 46.96 & 1 \\ 
K02521.01 & 28.5 & 2.50 & 4.31 & 1.97 & 4.92 & 0.167 & 9.98 & 1 \\ 
K02521.02 & 4.9 & 1.74 & 1.72 & 1.37 & 2.75 & 0.052 & 102.74 & 1 \\ 
K02522.01 & 5.6 & 1.37 & 0.99 & 1.16 & 3.01 & 0.058 & 78.65 & 0 \\ 
K02525.01 & 57.3 & 2.51 & 4.68 & 1.87 & 6.06 & 0.263 & 2.88 & 1 \\ 
K02527.01 & 1.4 & 0.86 & 1.55 & 0.62 & 1.71 & 0.022 & 268.34 & 1 \\ 
K02529.01 & 16.8 & 2.88 & 3.29 & 2.12 & 3.98 & 0.116 & 13.16 & 1 \\ 
K02529.02 & 64.0 & 3.01 & 4.35 & 2.21 & 6.19 & 0.281 & 2.25 & 1 \\ 
K02530.01 & 37.3 & 1.25 & 7.24 & 2.39 & 10.76 & 0.239 & 56.93 & 1 \\ 
K02531.01 & 17.7 & 2.48 & 2.66 & 1.88 & 4.19 & 0.123 & 14.43 & 1 \\ 
K02534.01 & 3.0 & 1.05 & 2.87 & 1.33 & 3.25 & 0.044 & 850.61 & 1 \\ 
K02535.01 & 48.9 & 1.84 & 4.70 & 1.56 & 6.24 & 0.246 & 5.31 & 1 \\ 
K02548.01 & 0.8 & 1.49 & 1.32 & 1.23 & 1.51 & 0.016 & 826.75 & 1 \\ 
K02555.01 & 12.6 & 0.86 & 4.58 & 1.04 & 5.04 & 0.112 & 127.62 & 1 \\ 
K02556.01 & 40.8 & 1.49 & 4.83 & 1.38 & 6.16 & 0.225 & 11.76 & 1 \\ 
K02559.01 & 9.3 & 0.99 & 3.35 & 1.20 & 4.59 & 0.091 & 157.69 & 1 \\ 
K02560.01 & 18.1 & 2.03 & 3.67 & 1.58 & 4.13 & 0.122 & 13.53 & 1 \\ 
K02561.01 & 3.2 & 0.82 & 2.51 & 1.24 & 3.96 & 0.046 & 1034.47 & 1 \\ 
K02563.01 & 23.5 & 1.11 & 6.57 & 2.36 & 10.02 & 0.181 & 141.43 & 1 \\ 
K02564.01 & 66.6 & 1.34 & 10.22 & 2.87 & 14.78 & 0.345 & 38.49 & 1 \\ 
K02577.01 & 18.6 & 2.19 & 5.19 & 3.57 & 8.05 & 0.137 & 122.74 & 0 \\ 
K02581.01 & 12.7 & 0.92 & 3.20 & 0.88 & 4.26 & 0.108 & 56.03 & 1 \\ 
K02582.01 & 40.0 & 1.35 & 4.70 & 1.94 & 8.56 & 0.245 & 30.53 & 0 \\ 
K02583.01 & 3.0 & 0.60 & 1.75 & 0.62 & 2.83 & 0.042 & 455.01 & 1 \\ 
K02585.01 & 5.3 & 0.78 & 3.50 & 0.97 & 4.12 & 0.060 & 415.37 & 1 \\ 
K02588.01 & 5.8 & 1.82 & 2.11 & 1.33 & 2.80 & 0.056 & 36.54 & 1 \\ 
K02593.01 & 14.8 & 0.70 & 5.45 & 1.12 & 6.62 & 0.132 & 166.97 & 1 \\ 
K02595.01 & 9.2 & 0.87 & 4.24 & 1.43 & 5.87 & 0.095 & 356.26 & 1 \\ 
K02595.02 & 14.6 & 0.79 & 5.20 & 1.30 & 6.85 & 0.130 & 192.93 & 1 \\ 
K02603.01 & 73.7 & 1.09 & 9.77 & 2.09 & 13.55 & 0.376 & 28.71 & 1 \\ 
K02612.01 & 4.6 & 0.49 & 2.66 & 0.55 & 3.43 & 0.056 & 279.31 & 1 \\ 
K02623.01 & 5.6 & 0.68 & 3.56 & 1.27 & 5.56 & 0.069 & 780.63 & 1 \\ 
K02631.01 & 45.0 & 1.20 & 8.74 & 2.02 & 11.28 & 0.242 & 39.22 & 1 \\ 
K02632.01 & 7.1 & 0.63 & 5.44 & 1.53 & 7.64 & 0.083 & 939.55 & 1 \\ 
K02635.01 & 22.2 & 0.74 & 7.12 & 1.48 & 9.77 & 0.166 & 143.37 & 1 \\ 
K02636.01 & 3.9 & 0.56 & 2.53 & 0.60 & 3.11 & 0.050 & 412.16 & 1 \\ 
K02650.01 & 35.0 & 2.04 & 4.05 & 1.43 & 4.89 & 0.181 & 2.68 & 1 \\ 
K02662.01 & 2.1 & 1.45 & 1.03 & 0.76 & 1.62 & 0.026 & 45.68 & 1 \\ 
K02663.01 & 9.9 & 0.76 & 4.08 & 1.07 & 5.56 & 0.093 & 177.51 & 1 \\ 
K02668.01 & 0.7 & 1.43 & 1.18 & 1.35 & 1.61 & 0.015 & 2614.19 & 1 \\ 
K02672.01 & 88.5 & 4.59 & 6.42 & 4.51 & 8.19 & 0.391 & 4.97 & 1 \\ 
K02672.02 & 43.0 & 3.07 & 4.44 & 3.01 & 6.46 & 0.243 & 12.89 & 1 \\ 
K02674.01 & 197.5 & 5.19 & 9.49 & 9.61 & 19.05 & 0.686 & 5.70 & 0 \\ 
K02674.02 & 11.2 & 0.80 & 6.05 & 1.49 & 7.38 & 0.103 & 252.54 & 1 \\ 
K02674.03 & 2.5 & 0.75 & 3.95 & 1.40 & 4.52 & 0.039 & 1788.44 & 1 \\ 
K02675.01 & 5.4 & 2.11 & 2.14 & 2.07 & 3.26 & 0.062 & 206.54 & 1 \\ 
K02675.02 & 1.1 & 0.97 & 1.31 & 0.94 & 1.93 & 0.022 & 1674.48 & 1 \\ 
K02677.01 & 237.8 & 4.92 & 7.26 & 9.03 & 19.17 & 0.811 & 5.20 & 0 \\ 
K02678.01 & 3.8 & 1.97 & 1.32 & 1.71 & 2.67 & 0.047 & 215.40 & 0 \\ 
K02686.01 & 211.0 & 3.96 & 6.29 & 3.01 & 9.36 & 0.624 & 0.50 & 1 \\ 
K02687.01 & 1.7 & 0.72 & 1.94 & 0.74 & 2.30 & 0.029 & 1045.06 & 1 \\ 
K02687.02 & 8.2 & 0.94 & 3.17 & 0.97 & 3.84 & 0.081 & 133.36 & 1 \\ 
K02690.01 & 3.6 & 1.94 & 0.96 & 1.78 & 2.74 & 0.046 & 273.83 & 0 \\ 
K02691.01 & 97.4 & 4.13 & 6.41 & 3.14 & 7.28 & 0.376 & 1.41 & 1 \\ 
K02693.01 & 4.1 & 1.18 & 2.22 & 0.86 & 2.43 & 0.045 & 68.41 & 1 \\ 
K02693.02 & 11.4 & 1.11 & 3.09 & 0.81 & 3.42 & 0.088 & 17.59 & 1 \\ 
K02693.03 & 6.8 & 1.20 & 2.17 & 0.87 & 2.89 & 0.063 & 34.64 & 1 \\ 
K02694.01 & 0.8 & 1.67 & 1.39 & 1.34 & 1.55 & 0.016 & 722.09 & 1 \\ 
K02694.02 & 6.6 & 1.81 & 1.77 & 1.45 & 3.05 & 0.064 & 48.09 & 0 \\ 
K02698.01 & 88.0 & 2.70 & 13.97 & 3.49 & 10.09 & 0.403 & 9.33 & 1 \\ 
K02700.01 & 0.9 & 1.75 & 1.66 & 1.38 & 1.58 & 0.017 & 651.30 & 1 \\ 
K02703.01 & 213.3 & 3.99 & 7.35 & 3.07 & 9.35 & 0.625 & 0.44 & 1 \\ 
K02705.01 & 2.9 & 2.31 & 0.86 & 1.26 & 1.83 & 0.032 & 31.62 & 1 \\ 
K02706.01 & 3.1 & 0.85 & 4.41 & 1.80 & 5.07 & 0.048 & 2299.92 & 1 \\ 
K02712.01 & 7.5 & 1.11 & 5.32 & 2.20 & 6.31 & 0.087 & 618.15 & 1 \\ 
K02714.01 & 14.4 & 1.24 & 8.08 & 2.32 & 7.82 & 0.125 & 210.58 & 1 \\ 
K02714.02 & 47.3 & 1.51 & 10.11 & 2.83 & 11.58 & 0.274 & 43.73 & 1 \\ 
K02714.03 & 184.3 & 1.58 & 10.92 & 2.96 & 18.14 & 0.673 & 7.27 & 1 \\ 
K02717.01 & 0.9 & 0.97 & 1.70 & 1.31 & 2.38 & 0.020 & 4479.54 & 1 \\ 
K02719.01 & 4.1 & 1.87 & 1.41 & 1.40 & 2.54 & 0.046 & 87.61 & 0 \\ 
K02719.02 & 106.3 & 1.72 & 5.24 & 1.28 & 7.44 & 0.397 & 1.20 & 1 \\ 
K02720.01 & 6.6 & 0.75 & 3.03 & 1.25 & 5.60 & 0.072 & 490.38 & 0 \\ 
K02722.01 & 6.1 & 1.05 & 3.34 & 1.26 & 3.93 & 0.069 & 314.82 & 1 \\ 
K02722.02 & 11.2 & 1.08 & 4.09 & 1.29 & 4.81 & 0.103 & 141.21 & 1 \\ 
K02722.03 & 4.0 & 0.93 & 3.07 & 1.11 & 3.43 & 0.052 & 547.26 & 1 \\ 
K02722.04 & 8.9 & 0.98 & 3.80 & 1.17 & 4.45 & 0.089 & 191.63 & 1 \\ 
K02730.01 & 4.5 & 0.95 & 3.37 & 1.34 & 4.34 & 0.054 & 500.32 & 1 \\ 
K02732.01 & 7.0 & 0.86 & 5.75 & 1.71 & 6.41 & 0.081 & 612.26 & 1 \\ 
K02732.02 & 13.6 & 0.91 & 7.44 & 1.80 & 7.97 & 0.125 & 256.02 & 1 \\ 
K02732.03 & 54.3 & 1.13 & 5.25 & 2.24 & 12.57 & 0.310 & 41.24 & 0 \\ 
K02736.01 & 9.3 & 2.68 & 2.22 & 1.90 & 3.22 & 0.078 & 24.15 & 1 \\ 
K02742.01 & 0.8 & 1.34 & 0.90 & 0.91 & 1.37 & 0.015 & 466.30 & 1 \\ 
K02743.01 & 11.9 & 1.37 & 1.92 & 1.38 & 4.36 & 0.101 & 71.17 & 0 \\ 
K02748.01 & 23.2 & 1.37 & 9.52 & 2.63 & 10.04 & 0.161 & 92.89 & 1 \\ 
K02748.02 & 5.8 & 1.06 & 2.38 & 2.04 & 6.35 & 0.064 & 581.99 & 0 \\ 
K02751.01 & 24.4 & 2.64 & 2.58 & 2.04 & 4.51 & 0.148 & 6.81 & 0 \\ 
K02753.01 & 0.9 & 0.75 & 1.55 & 1.05 & 2.46 & 0.020 & 4095.33 & 1 \\ 
K02755.01 & 8.5 & 0.77 & 2.40 & 0.81 & 4.05 & 0.082 & 138.28 & 0 \\ 
K02759.01 & 1.1 & 1.12 & 0.90 & 0.88 & 1.68 & 0.019 & 643.79 & 1 \\ 
K02762.01 & 133.0 & 3.20 & 6.90 & 2.66 & 8.21 & 0.463 & 0.80 & 1 \\ 
K02764.01 & 2.3 & 1.99 & 1.64 & 1.35 & 1.93 & 0.029 & 97.74 & 1 \\ 
K02770.01 & 205.4 & 3.16 & 8.26 & 2.39 & 8.83 & 0.591 & 0.35 & 1 \\ 
K02785.01 & 4.8 & 1.48 & 3.17 & 1.83 & 3.82 & 0.057 & 402.77 & 1 \\ 
K02792.01 & 2.1 & 0.47 & 3.17 & 0.70 & 3.37 & 0.035 & 1674.09 & 1 \\ 
K02798.01 & 0.9 & 0.91 & 1.13 & 0.57 & 1.33 & 0.016 & 361.84 & 1 \\ 
K02801.01 & 7.0 & 0.54 & 4.75 & 0.86 & 5.39 & 0.077 & 422.71 & 1 \\ 
K02803.01 & 2.4 & 0.52 & 2.35 & 0.55 & 2.66 & 0.036 & 641.90 & 1 \\ 
K02805.01 & 1.9 & 0.65 & 2.29 & 0.88 & 3.17 & 0.030 & 1792.49 & 1 \\ 
K02806.01 & 24.8 & 2.20 & 3.21 & 1.73 & 4.74 & 0.154 & 9.44 & 1 \\ 
K02828.01 & 59.5 & 3.18 & 5.16 & 2.32 & 6.07 & 0.269 & 2.46 & 1 \\ 
K02828.02 & 505.5 & 3.72 & 9.60 & 2.70 & 12.29 & 1.104 & 0.15 & 1 \\ 
K02829.01 & 10.6 & 1.14 & 0.98 & 1.80 & 6.15 & 0.100 & 224.02 & 0 \\ 
K02830.01 & 40.5 & 1.76 & 10.22 & 3.91 & 12.22 & 0.265 & 88.10 & 0 \\ 
K02832.01 & 3.6 & 0.88 & 2.31 & 0.74 & 2.65 & 0.044 & 186.23 & 1 \\ 
K02833.01 & 1.8 & 0.64 & 1.14 & 0.88 & 2.99 & 0.031 & 2232.43 & 1 \\ 
K02834.01 & 136.2 & 3.12 & 5.29 & 2.41 & 8.24 & 0.472 & 0.97 & 1 \\ 
K02835.01 & 6.3 & 2.41 & 1.28 & 1.77 & 2.83 & 0.060 & 40.56 & 0 \\ 
K02836.01 & 2.9 & 1.51 & 1.99 & 1.18 & 2.33 & 0.037 & 159.13 & 1 \\ 
K02838.01 & 7.7 & 0.78 & 4.32 & 1.38 & 6.22 & 0.081 & 370.63 & 1 \\ 
K02838.02 & 4.8 & 0.68 & 3.73 & 1.21 & 5.31 & 0.059 & 696.46 & 1 \\ 
K02839.01 & 2.2 & 2.11 & 1.27 & 1.56 & 1.97 & 0.029 & 111.08 & 1 \\ 
K02840.01 & 3.7 & 0.85 & 3.36 & 1.43 & 4.76 & 0.048 & 894.60 & 1 \\ 
K02845.01 & 1.6 & 1.35 & 1.48 & 1.00 & 1.83 & 0.024 & 193.54 & 1 \\ 
K02869.01 & 3.3 & 0.92 & 4.37 & 2.08 & 5.37 & 0.051 & 2394.32 & 0 \\ 
K02883.01 & 12.0 & 2.63 & 2.51 & 1.78 & 3.29 & 0.089 & 12.80 & 1 \\ 
K02906.01 & 13.9 & 0.86 & 6.64 & 1.48 & 7.37 & 0.118 & 211.45 & 1 \\ 
K02914.01 & 21.1 & 0.99 & 9.38 & 2.33 & 11.03 & 0.164 & 232.16 & 0 \\ 
K02915.01 & 5.1 & 0.78 & 2.41 & 0.78 & 3.25 & 0.058 & 218.93 & 1 \\ 
K02925.01 & 0.7 & 0.95 & 0.46 & 0.88 & 1.61 & 0.016 & 2285.98 & 1 \\ 
K02935.01 & 27.9 & 1.35 & 6.12 & 2.77 & 10.30 & 0.202 & 136.01 & 0 \\ 
K02943.01 & 54.4 & 1.28 & 9.05 & 2.17 & 11.05 & 0.304 & 25.89 & 1 \\ 
K02948.01 & 11.4 & 0.66 & 4.84 & 1.16 & 6.96 & 0.105 & 190.15 & 1 \\ 
K02949.01 & 10.2 & 0.68 & 4.68 & 1.02 & 5.79 & 0.097 & 213.58 & 1 \\ 
K02956.01 & 3.9 & 0.46 & 4.65 & 1.01 & 5.79 & 0.056 & 1805.31 & 1 \\ 
K02961.01 & 3.8 & 0.53 & 2.98 & 0.69 & 3.58 & 0.051 & 650.63 & 1 \\ 
K02964.01 & 47.4 & 1.33 & 10.36 & 2.49 & 11.99 & 0.267 & 50.52 & 1 \\ 
K02968.01 & 10.2 & 0.57 & 5.76 & 1.35 & 8.67 & 0.102 & 582.05 & 1 \\ 
K02970.01 & 4.8 & 0.59 & 3.40 & 0.73 & 3.75 & 0.059 & 470.99 & 1 \\ 
K02971.01 & 6.1 & 0.75 & 5.20 & 1.44 & 5.75 & 0.074 & 731.79 & 1 \\ 
K02977.01 & 2.8 & 0.69 & 3.32 & 0.96 & 3.58 & 0.041 & 1091.79 & 1 \\ 
K02977.02 & 4.1 & 0.73 & 3.39 & 1.03 & 4.08 & 0.053 & 648.28 & 1 \\ 
K02984.01 & 11.5 & 0.77 & 4.81 & 1.43 & 7.07 & 0.111 & 293.78 & 1 \\ 
K02992.01 & 82.7 & 3.24 & 3.28 & 2.19 & 6.16 & 0.315 & 0.85 & 0 \\ 
K03015.01 & 3.6 & 0.61 & 3.21 & 1.01 & 4.64 & 0.048 & 953.83 & 1 \\ 
K03017.01 & 2.5 & 0.64 & 1.63 & 0.62 & 2.53 & 0.035 & 531.45 & 1 \\ 
K03034.01 & 31.0 & 2.68 & 1.78 & 1.91 & 4.78 & 0.168 & 3.45 & 0 \\ 
K03039.01 & 20.4 & 0.93 & 7.00 & 1.56 & 8.46 & 0.146 & 105.57 & 1 \\ 
K03052.01 & 10.1 & 0.83 & 2.93 & 1.02 & 5.19 & 0.089 & 120.72 & 0 \\ 
K03052.02 & 15.6 & 0.97 & 3.82 & 1.20 & 5.99 & 0.118 & 68.21 & 0 \\ 
K03060.01 & 6.9 & 0.58 & 4.75 & 1.05 & 5.95 & 0.078 & 583.57 & 1 \\ 
K03068.01 & 3.9 & 1.15 & 2.03 & 0.86 & 2.48 & 0.045 & 106.13 & 1 \\ 
K03075.01 & 4.8 & 0.76 & 2.19 & 0.70 & 3.15 & 0.052 & 192.27 & 1 \\ 
K03077.01 & 4.1 & 1.83 & 1.61 & 1.34 & 2.55 & 0.047 & 91.57 & 1 \\ 
K03094.01 & 4.6 & 2.49 & 0.90 & 1.36 & 2.12 & 0.044 & 23.10 & 0 \\ 
K03096.01 & 14.5 & 0.83 & 6.81 & 1.50 & 8.16 & 0.118 & 157.06 & 1 \\ 
K03097.01 & 11.9 & 0.61 & 4.77 & 1.08 & 7.15 & 0.108 & 240.99 & 1 \\ 
K03097.02 & 6.8 & 0.53 & 4.49 & 0.93 & 5.94 & 0.075 & 505.40 & 1 \\ 
K03097.03 & 8.7 & 0.53 & 4.55 & 0.93 & 6.44 & 0.088 & 365.08 & 1 \\ 
K03109.01 & 10.7 & 1.14 & 4.49 & 3.08 & 9.41 & 0.112 & 641.07 & 0 \\ 
K03111.01 & 10.8 & 0.74 & 3.42 & 0.89 & 4.80 & 0.098 & 135.12 & 1 \\ 
K03114.01 & 7.5 & 0.55 & 6.10 & 1.45 & 8.20 & 0.089 & 952.86 & 1 \\ 
K03122.01 & 8.1 & 0.57 & 5.41 & 1.43 & 8.02 & 0.093 & 786.09 & 1 \\ 
K03125.01 & 4.5 & 0.63 & 3.62 & 0.95 & 4.31 & 0.058 & 789.80 & 1 \\ 
K03128.01 & 21.2 & 0.94 & 4.01 & 2.13 & 10.62 & 0.164 & 189.68 & 0 \\ 
K03130.01 & 14.9 & 1.31 & \nodata & 0.95 & 3.75 & 0.106 & 19.46 & 0 \\ 
K03130.02 & 5.7 & 1.01 & 1.90 & 0.74 & 2.72 & 0.056 & 69.74 & 1 \\ 
K03136.01 & 2.4 & 1.25 & 1.86 & 1.02 & 2.16 & 0.032 & 235.68 & 1 \\ 
K03145.01 & 4.5 & 2.05 & 1.71 & 1.50 & 2.45 & 0.047 & 62.78 & 1 \\ 
K03145.02 & 1.0 & 1.44 & 1.36 & 1.06 & 1.48 & 0.017 & 476.36 & 1 \\ 
K03146.01 & 39.9 & 1.14 & 7.96 & 1.92 & 10.04 & 0.241 & 37.58 & 1 \\ 
K03158.01 & 3.6 & 0.65 & 2.34 & 0.59 & 2.76 & 0.043 & 194.40 & 1 \\ 
K03158.02 & 4.5 & 0.80 & 1.73 & 0.73 & 2.98 & 0.050 & 142.88 & 0 \\ 
K03158.03 & 6.2 & 0.83 & 2.28 & 0.75 & 3.30 & 0.061 & 95.07 & 1 \\ 
K03158.04 & 7.7 & 0.80 & 2.75 & 0.73 & 3.55 & 0.071 & 70.73 & 1 \\ 
K03158.05 & 9.7 & 1.01 & 1.62 & 0.91 & 3.83 & 0.082 & 52.25 & 0 \\ 
K03165.01 & 4.1 & 0.55 & 4.21 & 1.09 & 5.46 & 0.056 & 1446.27 & 1 \\ 
K03190.01 & 9.0 & 0.61 & 2.93 & 0.79 & 4.90 & 0.087 & 212.93 & 0 \\ 
K03196.01 & 5.0 & 0.42 & 2.83 & 0.58 & 4.18 & 0.061 & 532.56 & 1 \\ 
K03196.02 & 6.9 & 0.53 & 1.83 & 0.72 & 4.65 & 0.076 & 345.63 & 0 \\ 
K03197.01 & 22.6 & 1.20 & 19.22 & 1.43 & 6.03 & 0.164 & 58.11 & 1 \\ 
K03203.01 & 96.8 & 1.20 & 9.91 & 2.21 & 14.10 & 0.456 & 22.28 & 1 \\ 
K03209.01 & 11.9 & 1.03 & 5.99 & 2.50 & 8.85 & 0.120 & 511.86 & 0 \\ 
K03220.01 & 81.4 & 2.61 & 11.77 & 4.81 & 12.96 & 0.412 & 24.12 & 1 \\ 
K03224.01 & 3.4 & 0.64 & 1.15 & 0.57 & 2.63 & 0.044 & 256.40 & 0 \\ 
K03232.01 & 6.1 & 1.17 & 1.25 & 1.19 & 3.49 & 0.067 & 197.04 & 0 \\ 
K03237.01 & 33.4 & 1.90 & 4.85 & 2.07 & 6.39 & 0.211 & 23.81 & 1 \\ 
K03245.01 & 10.6 & 0.73 & 4.33 & 1.05 & 5.68 & 0.100 & 218.71 & 1 \\ 
K03246.01 & 0.7 & 1.01 & 1.15 & 0.78 & 1.45 & 0.015 & 1078.29 & 1 \\ 
K03248.01 & 6.9 & 0.54 & 2.29 & 0.66 & 4.32 & 0.072 & 227.55 & 0 \\ 
K03266.01 & 54.5 & 2.26 & 4.21 & 1.76 & 5.96 & 0.254 & 2.43 & 1 \\ 
K03277.01 & 42.9 & 1.17 & 5.10 & 2.66 & 13.45 & 0.262 & 71.58 & 0 \\ 
K03282.01 & 49.3 & 3.08 & 3.62 & 1.93 & 5.06 & 0.220 & 1.39 & 1 \\ 
K03283.02 & 20.6 & 1.76 & 3.30 & 1.32 & 4.37 & 0.135 & 12.30 & 1 \\ 
K03287.01 & 51.1 & 1.69 & 7.43 & 2.29 & 9.18 & 0.273 & 21.77 & 1 \\ 
K03288.01 & 48.0 & 2.68 & 4.75 & 2.34 & 6.21 & 0.252 & 8.18 & 1 \\ 
K03296.01 & 62.9 & 1.67 & 5.55 & 1.43 & 6.64 & 0.286 & 2.94 & 1 \\ 
K03298.01 & 30.0 & 2.70 & 2.34 & 1.95 & 4.48 & 0.163 & 3.91 & 0 \\ 
K03301.01 & 20.7 & 1.10 & 2.53 & 2.18 & 9.22 & 0.161 & 120.94 & 0 \\ 
K03303.01 & 29.3 & 2.33 & 4.06 & 1.76 & 4.84 & 0.169 & 8.23 & 1 \\ 
K03308.01 & 31.8 & 1.49 & 7.84 & 2.64 & 9.73 & 0.208 & 63.49 & 1 \\ 
K03308.02 & 5.3 & 0.86 & 4.53 & 1.53 & 5.40 & 0.064 & 670.59 & 1 \\ 
K03310.01 & 20.6 & 1.27 & 4.07 & 1.22 & 4.99 & 0.147 & 28.49 & 1 \\ 
K03313.01 & 35.0 & 7468.98 & \nodata & 6062.75 & 5.37 & 0.194 & 6.27 & 0 \\ 
K03315.01 & 31.2 & 1.31 & 3.75 & 1.38 & 6.57 & 0.183 & 24.43 & 0 \\ 
K03330.01 & 16.3 & 1.27 & 3.55 & 1.11 & 4.27 & 0.117 & 18.34 & 1 \\ 
K03346.01 & 14.4 & 1.00 & 3.84 & 1.26 & 5.57 & 0.120 & 101.75 & 1 \\ 
K03358.01 & 10.1 & 3.39 & 0.76 & 3.12 & 3.86 & 0.089 & 66.74 & 0 \\ 
K03363.01 & 14.5 & 1.68 & 2.38 & 2.17 & 5.88 & 0.117 & 94.68 & 0 \\ 
K03370.02 & 5.9 & 1.42 & 2.07 & 1.09 & 2.96 & 0.060 & 69.40 & 1 \\ 
K03384.02 & 19.9 & 1.11 & 5.97 & 1.52 & 6.61 & 0.151 & 76.35 & 1 \\ 
K03398.02 & 35.8 & 1.88 & 7.91 & 3.09 & 9.10 & 0.236 & 61.20 & 0 \\ 
K03403.01 & 39.8 & 1.30 & 10.36 & 2.72 & 12.35 & 0.244 & 59.26 & 1 \\ 
K03403.02 & 6.2 & 0.70 & 6.07 & 1.46 & 6.67 & 0.071 & 696.28 & 1 \\ 
K03412.01 & 16.8 & 1.65 & 3.03 & 1.16 & 3.90 & 0.115 & 12.10 & 1 \\ 
K03425.01 & 20.0 & 1.04 & 6.29 & 2.33 & 10.05 & 0.163 & 197.96 & 1 \\ 
K03425.02 & 3.2 & 0.65 & 3.61 & 1.47 & 5.46 & 0.048 & 2269.08 & 1 \\ 
K03436.01 & 44.2 & 1.39 & 4.80 & 1.19 & 6.14 & 0.235 & 6.91 & 1 \\ 
K03438.01 & 14.6 & 0.94 & 4.49 & 1.15 & 5.43 & 0.120 & 102.14 & 1 \\ 
K03439.01 & 41.7 & 1.69 & 8.18 & 3.25 & 11.60 & 0.248 & 57.70 & 0 \\ 
K03469.01 & 60.5 & 1.99 & 6.76 & 2.87 & 10.60 & 0.298 & 15.58 & 0 \\ 
K03473.01 & 27.6 & 2.47 & 1.66 & 1.96 & 5.12 & 0.171 & 13.20 & 0 \\ 
K03478.01 & 33.5 & 1.16 & 4.09 & 0.92 & 5.31 & 0.189 & 6.89 & 1 \\ 
K03500.01 & 73.8 & 1.41 & 12.88 & 3.20 & 15.30 & 0.391 & 32.82 & 1 \\ 
K03663.01 & 282.5 & 9.00 & 9.70 & 9.19 & 12.47 & 0.835 & 1.21 & 1 \\ 
K03678.01 & 160.9 & 7.96 & 9.85 & 7.69 & 9.88 & 0.574 & 1.98 & 1 \\ 
K03681.01 & 217.8 & 8.77 & 19.15 & 11.94 & 13.95 & 0.762 & 3.62 & 1 \\ 
K03681.02 & 10.5 & 0.86 & 3.72 & 1.17 & 5.13 & 0.103 & 197.68 & 1 \\ 
K03683.01 & 214.3 & 6.20 & 15.04 & 10.44 & 16.98 & 0.759 & 5.77 & 1 \\ 
K03689.01 & 5.2 & 8.92 & 2.90 & 12.62 & 4.39 & 0.063 & 488.12 & 1 \\ 
K03741.03 & 5.1 & 1.52 & 2.67 & 2.58 & 5.14 & 0.062 & 856.81 & 0 \\ 
K03794.01 & 0.7 & 106.53 & \nodata & 82.25 & 1.38 & 0.014 & 892.68 & 0 \\ 
K03811.01 & 290.1 & 76.11 & \nodata & 121.09 & 19.42 & 0.848 & 2.88 & 0 \\ 
K03823.01 & 202.1 & 5.72 & 3.59 & 5.57 & 10.76 & 0.670 & 1.67 & 0 \\ 
K03835.01 & 47.1 & 3.02 & 2.96 & 2.30 & 5.91 & 0.239 & 5.41 & 0 \\ 
K03864.01 & 1.2 & 1.15 & 1.38 & 0.90 & 1.80 & 0.022 & 729.09 & 1 \\ 
K03864.02 & 18.3 & 1.14 & 3.36 & 0.89 & 4.40 & 0.129 & 20.29 & 1 \\ 
K03876.01 & 19.6 & 1.91 & 1.91 & 1.86 & 4.96 & 0.144 & 37.23 & 0 \\ 
K03878.01 & 71.0 & 2.57 & 6.63 & 2.68 & 7.95 & 0.343 & 8.32 & 1 \\ 
K03892.01 & 2.4 & 0.83 & 1.97 & 0.92 & 2.71 & 0.037 & 685.70 & 1 \\ 
K03893.01 & 3.9 & 2.65 & 1.70 & 1.99 & 2.45 & 0.044 & 78.53 & 1 \\ 
K03925.01 & 9.2 & 3.22 & 2.86 & 2.84 & 3.60 & 0.085 & 68.98 & 1 \\ 
K03925.02 & 2.6 & 1.67 & 1.99 & 1.46 & 2.37 & 0.037 & 367.91 & 1 \\ 
K03925.03 & 5.3 & 1.71 & 2.54 & 1.49 & 3.01 & 0.059 & 142.17 & 1 \\ 
K03936.02 & 13.0 & 1.87 & 0.59 & 1.52 & 4.02 & 0.104 & 33.47 & 0 \\ 
K03943.01 & 38.6 & 1.55 & 19.08 & 2.50 & 9.44 & 0.241 & 49.83 & 1 \\ 
K03946.01 & 308.5 & 2.24 & 17.70 & 4.24 & 21.55 & 0.961 & 4.55 & 1 \\ 
K03975.01 & 364.8 & 3.49 & 10.95 & 2.49 & 10.68 & 0.869 & 0.17 & 1 \\ 
K04004.01 & 4.9 & 1.03 & 2.71 & 1.01 & 3.16 & 0.058 & 236.26 & 1 \\ 
K04014.01 & 234.2 & 1.97 & 10.79 & 2.31 & 12.85 & 0.766 & 2.22 & 1 \\ 
K04016.01 & 125.4 & 3.30 & 2.11 & 2.39 & 7.57 & 0.431 & 0.70 & 0 \\ 
K04022.01 & 4.9 & 0.81 & 5.23 & 1.74 & 6.26 & 0.061 & 1156.98 & 1 \\ 
K04024.01 & 8.4 & 1.18 & 1.67 & 1.07 & 3.62 & 0.078 & 75.52 & 0 \\ 
K04032.01 & 4.0 & 0.72 & 2.51 & 0.92 & 3.79 & 0.050 & 475.42 & 1 \\ 
K04032.02 & 2.9 & 0.61 & 2.44 & 0.78 & 3.41 & 0.040 & 717.67 & 1 \\ 
K04032.03 & 6.0 & 0.77 & 2.55 & 0.99 & 4.34 & 0.065 & 274.34 & 0 \\ 
K04032.04 & 5.1 & 0.74 & 2.59 & 0.95 & 4.12 & 0.059 & 339.34 & 1 \\ 
K04036.01 & 168.8 & 2.22 & 6.38 & 1.72 & 8.86 & 0.543 & 0.79 & 1 \\ 
K04037.01 & 216.0 & 1.81 & 8.30 & 2.42 & 13.83 & 0.745 & 3.64 & 1 \\ 
K04051.01 & 163.7 & 3.04 & 6.59 & 2.78 & 9.69 & 0.557 & 1.42 & 1 \\ 
K04053.01 & 1.4 & 0.71 & 1.47 & 0.76 & 2.25 & 0.026 & 1767.30 & 1 \\ 
K04067.01 & 9.7 & 2.40 & 1.89 & 2.86 & 4.56 & 0.094 & 155.40 & 0 \\ 
K04069.01 & 13.1 & 1.94 & 3.16 & 1.47 & 3.76 & 0.100 & 20.22 & 1 \\ 
K04072.01 & 0.7 & 0.73 & 1.07 & 0.96 & 2.11 & 0.016 & 5673.56 & 1 \\ 
K04087.01 & 101.1 & 2.68 & 7.70 & 1.91 & 6.88 & 0.363 & 0.59 & 1 \\ 
K04097.01 & 2.8 & 1.39 & 0.60 & 1.05 & 2.22 & 0.036 & 117.02 & 1 \\ 
K04109.01 & 0.7 & 0.78 & 1.25 & 0.64 & 1.51 & 0.015 & 1659.44 & 1 \\ 
K04123.01 & 44.6 & 1.07 & 11.78 & 2.69 & 14.37 & 0.279 & 81.47 & 1 \\ 
K04129.01 & 2.3 & 0.70 & 2.06 & 0.59 & 2.32 & 0.034 & 355.63 & 1 \\ 
K04136.01 & 2.4 & 0.70 & 4.15 & 1.41 & 4.74 & 0.038 & 2161.56 & 1 \\ 
K04136.02 & 4.0 & 0.75 & 5.60 & 1.51 & 5.62 & 0.054 & 1099.77 & 1 \\ 
K04146.01 & 3.5 & 0.86 & 1.94 & 0.70 & 2.62 & 0.044 & 196.72 & 1 \\ 
K04156.01 & 4.9 & 0.73 & 4.47 & 1.29 & 5.13 & 0.061 & 667.84 & 1 \\ 
K04157.01 & 3.8 & 0.64 & 2.12 & 0.86 & 3.66 & 0.052 & 749.08 & 0 \\ 
K04160.01 & 3.0 & 0.84 & 1.66 & 0.87 & 2.81 & 0.043 & 511.79 & 0 \\ 
K04188.01 & 7.0 & 0.77 & 3.16 & 0.87 & 3.91 & 0.075 & 219.24 & 1 \\ 
K04204.01 & 20.9 & 0.96 & 6.56 & 1.28 & 6.53 & 0.156 & 64.25 & 1 \\ 
K04207.01 & 0.7 & 1.41 & 0.58 & 0.98 & 1.35 & 0.014 & 558.18 & 1 \\ 
K04212.01 & 5.8 & 1.01 & 3.26 & 1.38 & 4.23 & 0.069 & 427.89 & 1 \\ 
K04222.01 & 3.4 & 1.02 & 1.82 & 1.39 & 3.85 & 0.045 & 682.09 & 0 \\ 
K04230.01 & 5.5 & 0.87 & 2.37 & 1.36 & 5.23 & 0.061 & 570.13 & 0 \\ 
K04235.01 & 66.6 & 1.47 & 1.72 & 2.26 & 10.57 & 0.350 & 22.78 & 0 \\ 
K04245.01 & 24.7 & 0.97 & 8.14 & 2.23 & 10.88 & 0.189 & 139.27 & 1 \\ 
K04255.01 & 6.3 & 1.25 & 2.52 & 0.95 & 2.99 & 0.062 & 57.88 & 1 \\ 
K04276.01 & 56.6 & 0.96 & 15.39 & 2.57 & 16.15 & 0.337 & 69.12 & 1 \\ 
K04288.01 & 6.3 & 0.55 & 4.10 & 0.83 & 4.89 & 0.071 & 408.59 & 1 \\ 
K04292.01 & 9.3 & 0.61 & 3.97 & 0.70 & 4.55 & 0.086 & 120.68 & 1 \\ 
K04296.01 & 2.5 & 0.64 & 1.30 & 0.67 & 2.83 & 0.034 & 704.89 & 1 \\ 
K04301.01 & 15.6 & 0.80 & 4.38 & 0.98 & 5.47 & 0.129 & 103.79 & 1 \\ 
K04302.01 & 5.5 & 0.69 & 3.20 & 1.09 & 4.99 & 0.065 & 603.40 & 1 \\ 
K04304.01 & 9.4 & 0.82 & 4.89 & 1.21 & 5.59 & 0.092 & 226.23 & 1 \\ 
K04312.01 & 7.8 & 0.77 & 3.40 & 1.18 & 5.73 & 0.077 & 305.73 & 0 \\ 
K04318.01 & 14.8 & 0.96 & 4.81 & 1.33 & 5.84 & 0.130 & 151.85 & 1 \\ 
K04329.01 & 17.8 & 0.62 & 6.24 & 1.30 & 9.00 & 0.152 & 219.99 & 0 \\ 
K04334.01 & 2.4 & 1.36 & 1.88 & 1.01 & 2.02 & 0.032 & 152.89 & 1 \\ 
K04335.01 & 7.6 & 0.86 & 3.44 & 0.95 & 4.21 & 0.074 & 179.70 & 1 \\ 
K04356.01 & 174.5 & 3.56 & 6.40 & 2.63 & 8.78 & 0.552 & 0.64 & 1 \\ 
K04367.01 & 171.0 & 2.01 & 3.58 & 3.20 & 15.09 & 0.648 & 6.97 & 0 \\ 
K04372.01 & 6.2 & 1.32 & 2.30 & 1.04 & 3.01 & 0.062 & 57.50 & 1 \\ 
K04374.01 & 3.7 & 1.04 & 1.33 & 1.00 & 2.86 & 0.047 & 270.75 & 0 \\ 
K04382.01 & 2.9 & 0.70 & 3.11 & 1.05 & 3.79 & 0.043 & 1310.64 & 1 \\ 
K04383.01 & 4.3 & 0.79 & 2.53 & 0.79 & 3.08 & 0.054 & 299.89 & 1 \\ 
K04399.01 & 42.1 & 1.35 & 1.02 & 1.23 & 6.11 & 0.231 & 10.77 & 0 \\ 
K04400.01 & 2.2 & 0.71 & 2.39 & 0.82 & 2.76 & 0.034 & 935.99 & 1 \\ 
K04407.01 & 1.3 & 0.40 & 1.55 & 0.66 & 3.09 & 0.027 & 4942.11 & 1 \\ 
K04409.01 & 14.3 & 0.75 & 3.53 & 1.00 & 5.71 & 0.123 & 107.54 & 1 \\ 
K04411.01 & 11.2 & 0.88 & 3.05 & 1.03 & 4.75 & 0.102 & 137.26 & 1 \\ 
K04419.01 & 0.3 & 1.57 & 0.45 & 0.97 & 0.86 & 0.007 & 1388.29 & 1 \\ 
K04427.01 & 147.7 & 3.01 & 5.91 & 1.83 & 7.23 & 0.450 & 0.28 & 1 \\ 
K04431.01 & 19.6 & 0.72 & 4.19 & 1.42 & 8.96 & 0.156 & 174.75 & 0 \\ 
K04444.01 & 5.9 & 1.55 & 1.84 & 0.99 & 2.41 & 0.054 & 23.01 & 1 \\ 
K04447.01 & 2.2 & 1.01 & 1.52 & 0.77 & 2.10 & 0.031 & 237.29 & 1 \\ 
K04452.01 & 12.9 & 0.95 & 4.67 & 1.54 & 7.08 & 0.107 & 186.77 & 1 \\ 
K04464.01 & 4.4 & 1.94 & 0.49 & 1.34 & 2.38 & 0.046 & 49.37 & 0 \\ 
K04509.01 & 12.0 & 1.52 & 2.69 & 1.13 & 3.42 & 0.090 & 14.00 & 1 \\ 
K04613.01 & 2.0 & 0.76 & 1.44 & 0.67 & 2.18 & 0.030 & 585.87 & 1 \\ 
K04617.01 & 27.5 & 0.82 & 7.86 & 1.23 & 8.17 & 0.183 & 60.59 & 1 \\ 
K04725.01 & 7.3 & 0.96 & 1.54 & 0.77 & 3.16 & 0.068 & 48.62 & 0 \\ 
K04742.01 & 112.3 & 2.02 & 5.66 & 1.40 & 6.76 & 0.386 & 0.78 & 1 \\ 
K04774.01 & 51.6 & 1.32 & 5.25 & 1.16 & 6.41 & 0.260 & 6.53 & 1 \\ 
K04928.01 & 3.3 & 10.52 & 1.57 & 6.56 & 2.09 & 0.037 & 37.09 & 1 \\ 
K05341.01 & 15.2 & 1.58 & 0.55 & 1.88 & 5.25 & 0.129 & 104.42 & 0 \\ 
K05475.01 & 224.2 & 1.74 & 11.97 & 2.85 & 17.45 & 0.744 & 4.42 & 1 \\ 
K05597.01 & 7.8 & 0.79 & 3.37 & 0.74 & 3.58 & 0.076 & 74.67 & 1 \\ 
K05663.01 & 140.9 & 1.15 & 10.36 & 1.46 & 11.61 & 0.553 & 5.11 & 1 \\ 
K05692.01 & 2.6 & 0.75 & 2.14 & 0.53 & 2.11 & 0.033 & 82.07 & 1 \\ 
K06166.01 & 12.2 & 3.33 & 2.30 & 2.85 & 4.04 & 0.101 & 41.31 & 0 \\ 
K06166.02 & 6.7 & 2.95 & 2.09 & 2.52 & 3.31 & 0.068 & 92.08 & 1 \\ 
K06186.01 & 5.3 & 2.40 & 2.38 & 2.11 & 3.06 & 0.057 & 103.69 & 1 \\ 
K06246.01 & 9.1 & 1.41 & 2.13 & 1.63 & 4.34 & 0.091 & 165.06 & 0 \\ 
K06299.01 & 0.9 & 0.75 & 1.05 & 0.73 & 1.83 & 0.019 & 1810.56 & 1 \\ 
K06401.01 & 2.0 & 35.05 & \nodata & 83.78 & 4.90 & 0.035 & 5948.18 & 0 \\ 
K06860.01 & 0.6 & 0.54 & 1.56 & 0.41 & 1.31 & 0.013 & 899.90 & 1 \\ 
K07073.01 & 279.0 & 719.74 & \nodata & 1099.40 & 17.24 & 0.884 & 3.15 & 0 \\ 
K07375.01 & 4.8 & 2.20 & 0.80 & 1.73 & 2.63 & 0.050 & 42.45 & 0 \\ 
K07923.01 & 395.1 & 1.01 & 20.75 & 0.91 & 13.06 & 0.950 & 0.40 & 1 \\ 

==> tab_star.tex <==
%id_koi & m17_kmag & gaia2_sparallax & cks_steff & cks_smet & cks_svsini & cks_sprov & gdir_srad & giso_smass & giso_srad & giso_srho & giso_sage & giso2_sparallax & rm_sb2 & in_cxm
1 & 9.85 & 4.67 & 5857 & 0.02 & 1.3 & syn & 1.04 & 1.02 & 1.03 & 0.91 & 3.7 & 4.76 & 1 & 1 \\ 
2 & 9.33 & 2.96 & 6403 & 0.22 & 5.1 & syn & 2.00 & 1.50 & 1.99 & 0.19 & 1.8 & 3.72 & 1 & 1 \\ 
3 & 7.01 & 26.50 & 4619 & 0.16 & \nodata & emp & 0.78 & 0.76 & 0.75 & 1.79 & 11.2 & 23.80 & 1 & 1 \\ 
4 & 10.20 & 1.29 & 5948 & -0.27 & 38.0 & syn & 3.26 & 1.45 & 3.22 & 0.04 & 2.0 & 0.93 & 3 & 0 \\ 
6 & 10.99 & 2.13 & 6356 & 0.05 & 11.8 & syn & 1.29 & 1.23 & 1.28 & 0.57 & 1.5 & 2.24 & 1 & 0 \\ 
7 & 10.80 & 2.07 & 5817 & 0.18 & 2.8 & syn & 1.52 & 1.16 & 1.50 & 0.34 & 5.5 & 1.99 & 1 & 1 \\ 
8 & 11.04 & 3.01 & 5895 & -0.06 & 3.0 & syn & 0.93 & 0.99 & 0.94 & 1.19 & 1.8 & 2.93 & 1 & 0 \\ 
10 & 12.29 & 1.00 & 6202 & -0.09 & 10.2 & syn & 1.54 & 1.20 & 1.53 & 0.33 & 3.6 & 1.17 & 1 & 1 \\ 
17 & 11.63 & 1.73 & 5673 & 0.36 & 2.6 & syn & 1.26 & 1.10 & 1.25 & 0.55 & 6.0 & 1.49 & 1 & 1 \\ 
18 & 11.77 & 1.14 & 6326 & 0.03 & 4.4 & syn & 1.74 & 1.33 & 1.72 & 0.26 & 2.6 & 1.31 & 1 & 1 \\ 
20 & 12.07 & 1.16 & 5934 & 0.04 & 1.7 & syn & 1.50 & 1.14 & 1.49 & 0.34 & 5.3 & 1.09 & 1 & 1 \\ 
22 & 12.04 & 1.41 & 5896 & 0.21 & 2.0 & syn & 1.26 & 1.13 & 1.25 & 0.57 & 4.2 & 1.30 & 1 & 1 \\ 
41 & 9.77 & 3.31 & 5865 & 0.11 & 2.7 & syn & 1.52 & 1.15 & 1.51 & 0.33 & 5.5 & 3.28 & 1 & 1 \\ 
42 & 8.14 & 6.80 & 6367 & 0.01 & 13.0 & syn & 1.49 & 1.27 & 1.49 & 0.38 & 2.4 & 8.22 & 1 & 1 \\ 
46 & 12.01 & 1.10 & 5623 & 0.39 & 2.5 & syn & 1.66 & 1.19 & 1.64 & 0.27 & 6.0 & 1.06 & 1 & 1 \\ 
49 & 11.92 & 1.47 & 5803 & -0.06 & 7.7 & syn & 1.29 & 0.99 & 1.28 & 0.47 & 8.5 & 1.76 & 1 & 1 \\ 
63 & 10.00 & 5.18 & 5633 & 0.23 & 4.8 & syn & 0.89 & 0.99 & 0.91 & 1.32 & 1.4 & 4.82 & 1 & 1 \\ 
64 & 11.23 & 1.13 & 5323 & 0.06 & 2.0 & syn & 2.41 & 1.25 & 2.42 & 0.09 & 4.4 & 1.58 & 1 & 0 \\ 
69 & 8.37 & 10.45 & 5619 & -0.10 & 0.0 & syn & 0.94 & 0.90 & 0.93 & 1.09 & 6.9 & 10.67 & 1 & 1 \\ 
70 & 10.87 & 3.56 & 5515 & 0.10 & 0.0 & syn & 0.88 & 0.94 & 0.88 & 1.37 & 2.8 & 3.36 & 1 & 1 \\ 
72 & 9.50 & 5.41 & 5635 & -0.11 & 0.0 & syn & 1.08 & 0.89 & 1.07 & 0.72 & 11.1 & 5.39 & 1 & 1 \\ 
75 & 9.39 & 2.38 & 5869 & -0.08 & 5.0 & syn & 2.55 & 1.32 & 2.53 & 0.08 & 3.2 & 2.94 & 1 & 1 \\ 
82 & 9.35 & 9.30 & 4763 & 0.09 & \nodata & emp & 0.74 & 0.76 & 0.74 & 1.83 & 8.3 & 8.12 & 1 & 1 \\ 
84 & 10.32 & 4.60 & 5509 & -0.05 & 0.0 & syn & 0.88 & 0.89 & 0.88 & 1.32 & 5.0 & 4.49 & 1 & 1 \\ 
85 & 9.81 & 3.32 & 6229 & 0.15 & 8.7 & syn & 1.44 & 1.27 & 1.43 & 0.43 & 2.4 & 3.49 & 1 & 1 \\ 
87 & 10.15 & 5.16 & 5555 & -0.22 & 0.0 & syn & 0.84 & 0.85 & 0.84 & 1.42 & 5.7 & 5.25 & 1 & 1 \\ 
92 & 10.30 & 3.67 & 5932 & 0.09 & 2.7 & syn & 1.06 & 1.07 & 1.06 & 0.89 & 2.4 & 3.55 & 1 & 1 \\ 
94 & 10.93 & 2.12 & 6170 & 0.07 & 7.4 & syn & 1.39 & 1.21 & 1.39 & 0.45 & 3.1 & 2.23 & 1 & 1 \\ 
97 & 11.54 & 1.11 & 6040 & 0.18 & 3.7 & syn & 1.99 & 1.39 & 1.98 & 0.18 & 2.9 & 1.13 & 1 & 1 \\ 
98 & 10.99 & \nodata & 6464 & 0.05 & 7.5 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
99 & 10.98 & 4.04 & 4941 & -0.26 & 0.3 & syn & 0.79 & 0.72 & 0.73 & 1.79 & 13.0 & 4.44 & 1 & 0 \\ 
102 & 11.05 & 2.57 & 5785 & 0.24 & 1.7 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
103 & 11.05 & 3.30 & 5578 & 0.00 & 0.2 & syn & 0.87 & 0.92 & 0.87 & 1.39 & 2.8 & 3.20 & 1 & 1 \\ 
104 & 10.59 & 5.24 & 4457 & 0.22 & \nodata & emp & 0.77 & 0.74 & 0.73 & 1.88 & 12.1 & 5.65 & 1 & 1 \\ 
105 & 11.21 & 2.56 & 5563 & -0.37 & 0.0 & syn & 1.08 & 0.80 & 1.07 & 0.65 & 16.6 & 2.83 & 1 & 1 \\ 
107 & 11.34 & 1.52 & 5937 & 0.28 & 3.9 & syn & 1.58 & 1.27 & 1.59 & 0.31 & 3.7 & 1.50 & 1 & 1 \\ 
108 & 10.87 & 2.05 & 5904 & 0.14 & 3.2 & syn & 1.50 & 1.17 & 1.49 & 0.35 & 4.9 & 2.00 & 1 & 1 \\ 
110 & 11.46 & 1.83 & 6241 & -0.16 & 6.9 & syn & 1.23 & 1.10 & 1.22 & 0.59 & 3.3 & 2.03 & 1 & 1 \\ 
111 & 11.21 & 2.52 & 5822 & -0.42 & 0.0 & syn & 1.04 & 0.84 & 1.03 & 0.76 & 11.2 & 2.85 & 1 & 1 \\ 
112 & 11.37 & 2.66 & 5830 & -0.03 & 2.9 & syn & 0.94 & 0.98 & 0.95 & 1.12 & 2.6 & 2.30 & 1 & 0 \\ 
113 & 10.72 & -1.56 & 5573 & 0.40 & 2.3 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
115 & 11.50 & 2.20 & 5961 & -0.08 & 2.9 & syn & 1.02 & 1.01 & 1.02 & 0.95 & 3.1 & 2.16 & 1 & 1 \\ 
116 & 11.43 & 2.28 & 5881 & -0.09 & 0.5 & syn & 1.03 & 0.98 & 1.03 & 0.90 & 4.6 & 2.26 & 1 & 1 \\ 
117 & 11.06 & 1.93 & 5858 & 0.33 & 3.1 & syn & 1.44 & 1.21 & 1.44 & 0.40 & 4.2 & 1.75 & 1 & 1 \\ 
118 & 10.90 & 2.17 & 5791 & 0.09 & 2.1 & syn & 1.39 & 1.07 & 1.38 & 0.40 & 7.0 & 2.24 & 1 & 1 \\ 
119 & 10.98 & \nodata & 5668 & 0.38 & 3.2 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
122 & 10.80 & 2.27 & 5660 & 0.27 & 0.9 & syn & 1.41 & 1.10 & 1.40 & 0.40 & 7.1 & 2.07 & 1 & 1 \\ 
123 & 11.00 & 2.13 & 5942 & -0.02 & 2.8 & syn & 1.34 & 1.07 & 1.33 & 0.45 & 5.9 & 2.18 & 1 & 1 \\ 
124 & 11.62 & 1.73 & 5977 & -0.10 & 3.3 & syn & 1.24 & 1.03 & 1.23 & 0.55 & 6.0 & 1.82 & 1 & 1 \\ 
125 & 12.03 & 2.28 & 5459 & 0.11 & 3.9 & syn & 0.81 & 0.91 & 0.83 & 1.58 & 1.6 & 2.14 & 1 & 1 \\ 
127 & 12.36 & 1.59 & 5575 & 0.36 & 2.0 & syn & 0.99 & 1.04 & 0.99 & 1.07 & 2.6 & 1.40 & 1 & 1 \\ 
128 & 12.22 & 1.38 & 5652 & 0.27 & 2.9 & syn & 1.21 & 1.05 & 1.20 & 0.60 & 7.0 & 1.20 & 1 & 1 \\ 
129 & 12.03 & 1.10 & 6662 & -0.03 & 20.9 & syn & 1.53 & 1.33 & 1.51 & 0.38 & 1.7 & 1.36 & 3 & 1 \\ 
130 & 11.87 & 1.10 & 6201 & -0.12 & 3.9 & syn & 1.75 & 1.24 & 1.73 & 0.24 & 3.4 & 1.30 & 1 & 0 \\ 
131 & 12.56 & 0.82 & 6498 & 0.21 & 29.0 & syn & 1.64 & 1.41 & 1.62 & 0.33 & 1.6 & 0.82 & 3 & 1 \\ 
134 & 12.32 & 0.89 & 6252 & 0.30 & 11.1 & syn & 1.70 & 1.39 & 1.69 & 0.28 & 2.2 & 0.97 & 1 & 0 \\ 
135 & 12.55 & 1.02 & 5971 & 0.37 & 5.4 & syn & 1.36 & 1.24 & 1.35 & 0.49 & 2.8 & 0.94 & 1 & 1 \\ 
137 & 11.76 & 2.33 & 5440 & 0.28 & 0.0 & syn & 0.91 & 0.97 & 0.91 & 1.27 & 3.0 & 2.09 & 1 & 1 \\ 
139 & 12.11 & 1.55 & 5928 & 0.23 & 2.8 & syn & 1.10 & 1.12 & 1.10 & 0.83 & 1.9 & 1.41 & 1 & 1 \\ 
141 & 11.99 & 1.89 & 5277 & 0.29 & 3.0 & syn & 1.05 & 0.92 & 0.98 & 0.94 & 10.6 & 1.94 & 1 & 0 \\ 
142 & 11.45 & 2.68 & 5473 & 0.27 & 0.0 & syn & 0.90 & 0.97 & 0.90 & 1.31 & 2.3 & 2.39 & 1 & 0 \\ 
144 & 11.46 & 3.29 & 4733 & 0.14 & \nodata & emp & 0.79 & 0.77 & 0.77 & 1.69 & 11.0 & 3.02 & 1 & 1 \\ 
145 & 11.38 & 0.52 & 4911 & 0.03 & 2.4 & syn & 5.22 & 1.38 & 5.19 & 0.01 & 2.9 & 0.63 & 1 & 0 \\ 
148 & 11.22 & 3.28 & 5206 & 0.24 & 0.3 & syn & 0.84 & 0.90 & 0.84 & 1.49 & 3.8 & 2.96 & 1 & 1 \\ 
149 & 11.73 & 1.13 & 5719 & 0.04 & 2.5 & syn & 1.87 & 1.13 & 1.85 & 0.18 & 6.5 & 1.27 & 1 & 1 \\ 
150 & 12.15 & 1.97 & 5567 & -0.39 & 0.7 & syn & 0.90 & 0.79 & 0.89 & 1.09 & 12.9 & 2.16 & 1 & 1 \\ 
152 & 12.61 & 1.00 & 6428 & 0.07 & 14.1 & syn & 1.31 & 1.27 & 1.30 & 0.57 & 1.2 & 1.05 & 1 & 1 \\ 
153 & 11.26 & 3.84 & 4647 & 0.12 & \nodata & emp & 0.76 & 0.75 & 0.74 & 1.84 & 10.2 & 3.49 & 1 & 1 \\ 
155 & 11.91 & 1.21 & 5682 & -0.17 & 1.3 & syn & 1.61 & 0.97 & 1.59 & 0.24 & 9.8 & 1.41 & 1 & 1 \\ 
156 & 11.37 & 3.88 & 4511 & 0.11 & \nodata & emp & 0.72 & 0.73 & 0.71 & 1.99 & 10.1 & 3.98 & 1 & 1 \\ 
157 & 12.18 & 1.57 & 5780 & 0.06 & 0.8 & syn & 1.08 & 1.01 & 1.07 & 0.81 & 5.4 & 1.50 & 1 & 1 \\ 
159 & 11.97 & 1.63 & 6055 & -0.01 & 3.5 & syn & 1.12 & 1.08 & 1.12 & 0.77 & 2.9 & 1.68 & 1 & 1 \\ 
160 & 12.38 & 1.35 & 5913 & -0.47 & 0.9 & syn & 1.14 & 0.86 & 1.12 & 0.60 & 10.8 & 1.51 & 1 & 0 \\ 
161 & 11.24 & 3.59 & 4778 & 0.15 & \nodata & emp & 0.80 & 0.78 & 0.77 & 1.65 & 10.6 & 3.07 & 1 & 1 \\ 
162 & 12.30 & \nodata & 5855 & 0.23 & 3.1 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
163 & 11.73 & \nodata & 5039 & -0.37 & 0.9 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
165 & 12.01 & 1.55 & 5121 & -0.21 & 1.7 & syn & 1.66 & 0.78 & 0.79 & 1.15 & 14.7 & 2.59 & 1 & 0 \\ 
166 & 11.72 & 2.92 & 5175 & -0.22 & 0.5 & syn & 0.76 & 0.77 & 0.76 & 1.71 & 8.5 & 2.97 & 1 & 1 \\ 
167 & 12.06 & 1.20 & 6209 & 0.04 & 2.4 & syn & 1.42 & 1.22 & 1.40 & 0.44 & 2.9 & 1.16 & 1 & 1 \\ 
168 & 12.00 & 1.22 & 5796 & -0.12 & 1.3 & syn & 1.50 & 1.01 & 1.49 & 0.30 & 8.6 & 1.20 & 1 & 1 \\ 
171 & 12.38 & 1.07 & 6237 & 0.10 & 7.9 & syn & 1.39 & 1.23 & 1.38 & 0.46 & 2.6 & 1.19 & 1 & 1 \\ 
172 & 12.23 & 1.39 & 5673 & -0.21 & 1.3 & syn & 1.20 & 0.88 & 1.19 & 0.52 & 12.7 & 1.52 & 1 & 1 \\ 
173 & 12.38 & 1.25 & 5670 & -0.00 & 2.0 & syn & 1.24 & 0.96 & 1.23 & 0.51 & 10.2 & 1.23 & 1 & 1 \\ 
174 & 11.54 & 3.22 & 4691 & -0.24 & \nodata & emp & 0.79 & 0.70 & 0.71 & 1.93 & 13.8 & 3.83 & 1 & 0 \\ 
176 & 12.22 & 1.19 & 6423 & -0.19 & 11.0 & syn & 1.32 & 1.18 & 1.32 & 0.51 & 2.5 & 1.41 & 1 & 1 \\ 
177 & 11.64 & \nodata & 5754 & 0.01 & 1.9 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
179 & 12.50 & 0.65 & 6134 & 0.23 & 9.3 & syn & 2.18 & 1.49 & 2.16 & 0.14 & 2.3 & 0.76 & 1 & 1 \\ 
180 & 11.48 & 2.64 & 5642 & 0.05 & 0.7 & syn & 0.89 & 0.95 & 0.89 & 1.34 & 2.2 & 2.57 & 1 & 1 \\ 
182 & 12.49 & 0.86 & 6016 & 0.18 & 21.1 & syn & 1.69 & 1.29 & 1.68 & 0.27 & 3.5 & 1.25 & 1 & 0 \\ 
186 & 13.43 & 0.90 & 5818 & 0.20 & 2.0 & syn & 1.05 & 1.07 & 1.05 & 0.92 & 2.4 & 0.86 & 1 & 0 \\ 
189 & 12.29 & 2.32 & 4748 & 0.13 & \nodata & emp & 0.77 & 0.77 & 0.76 & 1.73 & 9.9 & 2.04 & 1 & 1 \\ 
191 & 13.25 & 1.17 & 5475 & 0.14 & 1.0 & syn & 0.92 & 0.94 & 0.91 & 1.23 & 4.4 & 1.13 & 1 & 0 \\ 
193 & 13.48 & 0.76 & 5720 & 0.04 & 179.3 & syn & 1.23 & 0.99 & 1.20 & 0.56 & 8.5 & 0.17 & 1 & 0 \\ 
195 & 13.21 & 1.21 & 5541 & -0.17 & 0.1 & syn & 0.89 & 0.86 & 0.88 & 1.24 & 7.4 & 1.23 & 1 & 0 \\ 
197 & 11.96 & 2.73 & 4950 & 0.04 & 2.5 & syn & 0.75 & 0.79 & 0.77 & 1.73 & 7.0 & 2.64 & 1 & 1 \\ 
201 & 12.35 & 1.61 & 5572 & 0.40 & 2.0 & syn & 0.99 & 1.04 & 0.99 & 1.08 & 2.4 & 1.31 & 1 & 1 \\ 
203 & 12.59 & 1.41 & 5703 & 0.32 & 4.5 & syn & 0.99 & 1.06 & 1.00 & 1.06 & 1.8 & 1.36 & 1 & 0 \\ 
209 & 13.01 & 0.71 & 6068 & 0.02 & 7.4 & syn & 1.57 & 1.20 & 1.56 & 0.31 & 4.0 & 0.78 & 1 & 0 \\ 
211 & 13.59 & 0.60 & 5790 & -0.08 & 3.6 & syn & 1.47 & 1.01 & 1.44 & 0.33 & 8.6 & 0.50 & 1 & 0 \\ 
214 & 12.47 & 1.46 & 5471 & 0.43 & 2.4 & syn & 1.04 & 1.02 & 1.03 & 0.91 & 5.4 & 1.26 & 1 & 0 \\ 
222 & 12.31 & 2.60 & 4416 & 0.09 & \nodata & emp & 0.71 & 0.70 & 0.69 & 2.09 & 10.7 & 2.72 & 1 & 1 \\ 
232 & 12.83 & 1.00 & 5994 & -0.06 & 4.0 & syn & 1.24 & 1.05 & 1.23 & 0.56 & 5.3 & 1.01 & 1 & 0 \\ 
237 & 12.59 & 1.26 & 5764 & 0.26 & 2.8 & syn & 1.11 & 1.08 & 1.10 & 0.79 & 3.7 & 1.12 & 1 & 1 \\ 
238 & 12.65 & 1.00 & 6131 & -0.10 & 5.9 & syn & 1.32 & 1.11 & 1.32 & 0.48 & 4.3 & 1.09 & 1 & 1 \\ 
241 & 12.23 & 2.40 & 4939 & -0.44 & 1.4 & syn & 0.75 & 0.68 & 0.69 & 2.05 & 12.5 & 2.65 & 1 & 1 \\ 
244 & 9.49 & 4.14 & 6280 & -0.03 & 9.2 & syn & 1.33 & 1.19 & 1.32 & 0.51 & 2.7 & 4.52 & 1 & 1 \\ 
245 & 7.94 & 15.67 & 5373 & -0.26 & 0.0 & syn & 0.78 & 0.80 & 0.78 & 1.64 & 6.3 & 16.03 & 1 & 1 \\ 
246 & 8.59 & 6.96 & 5778 & 0.13 & 0.0 & syn & 1.25 & 1.05 & 1.24 & 0.54 & 6.7 & 6.22 & 1 & 1 \\ 
247 & 11.12 & 6.42 & 3840 & 0.05 & \nodata & emp & 0.58 & 0.57 & 0.58 & 2.92 & 11.6 & 7.90 & 1 & 1 \\ 
248 & 12.38 & 3.24 & 4011 & -0.16 & \nodata & emp & 0.62 & 0.60 & 0.60 & 2.69 & 12.8 & 4.06 & 1 & 1 \\ 
249 & 11.15 & 10.12 & 3506 & -0.32 & \nodata & emp & 0.41 & 0.40 & 0.41 & 5.73 & 11.8 & 23.17 & 1 & 1 \\ 
250 & 12.63 & 3.01 & 4055 & -0.17 & \nodata & emp & 0.60 & 0.59 & 0.59 & 2.83 & 11.6 & 3.45 & 1 & 1 \\ 
251 & 11.68 & 5.48 & 3788 & -0.03 & \nodata & emp & 0.54 & 0.53 & 0.54 & 3.36 & 11.6 & 7.09 & 1 & 1 \\ 
252 & 12.55 & 2.98 & 3889 & 0.10 & \nodata & emp & 0.63 & 0.60 & 0.61 & 2.55 & 12.3 & 3.70 & 1 & 1 \\ 
253 & 12.29 & 3.14 & 4033 & 0.38 & \nodata & emp & 0.66 & 0.63 & 0.66 & 2.17 & 9.4 & 3.18 & 1 & 1 \\ 
254 & 12.89 & 2.64 & 3919 & 0.24 & \nodata & emp & 0.62 & 0.60 & 0.61 & 2.55 & 10.1 & 2.80 & 1 & 1 \\ 
255 & 12.08 & 3.55 & 3913 & 0.13 & \nodata & emp & 0.64 & 0.61 & 0.63 & 2.41 & 12.7 & 4.37 & 1 & 0 \\ 
257 & 9.62 & 4.40 & 6220 & 0.12 & 7.5 & syn & 1.18 & 1.19 & 1.19 & 0.71 & 1.2 & 4.31 & 1 & 1 \\ 
260 & 9.34 & 4.24 & 6292 & -0.16 & 8.7 & syn & 1.39 & 1.17 & 1.38 & 0.43 & 3.3 & 5.11 & 1 & 1 \\ 
261 & 8.87 & 8.16 & 5752 & 0.09 & 0.2 & syn & 0.94 & 1.00 & 0.94 & 1.18 & 2.0 & 7.82 & 1 & 1 \\ 
262 & 9.20 & 4.02 & 6171 & -0.09 & 10.0 & syn & 1.59 & 1.20 & 1.58 & 0.30 & 3.8 & 4.68 & 1 & 1 \\ 
263 & 9.01 & \nodata & 5779 & -0.12 & 0.7 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
265 & 10.66 & 2.58 & 6015 & 0.14 & 2.3 & syn & 1.27 & 1.15 & 1.26 & 0.56 & 3.5 & 2.35 & 1 & 1 \\ 
266 & 10.38 & 3.10 & 6232 & -0.02 & 5.5 & syn & 1.18 & 1.14 & 1.18 & 0.69 & 2.0 & 3.25 & 1 & 1 \\ 
268 & 9.60 & 3.46 & 6472 & 0.02 & 8.5 & syn & 1.49 & 1.30 & 1.48 & 0.39 & 2.0 & 4.12 & 1 & 0 \\ 
269 & 9.75 & 3.41 & 6340 & -0.06 & 11.8 & syn & 1.42 & 1.23 & 1.42 & 0.43 & 2.5 & 4.06 & 1 & 1 \\ 
270 & 9.70 & \nodata & 5625 & -0.14 & 3.7 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
271 & 10.23 & 2.86 & 6158 & 0.27 & 6.6 & syn & 1.38 & 1.28 & 1.37 & 0.49 & 1.9 & 2.90 & 1 & 1 \\ 
273 & 9.97 & 4.36 & 5676 & 0.28 & 0.5 & syn & 1.07 & 1.06 & 1.06 & 0.87 & 3.9 & 3.61 & 1 & 1 \\ 
274 & 10.11 & 2.55 & 6081 & -0.04 & 6.1 & syn & 1.67 & 1.22 & 1.66 & 0.26 & 3.9 & 2.81 & 1 & 1 \\ 
275 & 10.25 & 2.47 & 5826 & 0.27 & 2.9 & syn & 1.63 & 1.25 & 1.62 & 0.29 & 4.4 & 2.43 & 1 & 1 \\ 
276 & 10.48 & 3.03 & 5993 & -0.01 & 2.4 & syn & 1.18 & 1.06 & 1.17 & 0.65 & 4.4 & 3.17 & 1 & 1 \\ 
277 & 10.79 & 1.92 & 5987 & -0.19 & 4.8 & syn & 1.63 & 1.08 & 1.61 & 0.25 & 6.3 & 2.30 & 1 & 1 \\ 
279 & 10.43 & 2.22 & 6294 & 0.18 & 12.9 & syn & 1.60 & 1.34 & 1.59 & 0.33 & 2.3 & 2.68 & 1 & 0 \\ 
280 & 9.79 & 4.71 & 6087 & -0.27 & 3.0 & syn & 1.04 & 0.99 & 1.04 & 0.88 & 3.9 & 5.11 & 1 & 1 \\ 
281 & 10.45 & 2.61 & 5720 & -0.35 & 0.1 & syn & 1.43 & 0.89 & 1.43 & 0.30 & 12.1 & 3.21 & 1 & 1 \\ 
282 & 10.49 & 3.18 & 5906 & -0.16 & 0.9 & syn & 1.13 & 0.97 & 1.13 & 0.67 & 7.1 & 3.30 & 1 & 1 \\ 
283 & 10.08 & 4.40 & 5782 & 0.19 & 0.4 & syn & 0.99 & 1.05 & 1.00 & 1.05 & 2.0 & 4.11 & 1 & 1 \\ 
284 & 10.42 & \nodata & 5973 & -0.19 & 3.5 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
285 & 10.40 & 2.12 & 5952 & 0.20 & 4.0 & syn & 1.75 & 1.30 & 1.75 & 0.24 & 3.6 & 2.21 & 1 & 1 \\ 
288 & 9.71 & 2.47 & 6195 & 0.23 & 7.9 & syn & 2.03 & 1.46 & 2.03 & 0.17 & 2.3 & 2.74 & 1 & 1 \\ 
289 & 11.19 & 1.56 & 5855 & -0.36 & 1.8 & syn & 1.70 & 0.98 & 1.68 & 0.20 & 8.3 & 2.02 & 1 & 1 \\ 
291 & 11.32 & 1.56 & 5673 & 0.28 & 4.1 & syn & 1.63 & 1.15 & 1.60 & 0.28 & 6.5 & 1.67 & 1 & 0 \\ 
292 & 11.35 & 2.52 & 5784 & -0.17 & 0.0 & syn & 0.98 & 0.92 & 0.97 & 0.98 & 6.4 & 2.66 & 1 & 1 \\ 
294 & 11.31 & 2.16 & 6076 & 0.05 & 4.4 & syn & 1.13 & 1.11 & 1.12 & 0.77 & 2.2 & 2.14 & 1 & 0 \\ 
295 & 10.95 & 3.01 & 5965 & -0.17 & 2.1 & syn & 0.97 & 0.98 & 0.97 & 1.08 & 2.8 & 3.06 & 1 & 1 \\ 
296 & 11.47 & 2.16 & 5764 & -0.12 & 1.8 & syn & 1.08 & 0.93 & 1.08 & 0.74 & 8.6 & 2.19 & 1 & 1 \\ 
297 & 10.88 & 2.22 & 6181 & 0.12 & 7.0 & syn & 1.32 & 1.21 & 1.31 & 0.54 & 2.4 & 2.38 & 1 & 0 \\ 
299 & 11.25 & 2.88 & 5538 & 0.18 & 0.2 & syn & 0.91 & 0.97 & 0.91 & 1.27 & 2.6 & 2.77 & 1 & 1 \\ 
301 & 11.46 & 1.63 & 5995 & -0.08 & 5.5 & syn & 1.41 & 1.08 & 1.40 & 0.39 & 5.8 & 1.59 & 1 & 1 \\ 
303 & 10.63 & 3.47 & 5616 & -0.13 & 1.3 & syn & 1.00 & 0.88 & 0.99 & 0.89 & 10.0 & 3.57 & 1 & 1 \\ 
304 & 11.11 & 2.98 & 5807 & -0.16 & 1.5 & syn & 0.92 & 0.93 & 0.91 & 1.21 & 3.5 & 3.05 & 1 & 1 \\ 
305 & 10.76 & 4.82 & 4614 & 0.13 & \nodata & emp & 0.76 & 0.75 & 0.74 & 1.84 & 10.7 & 4.52 & 1 & 1 \\ 
306 & 10.76 & 4.08 & 5341 & 0.18 & 2.6 & syn & 0.82 & 0.90 & 0.83 & 1.56 & 2.1 & 3.89 & 1 & 1 \\ 
307 & 11.49 & 1.39 & 6035 & -0.08 & 5.4 & syn & 1.67 & 1.14 & 1.56 & 0.29 & 4.9 & 2.14 & 1 & 0 \\ 
308 & 11.04 & 1.94 & 6256 & 0.03 & 10.0 & syn & 1.41 & 1.22 & 1.39 & 0.45 & 2.7 & 2.34 & 1 & 0 \\ 
309 & 10.48 & 5.96 & 4425 & 0.07 & \nodata & emp & 0.72 & 0.70 & 0.69 & 2.08 & 11.1 & 6.30 & 1 & 0 \\ 
312 & 10.52 & 2.40 & 6246 & 0.07 & 9.7 & syn & 1.45 & 1.26 & 1.43 & 0.42 & 2.5 & 2.67 & 1 & 1 \\ 
313 & 11.16 & 3.32 & 5234 & 0.05 & 0.1 & syn & 0.85 & 0.85 & 0.85 & 1.38 & 7.6 & 3.37 & 1 & 1 \\ 
314 & 9.51 & 14.98 & 3817 & -0.15 & \nodata & emp & 0.54 & 0.53 & 0.53 & 3.45 & 12.1 & 20.42 & 1 & 1 \\ 
315 & 10.81 & 5.14 & 4780 & -0.26 & \nodata & emp & 0.68 & 0.69 & 0.68 & 2.19 & 9.3 & 4.80 & 1 & 1 \\ 
316 & 11.17 & 2.58 & 5652 & 0.37 & 1.3 & syn & 1.05 & 1.07 & 1.04 & 0.94 & 2.8 & 2.20 & 1 & 1 \\ 
317 & 11.67 & 1.23 & 6520 & 0.05 & 15.9 & syn & 1.66 & 1.36 & 1.64 & 0.30 & 2.0 & 1.50 & 1 & 1 \\ 
318 & 11.07 & 1.59 & 6336 & 0.26 & 13.6 & syn & 1.67 & 1.39 & 1.66 & 0.30 & 2.0 & 1.70 & 1 & 1 \\ 
319 & 10.75 & 1.54 & 5945 & 0.16 & 5.3 & syn & 2.09 & 1.31 & 2.06 & 0.15 & 3.8 & 1.80 & 1 & 1 \\ 
321 & 10.97 & 2.77 & 5659 & 0.28 & 0.3 & syn & 1.06 & 1.05 & 1.05 & 0.89 & 4.0 & 2.42 & 1 & 1 \\ 
323 & 10.83 & 3.97 & 5462 & 0.06 & 4.7 & syn & 0.81 & 0.89 & 0.82 & 1.61 & 1.7 & 3.78 & 1 & 1 \\ 
327 & 11.71 & 1.74 & 6043 & -0.02 & 4.4 & syn & 1.17 & 1.07 & 1.16 & 0.68 & 3.8 & 1.69 & 1 & 1 \\ 
328 & 11.22 & 2.21 & 5769 & -0.08 & 2.3 & syn & 1.19 & 0.96 & 1.18 & 0.58 & 9.1 & 2.78 & 1 & 0 \\ 
330 & 12.38 & 0.97 & 5860 & 0.02 & 3.4 & syn & 1.59 & 1.11 & 1.57 & 0.29 & 6.4 & 1.03 & 1 & 1 \\ 
331 & 11.80 & 1.03 & 5517 & 0.11 & 2.4 & syn & 2.00 & 1.14 & 1.98 & 0.14 & 6.5 & 1.21 & 1 & 1 \\ 
332 & 11.47 & 1.53 & 5801 & 0.38 & 2.9 & syn & 1.51 & 1.23 & 1.51 & 0.35 & 4.4 & 1.50 & 1 & 1 \\ 
333 & 12.12 & 1.36 & 6237 & 0.11 & 8.2 & syn & 1.22 & 1.20 & 1.22 & 0.66 & 1.5 & 1.40 & 1 & 0 \\ 
337 & 12.41 & 1.30 & 5748 & 0.09 & 1.9 & syn & 1.17 & 1.01 & 1.16 & 0.64 & 7.1 & 1.30 & 1 & 1 \\ 
338 & 11.39 & 3.34 & 4997 & 0.34 & 1.9 & syn & 0.78 & 0.86 & 0.82 & 1.56 & 5.3 & 3.03 & 1 & 1 \\ 
339 & 12.42 & 0.60 & 5988 & -0.18 & 4.9 & syn & 4.36 & 1.04 & 1.35 & 0.35 & 5.5 & 1.55 & 1 & 0 \\ 
340 & 11.44 & 1.35 & 5705 & 0.36 & 7.1 & syn & 1.76 & 1.27 & 1.75 & 0.23 & 4.6 & 1.56 & 1 & 0 \\ 
341 & 11.70 & 2.44 & 5551 & 0.17 & 1.9 & syn & 0.88 & 0.96 & 0.89 & 1.36 & 2.0 & 2.31 & 1 & 1 \\ 
343 & 11.76 & 1.85 & 5758 & 0.04 & 2.1 & syn & 1.11 & 0.99 & 1.10 & 0.74 & 6.6 & 1.77 & 1 & 1 \\ 
344 & 11.90 & 2.21 & 5614 & -0.20 & 0.0 & syn & 0.88 & 0.87 & 0.88 & 1.28 & 6.2 & 2.32 & 1 & 1 \\ 
345 & 11.18 & 3.98 & 4908 & 0.06 & 0.9 & syn & 0.73 & 0.78 & 0.76 & 1.78 & 6.6 & 3.82 & 1 & 1 \\ 
346 & 11.54 & 3.22 & 5083 & 0.08 & 2.4 & syn & 0.75 & 0.82 & 0.79 & 1.67 & 4.9 & 3.04 & 1 & 1 \\ 
348 & 11.68 & 3.32 & 4633 & 0.13 & \nodata & emp & 0.72 & 0.75 & 0.72 & 1.94 & 8.2 & 2.86 & 1 & 1 \\ 
349 & 12.05 & \nodata & 5763 & 0.35 & 4.1 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
350 & 11.92 & 1.92 & 5785 & 0.05 & 1.4 & syn & 0.98 & 1.00 & 0.98 & 1.06 & 2.9 & 1.87 & 1 & 1 \\ 
351 & 12.48 & 1.20 & 5993 & 0.09 & 3.6 & syn & 1.19 & 1.11 & 1.19 & 0.66 & 3.5 & 1.12 & 1 & 1 \\ 
352 & 12.22 & 1.26 & 5816 & -0.02 & 2.4 & syn & 1.32 & 1.02 & 1.30 & 0.45 & 7.8 & 1.25 & 1 & 1 \\ 
355 & 11.85 & 1.48 & 6122 & 0.20 & 4.9 & syn & 1.28 & 1.21 & 1.28 & 0.57 & 2.3 & 1.46 & 1 & 1 \\ 
356 & 11.89 & 2.19 & 5473 & 0.03 & 1.6 & syn & 0.92 & 0.91 & 0.91 & 1.19 & 6.2 & 2.19 & 1 & 0 \\ 
360 & 11.58 & 1.87 & 6018 & -0.09 & 3.0 & syn & 1.16 & 1.04 & 1.16 & 0.66 & 4.8 & 1.87 & 1 & 0 \\ 
361 & 11.62 & 2.30 & 5701 & 0.15 & 0.7 & syn & 0.95 & 1.01 & 0.95 & 1.15 & 2.2 & 2.15 & 1 & 1 \\ 
364 & 8.64 & 6.04 & 5790 & 0.26 & 0.7 & syn & 1.40 & 1.15 & 1.40 & 0.42 & 5.5 & 5.41 & 1 & 0 \\ 
365 & 9.64 & 6.44 & 5490 & -0.10 & 0.0 & syn & 0.86 & 0.87 & 0.86 & 1.38 & 5.2 & 6.40 & 1 & 1 \\ 
366 & 10.63 & 1.79 & 6472 & 0.10 & 34.9 & syn & 1.79 & 1.41 & 1.78 & 0.24 & 2.0 & 1.67 & 3 & 1 \\ 
367 & 9.64 & 5.40 & 5755 & 0.20 & 2.7 & syn & 0.99 & 1.04 & 1.00 & 1.05 & 2.1 & 4.98 & 1 & 1 \\ 
369 & 10.79 & 2.62 & 6227 & -0.12 & 6.9 & syn & 1.17 & 1.10 & 1.16 & 0.69 & 2.6 & 2.72 & 1 & 1 \\ 
370 & 10.63 & 1.79 & 6117 & 0.07 & 6.7 & syn & 1.87 & 1.33 & 1.86 & 0.20 & 3.1 & 2.13 & 1 & 1 \\ 
371 & 10.17 & 1.39 & 5180 & 0.14 & 2.4 & syn & 3.32 & 1.52 & 3.31 & 0.04 & 2.3 & 1.82 & 1 & 0 \\ 
372 & 10.91 & 3.28 & 5780 & -0.03 & 3.0 & syn & 0.92 & 0.97 & 0.92 & 1.24 & 2.3 & 3.22 & 1 & 0 \\ 
373 & 11.32 & 2.69 & 5797 & -0.33 & 1.3 & syn & 0.93 & 0.87 & 0.92 & 1.10 & 7.0 & 2.89 & 1 & 1 \\ 
374 & 10.81 & 2.59 & 5878 & -0.18 & 0.5 & syn & 1.20 & 0.96 & 1.20 & 0.55 & 8.3 & 2.92 & 1 & 1 \\ 
375 & 11.79 & 1.22 & 5772 & 0.20 & 2.7 & syn & 1.64 & 1.19 & 1.62 & 0.28 & 5.4 & 1.21 & 1 & 0 \\ 
377 & 12.34 & 1.62 & 5800 & 0.09 & 1.1 & syn & 0.97 & 1.02 & 0.97 & 1.10 & 2.2 & 1.57 & 1 & 0 \\ 
379 & 11.52 & \nodata & 6121 & 0.17 & 7.5 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
384 & 11.73 & 0.97 & 6052 & -0.02 & 5.9 & syn & 2.13 & 1.27 & 2.10 & 0.14 & 3.8 & 1.08 & 1 & 1 \\ 
385 & 11.78 & 2.32 & 5479 & 0.12 & 0.3 & syn & 0.89 & 0.94 & 0.89 & 1.31 & 3.5 & 2.22 & 1 & 1 \\ 
386 & 12.47 & 1.42 & 5983 & 0.06 & 3.6 & syn & 1.02 & 1.06 & 1.02 & 0.99 & 1.6 & 1.33 & 1 & 1 \\ 
387 & 11.09 & 4.53 & 4598 & 0.02 & \nodata & emp & 0.70 & 0.72 & 0.70 & 2.07 & 8.5 & 4.50 & 1 & 0 \\ 
388 & 11.78 & 1.13 & 5797 & 0.13 & 3.9 & syn & 1.80 & 1.17 & 1.78 & 0.20 & 5.8 & 1.18 & 1 & 1 \\ 
392 & 12.42 & 0.98 & 5913 & 0.08 & 4.1 & syn & 1.54 & 1.16 & 1.52 & 0.33 & 5.0 & 1.00 & 1 & 1 \\ 
393 & 12.29 & 1.06 & 6280 & -0.19 & 8.0 & syn & 1.47 & 1.17 & 1.46 & 0.37 & 3.6 & 1.35 & 1 & 1 \\ 
396 & 11.76 & 2.17 & 5725 & 0.11 & 1.3 & syn & 0.95 & 1.00 & 0.95 & 1.16 & 2.3 & 2.12 & 1 & 1 \\ 
399 & 11.52 & 1.37 & 6147 & 0.01 & 6.4 & syn & 1.62 & 1.24 & 1.61 & 0.29 & 3.5 & 2.04 & 1 & 0 \\ 
401 & 12.18 & 1.78 & 5464 & 0.36 & 1.2 & syn & 0.98 & 1.00 & 0.97 & 1.07 & 4.1 & 1.68 & 1 & 1 \\ 
403 & 12.60 & 0.96 & 6236 & 0.04 & 10.1 & syn & 1.42 & 1.22 & 1.40 & 0.44 & 2.8 & 1.05 & 1 & 0 \\ 
408 & 13.37 & 1.15 & 5600 & 0.11 & 1.8 & syn & 0.87 & 0.95 & 0.88 & 1.38 & 1.8 & 1.08 & 1 & 0 \\ 
409 & 12.71 & 1.25 & 5863 & 0.18 & 1.7 & syn & 1.05 & 1.08 & 1.05 & 0.93 & 2.1 & 1.14 & 1 & 1 \\ 
415 & 12.66 & 1.09 & 5695 & -0.20 & 0.9 & syn & 1.26 & 0.90 & 1.24 & 0.46 & 12.2 & 1.17 & 1 & 1 \\ 
416 & 12.30 & 2.29 & 5067 & -0.12 & 1.7 & syn & 0.75 & 0.77 & 0.76 & 1.74 & 7.7 & 2.28 & 1 & 0 \\ 
420 & 12.00 & 2.66 & 4691 & 0.12 & \nodata & emp & 0.78 & 0.76 & 0.75 & 1.77 & 10.7 & 2.41 & 1 & 0 \\ 
427 & 12.83 & 1.60 & 5334 & 0.14 & 1.4 & syn & 0.81 & 0.89 & 0.83 & 1.57 & 2.4 & 1.51 & 1 & 0 \\ 
430 & 12.19 & 3.24 & 4190 & -0.11 & \nodata & emp & 0.64 & 0.63 & 0.62 & 2.58 & 11.3 & 3.60 & 1 & 1 \\ 
431 & 12.42 & 2.20 & 5187 & -0.26 & 0.2 & syn & 0.73 & 0.76 & 0.74 & 1.83 & 7.2 & 2.22 & 1 & 0 \\ 
433 & 13.06 & 1.40 & 5183 & 0.18 & 2.3 & syn & 0.86 & 0.88 & 0.85 & 1.39 & 6.5 & 1.30 & 1 & 0 \\ 
435 & 12.99 & 1.12 & 5693 & 0.00 & 1.1 & syn & 1.05 & 0.96 & 1.04 & 0.83 & 7.3 & 1.12 & 1 & 0 \\ 
439 & 12.62 & 1.47 & 5479 & 0.35 & 1.7 & syn & 0.96 & 1.01 & 0.96 & 1.13 & 3.2 & 1.32 & 1 & 0 \\ 
440 & 12.15 & 2.28 & 5074 & 0.18 & 2.6 & syn & 0.80 & 0.85 & 0.81 & 1.62 & 4.7 & 2.20 & 1 & 1 \\ 
442 & 12.57 & 1.32 & 5821 & -0.03 & 1.5 & syn & 1.07 & 0.99 & 1.06 & 0.81 & 5.7 & 1.31 & 1 & 1 \\ 
443 & 12.63 & 1.05 & 6066 & -0.16 & 1.1 & syn & 1.28 & 1.05 & 1.27 & 0.51 & 5.5 & 1.26 & 1 & 0 \\ 
444 & 12.67 & 1.51 & 5651 & -0.08 & 0.5 & syn & 0.91 & 0.92 & 0.91 & 1.22 & 4.4 & 1.48 & 1 & 1 \\ 
446 & 12.06 & 3.20 & 4505 & -0.36 & \nodata & emp & 0.64 & 0.63 & 0.62 & 2.59 & 10.9 & 3.45 & 1 & 1 \\ 
448 & 12.36 & 2.70 & 4485 & 0.04 & \nodata & emp & 0.67 & 0.70 & 0.68 & 2.21 & 8.1 & 2.64 & 1 & 1 \\ 
455 & 11.47 & 3.43 & 4227 & -0.13 & \nodata & emp & 0.83 & 0.66 & 0.67 & 2.22 & 15.1 & 4.90 & 1 & 0 \\ 
456 & 13.05 & 1.09 & 5624 & 0.20 & 1.1 & syn & 1.05 & 1.01 & 1.04 & 0.88 & 5.5 & 1.06 & 1 & 0 \\ 
457 & 12.25 & 2.32 & 5109 & 0.25 & 2.4 & syn & 0.75 & 0.87 & 0.81 & 1.61 & 3.6 & 2.05 & 1 & 1 \\ 
458 & 13.11 & 1.20 & 5696 & -0.16 & 1.3 & syn & 0.92 & 0.90 & 0.92 & 1.16 & 5.6 & 1.03 & 1 & 1 \\ 
459 & 12.66 & 1.19 & 5896 & 0.12 & 3.0 & syn & 1.14 & 1.08 & 1.12 & 0.75 & 3.7 & 1.16 & 1 & 0 \\ 
464 & 12.59 & 1.63 & 5483 & 0.26 & 1.6 & syn & 0.88 & 0.97 & 0.89 & 1.34 & 2.0 & 1.50 & 1 & 0 \\ 
465 & 12.81 & 0.89 & 6027 & -0.00 & 3.9 & syn & 1.41 & 1.13 & 1.39 & 0.41 & 4.7 & 0.94 & 1 & 0 \\ 
466 & 13.21 & 0.67 & 5960 & 0.04 & 6.0 & syn & 1.54 & 1.16 & 1.51 & 0.33 & 4.9 & 0.78 & 1 & 0 \\ 
474 & 12.94 & 1.15 & 5981 & 0.02 & 3.3 & syn & 1.02 & 1.05 & 1.02 & 0.99 & 1.8 & 1.09 & 1 & 0 \\ 
475 & 12.84 & 1.81 & 5103 & -0.25 & 1.3 & syn & 0.74 & 0.75 & 0.74 & 1.82 & 8.7 & 1.88 & 1 & 0 \\ 
476 & 12.93 & 1.80 & 4837 & -0.29 & 2.2 & syn & 0.74 & 0.69 & 0.69 & 2.03 & 11.9 & 1.93 & 1 & 1 \\ 
478 & 10.96 & 7.68 & 3688 & 0.21 & \nodata & emp & 0.55 & 0.53 & 0.54 & 3.28 & 10.9 & 9.21 & 1 & 1 \\ 
479 & 12.51 & 1.59 & 5540 & -0.08 & 0.8 & syn & 0.93 & 0.89 & 0.92 & 1.12 & 7.6 & 1.60 & 1 & 1 \\ 
481 & 12.88 & 1.68 & 5175 & -0.08 & 0.5 & syn & 0.78 & 0.80 & 0.79 & 1.61 & 7.1 & 1.67 & 1 & 0 \\ 
486 & 12.64 & 1.32 & 5658 & -0.30 & 0.6 & syn & 1.05 & 0.83 & 1.04 & 0.73 & 13.4 & 1.45 & 1 & 1 \\ 
490 & 11.83 & 2.95 & 4720 & -0.02 & \nodata & emp & 0.75 & 0.74 & 0.73 & 1.87 & 10.6 & 2.76 & 1 & 1 \\ 
494 & 12.86 & 1.93 & 4762 & -0.40 & 1.4 & syn & 0.71 & 0.66 & 0.66 & 2.25 & 12.1 & 2.12 & 1 & 1 \\ 
496 & 12.56 & 1.87 & 5313 & 0.14 & 2.7 & syn & 0.80 & 0.88 & 0.81 & 1.64 & 2.0 & 1.77 & 1 & 1 \\ 
500 & 12.25 & 2.73 & 4432 & 0.08 & \nodata & emp & 0.70 & 0.70 & 0.69 & 2.12 & 10.0 & 2.81 & 1 & 1 \\ 
503 & 12.31 & 3.11 & 4221 & -0.19 & \nodata & emp & 0.63 & 0.62 & 0.61 & 2.72 & 11.2 & 3.43 & 1 & 1 \\ 
505 & 12.19 & 2.48 & 5028 & 0.17 & 2.7 & syn & 0.72 & 0.83 & 0.78 & 1.71 & 4.1 & 2.23 & 1 & 1 \\ 
508 & 12.68 & 1.38 & 5581 & 0.39 & 1.8 & syn & 0.99 & 1.05 & 0.99 & 1.07 & 2.4 & 1.17 & 1 & 0 \\ 
509 & 13.21 & 1.18 & 5591 & 0.20 & 1.4 & syn & 0.91 & 0.99 & 0.92 & 1.24 & 2.2 & 1.14 & 1 & 0 \\ 
510 & 12.79 & 1.23 & 5604 & 0.40 & 2.2 & syn & 1.05 & 1.06 & 1.04 & 0.93 & 3.2 & 1.10 & 1 & 0 \\ 
511 & 12.67 & 1.22 & 5941 & 0.06 & 3.6 & syn & 1.08 & 1.06 & 1.07 & 0.85 & 2.8 & 1.25 & 1 & 0 \\ 
517 & 12.40 & 1.73 & 5553 & 0.27 & 2.8 & syn & 0.89 & 0.98 & 0.90 & 1.32 & 1.6 & 1.61 & 1 & 1 \\ 
518 & 12.18 & 2.62 & 4693 & -0.57 & 2.1 & syn & 0.72 & 0.64 & 0.64 & 2.42 & 14.1 & 3.15 & 1 & 1 \\ 
519 & 13.50 & 0.79 & 5727 & 0.04 & 2.3 & syn & 1.18 & 0.99 & 1.16 & 0.62 & 8.1 & 0.76 & 1 & 0 \\ 
520 & 12.57 & 1.92 & 5106 & 0.13 & 1.4 & syn & 0.79 & 0.85 & 0.80 & 1.66 & 4.1 & 1.85 & 1 & 1 \\ 
523 & 13.42 & 0.72 & 5752 & -0.09 & 1.7 & syn & 1.33 & 0.97 & 1.31 & 0.42 & 9.7 & 0.72 & 1 & 0 \\ 
528 & 12.90 & 1.42 & 5394 & -0.03 & 0.8 & syn & 0.88 & 0.87 & 0.88 & 1.26 & 7.8 & 1.46 & 1 & 0 \\ 
531 & 11.61 & 3.98 & 4081 & 0.24 & \nodata & emp & 0.69 & 0.65 & 0.67 & 2.10 & 12.2 & 4.42 & 1 & 1 \\ 
534 & 12.75 & 1.68 & 5262 & 0.12 & 1.8 & syn & 0.81 & 0.88 & 0.82 & 1.59 & 3.0 & 1.56 & 1 & 0 \\ 
543 & 12.88 & 1.67 & 5116 & -0.05 & 1.9 & syn & 0.79 & 0.80 & 0.79 & 1.62 & 7.2 & 1.66 & 1 & 0 \\ 
546 & 13.52 & 0.67 & 5971 & 0.12 & 3.6 & syn & 1.33 & 1.14 & 1.31 & 0.49 & 4.3 & 0.69 & 1 & 0 \\ 
548 & 12.71 & 1.00 & 6000 & -0.06 & 3.0 & syn & 1.29 & 1.07 & 1.28 & 0.50 & 5.4 & 1.03 & 1 & 1 \\ 
550 & 12.54 & 1.53 & 5724 & 0.18 & 1.7 & syn & 0.94 & 1.01 & 0.95 & 1.19 & 1.7 & 1.42 & 1 & 1 \\ 
551 & 13.31 & 0.98 & 5689 & 0.11 & 1.6 & syn & 1.04 & 1.00 & 1.03 & 0.90 & 5.2 & 0.97 & 1 & 0 \\ 
555 & 12.93 & 1.49 & 5297 & 0.10 & 1.0 & syn & 0.84 & 0.88 & 0.84 & 1.48 & 4.2 & 1.42 & 1 & 0 \\ 
561 & 12.13 & 2.43 & 5054 & -0.14 & 0.5 & syn & 0.76 & 0.77 & 0.76 & 1.71 & 9.1 & 2.46 & 1 & 1 \\ 
564 & 13.21 & 0.68 & 5860 & 0.34 & 4.6 & syn & 1.56 & 1.24 & 1.52 & 0.34 & 4.0 & 0.60 & 1 & 0 \\ 
567 & 12.69 & 1.66 & 5530 & -0.15 & 0.4 & syn & 0.83 & 0.87 & 0.83 & 1.52 & 3.7 & 1.66 & 1 & 0 \\ 
568 & 12.42 & 1.82 & 5358 & 0.07 & 1.2 & syn & 0.86 & 0.89 & 0.86 & 1.39 & 5.0 & 1.78 & 1 & 1 \\ 
569 & 12.52 & 2.17 & 5035 & -0.14 & 1.2 & syn & 0.72 & 0.76 & 0.74 & 1.86 & 7.0 & 2.14 & 1 & 1 \\ 
571 & 11.61 & 5.66 & 3830 & -0.18 & \nodata & emp & 0.54 & 0.53 & 0.53 & 3.44 & 12.3 & 7.78 & 1 & 1 \\ 
572 & 12.57 & 0.90 & 6003 & -0.06 & 4.3 & syn & 1.58 & 1.14 & 1.55 & 0.30 & 5.0 & 1.03 & 1 & 1 \\ 
573 & 13.14 & 1.06 & 5708 & 0.15 & 2.1 & syn & 1.03 & 1.02 & 1.02 & 0.94 & 4.1 & 1.03 & 1 & 0 \\ 
574 & 12.92 & 1.71 & 5055 & -0.03 & 1.8 & syn & 0.75 & 0.79 & 0.77 & 1.69 & 6.8 & 1.66 & 1 & 1 \\ 
577 & 12.43 & 1.95 & 5072 & 0.11 & 1.4 & syn & 0.84 & 0.83 & 0.83 & 1.43 & 9.1 & 1.98 & 1 & 0 \\ 
579 & 12.23 & 2.33 & 5135 & 0.06 & 1.7 & syn & 0.75 & 0.83 & 0.79 & 1.66 & 4.6 & 2.19 & 1 & 1 \\ 
582 & 12.88 & 1.71 & 5191 & 0.13 & 1.9 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
584 & 12.43 & 1.56 & 5523 & 0.31 & 1.2 & syn & 0.99 & 1.01 & 0.98 & 1.06 & 3.9 & 1.43 & 1 & 1 \\ 
590 & 13.22 & 1.02 & 5981 & -0.00 & 3.7 & syn & 1.01 & 1.04 & 1.01 & 0.99 & 1.9 & 0.97 & 1 & 0 \\ 
596 & 11.57 & 5.79 & 3707 & -0.03 & \nodata & emp & 0.54 & 0.53 & 0.54 & 3.40 & 12.3 & 8.67 & 1 & 1 \\ 
597 & 13.51 & 0.94 & 5729 & -0.02 & 0.7 & syn & 0.98 & 0.96 & 0.97 & 1.02 & 4.9 & 0.86 & 1 & 0 \\ 
598 & 12.96 & 1.56 & 5238 & 0.04 & 0.4 & syn & 0.80 & 0.85 & 0.80 & 1.63 & 3.6 & 1.52 & 1 & 0 \\ 
600 & 13.34 & 0.84 & 5741 & -0.05 & 0.9 & syn & 1.19 & 0.96 & 1.17 & 0.59 & 9.0 & 0.91 & 1 & 0 \\ 
601 & 13.29 & 1.13 & 5838 & 0.09 & 4.1 & syn & 0.89 & 0.99 & 0.91 & 1.29 & 1.1 & 1.03 & 1 & 0 \\ 
610 & 11.91 & 3.54 & 4122 & 0.17 & \nodata & emp & 0.67 & 0.64 & 0.66 & 2.17 & 11.1 & 3.83 & 1 & 1 \\ 
611 & 12.71 & 0.98 & 6421 & 0.14 & 12.4 & syn & 1.29 & 1.28 & 1.29 & 0.60 & 0.9 & 0.99 & 1 & 1 \\ 
612 & 12.23 & 2.24 & 5137 & 0.02 & 1.7 & syn & 0.79 & 0.83 & 0.79 & 1.66 & 4.9 & 2.19 & 1 & 1 \\ 
620 & 13.20 & 1.30 & 5690 & 0.06 & 5.5 & syn & 0.82 & 0.93 & 0.85 & 1.50 & 1.1 & 1.18 & 1 & 0 \\ 
623 & 10.54 & 3.05 & 5970 & -0.42 & 0.6 & syn & 1.15 & 0.90 & 1.15 & 0.59 & 9.3 & 3.63 & 1 & 1 \\ 
624 & 12.03 & 2.04 & 5671 & 0.12 & 3.1 & syn & 0.89 & 0.97 & 0.90 & 1.33 & 1.6 & 1.93 & 1 & 1 \\ 
626 & 12.21 & 1.36 & 6131 & -0.17 & 4.0 & syn & 1.19 & 1.05 & 1.18 & 0.64 & 4.3 & 1.44 & 1 & 1 \\ 
627 & 11.90 & 1.34 & 6050 & 0.18 & 5.4 & syn & 1.41 & 1.21 & 1.40 & 0.44 & 3.4 & 1.34 & 1 & 1 \\ 
628 & 12.39 & 1.60 & 5769 & -0.32 & 0.6 & syn & 0.96 & 0.86 & 0.96 & 0.97 & 8.8 & 1.78 & 1 & 1 \\ 
629 & 12.61 & 1.04 & 6059 & -0.29 & 2.7 & syn & 1.32 & 1.00 & 1.31 & 0.44 & 6.8 & 1.29 & 1 & 1 \\ 
631 & 11.60 & 1.14 & 5835 & 0.03 & 4.5 & syn & 1.93 & 1.17 & 1.91 & 0.17 & 5.4 & 1.44 & 1 & 1 \\ 
632 & 11.65 & 2.71 & 5406 & 0.12 & 0.6 & syn & 0.82 & 0.90 & 0.83 & 1.58 & 1.9 & 2.55 & 1 & 1 \\ 
633 & 12.29 & 1.22 & 5761 & -0.17 & 1.9 & syn & 1.34 & 0.94 & 1.33 & 0.40 & 10.4 & 1.26 & 1 & 1 \\ 
635 & 11.75 & 1.81 & 6141 & 0.05 & 6.0 & syn & 1.09 & 1.12 & 1.09 & 0.86 & 1.2 & 1.79 & 1 & 1 \\ 
638 & 12.08 & 1.94 & 5740 & -0.00 & 1.4 & syn & 0.91 & 0.96 & 0.91 & 1.27 & 2.2 & 1.87 & 1 & 1 \\ 
639 & 12.21 & 1.34 & 6184 & 0.05 & 7.4 & syn & 1.22 & 1.16 & 1.21 & 0.65 & 2.1 & 1.37 & 1 & 1 \\ 
640 & 11.48 & \nodata & 5296 & 0.16 & 0.9 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
644 & 11.86 & 1.47 & 5749 & -0.08 & 1.5 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
645 & 11.98 & \nodata & 5856 & -0.19 & 2.3 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
647 & 12.16 & 1.15 & 6125 & -0.37 & 2.7 & syn & 1.45 & 1.02 & 1.43 & 0.34 & 6.5 & 1.56 & 1 & 1 \\ 
649 & 11.90 & 0.90 & 6244 & 0.22 & 7.8 & syn & 2.05 & 1.47 & 2.04 & 0.17 & 2.2 & 1.12 & 1 & 1 \\ 
650 & 11.57 & 3.00 & 5051 & 0.06 & 0.8 & syn & 0.79 & 0.82 & 0.80 & 1.61 & 6.8 & 2.98 & 1 & 1 \\ 
654 & 12.46 & 1.53 & 5822 & -0.01 & 1.3 & syn & 0.98 & 0.99 & 0.97 & 1.06 & 3.1 & 1.55 & 1 & 1 \\ 
655 & 11.74 & 1.60 & 6171 & -0.02 & 2.7 & syn & 1.24 & 1.13 & 1.24 & 0.59 & 3.0 & 1.56 & 1 & 1 \\ 
657 & 11.64 & 3.53 & 4686 & -0.17 & \nodata & emp & 0.70 & 0.69 & 0.68 & 2.14 & 9.6 & 3.95 & 1 & 1 \\ 
658 & 12.45 & 1.45 & 5910 & 0.09 & 2.8 & syn & 1.03 & 1.06 & 1.03 & 0.96 & 2.1 & 1.40 & 1 & 1 \\ 
659 & 12.18 & 1.30 & 6374 & -0.03 & 8.8 & syn & 1.23 & 1.20 & 1.22 & 0.65 & 1.4 & 1.37 & 1 & 1 \\ 
660 & 11.68 & 1.03 & 5314 & -0.08 & 1.7 & syn & 2.16 & 1.08 & 2.15 & 0.11 & 7.0 & 1.23 & 1 & 0 \\ 
661 & 12.48 & 1.48 & 5903 & 0.07 & 2.6 & syn & 0.98 & 1.04 & 0.98 & 1.08 & 1.5 & 1.38 & 1 & 1 \\ 
662 & 11.89 & 1.20 & 5806 & -0.03 & 1.8 & syn & 1.61 & 1.07 & 1.59 & 0.26 & 7.4 & 1.20 & 1 & 1 \\ 
664 & 12.00 & 1.71 & 5724 & 0.06 & 0.6 & syn & 1.08 & 0.99 & 1.07 & 0.80 & 6.4 & 1.64 & 1 & 1 \\ 
665 & 11.80 & 1.17 & 5980 & 0.30 & 5.3 & syn & 1.69 & 1.32 & 1.67 & 0.28 & 3.3 & 1.19 & 1 & 1 \\ 
666 & 12.11 & 1.82 & 5630 & 0.15 & 1.8 & syn & 0.97 & 0.99 & 0.97 & 1.08 & 3.7 & 1.75 & 1 & 1 \\ 
670 & 12.19 & 1.06 & 5625 & 0.19 & 2.3 & syn & 1.61 & 1.09 & 1.59 & 0.27 & 8.1 & 1.04 & 1 & 1 \\ 
671 & 12.21 & 1.31 & 6093 & 0.03 & 5.1 & syn & 1.24 & 1.12 & 1.23 & 0.60 & 3.3 & 1.27 & 1 & 1 \\ 
672 & 12.36 & 1.76 & 5562 & 0.13 & 0.6 & syn & 0.90 & 0.96 & 0.90 & 1.30 & 2.6 & 1.65 & 1 & 1 \\ 
673 & 12.10 & 1.30 & 6477 & 0.10 & 12.7 & syn & 1.27 & 1.27 & 1.27 & 0.62 & 0.7 & 1.34 & 1 & 0 \\ 
674 & 11.58 & 0.96 & 4915 & 0.24 & 3.1 & syn & 2.53 & 1.16 & 2.53 & 0.07 & 6.7 & 0.85 & 1 & 0 \\ 
676 & 11.31 & 4.32 & 4356 & 0.14 & \nodata & emp & 0.68 & 0.70 & 0.68 & 2.18 & 9.2 & 4.33 & 1 & 1 \\ 
678 & 11.45 & 3.26 & 5192 & 0.18 & 2.8 & syn & 0.76 & 0.87 & 0.82 & 1.55 & 3.8 & 2.97 & 1 & 1 \\ 
679 & 11.62 & 1.48 & 5864 & 0.21 & 3.8 & syn & 1.46 & 1.18 & 1.45 & 0.38 & 4.9 & 1.43 & 1 & 1 \\ 
680 & 12.29 & 0.73 & 6124 & -0.03 & 6.4 & syn & 2.14 & 1.29 & 2.11 & 0.14 & 3.5 & 0.78 & 1 & 1 \\ 
682 & 12.26 & 1.56 & 5664 & 0.36 & 2.0 & syn & 1.04 & 1.07 & 1.04 & 0.94 & 2.7 & 1.40 & 1 & 0 \\ 
683 & 12.24 & 1.51 & 5913 & 0.18 & 1.4 & syn & 1.08 & 1.10 & 1.08 & 0.88 & 2.1 & 1.43 & 1 & 1 \\ 
684 & 12.00 & 0.93 & 5264 & 0.10 & 2.7 & syn & 2.06 & 1.10 & 2.05 & 0.13 & 7.5 & 0.95 & 1 & 0 \\ 
685 & 12.57 & 0.78 & 6593 & -0.03 & 14.9 & syn & 1.71 & 1.36 & 1.69 & 0.28 & 2.0 & 1.05 & 1 & 1 \\ 
686 & 11.85 & 1.93 & 5643 & 0.02 & 1.3 & syn & 1.05 & 0.94 & 1.04 & 0.82 & 8.2 & 1.95 & 1 & 1 \\ 
687 & 12.12 & 3.08 & 5852 & 0.06 & 4.5 & syn & 0.57 & 0.92 & 0.83 & 1.62 & 0.6 & 1.64 & 1 & 0 \\ 
688 & 12.59 & 0.88 & 6218 & -0.06 & 8.9 & syn & 1.55 & 1.22 & 1.54 & 0.33 & 3.4 & 1.08 & 1 & 0 \\ 
689 & 12.09 & 2.24 & 5356 & -0.45 & 0.4 & syn & 0.83 & 0.74 & 0.82 & 1.35 & 14.6 & 2.46 & 1 & 1 \\ 
691 & 12.61 & 0.94 & 5933 & -0.31 & 2.5 & syn & 1.45 & 0.97 & 1.44 & 0.32 & 8.5 & 1.12 & 1 & 1 \\ 
692 & 12.12 & 1.60 & 5679 & 0.17 & 2.2 & syn & 1.09 & 1.01 & 1.08 & 0.79 & 5.9 & 1.48 & 1 & 1 \\ 
693 & 12.61 & 0.85 & 6018 & -0.03 & 6.5 & syn & 1.59 & 1.18 & 1.57 & 0.30 & 4.5 & 0.89 & 1 & 1 \\ 
694 & 12.44 & 1.60 & 5695 & 0.23 & 1.7 & syn & 0.94 & 1.02 & 0.95 & 1.18 & 1.6 & 1.44 & 1 & 1 \\ 
695 & 12.04 & 1.97 & 5730 & -0.42 & 0.0 & syn & 0.92 & 0.82 & 0.92 & 1.06 & 10.0 & 2.15 & 1 & 1 \\ 
697 & 12.14 & 0.50 & 5835 & 0.14 & 2.0 & syn & 5.62 & 1.13 & 1.42 & 0.33 & 4.8 & 1.11 & 1 & 0 \\ 
700 & 12.00 & 2.08 & 5705 & -0.44 & 0.6 & syn & 0.89 & 0.82 & 0.89 & 1.15 & 9.6 & 2.30 & 1 & 1 \\ 
701 & 11.66 & 3.35 & 4863 & -0.34 & 0.6 & syn & 0.71 & 0.69 & 0.68 & 2.13 & 10.6 & 3.57 & 1 & 1 \\ 
703 & 11.90 & 0.90 & 6383 & 0.26 & 7.5 & syn & 2.02 & 1.52 & 2.01 & 0.19 & 1.8 & 1.17 & 1 & 0 \\ 
704 & 11.97 & 2.58 & 5277 & -0.08 & 1.8 & syn & 0.75 & 0.82 & 0.79 & 1.66 & 4.5 & 2.46 & 1 & 1 \\ 
707 & 12.59 & 0.85 & 5953 & 0.14 & 4.4 & syn & 1.62 & 1.23 & 1.60 & 0.29 & 4.2 & 0.88 & 1 & 1 \\ 
708 & 12.62 & 0.87 & 6100 & -0.10 & 7.1 & syn & 1.56 & 1.17 & 1.54 & 0.31 & 4.3 & 1.01 & 1 & 1 \\ 
709 & 12.27 & 1.99 & 5385 & -0.13 & 0.3 & syn & 0.85 & 0.84 & 0.84 & 1.37 & 7.8 & 2.07 & 1 & 1 \\ 
710 & 12.10 & 0.93 & 6540 & -0.06 & 15.0 & syn & 1.75 & 1.35 & 1.74 & 0.25 & 2.2 & 1.22 & 1 & 1 \\ 
711 & 12.31 & 1.55 & 5630 & 0.40 & 1.4 & syn & 1.04 & 1.07 & 1.03 & 0.96 & 2.7 & 1.35 & 1 & 1 \\ 
712 & 12.18 & \nodata & 5472 & 0.03 & 1.4 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
714 & 11.74 & 2.56 & 5380 & 0.15 & 0.6 & syn & 0.83 & 0.91 & 0.84 & 1.52 & 2.4 & 2.42 & 1 & 1 \\ 
716 & 12.21 & 0.96 & 6063 & 0.13 & 5.1 & syn & 1.70 & 1.28 & 1.69 & 0.26 & 3.4 & 1.05 & 1 & 1 \\ 
717 & 11.79 & 1.70 & 5641 & 0.34 & 1.3 & syn & 1.19 & 1.07 & 1.18 & 0.64 & 6.1 & 1.55 & 1 & 1 \\ 
718 & 12.39 & 1.29 & 5907 & 0.37 & 3.5 & syn & 1.16 & 1.17 & 1.16 & 0.75 & 1.8 & 1.18 & 1 & 1 \\ 
719 & 10.55 & 5.87 & 4542 & 0.08 & \nodata & emp & 0.69 & 0.72 & 0.70 & 2.08 & 8.4 & 5.77 & 1 & 0 \\ 
720 & 11.90 & 2.62 & 5197 & 0.00 & 4.5 & syn & 0.77 & 0.83 & 0.78 & 1.75 & 3.1 & 2.54 & 1 & 1 \\ 
721 & 12.16 & 1.05 & 5820 & 0.12 & 1.9 & syn & 1.62 & 1.15 & 1.60 & 0.28 & 5.9 & 1.08 & 1 & 1 \\ 
722 & 12.21 & 1.35 & 6188 & -0.11 & 5.5 & syn & 1.19 & 1.09 & 1.18 & 0.66 & 3.1 & 1.44 & 1 & 1 \\ 
723 & 13.23 & 1.34 & 5309 & 0.32 & 4.2 & syn & 0.80 & 0.92 & 0.84 & 1.56 & 1.7 & 1.19 & 1 & 0 \\ 
730 & 13.63 & 0.56 & 5952 & 0.27 & 2.4 & syn & 1.54 & 1.24 & 1.50 & 0.36 & 3.7 & 0.62 & 1 & 0 \\ 
732 & 13.50 & 1.15 & 5259 & 0.30 & 1.7 & syn & 0.84 & 0.92 & 0.85 & 1.48 & 2.8 & 1.01 & 1 & 0 \\ 
733 & 13.70 & 1.30 & 5040 & -0.08 & 2.8 & syn & 0.70 & 0.77 & 0.74 & 1.90 & 4.9 & 1.21 & 1 & 0 \\ 
734 & 13.76 & 0.62 & 5909 & 0.25 & 2.6 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
736 & 13.25 & 1.81 & 4180 & 0.10 & \nodata & emp & 0.70 & 0.66 & 0.67 & 2.22 & 11.9 & 2.04 & 1 & 1 \\ 
738 & 13.66 & 1.23 & 5380 & -0.43 & 1.1 & syn & 0.73 & 0.76 & 0.75 & 1.78 & 7.1 & 1.21 & 1 & 0 \\ 
739 & 12.63 & 2.60 & 4093 & 0.17 & \nodata & emp & 0.67 & 0.64 & 0.66 & 2.19 & 11.3 & 2.84 & 1 & 1 \\ 
740 & 13.35 & 1.41 & 4687 & 0.08 & \nodata & emp & 0.79 & 0.76 & 0.75 & 1.77 & 11.4 & 1.35 & 1 & 1 \\ 
746 & 13.03 & 1.78 & 4532 & -0.35 & \nodata & emp & 0.74 & 0.66 & 0.66 & 2.26 & 13.7 & 2.17 & 1 & 1 \\ 
747 & 13.23 & 1.89 & 4316 & -0.13 & \nodata & emp & 0.66 & 0.64 & 0.64 & 2.46 & 11.1 & 2.06 & 1 & 1 \\ 
749 & 13.63 & 1.04 & 5356 & 0.09 & 0.6 & syn & 0.86 & 0.89 & 0.86 & 1.37 & 4.8 & 1.01 & 1 & 0 \\ 
750 & 13.20 & 1.25 & 4908 & -0.11 & 5.2 & syn & 0.93 & 0.78 & 0.87 & 1.17 & 17.7 & 1.61 & 1 & 0 \\ 
752 & 13.65 & 0.95 & 5556 & 0.11 & 0.8 & syn & 0.93 & 0.95 & 0.92 & 1.19 & 3.9 & 0.92 & 1 & 0 \\ 
756 & 14.13 & 0.63 & 5651 & 0.17 & 2.6 & syn & 1.11 & 1.01 & 1.08 & 0.77 & 6.5 & 0.59 & 1 & 0 \\ 
757 & 13.79 & 1.24 & 4996 & 0.06 & 2.1 & syn & 0.70 & 0.80 & 0.76 & 1.80 & 4.7 & 1.12 & 1 & 0 \\ 
759 & 13.30 & 1.37 & 5257 & -0.21 & 0.5 & syn & 0.77 & 0.79 & 0.77 & 1.69 & 6.9 & 1.39 & 1 & 0 \\ 
760 & 13.80 & 0.79 & 5758 & 0.11 & 1.1 & syn & 1.02 & 1.02 & 1.01 & 0.97 & 3.5 & 0.75 & 1 & 0 \\ 
771 & 13.25 & \nodata & 5658 & 0.17 & 2.4 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
775 & 12.36 & 3.13 & 4148 & -0.07 & \nodata & emp & 0.61 & 0.62 & 0.61 & 2.60 & 10.6 & 3.38 & 1 & 1 \\ 
778 & 12.39 & 2.95 & 4150 & -0.18 & \nodata & emp & 0.65 & 0.62 & 0.61 & 2.61 & 12.6 & 3.52 & 1 & 1 \\ 
780 & 13.20 & 1.53 & 4755 & 0.10 & \nodata & emp & 0.77 & 0.77 & 0.75 & 1.76 & 9.8 & 1.39 & 1 & 0 \\ 
781 & 12.63 & 3.41 & 3730 & 0.42 & \nodata & emp & 0.57 & 0.55 & 0.57 & 2.99 & 9.2 & 3.49 & 1 & 1 \\ 
784 & 12.59 & 3.18 & 4423 & 0.10 & \nodata & emp & 0.51 & 0.60 & 0.57 & 3.17 & 2.7 & 2.37 & 1 & 1 \\ 
800 & 14.06 & 0.60 & 5919 & 0.22 & 3.5 & syn & 1.18 & 1.13 & 1.16 & 0.71 & 2.9 & 0.55 & 1 & 0 \\ 
806 & 13.58 & 1.12 & 5470 & 0.16 & 2.2 & syn & 0.82 & 0.93 & 0.85 & 1.48 & 1.9 & 1.04 & 1 & 0 \\ 
811 & 13.22 & 1.60 & 4787 & 0.13 & \nodata & emp & 0.73 & 0.77 & 0.75 & 1.82 & 7.1 & 1.25 & 1 & 1 \\ 
812 & 13.12 & 2.36 & 4014 & -0.43 & \nodata & emp & 0.61 & 0.56 & 0.55 & 3.24 & 14.0 & 3.23 & 1 & 1 \\ 
817 & 12.31 & 3.49 & 3926 & 0.11 & \nodata & emp & 0.61 & 0.59 & 0.60 & 2.66 & 11.0 & 3.93 & 1 & 1 \\ 
818 & 12.49 & 3.61 & 3702 & 0.31 & \nodata & emp & 0.57 & 0.55 & 0.57 & 3.02 & 10.6 & 4.12 & 1 & 1 \\ 
824 & 14.18 & 0.89 & 5078 & 0.15 & 1.6 & syn & 0.82 & 0.84 & 0.82 & 1.51 & 6.9 & 0.83 & 1 & 0 \\ 
825 & 13.17 & 1.54 & 4727 & 0.13 & \nodata & emp & 0.78 & 0.77 & 0.76 & 1.74 & 10.3 & 1.41 & 1 & 1 \\ 
829 & 13.81 & 0.76 & 5814 & 0.03 & 2.2 & syn & 1.05 & 1.00 & 1.03 & 0.89 & 4.3 & 0.72 & 1 & 0 \\ 
834 & 13.51 & 0.58 & 5764 & 0.33 & 3.0 & syn & 1.58 & 1.21 & 1.55 & 0.32 & 4.9 & 0.57 & 1 & 0 \\ 
835 & 13.13 & 1.57 & 4790 & 0.13 & \nodata & emp & 0.77 & 0.78 & 0.76 & 1.72 & 9.3 & 1.29 & 1 & 1 \\ 
837 & 13.46 & 1.36 & 4677 & 0.19 & \nodata & emp & 0.78 & 0.77 & 0.76 & 1.76 & 10.0 & 1.22 & 1 & 1 \\ 
841 & 14.12 & 0.98 & 5273 & 0.13 & 3.0 & syn & 0.75 & 0.88 & 0.82 & 1.55 & 3.3 & 0.87 & 1 & 0 \\ 
842 & 12.88 & 1.69 & 4548 & 0.10 & \nodata & emp & 0.85 & 0.74 & 0.73 & 1.87 & 12.1 & 2.01 & 1 & 0 \\ 
853 & 13.24 & 1.69 & 4789 & -0.02 & \nodata & emp & 0.68 & 0.73 & 0.71 & 2.03 & 6.4 & 1.39 & 1 & 0 \\ 
854 & 12.54 & 3.64 & 3694 & 0.24 & \nodata & emp & 0.56 & 0.54 & 0.55 & 3.18 & 10.8 & 4.31 & 1 & 1 \\ 
855 & 13.31 & 1.15 & 5245 & -0.39 & 1.3 & syn & 0.93 & 0.75 & 0.89 & 1.07 & 17.7 & 1.44 & 1 & 0 \\ 
857 & 13.06 & 1.47 & 5152 & 0.26 & 2.4 & syn & 0.82 & 0.89 & 0.83 & 1.56 & 3.5 & 1.37 & 1 & 0 \\ 
864 & 13.73 & 0.99 & 5500 & 0.08 & 1.2 & syn & 0.86 & 0.92 & 0.87 & 1.38 & 2.9 & 0.94 & 1 & 0 \\ 
868 & 12.52 & 2.50 & 4295 & 0.21 & \nodata & emp & 0.68 & 0.70 & 0.68 & 2.17 & 9.7 & 2.54 & 1 & 1 \\ 
869 & 13.64 & 1.19 & 5102 & 0.12 & 3.1 & syn & 0.79 & 0.84 & 0.81 & 1.54 & 6.2 & 1.16 & 1 & 0 \\ 
870 & 12.72 & 2.31 & 4550 & 0.09 & \nodata & emp & 0.65 & 0.71 & 0.68 & 2.21 & 5.9 & 2.21 & 1 & 1 \\ 
872 & 13.35 & 1.31 & 5155 & 0.16 & 1.3 & syn & 0.80 & 0.86 & 0.81 & 1.61 & 3.8 & 1.25 & 1 & 0 \\ 
874 & 13.04 & 1.62 & 5087 & 0.20 & 2.5 & syn & 0.75 & 0.85 & 0.81 & 1.62 & 4.2 & 1.47 & 1 & 1 \\ 
875 & 13.10 & 1.76 & 4359 & 0.25 & \nodata & emp & 0.74 & 0.72 & 0.71 & 2.01 & 11.4 & 1.88 & 1 & 1 \\ 
877 & 12.39 & 2.90 & 4302 & -0.09 & \nodata & emp & 0.63 & 0.64 & 0.63 & 2.55 & 9.7 & 2.97 & 1 & 1 \\ 
878 & 13.06 & 1.63 & 4736 & -0.09 & \nodata & emp & 0.79 & 0.73 & 0.73 & 1.82 & 12.3 & 1.62 & 1 & 1 \\ 
880 & 13.52 & 1.13 & 5421 & 0.21 & 2.4 & syn & 0.84 & 0.93 & 0.86 & 1.45 & 2.1 & 0.95 & 1 & 0 \\ 
881 & 13.84 & 1.17 & 5065 & 0.01 & 1.5 & syn & 0.72 & 0.80 & 0.77 & 1.73 & 5.3 & 1.09 & 1 & 0 \\ 
883 & 13.52 & 1.39 & 4812 & 0.21 & 4.8 & syn & 0.74 & 0.80 & 0.77 & 1.76 & 6.5 & 1.23 & 1 & 1 \\ 
884 & 13.05 & 1.53 & 5063 & 0.30 & 1.6 & syn & 0.79 & 0.87 & 0.81 & 1.65 & 3.2 & 1.39 & 1 & 0 \\ 
886 & 12.65 & 3.71 & 3736 & -0.19 & \nodata & emp & 0.52 & 0.51 & 0.51 & 3.72 & 12.5 & 5.96 & 1 & 1 \\ 
889 & 13.12 & 1.22 & 5340 & 0.26 & 3.2 & syn & 0.95 & 0.94 & 0.94 & 1.12 & 6.8 & 1.25 & 1 & 0 \\ 
892 & 13.13 & 1.60 & 5063 & -0.06 & 2.6 & syn & 0.73 & 0.78 & 0.76 & 1.77 & 6.0 & 1.56 & 1 & 0 \\ 
896 & 13.36 & 1.38 & 5129 & 0.19 & 0.7 & syn & 0.76 & 0.86 & 0.81 & 1.58 & 4.2 & 1.22 & 1 & 0 \\ 
898 & 12.95 & 2.52 & 4013 & -0.21 & \nodata & emp & 0.61 & 0.59 & 0.60 & 2.75 & 13.0 & 3.22 & 1 & 1 \\ 
899 & 11.97 & 5.28 & 3686 & 0.02 & \nodata & emp & 0.51 & 0.50 & 0.51 & 3.79 & 11.4 & 7.11 & 1 & 1 \\ 
901 & 13.18 & 1.92 & 4205 & 0.01 & \nodata & emp & 0.67 & 0.65 & 0.65 & 2.35 & 11.5 & 2.13 & 1 & 1 \\ 
902 & 13.21 & 1.78 & 4379 & 0.05 & \nodata & emp & 0.69 & 0.69 & 0.68 & 2.19 & 10.4 & 1.86 & 1 & 1 \\ 
904 & 13.29 & 1.75 & 4356 & 0.06 & \nodata & emp & 0.68 & 0.68 & 0.67 & 2.23 & 10.1 & 1.81 & 1 & 1 \\ 
906 & 13.48 & 1.34 & 5009 & 0.01 & 2.1 & syn & 0.75 & 0.79 & 0.77 & 1.71 & 6.6 & 1.29 & 1 & 0 \\ 
907 & 13.63 & 1.11 & 5542 & -0.05 & 1.7 & syn & 0.80 & 0.89 & 0.82 & 1.58 & 2.1 & 1.02 & 1 & 0 \\ 
912 & 12.47 & 2.66 & 4375 & 0.01 & \nodata & emp & 0.66 & 0.67 & 0.66 & 2.31 & 9.2 & 2.68 & 1 & 1 \\ 
918 & 13.22 & 1.34 & 5412 & 0.14 & 2.1 & syn & 0.81 & 0.90 & 0.83 & 1.57 & 1.8 & 1.24 & 1 & 0 \\ 
921 & 13.53 & 1.22 & 5083 & 0.15 & 0.6 & syn & 0.80 & 0.85 & 0.80 & 1.61 & 4.9 & 1.18 & 1 & 0 \\ 
934 & 14.25 & 0.74 & 5502 & -0.13 & 0.5 & syn & 0.90 & 0.86 & 0.88 & 1.21 & 7.8 & 0.78 & 1 & 0 \\ 
935 & 13.87 & 0.63 & 6089 & -0.07 & 74.3 & syn & 1.22 & 1.08 & 1.20 & 0.61 & 4.0 & 0.52 & 1 & 0 \\ 
936 & 11.72 & 5.74 & 3646 & 0.10 & \nodata & emp & 0.52 & 0.51 & 0.52 & 3.61 & 11.5 & 7.79 & 1 & 1 \\ 
939 & 13.42 & 1.00 & 5655 & 0.28 & 1.9 & syn & 0.96 & 1.03 & 0.97 & 1.12 & 2.0 & 0.85 & 1 & 0 \\ 
941 & 13.37 & 1.31 & 5126 & 0.39 & 2.6 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
947 & 12.10 & 4.90 & 3761 & -0.12 & \nodata & emp & 0.51 & 0.50 & 0.51 & 3.80 & 11.6 & 6.74 & 1 & 1 \\ 
950 & 12.75 & 3.32 & 3831 & -0.09 & \nodata & emp & 0.54 & 0.53 & 0.54 & 3.38 & 11.7 & 4.23 & 1 & 1 \\ 
951 & 12.96 & 1.76 & 4689 & 0.13 & \nodata & emp & 0.75 & 0.76 & 0.74 & 1.82 & 9.4 & 1.58 & 1 & 1 \\ 
952 & 12.76 & 3.11 & 3855 & 0.10 & \nodata & emp & 0.57 & 0.56 & 0.57 & 3.00 & 10.7 & 3.51 & 1 & 1 \\ 
954 & 13.55 & 1.02 & 5517 & -0.08 & 1.2 & syn & 0.90 & 0.88 & 0.89 & 1.23 & 6.6 & 1.05 & 1 & 0 \\ 
956 & 12.82 & 2.07 & 4490 & 0.07 & \nodata & emp & 0.70 & 0.71 & 0.69 & 2.09 & 9.4 & 2.09 & 1 & 1 \\ 
958 & 10.41 & 5.91 & 4902 & 0.01 & 3.1 & syn & 0.70 & 0.77 & 0.74 & 1.90 & 5.6 & 5.59 & 1 & 1 \\ 
974 & 8.41 & 4.73 & 6274 & -0.05 & 7.9 & syn & 1.92 & 1.33 & 1.91 & 0.19 & 2.8 & 5.90 & 1 & 1 \\ 
975 & 6.95 & 9.24 & 6186 & -0.05 & 7.3 & syn & 1.94 & 1.32 & 1.93 & 0.18 & 3.0 & 11.61 & 1 & 1 \\ 
981 & 8.72 & 1.76 & 4990 & -0.19 & 2.1 & syn & 5.18 & 1.32 & 5.17 & 0.01 & 3.0 & 2.29 & 1 & 0 \\ 
982 & 13.00 & 2.09 & 4338 & -0.16 & \nodata & emp & 0.66 & 0.64 & 0.63 & 2.49 & 10.9 & 2.26 & 1 & 0 \\ 
986 & 12.49 & 1.62 & 5527 & 0.28 & 2.1 & syn & 0.92 & 1.00 & 0.93 & 1.24 & 2.2 & 1.53 & 1 & 1 \\ 
987 & 10.78 & 3.61 & 5499 & 0.11 & 0.5 & syn & 0.91 & 0.94 & 0.90 & 1.26 & 4.0 & 3.65 & 1 & 1 \\ 
988 & 11.59 & 3.17 & 5093 & 0.10 & 3.3 & syn & 0.74 & 0.83 & 0.79 & 1.67 & 4.5 & 2.97 & 1 & 1 \\ 
991 & 11.93 & 2.25 & 5538 & -0.13 & 1.6 & syn & 0.86 & 0.87 & 0.86 & 1.38 & 5.0 & 2.27 & 1 & 0 \\ 
993 & 12.73 & 1.66 & 5557 & -0.31 & 0.4 & syn & 0.81 & 0.82 & 0.81 & 1.53 & 5.6 & 1.68 & 1 & 0 \\ 
999 & 13.55 & 1.35 & 5113 & -0.08 & 2.1 & syn & 0.72 & 0.79 & 0.76 & 1.80 & 5.1 & 1.28 & 1 & 1 \\ 
1001 & 11.59 & 1.09 & 6298 & 0.14 & 9.0 & syn & 1.97 & 1.43 & 1.95 & 0.19 & 2.3 & 1.39 & 1 & 1 \\ 
1002 & 11.81 & 1.34 & 5389 & 0.12 & 1.7 & syn & 4.22 & 0.92 & 1.12 & 0.54 & 11.6 & 2.17 & 1 & 0 \\ 
1006 & 12.92 & 2.71 & 4005 & -0.38 & \nodata & emp & 0.59 & 0.56 & 0.56 & 3.18 & 13.5 & 3.57 & 1 & 0 \\ 
1010 & 12.19 & 1.04 & 6098 & -0.05 & 7.5 & syn & 1.58 & 1.19 & 1.56 & 0.31 & 4.1 & 1.19 & 1 & 0 \\ 
1014 & 13.52 & 1.41 & 4967 & -0.46 & 1.5 & syn & 0.72 & 0.68 & 0.68 & 2.13 & 10.9 & 1.52 & 1 & 1 \\ 
1015 & 13.10 & 0.80 & 5950 & -0.10 & 4.4 & syn & 1.36 & 1.04 & 1.35 & 0.42 & 6.6 & 0.81 & 1 & 0 \\ 
1019 & 8.21 & 3.36 & 4980 & 0.15 & 2.1 & syn & 3.39 & 1.33 & 3.41 & 0.03 & 3.6 & 3.59 & 1 & 0 \\ 
1024 & 11.88 & 3.66 & 4235 & -0.11 & \nodata & emp & 0.64 & 0.63 & 0.63 & 2.55 & 11.0 & 3.99 & 4 & 1 \\ 
1032 & 11.58 & 0.96 & 4916 & 0.08 & 3.1 & syn & 2.61 & 1.06 & 2.60 & 0.06 & 8.2 & 0.85 & 1 & 0 \\ 
1048 & 12.41 & 3.10 & 4162 & -0.18 & \nodata & emp & 0.61 & 0.60 & 0.60 & 2.79 & 11.2 & 3.44 & 1 & 0 \\ 
1050 & 11.88 & 2.53 & 5062 & 0.09 & 2.1 & syn & 0.82 & 0.83 & 0.82 & 1.50 & 8.3 & 2.59 & 1 & 1 \\ 
1052 & 13.90 & 0.81 & 5920 & -0.10 & 1.6 & syn & 0.94 & 0.98 & 0.95 & 1.14 & 2.2 & 0.73 & 1 & 0 \\ 
1054 & 10.07 & 0.61 & 5286 & -0.85 & 5.8 & syn & 7.91 & 1.53 & 7.98 & 0.00 & 1.3 & 0.50 & 1 & 0 \\ 
1060 & 13.11 & 0.69 & 6351 & -0.29 & 12.2 & syn & 1.52 & 1.17 & 1.51 & 0.33 & 3.5 & 0.76 & 1 & 0 \\ 
1069 & 13.24 & 1.29 & 5241 & 0.30 & 1.9 & syn & 0.85 & 0.92 & 0.86 & 1.45 & 3.3 & 1.19 & 1 & 0 \\ 
1075 & 11.53 & 1.42 & 6469 & 0.04 & 8.4 & syn & 1.54 & 1.32 & 1.52 & 0.36 & 2.0 & 1.60 & 1 & 0 \\ 
1076 & 12.88 & 1.62 & 4857 & -0.25 & 5.4 & syn & 0.84 & 0.74 & 0.79 & 1.48 & 17.2 & 2.06 & 5 & 0 \\ 
1078 & 12.48 & 3.80 & 3843 & -0.14 & \nodata & emp & 0.54 & 0.53 & 0.53 & 3.46 & 11.8 & 4.89 & 1 & 1 \\ 
1082 & 13.75 & 1.06 & 5059 & 0.08 & 1.5 & syn & 0.84 & 0.82 & 0.82 & 1.44 & 9.8 & 1.10 & 1 & 1 \\ 
1085 & 12.25 & 4.10 & 3804 & -0.26 & \nodata & emp & 0.55 & 0.54 & 0.54 & 3.37 & 13.4 & 6.61 & 1 & 1 \\ 
1089 & 13.10 & 1.02 & 5876 & 0.16 & 2.5 & syn & 1.08 & 1.08 & 1.07 & 0.87 & 2.5 & 1.00 & 1 & 0 \\ 
1101 & 13.51 & 1.30 & 4974 & 0.03 & 1.3 & syn & 0.78 & 0.79 & 0.78 & 1.64 & 8.3 & 1.32 & 1 & 1 \\ 
1102 & 13.37 & 0.89 & 6052 & -0.05 & 26.0 & syn & 1.09 & 1.06 & 1.07 & 0.84 & 2.7 & 0.64 & 1 & 0 \\ 
1104 & 13.37 & 1.33 & 4664 & 0.15 & \nodata & emp & 0.83 & 0.77 & 0.79 & 1.56 & 15.2 & 1.30 & 1 & 0 \\ 
1108 & 12.92 & 1.10 & 5657 & 0.28 & 2.0 & syn & 1.11 & 1.05 & 1.09 & 0.79 & 5.1 & 1.02 & 1 & 1 \\ 
1113 & 12.38 & 1.20 & 6099 & 0.04 & 5.2 & syn & 1.25 & 1.13 & 1.24 & 0.58 & 3.3 & 1.20 & 1 & 1 \\ 
1115 & 12.30 & 0.91 & 5646 & 0.12 & 2.5 & syn & 1.79 & 1.11 & 1.77 & 0.20 & 7.2 & 1.03 & 1 & 1 \\ 
1116 & 11.89 & 1.85 & 5754 & 0.04 & 2.3 & syn & 1.05 & 0.99 & 1.04 & 0.87 & 5.4 & 1.80 & 1 & 1 \\ 
1117 & 11.64 & 1.11 & 6401 & -0.05 & 9.6 & syn & 1.85 & 1.35 & 1.84 & 0.21 & 2.5 & 1.33 & 1 & 1 \\ 
1118 & 12.43 & 1.11 & 6030 & -0.05 & 3.5 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
1120 & 9.95 & 1.15 & 4930 & 0.17 & 4.8 & syn & 4.53 & 1.43 & 4.53 & 0.02 & 2.9 & 1.79 & 1 & 0 \\ 
1126 & 13.35 & 1.20 & 5315 & 0.05 & 1.4 & syn & 0.87 & 0.87 & 0.86 & 1.34 & 6.5 & 1.21 & 1 & 0 \\ 
1127 & 13.96 & 0.47 & 5626 & 0.40 & 2.4 & syn & 1.63 & 1.17 & 1.54 & 0.31 & 5.9 & 0.49 & 1 & 0 \\ 
1128 & 11.77 & 2.53 & 5356 & -0.03 & 0.6 & syn & 0.83 & 0.86 & 0.83 & 1.50 & 4.6 & 2.46 & 1 & 1 \\ 
1140 & 11.66 & 2.04 & 5928 & -0.28 & 1.5 & syn & 1.06 & 0.93 & 1.05 & 0.80 & 7.1 & 2.34 & 1 & 0 \\ 
1141 & 13.05 & 2.28 & 4083 & -0.15 & \nodata & emp & 0.64 & 0.61 & 0.61 & 2.62 & 12.5 & 2.75 & 1 & 1 \\ 
1145 & 12.69 & 1.23 & 5977 & 0.07 & 4.1 & syn & 1.08 & 1.08 & 1.07 & 0.87 & 2.3 & 1.17 & 1 & 1 \\ 
1146 & 12.61 & 3.56 & 3780 & 0.06 & \nodata & emp & 0.55 & 0.54 & 0.54 & 3.30 & 11.1 & 4.32 & 1 & 1 \\ 
1148 & 12.63 & 1.08 & 6127 & 0.16 & 5.5 & syn & 1.23 & 1.19 & 1.22 & 0.65 & 1.9 & 1.04 & 1 & 1 \\ 
1150 & 11.82 & 0.73 & 5736 & 0.08 & 3.8 & syn & 5.13 & 1.08 & 1.51 & 0.26 & 6.2 & 1.74 & 1 & 0 \\ 
1151 & 11.74 & 2.50 & 5494 & -0.17 & 0.6 & syn & 0.85 & 0.85 & 0.85 & 1.40 & 6.1 & 2.52 & 1 & 0 \\ 
1161 & 12.71 & 1.15 & 5443 & 0.04 & 2.7 & syn & 1.21 & 0.90 & 1.20 & 0.52 & 14.5 & 1.47 & 1 & 0 \\ 
1162 & 11.32 & 2.26 & 5754 & -0.20 & 1.0 & syn & 1.11 & 0.90 & 1.10 & 0.67 & 10.3 & 2.48 & 1 & 1 \\ 
1163 & 13.22 & 1.43 & 5244 & -0.27 & 0.4 & syn & 0.77 & 0.77 & 0.77 & 1.66 & 9.0 & 1.48 & 1 & 0 \\ 
1165 & 12.29 & 1.96 & 5400 & 0.00 & 1.0 & syn & 0.85 & 0.88 & 0.85 & 1.44 & 4.4 & 1.93 & 1 & 1 \\ 
1168 & 12.60 & 0.61 & 6107 & 0.04 & 6.4 & syn & 2.24 & 1.35 & 2.20 & 0.13 & 3.1 & 0.94 & 1 & 0 \\ 
1169 & 11.71 & 2.01 & 5648 & 0.14 & 0.2 & syn & 1.05 & 0.99 & 1.04 & 0.87 & 6.0 & 1.89 & 1 & 1 \\ 
1175 & 11.62 & 0.79 & 5588 & 0.08 & 4.4 & syn & 2.82 & 1.43 & 2.82 & 0.06 & 2.7 & 1.07 & 1 & 0 \\ 
1176 & 13.38 & 1.58 & 4420 & 0.11 & \nodata & emp & 0.72 & 0.71 & 0.69 & 2.08 & 10.5 & 1.65 & 1 & 1 \\ 
1194 & 13.38 & 1.91 & 4319 & -0.31 & \nodata & emp & 0.61 & 0.60 & 0.59 & 2.88 & 10.7 & 2.07 & 1 & 1 \\ 
1196 & 13.46 & 0.77 & 5686 & -0.16 & 1.6 & syn & 1.24 & 0.91 & 1.21 & 0.50 & 11.8 & 0.77 & 1 & 0 \\ 
1198 & 13.96 & 0.52 & 6323 & 0.10 & 8.4 & syn & 1.38 & 1.26 & 1.33 & 0.52 & 1.8 & 0.58 & 1 & 0 \\ 
1199 & 12.71 & 2.09 & 4664 & 0.12 & \nodata & emp & 0.71 & 0.75 & 0.73 & 1.93 & 7.8 & 1.77 & 1 & 1 \\ 
1202 & 13.11 & 2.01 & 4140 & 0.08 & \nodata & emp & 0.68 & 0.64 & 0.66 & 2.25 & 11.7 & 2.26 & 1 & 1 \\ 
1203 & 13.84 & 0.90 & 5693 & -0.29 & 0.7 & syn & 0.89 & 0.86 & 0.88 & 1.24 & 6.5 & 0.96 & 1 & 0 \\ 
1206 & 12.05 & 0.66 & 5769 & 0.10 & 5.3 & syn & 2.75 & 1.41 & 2.70 & 0.07 & 2.8 & 0.83 & 1 & 0 \\ 
1208 & 12.36 & 0.52 & 6334 & -0.09 & 8.2 & syn & 3.02 & 1.46 & 2.53 & 0.08 & 2.1 & 1.14 & 1 & 0 \\ 
1209 & 13.35 & 1.06 & 5777 & 0.06 & 1.5 & syn & 0.98 & 1.00 & 0.98 & 1.03 & 3.2 & 0.94 & 1 & 0 \\ 
1215 & 11.97 & 1.05 & 6054 & 0.09 & 2.9 & syn & 1.74 & 1.28 & 1.73 & 0.24 & 3.5 & 1.07 & 1 & 1 \\ 
1216 & 12.01 & 1.10 & 5931 & -0.10 & 3.5 & syn & 1.65 & 1.09 & 1.63 & 0.25 & 6.3 & 1.19 & 1 & 1 \\ 
1218 & 11.71 & 2.06 & 5575 & -0.03 & 2.2 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
1219 & 12.47 & 2.03 & 5078 & 0.12 & 0.7 & syn & 0.78 & 0.84 & 0.81 & 1.57 & 6.2 & 1.95 & 1 & 0 \\ 
1220 & 11.07 & 1.25 & 5289 & 0.16 & 2.8 & syn & 2.41 & 1.27 & 2.40 & 0.09 & 4.4 & 1.45 & 1 & 0 \\ 
1221 & 9.47 & 2.28 & 4979 & 0.34 & 2.1 & syn & 2.82 & 1.34 & 2.82 & 0.06 & 4.0 & 2.18 & 1 & 0 \\ 
1222 & 10.21 & 1.30 & 5033 & 0.06 & 3.2 & syn & 3.50 & 1.35 & 3.50 & 0.03 & 3.3 & 1.46 & 1 & 0 \\ 
1225 & 12.61 & 2.00 & 4102 & 0.14 & \nodata & emp & 0.87 & 0.66 & 0.68 & 2.06 & 14.6 & 2.86 & 4 & 0 \\ 
1230 & 9.99 & 0.79 & 5017 & -0.04 & 3.9 & syn & 6.54 & 1.59 & 6.52 & 0.01 & 1.7 & 1.17 & 1 & 0 \\ 
1239 & 13.52 & 1.02 & 5748 & -0.04 & 1.3 & syn & 0.90 & 0.95 & 0.91 & 1.26 & 2.6 & 0.91 & 1 & 0 \\ 
1240 & 12.84 & 1.31 & 5553 & 0.15 & 0.9 & syn & 0.97 & 0.97 & 0.97 & 1.05 & 5.2 & 1.24 & 1 & 0 \\ 
1241 & 10.23 & 1.12 & 4839 & 0.37 & 3.2 & syn & 4.09 & 1.39 & 4.10 & 0.02 & 3.6 & 1.02 & 1 & 0 \\ 
1242 & 12.47 & 1.12 & 6162 & -0.01 & 5.5 & syn & 1.27 & 1.14 & 1.26 & 0.56 & 3.2 & 1.15 & 1 & 1 \\ 
1245 & 12.84 & 1.05 & 6038 & -0.05 & 3.3 & syn & 1.16 & 1.06 & 1.15 & 0.69 & 3.9 & 1.04 & 1 & 1 \\ 
1257 & 12.73 & -0.28 & 5493 & 0.31 & 3.5 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
1266 & 12.76 & 2.29 & 4335 & -0.06 & \nodata & emp & 0.67 & 0.66 & 0.65 & 2.35 & 10.8 & 2.44 & 1 & 1 \\ 
1270 & 12.90 & 1.58 & 5202 & 0.08 & 1.6 & syn & 0.81 & 0.86 & 0.82 & 1.56 & 4.7 & 1.54 & 1 & 0 \\ 
1271 & 12.35 & 0.96 & 6312 & -0.28 & 6.9 & syn & 1.57 & 1.18 & 1.56 & 0.31 & 3.7 & 1.31 & 1 & 1 \\ 
1274 & 11.54 & 2.89 & 5238 & -0.22 & 1.4 & syn & 0.82 & 0.78 & 0.82 & 1.40 & 12.5 & 3.14 & 1 & 0 \\ 
1275 & 11.99 & 1.59 & 5877 & 0.04 & 2.8 & syn & 1.18 & 1.04 & 1.17 & 0.65 & 5.6 & 1.57 & 1 & 1 \\ 
1276 & 13.07 & 1.19 & 5488 & 0.14 & 1.4 & syn & 0.96 & 0.94 & 0.96 & 1.07 & 6.3 & 1.17 & 1 & 0 \\ 
1278 & 13.65 & 0.77 & 5705 & -0.20 & 0.7 & syn & 1.13 & 0.89 & 1.11 & 0.64 & 11.4 & 0.80 & 1 & 0 \\ 
1279 & 12.25 & 1.56 & 5696 & -0.03 & 1.3 & syn & 1.05 & 0.94 & 1.04 & 0.82 & 7.9 & 1.50 & 1 & 1 \\ 
1282 & 11.20 & 1.59 & 6087 & -0.13 & 6.2 & syn & 1.62 & 1.16 & 1.61 & 0.28 & 4.6 & 1.88 & 1 & 1 \\ 
1283 & 10.13 & 2.79 & 5781 & -0.26 & 0.3 & syn & 1.56 & 0.96 & 1.55 & 0.25 & 9.5 & 3.55 & 1 & 1 \\ 
1288 & 13.69 & 0.69 & 6072 & 0.07 & 1.7 & syn & 1.18 & 1.12 & 1.17 & 0.69 & 2.7 & 0.70 & 1 & 0 \\ 
1298 & 13.14 & 2.16 & 4236 & -0.23 & \nodata & emp & 0.61 & 0.61 & 0.60 & 2.82 & 11.0 & 2.37 & 1 & 1 \\ 
1299 & 10.12 & 1.20 & 4951 & 0.05 & 3.0 & syn & 3.97 & 1.30 & 3.96 & 0.02 & 3.7 & 1.33 & 1 & 0 \\ 
1300 & 11.88 & 2.97 & 4687 & 0.08 & \nodata & emp & 0.73 & 0.75 & 0.73 & 1.89 & 9.0 & 2.64 & 1 & 0 \\ 
1301 & 14.08 & 0.99 & 5224 & -0.26 & 0.9 & syn & 0.76 & 0.77 & 0.76 & 1.71 & 8.3 & 1.00 & 1 & 0 \\ 
1305 & 13.32 & 1.24 & 5297 & 0.17 & 0.5 & syn & 0.84 & 0.90 & 0.85 & 1.46 & 3.7 & 1.21 & 1 & 0 \\ 
1306 & 14.12 & 0.84 & 5608 & -0.26 & 0.3 & syn & 0.86 & 0.85 & 0.84 & 1.38 & 5.8 & 0.83 & 1 & 0 \\ 
1307 & 13.13 & 1.22 & 5552 & 0.12 & 0.8 & syn & 0.91 & 0.95 & 0.91 & 1.24 & 3.3 & 1.18 & 1 & 0 \\ 
1308 & 12.46 & 1.04 & 5654 & 0.03 & 2.4 & syn & 1.43 & 1.00 & 1.42 & 0.35 & 9.9 & 1.00 & 1 & 1 \\ 
1309 & 12.83 & 0.70 & 6485 & -0.00 & 21.2 & syn & 1.68 & 1.34 & 1.67 & 0.28 & 2.2 & 0.82 & 3 & 1 \\ 
1311 & 12.12 & 1.62 & 5919 & -0.25 & 2.0 & syn & 1.05 & 0.93 & 1.05 & 0.80 & 6.9 & 1.73 & 1 & 1 \\ 
1314 & 11.19 & 0.82 & 5045 & 0.11 & 2.9 & syn & 3.52 & 1.39 & 3.53 & 0.03 & 3.0 & 0.97 & 1 & 0 \\ 
1315 & 11.84 & 1.61 & 6096 & 0.06 & 4.7 & syn & 1.19 & 1.13 & 1.18 & 0.68 & 2.6 & 1.58 & 1 & 1 \\ 
1316 & 10.56 & 1.88 & 5852 & 0.33 & 3.9 & syn & 1.86 & 1.35 & 1.85 & 0.21 & 3.5 & 1.85 & 1 & 1 \\ 
1331 & 12.97 & 1.79 & 4696 & 0.12 & \nodata & emp & 0.73 & 0.76 & 0.74 & 1.86 & 8.5 & 1.55 & 1 & 1 \\ 
1332 & 13.59 & 0.86 & 5705 & -0.24 & 0.8 & syn & 1.05 & 0.87 & 1.03 & 0.77 & 11.0 & 0.93 & 1 & 0 \\ 
1335 & 12.53 & 0.75 & 6393 & 0.16 & 12.9 & syn & 1.85 & 1.42 & 1.83 & 0.23 & 2.1 & 0.90 & 1 & 0 \\ 
1336 & 13.28 & 1.06 & 5779 & 0.10 & 2.1 & syn & 0.96 & 1.01 & 0.97 & 1.11 & 2.2 & 1.01 & 1 & 0 \\ 
1338 & 13.05 & 1.19 & 5684 & -0.17 & 1.7 & syn & 0.97 & 0.89 & 0.96 & 0.99 & 8.0 & 1.16 & 1 & 0 \\ 
1344 & 12.00 & 1.31 & 6094 & -0.31 & 2.4 & syn & 1.37 & 1.02 & 1.36 & 0.40 & 6.5 & 1.68 & 1 & 1 \\ 
1353 & 12.51 & 1.44 & 5991 & 0.02 & 5.8 & syn & 1.00 & 1.05 & 1.00 & 1.04 & 1.4 & 1.42 & 1 & 1 \\ 
1356 & 13.61 & 0.52 & 5722 & 0.22 & 3.6 & syn & 1.71 & 1.16 & 1.66 & 0.25 & 6.2 & 0.50 & 1 & 0 \\ 
1358 & 13.15 & 1.70 & 4611 & 0.10 & \nodata & emp & 0.73 & 0.74 & 0.72 & 1.95 & 9.1 & 1.54 & 1 & 1 \\ 
1359 & 13.53 & 0.94 & 5771 & -0.16 & 0.2 & syn & 0.97 & 0.92 & 0.95 & 1.04 & 5.8 & 0.99 & 1 & 0 \\ 
1360 & 13.45 & 1.46 & 4960 & -0.12 & 2.3 & syn & 0.70 & 0.75 & 0.72 & 1.94 & 6.5 & 1.43 & 1 & 0 \\ 
1363 & 14.15 & 0.58 & 5647 & 0.24 & 2.1 & syn & 1.19 & 1.04 & 1.15 & 0.65 & 6.8 & 0.56 & 1 & 0 \\ 
1364 & 13.97 & 0.97 & 5310 & 0.08 & 1.4 & syn & 0.81 & 0.88 & 0.83 & 1.53 & 3.5 & 0.90 & 1 & 0 \\ 
1366 & 13.66 & 1.05 & 5480 & 0.10 & 0.7 & syn & 0.83 & 0.92 & 0.85 & 1.48 & 2.2 & 0.97 & 1 & 0 \\ 
1367 & 12.99 & 1.76 & 4967 & -0.08 & 1.4 & syn & 0.72 & 0.76 & 0.74 & 1.87 & 6.8 & 1.73 & 1 & 0 \\ 
1375 & 12.23 & 1.05 & 6229 & -0.20 & 8.8 & syn & 1.52 & 1.16 & 1.50 & 0.34 & 4.0 & 1.36 & 1 & 0 \\ 
1378 & 11.70 & 1.22 & 5602 & -0.26 & 2.2 & syn & 1.78 & 0.96 & 1.76 & 0.17 & 9.5 & 1.52 & 1 & 0 \\ 
1379 & 12.16 & 1.71 & 5688 & -0.09 & 1.6 & syn & 1.00 & 0.92 & 1.00 & 0.92 & 7.6 & 1.70 & 1 & 1 \\ 
1390 & 12.96 & 1.53 & 4358 & 0.17 & \nodata & emp & 0.92 & 0.76 & 0.79 & 1.56 & 18.4 & 2.04 & 1 & 0 \\ 
1393 & 12.77 & 2.67 & 3920 & 0.22 & \nodata & emp & 0.63 & 0.61 & 0.63 & 2.45 & 11.1 & 2.99 & 1 & 1 \\ 
1396 & 14.17 & 0.76 & 5502 & 0.10 & 1.5 & syn & 0.91 & 0.93 & 0.91 & 1.23 & 4.4 & 0.76 & 1 & 0 \\ 
1397 & 12.43 & 3.09 & 3974 & -0.33 & \nodata & emp & 0.62 & 0.59 & 0.59 & 2.79 & 14.5 & 4.54 & 1 & 1 \\ 
1399 & 13.74 & 1.24 & 4657 & 0.13 & \nodata & emp & 0.76 & 0.76 & 0.74 & 1.84 & 9.8 & 1.11 & 1 & 1 \\ 
1403 & 12.88 & 2.16 & 4328 & 0.15 & \nodata & emp & 0.67 & 0.69 & 0.67 & 2.24 & 8.7 & 2.14 & 1 & 1 \\ 
1404 & 13.48 & 1.60 & 4360 & -0.05 & \nodata & emp & 0.69 & 0.67 & 0.66 & 2.30 & 10.9 & 1.72 & 1 & 1 \\ 
1408 & 11.81 & 3.75 & 4106 & -0.06 & \nodata & emp & 0.67 & 0.63 & 0.64 & 2.41 & 12.8 & 4.51 & 1 & 1 \\ 
1411 & 11.69 & 1.87 & 5698 & 0.36 & 2.6 & syn & 1.16 & 1.09 & 1.15 & 0.71 & 4.5 & 1.64 & 1 & 1 \\ 
1412 & 12.25 & 1.08 & 5935 & 0.12 & 3.8 & syn & 1.48 & 1.17 & 1.47 & 0.36 & 4.7 & 1.09 & 1 & 1 \\ 
1413 & 12.72 & 0.61 & 5286 & -0.01 & 2.7 & syn & 2.27 & 1.13 & 2.24 & 0.10 & 6.1 & 0.68 & 1 & 0 \\ 
1420 & 13.49 & 1.30 & 4574 & 0.15 & \nodata & emp & 0.82 & 0.75 & 0.74 & 1.78 & 12.5 & 1.30 & 1 & 1 \\ 
1421 & 13.70 & 0.84 & 5632 & 0.04 & 2.2 & syn & 1.02 & 0.95 & 1.00 & 0.93 & 6.7 & 0.82 & 1 & 0 \\ 
1424 & 12.91 & 1.90 & 4604 & 0.10 & \nodata & emp & 0.72 & 0.74 & 0.72 & 1.96 & 9.0 & 1.71 & 1 & 1 \\ 
1426 & 12.78 & 1.47 & 5689 & -0.13 & 1.3 & syn & 0.87 & 0.91 & 0.87 & 1.35 & 3.2 & 1.44 & 1 & 0 \\ 
1427 & 13.06 & 2.34 & 4096 & -0.24 & \nodata & emp & 0.62 & 0.59 & 0.59 & 2.85 & 12.3 & 2.80 & 1 & 1 \\ 
1428 & 12.52 & 2.34 & 4716 & -0.09 & \nodata & emp & 0.69 & 0.71 & 0.70 & 2.07 & 8.5 & 2.08 & 1 & 1 \\ 
1430 & 13.07 & 1.95 & 4382 & -0.30 & \nodata & emp & 0.68 & 0.64 & 0.63 & 2.50 & 12.4 & 2.27 & 1 & 1 \\ 
1431 & 11.81 & 2.14 & 5532 & 0.26 & 0.3 & syn & 0.95 & 1.00 & 0.95 & 1.17 & 3.0 & 1.90 & 1 & 1 \\ 
1432 & 13.44 & 0.97 & 5676 & 0.11 & 1.8 & syn & 0.97 & 0.99 & 0.97 & 1.08 & 3.4 & 0.89 & 1 & 0 \\ 
1434 & 12.71 & 1.97 & 4640 & 0.14 & \nodata & emp & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
1436 & 12.71 & 1.41 & 5658 & 0.18 & 1.5 & syn & 0.94 & 1.00 & 0.94 & 1.18 & 2.2 & 1.33 & 1 & 0 \\ 
1438 & 12.43 & 0.75 & 5675 & 0.17 & 3.9 & syn & 2.02 & 1.21 & 2.00 & 0.15 & 5.4 & 0.81 & 1 & 1 \\ 
1439 & 11.53 & 1.24 & 5974 & 0.13 & 4.9 & syn & 1.80 & 1.29 & 1.78 & 0.22 & 3.7 & 1.31 & 1 & 1 \\ 
1442 & 10.91 & 2.98 & 5555 & 0.42 & 0.6 & syn & 1.02 & 1.05 & 1.02 & 0.98 & 3.3 & 2.33 & 1 & 1 \\ 
1444 & 12.59 & 0.64 & 6191 & 0.10 & 8.3 & syn & 2.12 & 1.42 & 2.09 & 0.15 & 2.5 & 0.86 & 1 & 1 \\ 
1445 & 11.15 & 1.78 & 6351 & 0.14 & 13.8 & syn & 1.44 & 1.30 & 1.43 & 0.44 & 1.9 & 1.90 & 1 & 1 \\ 
1459 & 12.78 & 1.95 & 4122 & 0.17 & \nodata & emp & 0.82 & 0.67 & 0.68 & 2.07 & 14.4 & 2.58 & 1 & 0 \\ 
1461 & 13.54 & 1.01 & 4732 & -0.01 & \nodata & emp & 1.01 & 0.79 & 0.84 & 1.31 & 18.0 & 1.22 & 1 & 0 \\ 
1463 & 10.97 & 1.64 & 6475 & -0.04 & 10.3 & syn & 1.69 & 1.32 & 1.66 & 0.28 & 2.3 & 2.16 & 1 & 0 \\ 
1466 & 13.95 & 1.17 & 4610 & 0.14 & \nodata & emp & 0.73 & 0.75 & 0.73 & 1.92 & 8.9 & 1.02 & 1 & 1 \\ 
1474 & 11.86 & 1.01 & 6413 & 0.18 & 13.6 & syn & 1.82 & 1.43 & 1.80 & 0.24 & 2.0 & 1.28 & 1 & 1 \\ 
1475 & 13.20 & 1.87 & 4257 & -0.11 & \nodata & emp & 0.69 & 0.65 & 0.65 & 2.38 & 12.6 & 2.17 & 1 & 1 \\ 
1477 & 14.00 & 0.99 & 5252 & -0.02 & 2.4 & syn & 0.78 & 0.84 & 0.79 & 1.66 & 3.8 & 0.96 & 1 & 0 \\ 
1478 & 10.86 & 3.37 & 5551 & 0.04 & 0.6 & syn & 0.93 & 0.93 & 0.92 & 1.17 & 5.2 & 3.21 & 1 & 1 \\ 
1480 & 13.86 & 1.22 & 4938 & -0.19 & 2.9 & syn & 0.70 & 0.73 & 0.71 & 2.00 & 7.8 & 1.22 & 1 & 1 \\ 
1483 & 12.81 & 0.87 & 5807 & 0.29 & 1.8 & syn & 1.46 & 1.18 & 1.45 & 0.38 & 5.0 & 0.76 & 1 & 0 \\ 
1484 & 12.93 & 1.55 & 4725 & 0.13 & \nodata & emp & 0.86 & 0.78 & 0.79 & 1.52 & 15.0 & 1.57 & 1 & 0 \\ 
1486 & 13.90 & 0.74 & 5715 & 0.16 & 1.6 & syn & 1.05 & 1.02 & 1.03 & 0.90 & 4.2 & 0.67 & 1 & 0 \\ 
1494 & 13.44 & 1.42 & 4373 & -0.02 & \nodata & emp & 0.79 & 0.69 & 0.69 & 2.08 & 13.6 & 1.72 & 1 & 1 \\ 
1501 & 13.48 & 1.57 & 4510 & -0.41 & \nodata & emp & 0.68 & 0.63 & 0.63 & 2.51 & 12.3 & 1.82 & 1 & 1 \\ 
1510 & 13.87 & 1.34 & 4680 & -0.03 & \nodata & emp & 0.65 & 0.71 & 0.68 & 2.18 & 6.4 & 1.13 & 1 & 1 \\ 
1514 & 12.78 & 2.66 & 4181 & -0.50 & \nodata & emp & 0.60 & 0.57 & 0.55 & 3.27 & 13.4 & 3.19 & 1 & 0 \\ 
1515 & 11.60 & 4.79 & 4009 & -0.44 & \nodata & emp & 0.60 & 0.56 & 0.55 & 3.24 & 14.2 & 6.57 & 1 & 1 \\ 
1527 & 13.12 & 1.24 & 5418 & 0.02 & 0.4 & syn & 0.93 & 0.89 & 0.92 & 1.14 & 8.3 & 1.18 & 1 & 0 \\ 
1528 & 12.27 & 2.01 & 5342 & 0.09 & 1.5 & syn & 0.84 & 0.89 & 0.84 & 1.47 & 3.8 & 1.91 & 1 & 1 \\ 
1529 & 12.93 & 0.88 & 5887 & -0.20 & 1.9 & syn & 1.34 & 0.97 & 1.33 & 0.41 & 8.6 & 0.97 & 1 & 0 \\ 
1530 & 11.75 & 1.62 & 6015 & -0.43 & 1.0 & syn & 1.25 & 0.92 & 1.24 & 0.48 & 8.9 & 2.09 & 1 & 1 \\ 
1531 & 11.55 & 3.14 & 5799 & -0.06 & 3.1 & syn & 0.72 & 0.94 & 0.88 & 1.38 & 1.6 & 2.27 & 1 & 0 \\ 
1532 & 11.54 & 1.56 & 6143 & 0.15 & 6.6 & syn & 1.41 & 1.23 & 1.40 & 0.44 & 2.9 & 1.62 & 1 & 1 \\ 
1533 & 12.56 & 1.43 & 5883 & -0.23 & 0.9 & syn & 0.98 & 0.93 & 0.97 & 1.00 & 5.3 & 1.53 & 1 & 1 \\ 
1534 & 12.24 & 1.15 & 6208 & 0.04 & 8.1 & syn & 1.37 & 1.20 & 1.36 & 0.46 & 3.0 & 1.27 & 1 & 1 \\ 
1535 & 11.59 & 2.40 & 5779 & -0.33 & 0.5 & syn & 0.91 & 0.87 & 0.91 & 1.14 & 6.9 & 2.56 & 1 & 1 \\ 
1536 & 11.33 & 1.70 & 5906 & 0.22 & 3.1 & syn & 1.45 & 1.19 & 1.44 & 0.39 & 4.4 & 1.61 & 1 & 1 \\ 
1537 & 10.51 & 1.96 & 6209 & -0.13 & 6.2 & syn & 1.79 & 1.25 & 1.77 & 0.22 & 3.4 & 2.54 & 1 & 1 \\ 
1546 & 12.85 & 2.81 & 6167 & -0.01 & 4.9 & syn & 0.44 & 0.00 & 0.00 & 0.00 & 0.0 & 1.00 & 1 & 0 \\ 
1552 & 13.59 & 1.34 & 4724 & 0.11 & \nodata & emp & 0.75 & 0.76 & 0.74 & 1.83 & 8.7 & 1.19 & 1 & 1 \\ 
1557 & 12.63 & 2.33 & 4678 & 0.05 & \nodata & emp & 0.66 & 0.72 & 0.70 & 2.12 & 5.7 & 1.92 & 1 & 1 \\ 
1563 & 13.70 & 1.18 & 5101 & 0.10 & 2.0 & syn & 0.77 & 0.83 & 0.80 & 1.59 & 5.8 & 1.12 & 1 & 0 \\ 
1567 & 13.50 & 1.31 & 4912 & -0.08 & 2.2 & syn & 0.77 & 0.75 & 0.75 & 1.74 & 10.2 & 1.34 & 1 & 1 \\ 
1569 & 13.34 & 1.78 & 4546 & -0.27 & \nodata & emp & 0.64 & 0.65 & 0.63 & 2.50 & 9.6 & 1.82 & 1 & 1 \\ 
1576 & 12.32 & 1.76 & 5579 & 0.25 & 2.0 & syn & 0.91 & 0.99 & 0.92 & 1.26 & 1.9 & 1.58 & 1 & 1 \\ 
1577 & 13.39 & 1.88 & 4189 & -0.06 & \nodata & emp & 0.64 & 0.63 & 0.62 & 2.54 & 10.7 & 2.03 & 1 & 1 \\ 
1581 & 13.66 & 0.45 & 5437 & 0.24 & 2.6 & syn & 1.98 & 1.14 & 1.89 & 0.16 & 7.2 & 0.55 & 1 & 0 \\ 
1584 & 13.19 & 2.09 & 4156 & -0.10 & \nodata & emp & 0.64 & 0.62 & 0.62 & 2.58 & 11.4 & 2.35 & 1 & 1 \\ 
1586 & 12.70 & 2.08 & 4622 & 0.11 & \nodata & emp & 0.73 & 0.74 & 0.72 & 1.93 & 9.0 & 1.81 & 1 & 1 \\ 
1588 & 11.91 & 3.96 & 4108 & -0.28 & \nodata & emp & 0.61 & 0.59 & 0.58 & 2.91 & 12.6 & 4.76 & 1 & 1 \\ 
1589 & 13.19 & 0.75 & 6030 & -0.12 & 4.5 & syn & 3.57 & 1.04 & 1.17 & 0.56 & 4.4 & 1.09 & 1 & 0 \\ 
1590 & 13.45 & 1.42 & 4828 & -0.12 & 3.0 & syn & 0.77 & 0.73 & 0.72 & 1.93 & 9.6 & 1.48 & 1 & 0 \\ 
1596 & 12.85 & 1.86 & 4525 & 0.16 & \nodata & emp & 0.76 & 0.74 & 0.73 & 1.89 & 11.3 & 1.86 & 1 & 1 \\ 
1598 & 12.63 & 1.68 & 5452 & -0.12 & 0.4 & syn & 0.84 & 0.86 & 0.84 & 1.45 & 5.2 & 1.70 & 1 & 0 \\ 
1601 & 12.99 & 0.75 & 5558 & -0.10 & 1.7 & syn & 1.59 & 0.95 & 1.56 & 0.24 & 11.1 & 0.74 & 1 & 0 \\ 
1606 & 12.26 & 1.91 & 5440 & 0.14 & 1.6 & syn & 0.87 & 0.93 & 0.88 & 1.37 & 3.1 & 1.85 & 1 & 1 \\ 
1608 & 12.42 & 1.31 & 5916 & -0.03 & 2.8 & syn & 1.14 & 1.02 & 1.13 & 0.70 & 5.3 & 1.29 & 1 & 1 \\ 
1609 & 12.59 & 1.34 & 5970 & -0.43 & 2.7 & syn & 1.02 & 0.89 & 1.02 & 0.84 & 7.8 & 1.55 & 1 & 1 \\ 
1612 & 7.49 & 11.29 & 6095 & -0.14 & 2.8 & syn & 1.25 & 1.06 & 1.24 & 0.55 & 4.9 & 11.86 & 1 & 1 \\ 
1615 & 9.99 & 3.46 & 6013 & 0.22 & 7.9 & syn & 1.29 & 1.18 & 1.28 & 0.55 & 3.1 & 3.91 & 1 & 1 \\ 
1616 & 10.27 & 3.25 & 6067 & 0.18 & 5.3 & syn & 1.20 & 1.17 & 1.20 & 0.68 & 2.1 & 3.15 & 1 & 1 \\ 
1618 & 10.33 & 2.52 & 6209 & 0.13 & 10.1 & syn & 1.49 & 1.27 & 1.47 & 0.39 & 2.6 & 2.59 & 1 & 1 \\ 
1619 & 9.59 & 8.42 & 4838 & -0.25 & 2.7 & syn & 0.72 & 0.70 & 0.70 & 2.02 & 11.0 & 9.07 & 1 & 1 \\ 
1621 & 10.51 & 1.82 & 6089 & 0.02 & 5.9 & syn & 1.96 & 1.30 & 1.93 & 0.18 & 3.3 & 2.22 & 1 & 1 \\ 
1623 & 10.48 & 2.28 & 5700 & 0.03 & 2.1 & syn & 1.62 & 1.05 & 1.61 & 0.25 & 8.2 & 2.47 & 1 & 0 \\ 
1628 & 11.60 & 1.28 & 6264 & 0.15 & 10.4 & syn & 1.68 & 1.34 & 1.66 & 0.29 & 2.5 & 1.81 & 1 & 1 \\ 
1629 & 12.13 & 1.35 & 5802 & 0.26 & 3.2 & syn & 1.27 & 1.12 & 1.26 & 0.55 & 5.0 & 1.19 & 1 & 1 \\ 
1631 & 13.44 & 1.61 & 5149 & 0.36 & 3.1 & syn & 0.63 & 0.89 & 0.82 & 1.59 & 2.5 & 1.03 & 1 & 0 \\ 
1632 & 12.04 & 1.20 & 6088 & 0.02 & 7.6 & syn & 1.47 & 1.18 & 1.46 & 0.37 & 4.1 & 1.25 & 1 & 1 \\ 
1639 & 12.24 & 0.69 & 6025 & 0.03 & 6.1 & syn & 2.33 & 1.33 & 2.30 & 0.11 & 3.3 & 0.38 & 1 & 0 \\ 
1647 & 12.52 & 0.98 & 5697 & 0.26 & 3.7 & syn & 1.50 & 1.12 & 1.43 & 0.37 & 6.4 & 1.01 & 1 & 0 \\ 
1649 & 11.79 & 4.55 & 3865 & 0.26 & \nodata & emp & 0.60 & 0.58 & 0.60 & 2.68 & 10.1 & 4.85 & 1 & 1 \\ 
1655 & 12.19 & 1.89 & 5541 & -0.09 & 0.3 & syn & 0.91 & 0.89 & 0.90 & 1.19 & 6.7 & 1.90 & 1 & 1 \\ 
1658 & 12.09 & 1.24 & 6278 & 0.16 & 9.7 & syn & 1.35 & 1.27 & 1.33 & 0.53 & 1.6 & 1.27 & 1 & 1 \\ 
1665 & 12.66 & 1.02 & 5978 & 0.32 & 2.9 & syn & 1.30 & 1.21 & 1.28 & 0.56 & 2.6 & 0.85 & 1 & 1 \\ 
1666 & 13.26 & 0.75 & 6420 & 0.11 & 14.2 & syn & 1.31 & 1.27 & 1.29 & 0.58 & 1.0 & 0.76 & 1 & 0 \\ 
1669 & 12.74 & 0.97 & 6140 & -0.05 & 6.9 & syn & 1.30 & 1.12 & 1.28 & 0.52 & 3.8 & 0.99 & 1 & 1 \\ 
1671 & 12.13 & 1.35 & 5961 & 0.07 & 3.5 & syn & 1.26 & 1.10 & 1.25 & 0.56 & 4.7 & 1.26 & 1 & 1 \\ 
1672 & 13.34 & 1.66 & 4438 & 0.12 & \nodata & emp & 0.70 & 0.71 & 0.69 & 2.10 & 9.5 & 1.68 & 1 & 1 \\ 
1687 & 12.93 & 1.99 & 4575 & -0.09 & \nodata & emp & 0.68 & 0.69 & 0.68 & 2.19 & 9.3 & 2.01 & 1 & 1 \\ 
1688 & 12.85 & 0.79 & 5993 & 0.18 & 5.6 & syn & 1.58 & 1.24 & 1.56 & 0.32 & 3.8 & 0.78 & 1 & 0 \\ 
1692 & 10.78 & 3.74 & 5440 & 0.38 & 2.7 & syn & 0.87 & 0.98 & 0.89 & 1.37 & 1.7 & 3.31 & 1 & 1 \\ 
1695 & 12.26 & 1.20 & 5885 & 0.14 & 3.8 & syn & 1.36 & 1.12 & 1.34 & 0.45 & 5.3 & 1.15 & 1 & 1 \\ 
1702 & 12.20 & 7.47 & 3403 & -0.20 & \nodata & emp & 0.36 & 0.34 & 0.36 & 7.09 & 10.9 & 15.13 & 1 & 0 \\ 
1706 & 12.21 & 2.17 & 5106 & 0.02 & 2.4 & syn & 0.83 & 0.82 & 0.82 & 1.44 & 9.6 & 1.80 & 1 & 1 \\ 
1707 & 13.58 & 0.89 & 5688 & -0.27 & 0.5 & syn & 1.02 & 0.85 & 1.01 & 0.81 & 11.4 & 1.00 & 1 & 0 \\ 
1711 & 12.97 & 1.67 & 4994 & 0.24 & 2.1 & syn & 0.76 & 0.84 & 0.80 & 1.62 & 5.3 & 1.56 & 1 & 1 \\ 
1713 & 12.54 & 2.62 & 4221 & -0.06 & \nodata & emp & 0.66 & 0.64 & 0.64 & 2.44 & 11.5 & 2.90 & 1 & 1 \\ 
1715 & 11.47 & 2.02 & 5820 & -0.25 & 1.1 & syn & 1.14 & 0.91 & 1.14 & 0.61 & 10.0 & 2.24 & 1 & 1 \\ 
1716 & 12.62 & 2.14 & 4683 & 0.13 & \nodata & emp & 0.72 & 0.75 & 0.73 & 1.90 & 7.8 & 1.84 & 1 & 1 \\ 
1726 & 10.84 & 4.65 & 4648 & 0.12 & \nodata & emp & 0.75 & 0.75 & 0.74 & 1.84 & 10.2 & 4.24 & 1 & 0 \\ 
1731 & 13.36 & \nodata & 4629 & 0.15 & \nodata & emp & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
1738 & 11.51 & 2.82 & 5310 & 0.26 & 2.3 & syn & 0.85 & 0.93 & 0.86 & 1.46 & 2.7 & 2.59 & 1 & 1 \\ 
1739 & 13.48 & 0.65 & 5795 & 0.08 & 2.6 & syn & 1.44 & 1.08 & 1.40 & 0.38 & 6.9 & 0.72 & 1 & 0 \\ 
1751 & 12.52 & 2.08 & 5134 & -0.01 & 2.5 & syn & 0.75 & 0.81 & 0.78 & 1.69 & 5.1 & 1.99 & 1 & 0 \\ 
1754 & 11.93 & 1.60 & 6184 & -0.05 & 6.8 & syn & 1.16 & 1.11 & 1.15 & 0.72 & 2.3 & 1.65 & 1 & 1 \\ 
1779 & 11.77 & 2.07 & 5867 & 0.33 & 7.0 & syn & 0.98 & 1.08 & 1.00 & 1.08 & 0.9 & 1.88 & 1 & 1 \\ 
1780 & 13.18 & 1.26 & 4905 & 0.15 & 7.7 & syn & 0.93 & 0.82 & 0.88 & 1.17 & 16.5 & 1.39 & 5 & 0 \\ 
1781 & 10.06 & 6.53 & 4906 & 0.19 & 3.8 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
1783 & 12.62 & 1.18 & 5936 & 0.12 & 3.1 & syn & 1.14 & 1.09 & 1.14 & 0.73 & 3.3 & 1.11 & 1 & 1 \\ 
1788 & 12.25 & 2.64 & 4692 & 0.08 & \nodata & emp & 0.69 & 0.74 & 0.72 & 1.99 & 7.0 & 2.23 & 1 & 1 \\ 
1790 & 13.66 & 0.79 & 5660 & 0.01 & 0.6 & syn & 1.10 & 0.95 & 1.08 & 0.74 & 8.8 & 0.75 & 1 & 0 \\ 
1792 & 10.29 & 0.94 & 5463 & 0.06 & 3.6 & syn & 8.34 & 1.42 & 2.81 & 0.05 & 2.5 & 3.15 & 1 & 0 \\ 
1795 & 12.99 & 1.26 & 4420 & -0.39 & \nodata & emp & 1.13 & 0.00 & 0.00 & 0.00 & 0.0 & 2.41 & 5 & 0 \\ 
1796 & 11.08 & 2.54 & 6050 & -0.00 & 4.3 & syn & 1.06 & 1.07 & 1.06 & 0.89 & 2.0 & 2.58 & 1 & 0 \\ 
1797 & 10.84 & 4.66 & 4973 & 0.18 & 4.3 & syn & 0.72 & 0.82 & 0.78 & 1.75 & 4.3 & 4.26 & 1 & 1 \\ 
1800 & 10.81 & 3.76 & 5567 & 0.05 & 6.9 & syn & 0.86 & 0.93 & 0.87 & 1.42 & 2.3 & 3.69 & 1 & 1 \\ 
1802 & 11.96 & 1.86 & 5903 & 0.03 & 3.2 & syn & 0.99 & 1.03 & 0.99 & 1.05 & 2.0 & 1.84 & 1 & 1 \\ 
1803 & 11.14 & 4.14 & 4921 & 0.05 & 2.8 & syn & 0.71 & 0.78 & 0.75 & 1.84 & 5.5 & 3.91 & 1 & 0 \\ 
1804 & 13.45 & 1.24 & 4963 & 0.17 & 9.8 & syn & 0.83 & 0.82 & 0.82 & 1.48 & 9.6 & 1.25 & 1 & 1 \\ 
1805 & 12.21 & 2.01 & 5562 & 0.03 & 3.4 & syn & 0.85 & 0.92 & 0.85 & 1.47 & 2.1 & 1.95 & 1 & 1 \\ 
1806 & 12.31 & 1.23 & 6146 & -0.05 & 6.9 & syn & 1.24 & 1.11 & 1.23 & 0.59 & 3.4 & 1.25 & 1 & 1 \\ 
1808 & 11.26 & 2.31 & 6188 & 0.06 & 6.7 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
1809 & 11.25 & 2.62 & 5758 & 0.12 & 2.8 & syn & 0.99 & 1.02 & 0.99 & 1.05 & 2.7 & 2.50 & 1 & 0 \\ 
1812 & 12.32 & 1.23 & 5977 & -0.03 & 2.4 & syn & 1.25 & 1.06 & 1.24 & 0.55 & 5.4 & 1.24 & 1 & 0 \\ 
1813 & 12.04 & 2.25 & 5420 & 0.07 & 2.1 & syn & 0.83 & 0.90 & 0.83 & 1.54 & 2.4 & 2.17 & 1 & 1 \\ 
1814 & 11.54 & 1.26 & 5791 & -0.50 & 85.3 & syn & 1.81 & 0.94 & 1.79 & 0.16 & 8.7 & 0.33 & 3 & 1 \\ 
1815 & 11.62 & 3.53 & 4641 & 0.11 & \nodata & emp & 0.70 & 0.74 & 0.72 & 2.00 & 7.3 & 2.96 & 1 & 1 \\ 
1818 & 12.48 & 1.77 & 5519 & 0.02 & 2.3 & syn & 0.85 & 0.91 & 0.86 & 1.45 & 2.6 & 1.73 & 1 & 1 \\ 
1819 & 11.90 & 2.45 & 5454 & 0.05 & 3.2 & syn & 0.80 & 0.89 & 0.81 & 1.65 & 1.6 & 2.32 & 1 & 1 \\ 
1820 & 11.84 & 2.52 & 5406 & 0.12 & 2.5 & syn & 0.80 & 0.90 & 0.82 & 1.62 & 1.6 & 2.35 & 1 & 1 \\ 
1822 & 11.10 & 2.58 & 6109 & -0.21 & 4.5 & syn & 1.06 & 1.01 & 1.05 & 0.86 & 3.3 & 2.74 & 1 & 1 \\ 
1824 & 11.35 & 2.22 & 5987 & -0.16 & 3.1 & syn & 1.08 & 0.99 & 1.08 & 0.79 & 4.9 & 2.25 & 1 & 1 \\ 
1825 & 12.14 & 2.22 & 5371 & 0.14 & 4.5 & syn & 0.80 & 0.89 & 0.82 & 1.63 & 1.7 & 2.08 & 1 & 1 \\ 
1826 & 11.91 & 1.74 & 5919 & -0.04 & 2.9 & syn & 1.09 & 1.02 & 1.08 & 0.80 & 4.5 & 1.72 & 1 & 1 \\ 
1831 & 12.29 & 2.02 & 5230 & 0.17 & 2.1 & syn & 0.84 & 0.89 & 0.84 & 1.49 & 4.2 & 1.90 & 1 & 1 \\ 
1832 & 13.35 & 1.24 & 5538 & 0.02 & 2.9 & syn & 0.81 & 0.90 & 0.83 & 1.57 & 1.7 & 1.18 & 1 & 0 \\ 
1833 & 11.83 & 3.47 & 4401 & 0.06 & \nodata & emp & 0.67 & 0.69 & 0.67 & 2.25 & 8.7 & 3.43 & 1 & 1 \\ 
1835 & 11.67 & 2.08 & 5137 & 0.18 & 4.7 & syn & 1.09 & 0.87 & 1.06 & 0.72 & 17.3 & 2.74 & 1 & 0 \\ 
1837 & 11.90 & 2.59 & 5219 & 0.14 & 2.9 & syn & 0.78 & 0.86 & 0.80 & 1.70 & 2.3 & 2.42 & 1 & 1 \\ 
1838 & 12.21 & 3.04 & 4401 & 0.04 & \nodata & emp & 0.64 & 0.67 & 0.65 & 2.38 & 7.2 & 2.90 & 1 & 1 \\ 
1839 & 11.42 & 2.98 & 5458 & 0.12 & 7.1 & syn & 0.83 & 0.92 & 0.85 & 1.50 & 2.0 & 2.81 & 1 & 0 \\ 
1840 & 13.37 & 0.86 & 6167 & 0.05 & 9.5 & syn & 1.11 & 1.13 & 1.11 & 0.82 & 1.3 & 0.88 & 1 & 0 \\ 
1841 & 11.30 & 3.07 & 5173 & 0.05 & 1.9 & syn & 0.87 & 0.83 & 0.86 & 1.28 & 10.8 & 3.28 & 1 & 0 \\ 
1843 & 11.06 & 7.47 & 3669 & 0.20 & \nodata & emp & 0.54 & 0.53 & 0.54 & 3.36 & 11.0 & 9.15 & 1 & 1 \\ 
1845 & 12.19 & 2.37 & 4580 & 0.16 & \nodata & emp & 0.82 & 0.75 & 0.75 & 1.77 & 12.7 & 2.30 & 1 & 1 \\ 
1848 & 12.01 & 1.01 & 6023 & -0.10 & 6.1 & syn & 2.28 & 1.11 & 1.48 & 0.31 & 4.9 & 1.75 & 1 & 0 \\ 
1850 & 12.66 & 1.06 & 5849 & 0.02 & 2.9 & syn & 1.25 & 1.03 & 1.24 & 0.53 & 6.8 & 1.01 & 1 & 1 \\ 
1852 & 11.89 & 1.27 & 6415 & -0.17 & 4.2 & syn & 1.43 & 1.21 & 1.43 & 0.41 & 2.7 & 1.55 & 1 & 0 \\ 
1854 & 11.83 & 2.20 & 5614 & 0.05 & 1.2 & syn & 0.92 & 0.95 & 0.92 & 1.22 & 3.5 & 2.17 & 1 & 1 \\ 
1856 & 12.28 & 2.20 & 5242 & 0.02 & 1.8 & syn & 0.77 & 0.84 & 0.78 & 1.75 & 2.5 & 2.08 & 1 & 1 \\ 
1857 & 12.15 & 1.02 & 5774 & -0.01 & 2.8 & syn & 2.03 & 1.04 & 1.44 & 0.31 & 7.4 & 1.72 & 1 & 0 \\ 
1858 & 13.02 & 1.50 & 5432 & 0.00 & 1.8 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
1860 & 12.51 & 1.47 & 5735 & 0.13 & 2.5 & syn & 0.99 & 1.02 & 0.99 & 1.04 & 2.9 & 1.45 & 1 & 1 \\ 
1861 & 12.51 & 1.38 & 6043 & 0.03 & 7.7 & syn & 1.02 & 1.07 & 1.02 & 0.99 & 1.3 & 1.37 & 1 & 1 \\ 
1862 & 12.11 & 1.85 & 5607 & 0.25 & 1.8 & syn & 0.96 & 1.01 & 0.96 & 1.14 & 2.5 & 1.62 & 1 & 0 \\ 
1863 & 12.31 & 1.40 & 5994 & 0.22 & 4.7 & syn & 1.10 & 1.14 & 1.10 & 0.84 & 1.4 & 1.35 & 1 & 1 \\ 
1864 & 11.75 & 1.17 & 5621 & 0.13 & 2.1 & syn & 1.79 & 1.11 & 1.77 & 0.20 & 7.3 & 1.27 & 1 & 1 \\ 
1867 & 11.96 & 4.16 & 3916 & 0.00 & \nodata & emp & 0.60 & 0.58 & 0.59 & 2.76 & 12.0 & 5.05 & 1 & 1 \\ 
1868 & 12.29 & 3.30 & 3988 & -0.17 & \nodata & emp & 0.63 & 0.60 & 0.61 & 2.63 & 13.5 & 4.38 & 1 & 1 \\ 
1871 & 12.53 & 2.29 & 4444 & 0.19 & \nodata & emp & 0.73 & 0.73 & 0.71 & 1.99 & 10.4 & 2.36 & 1 & 1 \\ 
1874 & 12.69 & 2.30 & 4322 & -0.34 & \nodata & emp & 0.72 & 0.64 & 0.64 & 2.40 & 14.4 & 2.95 & 1 & 1 \\ 
1875 & 12.93 & 1.27 & 5582 & -0.11 & 1.5 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
1876 & 12.61 & 2.59 & 4342 & -0.30 & \nodata & emp & 0.63 & 0.62 & 0.61 & 2.70 & 11.3 & 2.87 & 1 & 1 \\ 
1877 & 11.27 & 3.88 & 4890 & 0.03 & 2.8 & syn & 0.72 & 0.77 & 0.75 & 1.83 & 6.6 & 3.73 & 1 & 1 \\ 
1878 & 11.69 & 1.49 & 6214 & 0.18 & 6.9 & syn & 1.36 & 1.26 & 1.34 & 0.52 & 1.9 & 1.56 & 1 & 1 \\ 
1879 & 12.73 & 3.11 & 3896 & 0.29 & \nodata & emp & 0.59 & 0.57 & 0.59 & 2.80 & 8.7 & 3.03 & 1 & 1 \\ 
1880 & 11.45 & 5.34 & 3882 & -0.04 & \nodata & emp & 0.59 & 0.58 & 0.59 & 2.84 & 12.4 & 6.85 & 1 & 1 \\ 
1883 & 10.61 & 2.16 & 5937 & -0.01 & 6.7 & syn & 1.57 & 1.14 & 1.56 & 0.30 & 5.4 & 1.76 & 1 & 1 \\ 
1886 & 10.92 & 1.86 & 6221 & 0.05 & 10.5 & syn & 1.58 & 1.27 & 1.56 & 0.33 & 2.9 & 2.10 & 1 & 1 \\ 
1888 & 12.09 & 0.92 & 6382 & 0.09 & 17.1 & syn & 1.80 & 1.38 & 1.79 & 0.24 & 2.3 & 1.25 & 1 & 1 \\ 
1889 & 13.66 & 1.10 & 5437 & 0.04 & 2.1 & syn & 0.80 & 0.89 & 0.82 & 1.59 & 2.1 & 1.03 & 1 & 0 \\ 
1890 & 10.37 & 0.75 & 6087 & 0.10 & 7.2 & syn & 11.72 & 1.31 & 1.85 & 0.17 & 2.8 & 2.67 & 1 & 0 \\ 
1891 & 13.26 & 1.42 & 5027 & 0.16 & 1.1 & syn & 0.78 & 0.83 & 0.80 & 1.58 & 6.5 & 1.34 & 1 & 1 \\ 
1893 & 12.62 & 1.09 & 5729 & -0.28 & 2.0 & syn & 1.29 & 0.88 & 1.27 & 0.42 & 12.4 & 1.18 & 1 & 1 \\ 
1894 & 11.06 & 0.89 & 4991 & 0.18 & 3.1 & syn & 3.52 & 1.38 & 3.50 & 0.03 & 3.3 & 0.97 & 1 & 0 \\ 
1895 & 13.34 & 1.75 & 4435 & 0.06 & \nodata & emp & 0.66 & 0.69 & 0.67 & 2.25 & 8.0 & 1.70 & 1 & 1 \\ 
1897 & 12.51 & 1.25 & 5898 & -0.11 & 2.2 & syn & 1.16 & 0.99 & 1.15 & 0.65 & 6.7 & 1.32 & 1 & 1 \\ 
1898 & 11.72 & 1.79 & 5758 & 0.01 & 1.6 & syn & 1.17 & 0.99 & 1.16 & 0.63 & 7.8 & 1.87 & 1 & 1 \\ 
1901 & 12.01 & 1.55 & 6011 & 0.15 & 4.4 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
1902 & 11.45 & 4.57 & 3797 & -0.05 & \nodata & emp & 0.65 & 0.60 & 0.62 & 2.48 & 15.0 & 7.90 & 4 & 0 \\ 
1904 & 11.38 & 3.56 & 5054 & 0.01 & 2.7 & syn & 0.73 & 0.80 & 0.77 & 1.75 & 5.3 & 3.38 & 1 & 1 \\ 
1905 & 11.97 & 2.93 & 4943 & -0.12 & 1.3 & syn & 0.69 & 0.74 & 0.71 & 2.01 & 6.0 & 2.82 & 1 & 1 \\ 
1907 & 12.35 & 2.84 & 4041 & -0.05 & \nodata & emp & 0.68 & 0.63 & 0.64 & 2.33 & 13.8 & 3.75 & 1 & 0 \\ 
1908 & 12.12 & 3.11 & 4289 & -0.08 & \nodata & emp & 0.67 & 0.65 & 0.64 & 2.40 & 11.3 & 3.38 & 1 & 1 \\ 
1909 & 11.41 & 2.37 & 5906 & 0.03 & 2.4 & syn & 1.00 & 1.03 & 1.00 & 1.03 & 2.1 & 2.31 & 1 & 1 \\ 
1913 & 11.66 & 2.46 & 5507 & 0.23 & 2.7 & syn & 0.89 & 0.97 & 0.90 & 1.33 & 2.1 & 2.31 & 1 & 1 \\ 
1915 & 12.50 & 0.81 & 5956 & 0.33 & 6.5 & syn & 1.78 & 1.35 & 1.76 & 0.24 & 3.2 & 0.77 & 1 & 1 \\ 
1916 & 12.14 & 0.48 & 5873 & 0.22 & 5.8 & syn & 5.84 & 1.18 & 1.45 & 0.33 & 3.9 & 1.49 & 1 & 0 \\ 
1917 & 12.26 & 1.47 & 5945 & -0.07 & 3.2 & syn & 1.09 & 1.01 & 1.08 & 0.80 & 4.5 & 1.46 & 1 & 1 \\ 
1921 & 11.68 & 1.38 & 6479 & 0.04 & 18.6 & syn & 1.45 & 1.30 & 1.43 & 0.44 & 1.8 & 1.54 & 1 & 1 \\ 
1922 & 13.73 & 0.74 & 5774 & 0.03 & 1.7 & syn & 1.13 & 1.00 & 1.11 & 0.71 & 6.6 & 0.80 & 1 & 0 \\ 
1923 & 12.40 & 1.84 & 5413 & 0.21 & 1.9 & syn & 0.87 & 0.94 & 0.87 & 1.40 & 2.6 & 1.70 & 1 & 1 \\ 
1924 & 6.49 & 8.76 & 5948 & 0.34 & 4.7 & syn & 2.57 & 1.60 & 2.53 & 0.10 & 2.1 & 9.59 & 1 & 0 \\ 
1925 & 7.77 & 14.69 & 5422 & 0.12 & 2.4 & syn & 0.90 & 0.92 & 0.89 & 1.28 & 4.7 & 14.03 & 1 & 1 \\ 
1928 & 12.16 & 1.56 & 5879 & 0.25 & 2.8 & syn & 1.08 & 1.11 & 1.08 & 0.88 & 1.8 & 1.48 & 1 & 1 \\ 
1929 & 11.18 & 1.50 & 5651 & 0.07 & 2.1 & syn & 1.80 & 1.10 & 1.78 & 0.19 & 7.3 & 1.62 & 1 & 1 \\ 
1930 & 10.76 & 1.83 & 5860 & -0.04 & 5.1 & syn & 1.77 & 1.12 & 1.75 & 0.21 & 6.2 & 1.94 & 1 & 1 \\ 
1931 & 12.87 & 1.65 & 5460 & 0.00 & 1.6 & syn & 0.77 & 0.87 & 0.79 & 1.74 & 1.3 & 1.50 & 1 & 0 \\ 
1934 & 12.27 & 2.73 & 4526 & 0.10 & \nodata & emp & 0.69 & 0.72 & 0.70 & 2.10 & 7.9 & 2.65 & 1 & 1 \\ 
1937 & 11.00 & 5.17 & 4307 & 0.00 & \nodata & emp & 0.67 & 0.66 & 0.65 & 2.34 & 10.4 & 5.40 & 1 & 1 \\ 
1938 & 12.15 & 2.43 & 5114 & -0.22 & 1.6 & syn & 0.75 & 0.76 & 0.75 & 1.77 & 8.7 & 2.48 & 1 & 1 \\ 
1940 & 12.82 & 2.41 & 4237 & -0.16 & \nodata & emp & 0.64 & 0.62 & 0.62 & 2.63 & 11.2 & 2.65 & 1 & 1 \\ 
1944 & 12.53 & 1.64 & 5744 & 0.07 & 3.2 & syn & 0.88 & 0.97 & 0.90 & 1.34 & 1.4 & 1.54 & 1 & 1 \\ 
1945 & 12.76 & 1.47 & 5359 & 0.26 & 1.4 & syn & 0.91 & 0.95 & 0.91 & 1.24 & 4.6 & 1.40 & 1 & 0 \\ 
1947 & 10.94 & 2.35 & 5948 & 0.23 & 3.1 & syn & 1.23 & 1.15 & 1.23 & 0.62 & 3.3 & 1.56 & 1 & 1 \\ 
1951 & 12.22 & 1.27 & 6093 & -0.20 & 4.3 & syn & 1.28 & 1.04 & 1.26 & 0.51 & 5.5 & 1.46 & 1 & 0 \\ 
1952 & 12.99 & 0.98 & 5737 & 0.08 & 1.9 & syn & 1.20 & 1.01 & 1.18 & 0.60 & 7.6 & 0.94 & 1 & 0 \\ 
1955 & 11.96 & 1.30 & 6249 & 0.09 & 9.5 & syn & 1.37 & 1.23 & 1.36 & 0.48 & 2.5 & 1.37 & 1 & 1 \\ 
1958 & 13.62 & 0.86 & 5852 & 0.07 & 4.1 & syn & 1.02 & 1.03 & 1.01 & 0.98 & 2.6 & 0.90 & 1 & 0 \\ 
1959 & 12.08 & 2.87 & 4893 & -0.11 & 2.4 & syn & 0.67 & 0.73 & 0.70 & 2.07 & 5.6 & 2.72 & 1 & 1 \\ 
1960 & 12.68 & 1.10 & 5796 & 0.18 & 3.0 & syn & 1.21 & 1.07 & 1.19 & 0.62 & 5.4 & 0.97 & 1 & 1 \\ 
1961 & 11.12 & 2.49 & 5384 & 0.04 & 3.5 & syn & 1.14 & 0.88 & 1.13 & 0.61 & 15.5 & 3.35 & 1 & 0 \\ 
1962 & 9.46 & 0.96 & 5950 & -0.03 & 4.6 & syn & 11.01 & 1.84 & 4.53 & 0.02 & 1.1 & 4.16 & 1 & 0 \\ 
1963 & 12.64 & 0.61 & 5880 & 0.09 & 4.6 & syn & 2.34 & 1.26 & 2.02 & 0.14 & 4.2 & 1.05 & 1 & 0 \\ 
1964 & 8.95 & 7.41 & 5553 & 0.05 & 2.3 & syn & 1.02 & 0.93 & 1.01 & 0.88 & 8.8 & 8.19 & 1 & 0 \\ 
1967 & 12.17 & 2.75 & 4736 & -0.22 & \nodata & emp & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
1970 & 13.66 & 1.02 & 5461 & 0.09 & 0.3 & syn & 0.87 & 0.92 & 0.87 & 1.37 & 3.4 & 0.93 & 1 & 0 \\ 
1973 & 13.30 & 1.52 & 4512 & -0.01 & \nodata & emp & 0.78 & 0.71 & 0.70 & 2.02 & 11.7 & 1.71 & 1 & 0 \\ 
1978 & 13.58 & 1.04 & 5517 & 0.10 & 1.2 & syn & 0.87 & 0.93 & 0.88 & 1.36 & 2.8 & 1.00 & 1 & 0 \\ 
1979 & 11.42 & 1.81 & 5746 & 0.21 & 2.6 & syn & 1.33 & 1.09 & 1.32 & 0.47 & 6.4 & 2.05 & 1 & 0 \\ 
1980 & 12.12 & 2.07 & 5494 & 0.19 & 2.3 & syn & 0.86 & 0.94 & 0.87 & 1.44 & 1.8 & 1.92 & 1 & 1 \\ 
1984 & 12.29 & 1.38 & 6010 & 0.13 & 4.2 & syn & 1.15 & 1.12 & 1.14 & 0.75 & 2.4 & 1.33 & 1 & 1 \\ 
1985 & 11.58 & 3.29 & 4924 & 0.02 & 2.7 & syn & 0.74 & 0.78 & 0.76 & 1.77 & 7.3 & 3.25 & 1 & 1 \\ 
1988 & 11.75 & 3.28 & 4559 & 0.16 & \nodata & emp & 0.71 & 0.74 & 0.72 & 1.98 & 8.4 & 2.89 & 1 & 1 \\ 
1989 & 11.77 & 2.10 & 5709 & 0.09 & 2.2 & syn & 0.98 & 0.99 & 0.97 & 1.07 & 3.3 & 2.11 & 1 & 1 \\ 
1992 & 13.05 & 0.79 & 5704 & -0.14 & 1.7 & syn & 1.44 & 0.95 & 1.42 & 0.33 & 10.5 & 0.78 & 1 & 0 \\ 
2001 & 11.12 & 3.81 & 5146 & 0.08 & 3.1 & syn & 0.76 & 0.84 & 0.80 & 1.61 & 4.8 & 3.62 & 1 & 1 \\ 
2002 & 11.73 & 1.84 & 6016 & 0.03 & 4.8 & syn & 1.10 & 1.08 & 1.09 & 0.82 & 2.5 & 1.93 & 1 & 0 \\ 
2004 & 11.80 & 1.25 & 5651 & 0.29 & 4.6 & syn & 1.61 & 1.14 & 1.60 & 0.28 & 6.8 & 1.54 & 1 & 1 \\ 
2005 & 12.45 & 1.82 & 4501 & 0.09 & \nodata & emp & 0.95 & 0.80 & 0.86 & 1.27 & 19.2 & 2.45 & 1 & 0 \\ 
2006 & 11.18 & 6.20 & 3902 & -0.16 & \nodata & emp & 0.58 & 0.57 & 0.57 & 2.99 & 12.8 & 8.18 & 1 & 1 \\ 
2007 & 11.72 & 2.06 & 5881 & 0.13 & 2.5 & syn & 1.00 & 1.05 & 1.00 & 1.04 & 1.6 & 1.98 & 1 & 1 \\ 
2009 & 12.25 & 1.53 & 5661 & -0.23 & 1.2 & syn & 1.09 & 0.86 & 1.08 & 0.67 & 12.6 & 1.71 & 1 & 1 \\ 
2010 & 12.01 & 1.23 & 6416 & -0.00 & 10.0 & syn & 1.41 & 1.26 & 1.40 & 0.46 & 2.0 & 1.34 & 1 & 1 \\ 
2011 & 11.38 & 1.78 & 6455 & -0.02 & 15.2 & syn & 1.31 & 1.24 & 1.29 & 0.57 & 1.4 & 1.94 & 1 & 1 \\ 
2012 & 13.30 & 1.08 & 5727 & 0.11 & 3.3 & syn & 0.93 & 1.00 & 0.94 & 1.19 & 2.0 & 1.06 & 1 & 0 \\ 
2013 & 10.59 & 6.64 & 4209 & -0.14 & \nodata & emp & 0.65 & 0.63 & 0.62 & 2.56 & 11.7 & 7.50 & 1 & 1 \\ 
2016 & 12.69 & 0.94 & 5886 & 0.34 & 4.0 & syn & 1.39 & 1.21 & 1.38 & 0.45 & 3.7 & 0.86 & 1 & 1 \\ 
2017 & 11.57 & 2.59 & 5664 & 0.05 & 3.9 & syn & 0.86 & 0.94 & 0.87 & 1.41 & 1.6 & 2.47 & 1 & 1 \\ 
2022 & 13.18 & 1.09 & 5884 & 0.21 & 6.3 & syn & 0.97 & 1.06 & 0.99 & 1.09 & 1.1 & 1.01 & 1 & 0 \\ 
2025 & 12.39 & 1.07 & 6476 & 0.08 & 21.3 & syn & 1.37 & 1.29 & 1.35 & 0.52 & 1.2 & 1.12 & 3 & 1 \\ 
2026 & 11.93 & 1.86 & 6017 & -0.09 & 4.5 & syn & 0.98 & 1.02 & 0.98 & 1.06 & 1.8 & 1.85 & 1 & 1 \\ 
2029 & 11.13 & 3.98 & 5209 & -0.12 & 2.9 & syn & 0.72 & 0.80 & 0.76 & 1.79 & 4.6 & 3.82 & 1 & 1 \\ 
2031 & 12.33 & 2.54 & 4381 & 0.12 & \nodata & emp & 0.73 & 0.71 & 0.70 & 2.05 & 11.8 & 2.74 & 1 & 1 \\ 
2033 & 11.82 & \nodata & 5055 & -0.11 & 1.6 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
2035 & 11.36 & 2.93 & 5521 & 0.07 & 6.0 & syn & 0.88 & 0.93 & 0.88 & 1.38 & 2.8 & 2.92 & 1 & 1 \\ 
2036 & 12.81 & 2.62 & 4031 & -0.05 & \nodata & emp & 0.63 & 0.61 & 0.62 & 2.54 & 12.1 & 3.11 & 1 & 1 \\ 
2037 & 13.02 & 1.70 & 4751 & 0.15 & \nodata & emp & 0.75 & 0.77 & 0.75 & 1.79 & 8.3 & 1.44 & 1 & 0 \\ 
2038 & 13.08 & 1.33 & 5511 & 0.12 & 2.1 & syn & 0.86 & 0.93 & 0.87 & 1.42 & 2.2 & 1.26 & 1 & 0 \\ 
2039 & 12.66 & 1.52 & 5586 & 0.28 & 2.3 & syn & 0.90 & 1.00 & 0.92 & 1.28 & 1.6 & 1.44 & 1 & 0 \\ 
2040 & 12.66 & 1.37 & 5668 & 0.02 & 1.3 & syn & 1.00 & 0.96 & 0.99 & 0.97 & 5.9 & 1.37 & 1 & 1 \\ 
2042 & 11.76 & 0.96 & 5736 & -0.83 & 101.5 & syn & 2.23 & 0.94 & 2.20 & 0.09 & 7.5 & 0.08 & 3 & 1 \\ 
2043 & 12.63 & 1.18 & 5827 & 0.01 & 2.4 & syn & 1.15 & 1.01 & 1.14 & 0.67 & 6.4 & 1.15 & 1 & 1 \\ 
2044 & 14.16 & 0.70 & 5681 & 0.21 & 2.0 & syn & 0.98 & 1.02 & 0.99 & 1.05 & 2.8 & 0.68 & 1 & 0 \\ 
2045 & 13.16 & 1.83 & 4431 & -0.09 & \nodata & emp & 0.69 & 0.67 & 0.67 & 2.25 & 11.0 & 1.96 & 1 & 1 \\ 
2046 & 11.54 & 1.46 & 5582 & 0.23 & 2.7 & syn & 1.58 & 1.08 & 1.56 & 0.28 & 8.5 & 1.42 & 1 & 1 \\ 
2047 & 12.68 & 1.09 & 6172 & -0.02 & 5.3 & syn & 1.19 & 1.12 & 1.18 & 0.68 & 2.5 & 1.13 & 1 & 1 \\ 
2048 & 13.78 & 0.99 & 5166 & 0.15 & 2.8 & syn & 0.88 & 0.86 & 0.87 & 1.29 & 9.0 & 1.05 & 1 & 0 \\ 
2049 & 12.57 & 1.04 & 5972 & 0.07 & 4.1 & syn & 1.33 & 1.12 & 1.32 & 0.48 & 4.8 & 0.98 & 1 & 1 \\ 
2051 & 13.67 & 0.72 & 5754 & -0.06 & 1.5 & syn & 1.18 & 0.96 & 1.16 & 0.60 & 8.9 & 0.77 & 1 & 0 \\ 
2053 & 11.70 & 1.44 & 6183 & 0.08 & 6.8 & syn & 1.40 & 1.22 & 1.39 & 0.45 & 3.0 & 1.58 & 1 & 1 \\ 
2057 & 12.07 & 4.01 & 3906 & -0.17 & \nodata & emp & 0.59 & 0.57 & 0.58 & 2.90 & 13.2 & 5.43 & 1 & 1 \\ 
2058 & 12.41 & 3.46 & 3953 & -0.17 & \nodata & emp & 0.59 & 0.57 & 0.58 & 2.95 & 12.5 & 4.33 & 1 & 0 \\ 
2060 & 12.98 & 1.81 & 4691 & 0.12 & \nodata & emp & 0.72 & 0.75 & 0.73 & 1.90 & 7.8 & 1.54 & 1 & 1 \\ 
2071 & 11.91 & 2.40 & 5269 & 0.17 & 1.7 & syn & 0.84 & 0.90 & 0.84 & 1.50 & 3.5 & 2.27 & 1 & 1 \\ 
2072 & 11.97 & 1.38 & 5811 & -0.16 & 1.6 & syn & 1.35 & 0.96 & 1.34 & 0.40 & 9.4 & 1.45 & 1 & 1 \\ 
2073 & 13.41 & 1.48 & 4938 & 0.06 & 1.8 & syn & 0.71 & 0.79 & 0.75 & 1.82 & 5.3 & 1.36 & 1 & 1 \\ 
2076 & 13.89 & 0.76 & 5853 & 0.21 & 1.8 & syn & 1.00 & 1.07 & 1.02 & 1.01 & 1.5 & 0.63 & 1 & 0 \\ 
2078 & 12.94 & 2.17 & 4293 & 0.10 & \nodata & emp & 0.66 & 0.67 & 0.66 & 2.32 & 9.1 & 2.18 & 1 & 1 \\ 
2079 & 11.21 & 2.78 & 5468 & 0.39 & 1.6 & syn & 0.97 & 1.01 & 0.97 & 1.10 & 3.5 & 2.53 & 1 & 1 \\ 
2081 & 11.34 & 0.82 & 5072 & 0.19 & 2.8 & syn & 3.30 & 1.44 & 3.31 & 0.04 & 2.8 & 0.93 & 1 & 0 \\ 
2082 & 12.69 & 0.96 & 6004 & 0.33 & 3.9 & syn & 1.37 & 1.24 & 1.35 & 0.49 & 2.7 & 0.89 & 1 & 1 \\ 
2083 & 12.01 & 1.04 & 6023 & -0.04 & 5.6 & syn & 1.89 & 1.16 & 1.57 & 0.28 & 4.6 & 1.69 & 1 & 0 \\ 
2086 & 12.52 & 1.00 & 5825 & -0.05 & 3.0 & syn & 1.44 & 1.03 & 1.43 & 0.35 & 7.9 & 0.94 & 1 & 1 \\ 
2087 & 10.48 & 3.59 & 5983 & 0.03 & 3.6 & syn & 1.01 & 1.05 & 1.01 & 1.01 & 1.6 & 3.47 & 1 & 1 \\ 
2090 & 12.39 & 3.88 & 3725 & 0.38 & \nodata & emp & 0.56 & 0.55 & 0.56 & 3.08 & 9.4 & 4.01 & 1 & 1 \\ 
2092 & 14.49 & 0.72 & 5565 & -0.31 & 1.0 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
2093 & 14.00 & 0.69 & 5958 & 0.02 & 3.4 & syn & 1.06 & 1.05 & 1.05 & 0.89 & 2.7 & 0.66 & 1 & 0 \\ 
2094 & 13.07 & 1.19 & 5330 & 0.02 & 2.2 & syn & 1.00 & 0.85 & 0.98 & 0.90 & 14.0 & 1.44 & 1 & 0 \\ 
2098 & 12.48 & 0.96 & 6305 & -0.13 & 11.4 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
2101 & 12.38 & 2.67 & 4258 & 0.04 & \nodata & emp & 0.70 & 0.67 & 0.66 & 2.27 & 11.6 & 2.91 & 1 & 1 \\ 
2105 & 12.46 & 1.47 & 5926 & -0.05 & 2.6 & syn & 1.00 & 1.01 & 1.00 & 1.01 & 2.7 & 1.43 & 1 & 1 \\ 
2109 & 12.73 & 0.77 & 6028 & 0.04 & 7.4 & syn & 1.65 & 1.22 & 1.63 & 0.28 & 4.1 & 0.82 & 1 & 1 \\ 
2110 & 10.97 & 1.91 & 6404 & 0.23 & 16.4 & syn & 1.45 & 1.35 & 1.44 & 0.45 & 1.4 & 2.00 & 1 & 1 \\ 
2111 & 13.23 & 1.17 & 5604 & 0.15 & 3.7 & syn & 0.90 & 0.97 & 0.91 & 1.27 & 2.3 & 1.13 & 1 & 0 \\ 
2114 & 12.37 & 3.17 & 4101 & -0.13 & \nodata & emp & 0.62 & 0.61 & 0.61 & 2.62 & 11.9 & 3.67 & 1 & 1 \\ 
2115 & 14.15 & 0.91 & 5073 & 0.01 & 3.2 & syn & 0.81 & 0.81 & 0.80 & 1.53 & 8.7 & 0.49 & 1 & 0 \\ 
2119 & 12.15 & 2.36 & 5100 & 0.18 & 3.6 & syn & 0.77 & 0.85 & 0.81 & 1.56 & 5.1 & 2.20 & 1 & 1 \\ 
2120 & 11.67 & 3.25 & 5026 & -0.05 & 2.7 & syn & 0.72 & 0.78 & 0.75 & 1.85 & 5.4 & 3.10 & 1 & 1 \\ 
2124 & 11.58 & 3.31 & 4163 & -0.24 & \nodata & emp & 0.83 & 0.64 & 0.65 & 2.35 & 15.4 & 5.17 & 1 & 0 \\ 
2126 & 13.60 & 1.40 & 4707 & -0.16 & \nodata & emp & 0.71 & 0.70 & 0.69 & 2.09 & 9.8 & 1.39 & 1 & 1 \\ 
2130 & 12.78 & 2.56 & 4068 & -0.06 & \nodata & emp & 0.65 & 0.61 & 0.62 & 2.49 & 12.1 & 3.01 & 1 & 1 \\ 
2133 & 10.14 & 0.80 & 4606 & 0.37 & 3.2 & syn & 6.23 & 1.30 & 6.17 & 0.01 & 4.7 & 0.52 & 1 & 0 \\ 
2135 & 12.20 & 1.10 & 6171 & 0.05 & 7.6 & syn & 1.47 & 1.23 & 1.46 & 0.38 & 3.2 & 1.20 & 1 & 1 \\ 
2137 & 11.94 & 2.41 & 5292 & -0.12 & 1.4 & syn & 0.81 & 0.82 & 0.81 & 1.51 & 7.1 & 2.47 & 1 & 1 \\ 
2143 & 12.46 & 1.78 & 5435 & 0.23 & 2.3 & syn & 0.85 & 0.94 & 0.87 & 1.44 & 2.0 & 1.60 & 1 & 1 \\ 
2146 & 13.17 & 1.65 & 4733 & 0.14 & \nodata & emp & 0.73 & 0.77 & 0.74 & 1.86 & 7.5 & 1.37 & 1 & 1 \\ 
2147 & 12.78 & 0.94 & 5628 & -0.12 & 2.0 & syn & 1.39 & 0.92 & 1.35 & 0.36 & 12.0 & 1.39 & 1 & 0 \\ 
2148 & 11.70 & 1.34 & 5612 & 0.42 & 3.2 & syn & 1.60 & 1.21 & 1.58 & 0.30 & 5.6 & 1.18 & 1 & 1 \\ 
2149 & 10.79 & 2.10 & 6235 & 0.22 & 8.8 & syn & 1.46 & 1.30 & 1.46 & 0.42 & 2.2 & 2.24 & 1 & 1 \\ 
2153 & 12.39 & 1.15 & 6023 & -0.06 & 5.8 & syn & 1.31 & 1.08 & 1.30 & 0.49 & 5.3 & 1.14 & 1 & 1 \\ 
2156 & 12.83 & 3.47 & 3733 & -0.13 & \nodata & emp & 0.51 & 0.50 & 0.51 & 3.77 & 12.0 & 5.17 & 1 & 0 \\ 
2158 & 11.28 & 2.88 & 5357 & 0.02 & 1.8 & syn & 0.93 & 0.87 & 0.92 & 1.08 & 10.5 & 2.72 & 1 & 1 \\ 
2159 & 11.98 & 1.88 & 5764 & 0.12 & 2.3 & syn & 0.98 & 1.02 & 0.98 & 1.07 & 2.4 & 1.81 & 1 & 1 \\ 
2162 & 12.53 & 1.60 & 5686 & -0.43 & 1.3 & syn & 0.91 & 0.81 & 0.90 & 1.09 & 10.7 & 1.78 & 1 & 1 \\ 
2167 & 13.78 & 0.87 & 5751 & 0.13 & 3.0 & syn & 0.93 & 1.01 & 0.95 & 1.16 & 1.8 & 0.83 & 1 & 0 \\ 
2168 & 13.35 & 0.56 & 5913 & -0.07 & 3.8 & syn & 1.75 & 1.12 & 1.69 & 0.22 & 6.0 & 0.86 & 1 & 0 \\ 
2169 & 10.66 & 4.03 & 5396 & 0.18 & 0.3 & syn & 0.86 & 0.93 & 0.87 & 1.42 & 2.9 & 3.86 & 1 & 1 \\ 
2173 & 10.67 & 5.34 & 4703 & 0.12 & \nodata & emp & 0.70 & 0.75 & 0.73 & 1.94 & 6.8 & 4.47 & 1 & 1 \\ 
2175 & 11.18 & 1.32 & 5416 & 0.10 & 3.1 & syn & 2.10 & 1.15 & 2.09 & 0.13 & 6.3 & 1.52 & 1 & 0 \\ 
2183 & 13.55 & 0.88 & 5652 & 0.12 & 0.3 & syn & 1.04 & 0.99 & 1.02 & 0.91 & 5.6 & 0.90 & 1 & 0 \\ 
2188 & 13.74 & 0.87 & 5636 & -0.56 & 0.3 & syn & 0.97 & 0.77 & 0.95 & 0.88 & 15.7 & 1.04 & 1 & 0 \\ 
2191 & 11.81 & 4.54 & 3885 & 0.25 & \nodata & emp & 0.60 & 0.58 & 0.60 & 2.70 & 9.7 & 4.73 & 1 & 1 \\ 
2193 & 13.17 & 2.06 & 4341 & -0.34 & \nodata & emp & 0.62 & 0.61 & 0.59 & 2.84 & 11.1 & 2.26 & 1 & 1 \\ 
2194 & 12.34 & 1.25 & 5767 & -0.20 & 2.0 & syn & 1.25 & 0.92 & 1.24 & 0.47 & 10.8 & 1.31 & 1 & 1 \\ 
2195 & 13.56 & 0.69 & 6130 & -0.12 & 5.0 & syn & 1.25 & 1.08 & 1.24 & 0.56 & 4.3 & 0.70 & 1 & 0 \\ 
2201 & 12.40 & 0.85 & 6096 & 0.20 & 7.4 & syn & 1.75 & 1.34 & 1.74 & 0.25 & 3.0 & 0.97 & 1 & 0 \\ 
2202 & 12.34 & 2.04 & 5304 & 0.35 & 2.6 & syn & 0.80 & 0.92 & 0.83 & 1.59 & 1.5 & 1.73 & 1 & 1 \\ 
2204 & 12.58 & 0.79 & 6284 & -0.17 & 10.2 & syn & 1.71 & 1.24 & 1.69 & 0.25 & 3.3 & 1.07 & 1 & 1 \\ 
2205 & 13.30 & 1.55 & 4667 & -0.09 & \nodata & emp & 0.74 & 0.72 & 0.71 & 1.97 & 11.0 & 1.62 & 1 & 1 \\ 
2208 & 10.97 & 2.56 & 5849 & 0.11 & 3.3 & syn & 1.13 & 1.05 & 1.12 & 0.74 & 4.6 & 2.36 & 1 & 1 \\ 
2210 & 13.07 & 1.83 & 4888 & -0.11 & 2.2 & syn & 0.67 & 0.73 & 0.70 & 2.08 & 5.5 & 1.72 & 1 & 1 \\ 
2214 & 13.52 & 1.45 & 4583 & 0.12 & \nodata & emp & 0.72 & 0.74 & 0.72 & 1.97 & 9.0 & 1.30 & 1 & 1 \\ 
2218 & 12.86 & 0.94 & 5621 & 0.15 & 3.0 & syn & 1.33 & 1.02 & 1.32 & 0.44 & 9.4 & 1.29 & 1 & 0 \\ 
2219 & 12.16 & 2.47 & 4993 & 0.15 & 1.7 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
2220 & 13.14 & 0.81 & 5730 & 0.15 & 2.4 & syn & 1.34 & 1.06 & 1.33 & 0.45 & 7.4 & 0.82 & 1 & 0 \\ 
2223 & 13.20 & 1.62 & 4899 & 0.00 & 3.1 & syn & 0.71 & 0.77 & 0.74 & 1.87 & 6.3 & 1.56 & 1 & 0 \\ 
2225 & 12.13 & 2.81 & 4603 & 0.11 & \nodata & emp & 0.69 & 0.73 & 0.71 & 2.02 & 7.6 & 2.41 & 1 & 1 \\ 
2228 & 11.75 & 0.92 & 6535 & -0.17 & 12.8 & syn & 2.11 & 1.39 & 2.08 & 0.15 & 2.2 & 1.00 & 1 & 0 \\ 
2236 & 14.08 & 0.83 & 5501 & -0.03 & 0.5 & syn & 0.87 & 0.89 & 0.87 & 1.34 & 4.5 & 0.78 & 1 & 0 \\ 
2238 & 11.68 & 4.67 & 3934 & -0.09 & \nodata & emp & 0.60 & 0.58 & 0.59 & 2.76 & 12.7 & 5.93 & 1 & 1 \\ 
2246 & 12.66 & 1.47 & 5738 & -0.18 & 0.7 & syn & 0.92 & 0.91 & 0.92 & 1.16 & 5.2 & 1.54 & 1 & 1 \\ 
2247 & 12.02 & 2.95 & 4464 & 0.11 & \nodata & emp & 0.71 & 0.72 & 0.70 & 2.06 & 10.0 & 3.01 & 1 & 1 \\ 
2248 & 13.64 & \nodata & 5215 & 0.13 & 2.9 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
2250 & 13.39 & 1.40 & 4958 & 0.13 & 2.8 & syn & 0.75 & 0.81 & 0.78 & 1.68 & 6.3 & 1.34 & 1 & 1 \\ 
2252 & 12.27 & 0.70 & 6116 & 0.08 & 7.6 & syn & 2.26 & 1.43 & 2.22 & 0.13 & 2.5 & 0.90 & 1 & 1 \\ 
2256 & 13.14 & 1.85 & 4600 & 0.07 & \nodata & emp & 0.69 & 0.72 & 0.70 & 2.08 & 7.3 & 1.65 & 1 & 1 \\ 
2260 & 10.97 & 2.11 & 6188 & 0.01 & 7.9 & syn & 1.33 & 1.18 & 1.32 & 0.50 & 3.1 & 2.15 & 1 & 1 \\ 
2261 & 12.20 & 2.34 & 5158 & 0.06 & 3.1 & syn & 0.76 & 0.84 & 0.80 & 1.60 & 5.1 & 2.25 & 1 & 1 \\ 
2266 & 13.66 & 1.24 & 4727 & -0.07 & \nodata & emp & 0.78 & 0.73 & 0.73 & 1.86 & 11.5 & 1.20 & 1 & 1 \\ 
2273 & 11.41 & 1.94 & 6038 & 0.25 & 4.6 & syn & 1.20 & 1.18 & 1.19 & 0.69 & 1.9 & 1.78 & 1 & 1 \\ 
2278 & 12.32 & 1.11 & 5865 & -0.13 & 2.6 & syn & 1.43 & 1.01 & 1.41 & 0.36 & 8.1 & 1.13 & 1 & 1 \\ 
2279 & 12.47 & 1.24 & 5950 & 0.05 & 2.6 & syn & 1.18 & 1.07 & 1.17 & 0.66 & 4.3 & 1.17 & 1 & 1 \\ 
2281 & 11.88 & 2.68 & 5061 & 0.17 & 1.9 & syn & 0.77 & 0.84 & 0.80 & 1.59 & 5.5 & 2.49 & 1 & 1 \\ 
2287 & 10.20 & 6.60 & 4619 & 0.09 & \nodata & emp & 0.72 & 0.74 & 0.72 & 1.96 & 8.8 & 5.95 & 1 & 0 \\ 
2289 & 12.01 & 1.39 & 6048 & 0.09 & 4.9 & syn & 1.28 & 1.14 & 1.27 & 0.55 & 3.6 & 1.44 & 1 & 1 \\ 
2290 & 12.53 & 2.31 & 4966 & -0.24 & 1.7 & syn & 0.67 & 0.72 & 0.69 & 2.12 & 6.5 & 2.24 & 1 & 0 \\ 
2295 & 9.68 & \nodata & 5426 & -0.13 & 4.1 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
2298 & 11.73 & 2.10 & 5118 & -0.07 & 2.6 & syn & 1.06 & 0.82 & 1.03 & 0.76 & 18.3 & 2.87 & 1 & 0 \\ 
2300 & 12.19 & 2.43 & 5135 & -0.10 & 1.2 & syn & 0.74 & 0.79 & 0.76 & 1.74 & 6.1 & 2.39 & 1 & 1 \\ 
2311 & 10.98 & 2.20 & 5630 & 0.16 & 13.0 & syn & 1.34 & 1.02 & 1.33 & 0.43 & 9.1 & 3.07 & 5 & 1 \\ 
2312 & 11.32 & 1.05 & 6211 & -0.38 & 6.5 & syn & 2.34 & 1.24 & 2.31 & 0.10 & 3.4 & 1.02 & 1 & 0 \\ 
2318 & 12.21 & 2.94 & 4598 & -0.11 & \nodata & emp & 0.64 & 0.68 & 0.66 & 2.35 & 7.1 & 2.79 & 1 & 1 \\ 
2319 & 12.08 & 1.40 & 6114 & -0.01 & 4.7 & syn & 1.22 & 1.11 & 1.21 & 0.62 & 3.3 & 1.48 & 1 & 1 \\ 
2329 & 12.67 & 2.99 & 3882 & -0.07 & \nodata & emp & 0.60 & 0.58 & 0.59 & 2.81 & 12.8 & 3.98 & 1 & 1 \\ 
2331 & 12.06 & 1.27 & 5862 & 0.10 & 3.6 & syn & 1.38 & 1.11 & 1.37 & 0.42 & 5.8 & 1.26 & 1 & 1 \\ 
2332 & 11.17 & 1.48 & 5196 & -0.04 & 2.2 & syn & 1.92 & 0.98 & 1.92 & 0.14 & 10.5 & 1.42 & 1 & 0 \\ 
2333 & 12.29 & 1.25 & 6081 & -0.15 & 3.7 & syn & 1.24 & 1.05 & 1.23 & 0.55 & 5.1 & 1.42 & 1 & 0 \\ 
2335 & 12.45 & 0.89 & 5560 & -0.01 & 1.9 & syn & 1.87 & 0.99 & 1.57 & 0.24 & 9.9 & 1.63 & 1 & 0 \\ 
2336 & 12.32 & 2.76 & 4389 & 0.06 & \nodata & emp & 0.68 & 0.69 & 0.67 & 2.23 & 9.3 & 2.79 & 1 & 0 \\ 
2339 & 12.81 & 2.08 & 4573 & 0.14 & \nodata & emp & 0.69 & 0.73 & 0.71 & 2.04 & 7.3 & 1.78 & 1 & 1 \\ 
2342 & 11.58 & 1.77 & 5889 & -0.39 & 2.2 & syn & 1.26 & 0.89 & 1.22 & 0.48 & 10.6 & 2.12 & 1 & 0 \\ 
2344 & 13.20 & 1.72 & 4364 & 0.23 & \nodata & emp & 0.73 & 0.72 & 0.70 & 2.03 & 10.9 & 1.81 & 1 & 1 \\ 
2347 & 12.06 & 3.18 & 4083 & 0.27 & \nodata & emp & 0.70 & 0.65 & 0.68 & 2.06 & 12.4 & 3.55 & 1 & 0 \\ 
2352 & 9.50 & 3.77 & 6387 & -0.14 & 7.2 & syn & 1.44 & 1.22 & 1.44 & 0.40 & 2.8 & 4.44 & 1 & 1 \\ 
2355 & 13.74 & 1.34 & 4686 & 0.13 & \nodata & emp & 0.69 & 0.75 & 0.72 & 1.97 & 6.6 & 1.10 & 1 & 1 \\ 
2357 & 13.93 & 0.64 & 5640 & 0.03 & 1.2 & syn & 1.21 & 0.96 & 1.16 & 0.58 & 9.9 & 0.64 & 1 & 0 \\ 
2358 & 12.26 & 0.97 & 6285 & 0.21 & 13.6 & syn & 1.62 & 1.35 & 1.60 & 0.33 & 2.3 & 1.03 & 1 & 1 \\ 
2365 & 12.39 & 1.11 & 5952 & 0.21 & 3.7 & syn & 1.34 & 1.17 & 1.33 & 0.49 & 3.9 & 1.06 & 1 & 1 \\ 
2366 & 11.24 & 2.00 & 6165 & 0.01 & 6.6 & syn & 1.25 & 1.15 & 1.24 & 0.58 & 2.9 & 2.09 & 1 & 1 \\ 
2367 & 11.29 & 1.71 & 6059 & 0.15 & 6.3 & syn & 1.45 & 1.22 & 1.44 & 0.41 & 3.4 & 1.70 & 1 & 1 \\ 
2369 & 14.32 & 0.57 & 5781 & 0.10 & 2.9 & syn & 1.11 & 1.02 & 1.08 & 0.79 & 5.0 & 0.47 & 1 & 0 \\ 
2370 & 11.80 & 1.46 & 6461 & -0.15 & 19.2 & syn & 1.31 & 1.20 & 1.30 & 0.54 & 2.0 & 1.67 & 1 & 0 \\ 
2372 & 11.99 & 1.26 & 5970 & -0.09 & 3.9 & syn & 1.44 & 1.07 & 1.43 & 0.37 & 6.2 & 1.38 & 1 & 1 \\ 
2374 & 12.89 & 1.09 & 5720 & 0.13 & 2.4 & syn & 1.15 & 1.02 & 1.13 & 0.69 & 6.7 & 1.14 & 1 & 0 \\ 
2389 & 12.18 & 1.21 & 5835 & -0.08 & 2.4 & syn & 1.39 & 1.01 & 1.38 & 0.38 & 8.1 & 1.15 & 1 & 1 \\ 
2390 & 10.81 & 1.16 & 5949 & 0.12 & 5.5 & syn & 2.70 & 1.44 & 2.66 & 0.08 & 2.7 & 1.67 & 1 & 1 \\ 
2393 & 12.72 & 2.02 & 4760 & -0.05 & \nodata & emp & 0.72 & 0.73 & 0.72 & 1.93 & 9.1 & 1.80 & 1 & 1 \\ 
2396 & 12.85 & 1.64 & 5230 & 0.10 & 1.4 & syn & 0.80 & 0.86 & 0.81 & 1.63 & 3.1 & 1.57 & 1 & 0 \\ 
2398 & 12.28 & 0.99 & 6164 & -0.31 & 8.2 & syn & 1.58 & 1.09 & 1.56 & 0.28 & 5.4 & 1.31 & 1 & 0 \\ 
2399 & 12.19 & 2.43 & 5056 & -0.06 & 1.5 & syn & 0.74 & 0.78 & 0.76 & 1.75 & 6.4 & 2.35 & 1 & 1 \\ 
2401 & 12.48 & 1.78 & 4495 & 0.02 & \nodata & emp & 0.96 & 0.80 & 0.86 & 1.27 & 19.2 & 2.46 & 1 & 1 \\ 
2402 & 12.43 & 2.20 & 4544 & 0.16 & \nodata & emp & 0.78 & 0.75 & 0.74 & 1.84 & 11.9 & 2.12 & 1 & 1 \\ 
2403 & 11.59 & 1.81 & 6186 & 0.18 & 5.3 & syn & 1.18 & 1.20 & 1.17 & 0.73 & 1.1 & 1.75 & 1 & 1 \\ 
2407 & 12.64 & 0.91 & 5956 & 0.19 & 5.2 & syn & 1.47 & 1.20 & 1.45 & 0.38 & 4.1 & 0.89 & 1 & 0 \\ 
2408 & 12.51 & 1.63 & 5488 & -0.07 & 1.4 & syn & 0.92 & 0.87 & 0.92 & 1.13 & 8.5 & 1.72 & 1 & 1 \\ 
2409 & 12.80 & 1.96 & 4766 & -0.61 & 2.2 & syn & 0.73 & 0.64 & 0.64 & 2.40 & 13.8 & 2.33 & 1 & 0 \\ 
2410 & 13.55 & 0.96 & 5650 & -0.09 & 1.0 & syn & 0.95 & 0.91 & 0.94 & 1.08 & 6.3 & 1.00 & 1 & 0 \\ 
2414 & 12.04 & 1.14 & 5581 & -0.29 & 1.6 & syn & 1.61 & 0.90 & 1.60 & 0.22 & 11.8 & 1.36 & 1 & 1 \\ 
2422 & 12.96 & 1.60 & 5216 & -0.02 & 1.3 & syn & 0.78 & 0.83 & 0.78 & 1.71 & 3.6 & 1.55 & 1 & 0 \\ 
2426 & 12.20 & 1.87 & 5352 & 0.09 & 1.1 & syn & 0.92 & 0.89 & 0.92 & 1.14 & 8.7 & 1.75 & 1 & 1 \\ 
2433 & 13.82 & 0.72 & 5852 & 0.01 & 2.7 & syn & 1.09 & 1.02 & 1.08 & 0.79 & 4.9 & 0.61 & 1 & 0 \\ 
2440 & 12.36 & 1.18 & 5673 & 0.33 & 2.0 & syn & 1.32 & 1.10 & 1.31 & 0.48 & 6.4 & 1.09 & 1 & 0 \\ 
2442 & 13.61 & 1.16 & 5056 & 0.06 & 2.0 & syn & 0.82 & 0.82 & 0.81 & 1.51 & 8.6 & 1.18 & 1 & 0 \\ 
2443 & 12.54 & 1.27 & 5784 & -0.35 & 1.3 & syn & 1.13 & 0.86 & 1.12 & 0.61 & 12.0 & 1.38 & 1 & 1 \\ 
2460 & 12.59 & 2.32 & 4513 & -0.45 & \nodata & emp & 0.70 & 0.63 & 0.63 & 2.47 & 13.2 & 2.79 & 1 & 0 \\ 
2462 & 10.37 & 2.24 & 5970 & 0.06 & 5.6 & syn & 1.71 & 1.23 & 1.69 & 0.25 & 4.1 & 2.34 & 1 & 1 \\ 
2463 & 11.45 & \nodata & 6061 & 0.19 & 5.9 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
2469 & 12.73 & 1.97 & 4721 & 0.01 & \nodata & emp & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
2470 & 12.08 & 1.44 & 5860 & 0.31 & 3.0 & syn & 1.22 & 1.15 & 1.21 & 0.63 & 3.5 & 1.27 & 1 & 0 \\ 
2473 & 13.90 & 1.25 & 5075 & -0.10 & 0.9 & syn & 0.66 & 0.77 & 0.73 & 1.97 & 3.8 & 1.10 & 1 & 0 \\ 
2474 & 12.42 & \nodata & 5330 & -0.26 & 2.0 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
2479 & 11.14 & 1.30 & 5367 & 0.07 & 2.9 & syn & 2.18 & 1.16 & 2.17 & 0.11 & 5.9 & 1.58 & 1 & 0 \\ 
2480 & 12.88 & 2.36 & 4163 & 0.03 & \nodata & emp & 0.65 & 0.64 & 0.64 & 2.36 & 10.9 & 2.56 & 1 & 1 \\ 
2481 & 11.08 & 0.30 & 4683 & 0.11 & 4.1 & syn & 10.69 & 1.40 & 11.14 & 0.00 & 3.0 & 0.49 & 1 & 0 \\ 
2484 & 11.02 & 1.97 & 5768 & -0.32 & 1.8 & syn & 1.47 & 0.92 & 1.46 & 0.29 & 10.8 & 2.45 & 1 & 1 \\ 
2485 & 13.29 & 1.63 & 4953 & -0.16 & 1.2 & syn & 0.68 & 0.73 & 0.71 & 2.06 & 5.8 & 1.56 & 1 & 1 \\ 
2486 & 11.71 & \nodata & 6041 & 0.09 & 5.8 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
2488 & 12.23 & 1.15 & 5939 & -0.04 & 4.9 & syn & 1.42 & 1.08 & 1.41 & 0.38 & 6.2 & 1.10 & 1 & 1 \\ 
2490 & 13.59 & 1.43 & 4735 & -0.05 & \nodata & emp & 0.69 & 0.72 & 0.70 & 2.05 & 7.7 & 1.24 & 1 & 1 \\ 
2492 & 12.38 & 1.42 & 5704 & -0.30 & 1.0 & syn & 1.09 & 0.85 & 1.08 & 0.67 & 12.7 & 1.48 & 1 & 1 \\ 
2497 & 13.56 & 1.37 & 4937 & 0.02 & 1.9 & syn & 0.71 & 0.78 & 0.75 & 1.83 & 5.9 & 1.28 & 1 & 1 \\ 
2498 & 12.07 & 2.32 & 5146 & -0.08 & 1.8 & syn & 0.81 & 0.80 & 0.81 & 1.51 & 9.4 & 2.34 & 1 & 1 \\ 
2502 & 12.87 & 1.70 & 4927 & -0.02 & 2.3 & syn & 0.80 & 0.77 & 0.77 & 1.63 & 10.6 & 1.84 & 1 & 0 \\ 
2503 & 11.94 & 2.69 & 4750 & 0.14 & \nodata & emp & 0.78 & 0.78 & 0.76 & 1.72 & 10.0 & 2.38 & 1 & 1 \\ 
2516 & 11.58 & 1.17 & 5423 & 0.29 & 2.6 & syn & 1.98 & 1.17 & 1.96 & 0.15 & 6.6 & 1.28 & 1 & 0 \\ 
2517 & 12.90 & 1.27 & 5611 & -0.08 & 1.1 & syn & 0.97 & 0.90 & 0.96 & 1.00 & 7.8 & 1.44 & 1 & 0 \\ 
2519 & 12.04 & 3.03 & 4398 & 0.12 & \nodata & emp & 0.69 & 0.70 & 0.69 & 2.14 & 9.6 & 3.07 & 1 & 1 \\ 
2520 & 13.20 & 1.74 & 4562 & -0.07 & \nodata & emp & 0.70 & 0.69 & 0.68 & 2.15 & 9.7 & 1.78 & 1 & 1 \\ 
2521 & 13.82 & 1.20 & 4976 & -0.24 & 1.4 & syn & 0.72 & 0.72 & 0.71 & 1.97 & 8.9 & 1.23 & 1 & 1 \\ 
2522 & 11.53 & 3.25 & 4765 & 0.14 & \nodata & emp & 0.78 & 0.78 & 0.76 & 1.72 & 9.7 & 2.88 & 1 & 1 \\ 
2525 & 13.42 & 1.61 & 4641 & 0.00 & \nodata & emp & 0.68 & 0.71 & 0.69 & 2.11 & 7.5 & 1.45 & 1 & 1 \\ 
2527 & 11.56 & 4.02 & 4299 & 0.01 & \nodata & emp & 0.66 & 0.66 & 0.65 & 2.35 & 10.2 & 4.18 & 1 & 1 \\ 
2529 & 13.33 & 1.72 & 4560 & -0.02 & \nodata & emp & 0.67 & 0.70 & 0.68 & 2.20 & 7.9 & 1.67 & 1 & 1 \\ 
2530 & 12.22 & 0.94 & 5913 & 0.14 & 4.5 & syn & 1.74 & 1.25 & 1.73 & 0.24 & 4.1 & 0.99 & 1 & 1 \\ 
2531 & 13.16 & 1.74 & 4667 & 0.11 & \nodata & emp & 0.69 & 0.74 & 0.72 & 1.99 & 6.8 & 1.45 & 1 & 1 \\ 
2533 & 11.24 & 0.94 & 4959 & 0.01 & 3.2 & syn & 3.03 & 1.14 & 3.02 & 0.04 & 5.8 & 1.00 & 1 & 0 \\ 
2534 & 12.50 & 1.23 & 6118 & 0.02 & 4.4 & syn & 1.15 & 1.12 & 1.14 & 0.74 & 2.3 & 1.22 & 1 & 1 \\ 
2535 & 12.78 & 1.80 & 4930 & 0.10 & 2.3 & syn & 0.78 & 0.80 & 0.78 & 1.65 & 8.1 & 1.82 & 1 & 1 \\ 
2538 & 12.15 & 1.89 & 4966 & -0.23 & 6.6 & syn & 1.00 & 0.77 & 0.87 & 1.14 & 18.1 & 2.62 & 1 & 0 \\ 
2540 & 13.27 & 1.53 & 4460 & 0.20 & \nodata & emp & 0.78 & 0.74 & 0.73 & 1.89 & 12.1 & 1.68 & 1 & 0 \\ 
2541 & 10.97 & 1.17 & 5032 & 0.11 & 3.0 & syn & 2.71 & 1.23 & 2.71 & 0.06 & 4.8 & 1.20 & 1 & 0 \\ 
2543 & 13.39 & 1.20 & 5054 & 0.03 & 2.7 & syn & 0.87 & 0.81 & 0.85 & 1.30 & 13.3 & 1.33 & 1 & 0 \\ 
2545 & 10.45 & 1.65 & 6105 & 0.14 & 6.9 & syn & 2.18 & 1.44 & 2.16 & 0.14 & 2.5 & 1.95 & 1 & 0 \\ 
2547 & 12.59 & 1.20 & 5976 & -0.11 & 2.1 & syn & 1.16 & 1.01 & 1.15 & 0.66 & 5.6 & 1.34 & 1 & 0 \\ 
2548 & 12.66 & 2.02 & 4698 & -0.28 & \nodata & emp & 0.76 & 0.69 & 0.69 & 2.04 & 13.1 & 2.32 & 1 & 1 \\ 
2551 & 13.77 & 1.17 & 4921 & 0.04 & 1.8 & syn & 0.76 & 0.78 & 0.77 & 1.69 & 8.3 & 1.18 & 1 & 0 \\ 
2553 & 13.66 & 1.23 & 4947 & 0.05 & 2.3 & syn & 0.76 & 0.79 & 0.77 & 1.69 & 7.8 & 1.10 & 1 & 0 \\ 
2555 & 11.64 & 1.88 & 6180 & -0.07 & 6.1 & syn & 1.11 & 1.10 & 1.10 & 0.81 & 1.9 & 1.85 & 1 & 1 \\ 
2556 & 12.43 & 1.82 & 5526 & -0.14 & 1.3 & syn & 0.85 & 0.87 & 0.84 & 1.43 & 4.7 & 1.83 & 1 & 1 \\ 
2559 & 12.34 & 1.39 & 5881 & 0.15 & 2.7 & syn & 1.11 & 1.08 & 1.10 & 0.79 & 3.2 & 1.31 & 1 & 1 \\ 
2560 & 13.22 & 1.68 & 4686 & -0.23 & \nodata & emp & 0.71 & 0.69 & 0.68 & 2.13 & 11.1 & 1.79 & 1 & 1 \\ 
2561 & 12.27 & 1.15 & 6014 & 0.04 & 4.1 & syn & 1.38 & 1.14 & 1.37 & 0.43 & 4.6 & 1.14 & 1 & 1 \\ 
2563 & 12.62 & 0.69 & 6119 & 0.11 & 7.5 & syn & 1.94 & 1.36 & 1.92 & 0.19 & 2.9 & 0.74 & 1 & 1 \\ 
2564 & 12.60 & 0.70 & 6087 & -0.13 & 9.1 & syn & 1.96 & 1.20 & 1.93 & 0.16 & 4.4 & 0.87 & 1 & 1 \\ 
2570 & 12.54 & 3.73 & 3803 & -0.06 & \nodata & emp & 0.54 & 0.53 & 0.54 & 3.42 & 11.6 & 4.79 & 1 & 0 \\ 
2571 & 12.53 & 1.16 & 5275 & 0.27 & 6.0 & syn & 1.31 & 0.93 & 1.29 & 0.43 & 15.3 & 1.68 & 1 & 0 \\ 
2577 & 12.37 & 1.03 & 5866 & -0.36 & 73.9 & syn & 1.49 & 0.94 & 1.48 & 0.29 & 9.6 & 0.29 & 3 & 1 \\ 
2581 & 11.81 & 2.30 & 5504 & 0.28 & 2.1 & syn & 0.88 & 0.97 & 0.89 & 1.36 & 1.7 & 2.07 & 1 & 1 \\ 
2582 & 12.24 & 1.23 & 5880 & 0.31 & 3.5 & syn & 1.32 & 1.18 & 1.31 & 0.52 & 3.8 & 1.08 & 1 & 1 \\ 
2583 & 11.08 & 2.96 & 5607 & 0.11 & 0.4 & syn & 0.95 & 0.97 & 0.95 & 1.12 & 4.1 & 2.81 & 1 & 1 \\ 
2585 & 12.12 & 1.49 & 6005 & -0.36 & 1.9 & syn & 1.14 & 0.93 & 1.13 & 0.63 & 7.9 & 1.78 & 1 & 1 \\ 
2588 & 12.74 & 2.42 & 4140 & 0.14 & \nodata & emp & 0.67 & 0.65 & 0.66 & 2.20 & 11.0 & 2.62 & 1 & 1 \\ 
2590 & 10.41 & 1.70 & 6151 & -0.02 & 10.2 & syn & 2.16 & 1.31 & 2.13 & 0.14 & 3.3 & 2.10 & 1 & 0 \\ 
2593 & 10.48 & 2.39 & 6238 & 0.22 & 7.5 & syn & 1.47 & 1.30 & 1.46 & 0.42 & 2.2 & 2.66 & 1 & 1 \\ 
2595 & 11.99 & 1.16 & 6332 & 0.04 & 14.4 & syn & 1.51 & 1.27 & 1.50 & 0.37 & 2.5 & 1.38 & 1 & 1 \\ 
2597 & 13.38 & 0.97 & 5875 & -0.30 & 2.0 & syn & 1.00 & 0.90 & 0.99 & 0.93 & 7.0 & 1.07 & 1 & 0 \\ 
2603 & 11.36 & 1.36 & 6225 & -0.08 & 9.7 & syn & 1.75 & 1.26 & 1.74 & 0.24 & 3.2 & 1.68 & 1 & 1 \\ 
2604 & 13.13 & 1.78 & 4718 & -0.09 & \nodata & emp & 0.69 & 0.71 & 0.70 & 2.08 & 8.3 & 1.56 & 1 & 0 \\ 
2607 & 12.99 & 1.24 & 5782 & 0.21 & 3.0 & syn & 0.93 & 1.03 & 0.95 & 1.18 & 1.2 & 1.09 & 1 & 0 \\ 
2608 & 11.96 & 1.45 & 6429 & 0.06 & 18.1 & syn & 1.23 & 1.24 & 1.23 & 0.65 & 0.8 & 1.41 & 1 & 0 \\ 
2612 & 10.19 & 4.16 & 5548 & 0.32 & 2.3 & syn & 1.02 & 1.02 & 1.02 & 0.95 & 4.6 & 3.69 & 1 & 1 \\ 
2623 & 12.07 & 1.00 & 6178 & 0.13 & 7.2 & syn & 1.71 & 1.32 & 1.70 & 0.27 & 2.9 & 1.07 & 1 & 1 \\ 
2631 & 12.04 & 1.18 & 5773 & -0.43 & 2.1 & syn & 1.53 & 0.90 & 1.52 & 0.25 & 11.0 & 1.59 & 1 & 1 \\ 
2632 & 10.15 & 1.86 & 6209 & -0.02 & 10.3 & syn & 2.22 & 1.37 & 2.20 & 0.13 & 2.8 & 2.55 & 1 & 1 \\ 
2635 & 11.38 & 1.31 & 6052 & -0.14 & 7.0 & syn & 1.83 & 1.16 & 1.81 & 0.19 & 5.0 & 1.64 & 1 & 1 \\ 
2636 & 10.67 & 3.37 & 5892 & 0.09 & 3.0 & syn & 0.98 & 1.04 & 0.99 & 1.08 & 1.6 & 3.19 & 1 & 1 \\ 
2639 & 14.02 & 0.42 & 5594 & -0.02 & 2.5 & syn & 1.78 & 1.03 & 1.71 & 0.20 & 8.6 & 0.42 & 1 & 0 \\ 
2640 & 10.99 & 0.47 & 4835 & -0.21 & 3.6 & syn & 6.94 & 1.23 & 6.87 & 0.00 & 3.8 & 0.58 & 1 & 0 \\ 
2641 & 12.31 & 1.04 & 5779 & -0.01 & 2.9 & syn & 1.55 & 1.05 & 1.53 & 0.29 & 7.9 & 1.05 & 1 & 0 \\ 
2644 & 12.61 & 2.72 & 4560 & 0.16 & \nodata & emp & 0.58 & 0.69 & 0.65 & 2.47 & 2.7 & 1.92 & 4 & 0 \\ 
2650 & 12.95 & 2.40 & 3977 & 0.01 & \nodata & emp & 0.64 & 0.61 & 0.62 & 2.47 & 12.7 & 2.98 & 1 & 1 \\ 
2657 & 11.24 & \nodata & 5469 & -0.13 & 0.8 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
2659 & 10.91 & 0.96 & 5034 & 0.25 & 2.9 & syn & 3.41 & 1.45 & 3.43 & 0.04 & 2.8 & 1.03 & 1 & 0 \\ 
2662 & 11.02 & 8.90 & 3498 & 0.05 & \nodata & emp & 0.48 & 0.47 & 0.48 & 4.24 & 12.1 & 14.96 & 1 & 1 \\ 
2663 & 11.90 & 1.49 & 5667 & 0.10 & 2.2 & syn & 1.29 & 1.01 & 1.28 & 0.47 & 9.1 & 1.44 & 1 & 1 \\ 
2668 & 12.44 & 1.78 & 5489 & -0.02 & 1.1 & syn & 0.86 & 0.90 & 0.86 & 1.38 & 4.1 & 1.79 & 1 & 1 \\ 
2672 & 10.29 & 4.49 & 5657 & 0.18 & 3.6 & syn & 0.90 & 0.99 & 0.91 & 1.30 & 1.5 & 4.20 & 1 & 1 \\ 
2674 & 11.82 & 1.18 & 5703 & 0.07 & 1.8 & syn & 1.70 & 1.09 & 1.68 & 0.23 & 7.5 & 1.28 & 1 & 1 \\ 
2675 & 10.91 & 3.37 & 5730 & 0.11 & 7.7 & syn & 0.89 & 0.98 & 0.91 & 1.31 & 1.4 & 3.17 & 1 & 1 \\ 
2676 & 11.93 & 0.76 & 6063 & -0.23 & 4.8 & syn & 2.50 & 1.29 & 2.46 & 0.09 & 3.2 & 0.61 & 1 & 0 \\ 
2677 & 12.14 & 0.99 & 6094 & 0.04 & 6.6 & syn & 1.67 & 1.25 & 1.67 & 0.27 & 3.6 & 1.00 & 1 & 1 \\ 
2678 & 10.09 & 5.76 & 5373 & 0.08 & 6.8 & syn & 0.79 & 0.88 & 0.80 & 1.68 & 1.6 & 5.41 & 1 & 1 \\ 
2681 & 13.90 & \nodata & 5316 & -0.06 & 1.7 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
2686 & 11.56 & 3.67 & 4588 & 0.04 & \nodata & emp & 0.69 & 0.72 & 0.70 & 2.08 & 8.2 & 3.63 & 1 & 1 \\ 
2687 & 8.69 & 8.87 & 5778 & 0.06 & 2.3 & syn & 0.94 & 0.99 & 0.94 & 1.19 & 1.9 & 8.48 & 1 & 1 \\ 
2690 & 11.76 & 2.48 & 5473 & 0.13 & 3.7 & syn & 0.84 & 0.92 & 0.85 & 1.47 & 2.1 & 2.39 & 1 & 1 \\ 
2691 & 12.69 & 2.21 & 4602 & 0.09 & \nodata & emp & 0.69 & 0.73 & 0.71 & 2.05 & 7.4 & 1.91 & 1 & 1 \\ 
2693 & 10.79 & 5.66 & 4373 & -0.10 & \nodata & emp & 0.66 & 0.66 & 0.65 & 2.38 & 10.5 & 5.96 & 1 & 1 \\ 
2694 & 12.68 & 2.10 & 4528 & 0.18 & \nodata & emp & 0.73 & 0.74 & 0.72 & 1.94 & 9.7 & 1.93 & 1 & 1 \\ 
2698 & 12.44 & 1.27 & 5948 & 0.12 & 3.0 & syn & 1.18 & 1.10 & 1.16 & 0.69 & 3.5 & 1.22 & 1 & 1 \\ 
2700 & 12.84 & 2.01 & 4537 & 0.16 & \nodata & emp & 0.72 & 0.74 & 0.72 & 1.97 & 9.1 & 1.82 & 1 & 1 \\ 
2703 & 12.77 & 2.13 & 4482 & 0.06 & \nodata & emp & 0.70 & 0.71 & 0.69 & 2.10 & 9.5 & 2.16 & 1 & 1 \\ 
2705 & 10.73 & 9.65 & 3501 & 0.01 & \nodata & emp & 0.50 & 0.48 & 0.49 & 3.96 & 12.8 & 17.98 & 1 & 1 \\ 
2706 & 9.11 & 3.38 & 6332 & 0.13 & 10.8 & syn & 1.94 & 1.43 & 1.93 & 0.20 & 2.2 & 4.40 & 1 & 1 \\ 
2707 & 12.70 & 0.79 & 5574 & -0.10 & 1.6 & syn & 1.87 & 0.98 & 1.63 & 0.21 & 9.8 & 1.54 & 1 & 0 \\ 
2708 & 13.66 & 1.57 & 4600 & 0.04 & \nodata & emp & 0.62 & 0.70 & 0.67 & 2.31 & 4.8 & 1.31 & 1 & 0 \\ 
2711 & 12.30 & \nodata & 5946 & 0.09 & 4.0 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
2712 & 9.95 & 2.44 & 6335 & 0.27 & 13.2 & syn & 1.81 & 1.44 & 1.80 & 0.24 & 2.0 & 2.95 & 1 & 1 \\ 
2713 & 12.79 & 2.20 & 4687 & -0.03 & \nodata & emp & 0.65 & 0.71 & 0.68 & 2.20 & 6.0 & 1.85 & 1 & 0 \\ 
2714 & 11.99 & 1.06 & 5989 & -0.02 & 5.8 & syn & 1.71 & 1.18 & 1.69 & 0.24 & 4.8 & 1.14 & 1 & 1 \\ 
2717 & 11.12 & 2.17 & 6025 & -0.02 & 4.6 & syn & 1.24 & 1.08 & 1.23 & 0.58 & 4.5 & 2.16 & 1 & 1 \\ 
2719 & 12.83 & 2.10 & 4566 & 0.10 & \nodata & emp & 0.68 & 0.72 & 0.70 & 2.10 & 7.2 & 1.89 & 1 & 1 \\ 
2720 & 9.00 & 4.70 & 5943 & -0.13 & 2.6 & syn & 1.52 & 1.06 & 1.51 & 0.31 & 6.7 & 4.93 & 1 & 1 \\ 
2722 & 11.99 & 1.62 & 6140 & -0.07 & 6.3 & syn & 1.09 & 1.08 & 1.09 & 0.83 & 2.1 & 1.60 & 1 & 1 \\ 
2729 & 12.37 & 1.50 & 5598 & -0.32 & 1.5 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
2730 & 12.30 & 1.25 & 5647 & 0.01 & 1.9 & syn & 1.29 & 0.96 & 1.28 & 0.46 & 10.6 & 1.19 & 1 & 1 \\ 
2732 & 11.54 & 1.21 & 6082 & 0.08 & 4.9 & syn & 1.82 & 1.30 & 1.80 & 0.22 & 3.3 & 1.36 & 1 & 1 \\ 
2733 & 11.76 & 1.82 & 4734 & 0.05 & \nodata & emp & 1.54 & 0.88 & 1.91 & 0.10 & 17.1 & 2.80 & 1 & 0 \\ 
2736 & 13.44 & 1.73 & 4411 & 0.04 & \nodata & emp & 0.65 & 0.68 & 0.66 & 2.33 & 7.8 & 1.66 & 1 & 1 \\ 
2737 & 10.87 & 1.96 & 5667 & 0.37 & 2.3 & syn & 1.57 & 1.20 & 1.56 & 0.31 & 5.4 & 1.93 & 1 & 0 \\ 
2740 & 12.14 & 0.86 & 6083 & -0.27 & 6.7 & syn & 1.97 & 1.15 & 1.94 & 0.15 & 4.8 & 1.64 & 1 & 0 \\ 
2741 & 11.58 & 2.18 & 5880 & 0.07 & 0.8 & syn & 1.02 & 1.04 & 1.02 & 0.99 & 2.3 & 2.09 & 1 & 0 \\ 
2742 & 12.32 & 3.16 & 4177 & -0.09 & \nodata & emp & 0.62 & 0.62 & 0.62 & 2.61 & 10.7 & 3.39 & 1 & 1 \\ 
2743 & 12.12 & 1.92 & 5583 & -0.01 & 1.0 & syn & 0.92 & 0.92 & 0.92 & 1.18 & 5.1 & 2.00 & 1 & 1 \\ 
2748 & 12.37 & 0.91 & 5468 & -0.09 & 2.5 & syn & 1.75 & 0.98 & 1.74 & 0.18 & 10.1 & 0.96 & 1 & 1 \\ 
2749 & 10.02 & 1.85 & 6158 & -0.02 & 9.5 & syn & 2.36 & 1.35 & 2.33 & 0.11 & 2.9 & 2.56 & 1 & 0 \\ 
2750 & 14.57 & 0.31 & 6070 & 0.07 & 7.8 & syn & 1.83 & 1.24 & 1.64 & 0.26 & 3.6 & 0.33 & 1 & 0 \\ 
2751 & 13.29 & 1.69 & 4373 & 0.01 & \nodata & emp & 0.71 & 0.68 & 0.67 & 2.19 & 11.3 & 1.81 & 1 & 1 \\ 
2752 & 10.20 & 2.59 & 6065 & 0.14 & 7.6 & syn & 1.64 & 1.24 & 1.54 & 0.32 & 3.4 & 3.07 & 1 & 0 \\ 
2753 & 12.11 & 1.35 & 5811 & 0.22 & 2.3 & syn & 1.29 & 1.11 & 1.28 & 0.53 & 5.4 & 1.26 & 1 & 1 \\ 
2754 & 10.63 & 2.72 & 5898 & -0.08 & 3.2 & syn & 1.25 & 1.01 & 1.24 & 0.53 & 7.1 & 3.35 & 1 & 0 \\ 
2755 & 10.71 & 3.42 & 5791 & -0.14 & 2.2 & syn & 0.96 & 0.94 & 0.96 & 1.06 & 5.1 & 3.54 & 1 & 1 \\ 
2756 & 13.24 & 1.04 & 5896 & 0.10 & 3.1 & syn & 1.00 & 1.05 & 1.00 & 1.04 & 1.7 & 0.95 & 1 & 0 \\ 
2758 & 9.84 & 1.49 & 5210 & 0.35 & 4.0 & syn & 3.58 & 1.71 & 3.57 & 0.04 & 1.8 & 2.25 & 1 & 0 \\ 
2759 & 12.23 & 2.57 & 4765 & 0.00 & \nodata & emp & 0.72 & 0.74 & 0.72 & 1.93 & 8.1 & 2.25 & 1 & 1 \\ 
2760 & 12.47 & \nodata & 4568 & 0.11 & \nodata & emp & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
2762 & 12.64 & 2.12 & 4398 & 0.23 & \nodata & emp & 0.76 & 0.73 & 0.72 & 1.95 & 12.0 & 2.28 & 1 & 1 \\ 
2763 & 13.12 & 1.74 & 4638 & 0.05 & \nodata & emp & 0.72 & 0.73 & 0.71 & 1.98 & 8.8 & 1.57 & 1 & 0 \\ 
2764 & 12.87 & 2.56 & 4007 & -0.16 & \nodata & emp & 0.62 & 0.60 & 0.60 & 2.66 & 13.0 & 3.26 & 1 & 1 \\ 
2765 & 12.45 & 0.76 & 6183 & 0.08 & 3.4 & syn & 1.89 & 1.35 & 1.88 & 0.20 & 2.8 & 0.83 & 1 & 0 \\ 
2768 & 13.48 & 1.26 & 5328 & -0.03 & 1.0 & syn & 0.77 & 0.85 & 0.79 & 1.72 & 2.6 & 1.19 & 1 & 0 \\ 
2769 & 12.16 & 0.89 & 5767 & -0.05 & 2.8 & syn & 1.92 & 1.12 & 1.90 & 0.16 & 6.1 & 1.03 & 1 & 0 \\ 
2770 & 13.05 & 1.98 & 4286 & -0.19 & \nodata & emp & 0.69 & 0.64 & 0.64 & 2.41 & 12.9 & 2.34 & 1 & 1 \\ 
2771 & 10.46 & 3.26 & 6251 & -0.03 & 4.2 & syn & 1.08 & 1.12 & 1.09 & 0.87 & 1.0 & 3.23 & 1 & 0 \\ 
2781 & 11.11 & 1.76 & 5761 & -0.44 & 1.3 & syn & 1.61 & 0.91 & 1.59 & 0.22 & 10.6 & 2.35 & 1 & 0 \\ 
2783 & 11.88 & 3.73 & 4107 & -0.10 & \nodata & emp & 0.65 & 0.62 & 0.62 & 2.51 & 12.4 & 4.44 & 1 & 0 \\ 
2785 & 12.63 & 1.20 & 5860 & 0.02 & 2.4 & syn & 1.13 & 1.02 & 1.12 & 0.71 & 5.5 & 1.20 & 1 & 1 \\ 
2786 & 12.56 & 0.76 & 6367 & -0.13 & 7.5 & syn & 1.76 & 1.29 & 1.75 & 0.24 & 2.8 & 1.06 & 1 & 0 \\ 
2790 & 11.49 & \nodata & 5082 & -0.21 & 1.6 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
2792 & 9.76 & 3.64 & 5969 & 0.21 & 4.3 & syn & 1.37 & 1.19 & 1.36 & 0.46 & 3.9 & 3.53 & 1 & 1 \\ 
2796 & 13.38 & 0.94 & 5728 & 0.01 & 1.7 & syn & 1.04 & 0.97 & 1.03 & 0.88 & 6.0 & 0.95 & 1 & 0 \\ 
2798 & 11.47 & 4.96 & 4283 & -0.50 & \nodata & emp & 0.57 & 0.57 & 0.55 & 3.32 & 11.8 & 5.40 & 1 & 1 \\ 
2801 & 9.47 & 3.87 & 6027 & 0.03 & 3.6 & syn & 1.46 & 1.16 & 1.46 & 0.37 & 4.5 & 3.92 & 1 & 1 \\ 
2803 & 10.64 & 3.53 & 5594 & 0.17 & 2.7 & syn & 0.97 & 0.99 & 0.97 & 1.07 & 4.1 & 3.31 & 1 & 1 \\ 
2805 & 11.92 & 1.51 & 5879 & -0.24 & 1.6 & syn & 1.25 & 0.94 & 1.24 & 0.49 & 9.2 & 1.73 & 1 & 1 \\ 
2806 & 13.14 & 1.71 & 4661 & 0.14 & \nodata & emp & 0.72 & 0.75 & 0.73 & 1.92 & 7.8 & 1.45 & 1 & 1 \\ 
2807 & 12.54 & 0.98 & 6426 & 0.19 & 13.8 & syn & 1.39 & 1.32 & 1.37 & 0.50 & 1.2 & 1.03 & 1 & 0 \\ 
2811 & 12.60 & 2.23 & 4324 & -0.23 & \nodata & emp & 0.74 & 0.65 & 0.66 & 2.28 & 14.3 & 2.84 & 1 & 0 \\ 
2815 & 12.03 & 1.52 & 5896 & -0.06 & 1.9 & syn & 1.18 & 1.01 & 1.17 & 0.62 & 6.4 & 1.54 & 1 & 0 \\ 
2828 & 13.43 & 1.65 & 4543 & 0.06 & \nodata & emp & 0.66 & 0.70 & 0.68 & 2.18 & 7.0 & 1.56 & 1 & 1 \\ 
2829 & 11.44 & 1.62 & 5913 & 0.02 & 3.3 & syn & 1.44 & 1.10 & 1.43 & 0.37 & 5.9 & 1.68 & 1 & 1 \\ 
2830 & 12.55 & 0.68 & 6447 & 0.06 & 30.0 & syn & 2.03 & 1.45 & 2.00 & 0.18 & 2.1 & 0.83 & 3 & 1 \\ 
2831 & 11.05 & 1.30 & 5722 & -0.03 & 4.6 & syn & 2.21 & 1.20 & 2.19 & 0.11 & 4.7 & 1.65 & 1 & 0 \\ 
2832 & 11.98 & 2.59 & 5043 & 0.11 & 1.5 & syn & 0.77 & 0.82 & 0.79 & 1.62 & 6.2 & 2.46 & 1 & 1 \\ 
2833 & 11.12 & 2.13 & 6253 & -0.17 & 5.0 & syn & 1.26 & 1.11 & 1.25 & 0.56 & 3.4 & 2.50 & 1 & 1 \\ 
2834 & 13.63 & 1.39 & 4659 & 0.08 & \nodata & emp & 0.71 & 0.74 & 0.72 & 1.97 & 7.9 & 1.19 & 1 & 1 \\ 
2835 & 13.44 & 1.66 & 4414 & -0.07 & \nodata & emp & 0.67 & 0.67 & 0.66 & 2.33 & 9.8 & 1.71 & 1 & 1 \\ 
2836 & 12.96 & 1.87 & 4697 & 0.00 & \nodata & emp & 0.72 & 0.73 & 0.72 & 1.97 & 8.7 & 1.68 & 1 & 1 \\ 
2838 & 11.86 & 1.21 & 5690 & 0.15 & 1.8 & syn & 1.62 & 1.10 & 1.61 & 0.26 & 7.5 & 1.26 & 1 & 1 \\ 
2839 & 12.96 & 2.17 & 4012 & -0.10 & \nodata & emp & 0.68 & 0.62 & 0.63 & 2.40 & 14.1 & 3.01 & 1 & 1 \\ 
2840 & 12.26 & 1.09 & 5627 & -0.02 & 1.8 & syn & 1.53 & 0.99 & 1.51 & 0.28 & 10.1 & 1.05 & 1 & 1 \\ 
2841 & 13.98 & 0.97 & 5158 & -0.13 & 0.7 & syn & 0.82 & 0.79 & 0.80 & 1.48 & 10.6 & 1.01 & 1 & 0 \\ 
2845 & 12.70 & 2.52 & 4081 & 0.20 & \nodata & emp & 0.67 & 0.64 & 0.66 & 2.18 & 11.3 & 2.73 & 1 & 1 \\ 
2847 & 13.17 & 1.45 & 4564 & 0.18 & \nodata & emp & 0.84 & 0.77 & 0.79 & 1.52 & 17.2 & 1.45 & 1 & 0 \\ 
2848 & 10.92 & 2.28 & 5724 & 0.33 & 2.8 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
2857 & 12.35 & 1.02 & 6189 & 0.24 & 6.3 & syn & 1.47 & 1.30 & 1.46 & 0.41 & 2.3 & 0.99 & 1 & 0 \\ 
2858 & 13.44 & 1.45 & 4699 & 0.10 & \nodata & emp & 0.74 & 0.75 & 0.74 & 1.87 & 8.8 & 1.27 & 1 & 0 \\ 
2859 & 12.05 & 1.96 & 5262 & -0.07 & 1.5 & syn & 0.96 & 0.82 & 0.95 & 0.95 & 15.7 & 2.29 & 1 & 0 \\ 
2863 & 12.22 & 1.49 & 5717 & -0.23 & 0.7 & syn & 1.12 & 0.88 & 1.11 & 0.64 & 11.6 & 1.63 & 1 & 0 \\ 
2864 & 11.45 & 2.35 & 5821 & -0.12 & 0.8 & syn & 1.00 & 0.95 & 0.99 & 0.96 & 5.3 & 2.41 & 1 & 0 \\ 
2866 & 12.79 & 0.61 & 6290 & 0.10 & 5.4 & syn & 2.03 & 1.41 & 1.98 & 0.18 & 2.4 & 0.99 & 1 & 0 \\ 
2869 & 12.36 & 0.72 & 6407 & 0.18 & 24.7 & syn & 2.06 & 1.50 & 2.04 & 0.17 & 1.9 & 0.80 & 3 & 1 \\ 
2874 & 13.18 & 1.41 & 5262 & -0.06 & 1.6 & syn & 0.79 & 0.83 & 0.79 & 1.64 & 4.6 & 1.35 & 1 & 0 \\ 
2875 & 12.81 & 2.01 & 4993 & -0.06 & 2.1 & syn & 0.68 & 0.76 & 0.73 & 1.96 & 4.4 & 1.84 & 1 & 0 \\ 
2879 & 11.10 & \nodata & 5452 & -0.02 & 1.9 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
2883 & 13.33 & 2.00 & 4212 & -0.18 & \nodata & emp & 0.62 & 0.61 & 0.60 & 2.79 & 10.7 & 2.17 & 1 & 1 \\ 
2884 & 12.47 & 0.44 & 5687 & -0.02 & 3.5 & syn & 3.42 & 1.53 & 3.24 & 0.04 & 2.0 & 0.87 & 1 & 0 \\ 
2885 & 12.06 & 0.93 & 5498 & -0.39 & 1.8 & syn & 2.00 & 0.96 & 1.98 & 0.12 & 8.8 & 1.21 & 1 & 0 \\ 
2891 & 11.83 & 0.96 & 6091 & 0.13 & 5.7 & syn & 3.49 & 1.27 & 1.63 & 0.25 & 3.0 & 1.07 & 1 & 0 \\ 
2896 & 10.59 & \nodata & 6220 & -0.01 & 14.9 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
2901 & 12.39 & 2.74 & 4315 & 0.06 & \nodata & emp & 0.68 & 0.67 & 0.66 & 2.28 & 10.1 & 2.84 & 1 & 0 \\ 
2902 & 12.95 & 1.77 & 4770 & -0.35 & 1.8 & syn & 0.75 & 0.68 & 0.68 & 2.11 & 13.2 & 2.01 & 1 & 0 \\ 
2904 & 11.36 & 1.38 & 6077 & 0.30 & 7.5 & syn & 1.74 & 1.36 & 1.72 & 0.26 & 2.8 & 1.19 & 1 & 0 \\ 
2906 & 12.32 & 1.00 & 6087 & -0.28 & 6.0 & syn & 1.58 & 1.07 & 1.55 & 0.28 & 6.0 & 1.18 & 1 & 1 \\ 
2913 & 11.36 & 1.48 & 5762 & 0.34 & 2.1 & syn & 1.66 & 1.25 & 1.64 & 0.28 & 4.5 & 1.78 & 1 & 0 \\ 
2914 & 11.01 & 1.30 & 6252 & -0.27 & 25.7 & syn & 2.15 & 1.24 & 2.14 & 0.13 & 3.5 & 1.01 & 3 & 1 \\ 
2915 & 11.96 & 2.08 & 5617 & 0.02 & 0.8 & syn & 0.92 & 0.94 & 0.91 & 1.23 & 3.7 & 2.00 & 1 & 1 \\ 
2916 & 12.40 & 2.17 & 4991 & 0.02 & 1.8 & syn & 0.77 & 0.79 & 0.78 & 1.66 & 7.8 & 2.14 & 1 & 0 \\ 
2925 & 11.73 & 2.51 & 5453 & 0.19 & 1.4 & syn & 0.85 & 0.94 & 0.86 & 1.47 & 1.9 & 2.29 & 1 & 1 \\ 
2926 & 13.34 & 2.23 & 5028 & -0.51 & 2.5 & syn & 0.48 & 0.63 & 0.58 & 3.16 & 1.7 & 0.39 & 1 & 0 \\ 
2931 & 12.70 & 2.04 & 4955 & -0.12 & 2.0 & syn & 0.71 & 0.75 & 0.73 & 1.92 & 7.1 & 1.99 & 1 & 0 \\ 
2935 & 12.37 & 0.80 & 6510 & -0.14 & 26.9 & syn & 1.88 & 1.35 & 1.86 & 0.21 & 2.4 & 0.76 & 3 & 1 \\ 
2943 & 12.37 & 0.99 & 5785 & 0.34 & 2.7 & syn & 1.56 & 1.22 & 1.55 & 0.32 & 4.7 & 0.91 & 1 & 1 \\ 
2948 & 10.32 & 2.51 & 5515 & 0.44 & 3.7 & syn & 1.61 & 1.12 & 1.60 & 0.28 & 7.7 & 2.05 & 1 & 1 \\ 
2949 & 11.90 & 1.39 & 5895 & 0.07 & 2.8 & syn & 1.38 & 1.10 & 1.37 & 0.43 & 5.7 & 1.32 & 1 & 1 \\ 
2951 & 11.82 & 1.62 & 5626 & -0.17 & 2.3 & syn & 1.33 & 0.88 & 1.19 & 0.49 & 12.6 & 2.36 & 1 & 0 \\ 
2956 & 10.68 & 1.59 & 6280 & -0.05 & 9.9 & syn & 2.02 & 1.36 & 2.01 & 0.17 & 2.6 & 1.43 & 1 & 1 \\ 
2957 & 12.32 & 2.41 & 4712 & -0.23 & \nodata & emp & 0.73 & 0.70 & 0.69 & 2.04 & 12.0 & 2.64 & 1 & 0 \\ 
2960 & 11.85 & 1.65 & 5956 & 0.09 & 3.0 & syn & 1.17 & 1.09 & 1.16 & 0.69 & 3.7 & 1.52 & 1 & 0 \\ 
2961 & 11.29 & 2.05 & 6078 & 0.13 & 5.2 & syn & 1.19 & 1.15 & 1.18 & 0.68 & 2.3 & 1.94 & 1 & 1 \\ 
2964 & 12.47 & 0.86 & 6126 & -0.35 & 8.2 & syn & 1.72 & 1.08 & 1.69 & 0.22 & 5.7 & 1.17 & 1 & 1 \\ 
2968 & 10.29 & 1.78 & 6176 & -0.14 & 7.4 & syn & 2.17 & 1.27 & 2.15 & 0.13 & 3.5 & 2.44 & 1 & 1 \\ 
2969 & 11.12 & 1.39 & 5955 & 0.18 & 5.2 & syn & 7.36 & 1.19 & 1.44 & 0.34 & 3.5 & 1.51 & 1 & 0 \\ 
2970 & 11.57 & 1.91 & 6178 & -0.06 & 5.1 & syn & 1.14 & 1.10 & 1.13 & 0.76 & 2.2 & 1.93 & 1 & 1 \\ 
2971 & 11.44 & 1.32 & 6248 & 0.18 & 14.9 & syn & 1.74 & 1.37 & 1.72 & 0.26 & 2.5 & 1.54 & 1 & 1 \\ 
2974 & 12.59 & 0.37 & 6540 & 0.13 & 13.2 & syn & 3.54 & 1.91 & 3.40 & 0.05 & 1.1 & 0.83 & 1 & 0 \\ 
2977 & 12.36 & 1.20 & 5946 & -0.06 & 3.2 & syn & 1.28 & 1.04 & 1.27 & 0.51 & 6.2 & 1.20 & 1 & 1 \\ 
2979 & 11.90 & 1.51 & 6002 & -0.18 & 1.7 & syn & 1.26 & 1.01 & 1.25 & 0.52 & 6.5 & 1.68 & 1 & 0 \\ 
2983 & 12.28 & 4.39 & 3677 & -0.13 & \nodata & emp & 0.52 & 0.51 & 0.52 & 3.67 & 12.7 & 7.42 & 1 & 0 \\ 
2984 & 11.64 & 1.25 & 6128 & 0.11 & 6.2 & syn & 1.70 & 1.30 & 1.69 & 0.26 & 3.2 & 1.34 & 1 & 1 \\ 
2992 & 13.04 & 2.41 & 4082 & -0.27 & \nodata & emp & 0.62 & 0.59 & 0.58 & 2.89 & 12.6 & 2.95 & 1 & 1 \\ 
3008 & 10.69 & 1.89 & 5981 & -0.08 & 5.4 & syn & 1.74 & 1.14 & 1.72 & 0.22 & 5.5 & 2.20 & 1 & 0 \\ 
3009 & 13.25 & 1.46 & 5119 & 0.18 & 3.4 & syn & 0.76 & 0.86 & 0.81 & 1.61 & 4.1 & 1.34 & 1 & 0 \\ 
3012 & 11.25 & 1.49 & 5431 & -0.52 & 1.5 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
3015 & 11.77 & 1.35 & 5739 & -0.04 & 2.4 & syn & 1.51 & 1.02 & 1.50 & 0.30 & 8.8 & 1.37 & 1 & 1 \\ 
3017 & 11.76 & 2.36 & 5565 & -0.16 & 0.7 & syn & 0.88 & 0.87 & 0.88 & 1.28 & 6.3 & 2.40 & 1 & 1 \\ 
3021 & 12.30 & 1.55 & 5885 & 0.20 & 2.9 & syn & 1.01 & 1.08 & 1.02 & 1.02 & 1.4 & 1.43 & 1 & 0 \\ 
3023 & 11.85 & 1.52 & 6323 & -0.07 & 6.9 & syn & 1.23 & 1.16 & 1.22 & 0.63 & 2.0 & 1.64 & 1 & 0 \\ 
3032 & 13.95 & 0.98 & 5205 & 0.37 & 1.6 & syn & 0.80 & 0.92 & 0.85 & 1.49 & 2.8 & 0.82 & 1 & 0 \\ 
3034 & 12.61 & 2.76 & 4038 & 0.09 & \nodata & emp & 0.65 & 0.62 & 0.64 & 2.34 & 11.8 & 3.11 & 1 & 1 \\ 
3039 & 12.34 & 1.03 & 5765 & -0.24 & 2.8 & syn & 1.53 & 0.95 & 1.51 & 0.27 & 9.8 & 1.14 & 1 & 1 \\ 
3046 & 11.77 & 1.77 & 5681 & 0.28 & 2.4 & syn & 1.16 & 1.06 & 1.15 & 0.69 & 5.8 & 1.53 & 1 & 0 \\ 
3049 & 12.76 & \nodata & 4724 & 0.12 & \nodata & emp & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
3052 & 11.77 & 1.90 & 5396 & -0.12 & 3.3 & syn & 1.13 & 0.84 & 1.12 & 0.60 & 16.9 & 2.67 & 1 & 1 \\ 
3057 & 14.06 & 0.96 & 5464 & -0.06 & 0.0 & syn & 0.77 & 0.86 & 0.80 & 1.66 & 2.2 & 0.83 & 1 & 0 \\ 
3060 & 11.55 & 1.30 & 6187 & -0.06 & 6.2 & syn & 1.67 & 1.24 & 1.65 & 0.27 & 3.4 & 1.43 & 1 & 1 \\ 
3065 & 12.99 & 1.29 & 5747 & 0.01 & 2.7 & syn & 0.92 & 0.97 & 0.92 & 1.24 & 2.2 & 1.27 & 1 & 0 \\ 
3068 & 12.83 & 2.06 & 4738 & -0.16 & \nodata & emp & 0.68 & 0.70 & 0.68 & 2.16 & 8.4 & 1.85 & 1 & 1 \\ 
3075 & 11.53 & 2.79 & 5362 & -0.44 & 0.1 & syn & 0.85 & 0.75 & 0.84 & 1.27 & 15.4 & 3.11 & 1 & 1 \\ 
3077 & 13.70 & 1.43 & 4603 & 0.12 & \nodata & emp & 0.67 & 0.73 & 0.70 & 2.08 & 6.4 & 1.17 & 1 & 1 \\ 
3083 & 11.40 & 2.12 & 5861 & 0.34 & 2.3 & syn & 1.12 & 1.14 & 1.12 & 0.80 & 2.1 & 1.87 & 1 & 0 \\ 
3086 & 13.91 & 1.01 & 5227 & -0.16 & 0.9 & syn & 0.81 & 0.79 & 0.80 & 1.52 & 9.1 & 1.03 & 1 & 0 \\ 
3087 & 10.98 & 3.65 & 5317 & 0.29 & 1.0 & syn & 0.85 & 0.93 & 0.86 & 1.47 & 2.4 & 3.39 & 1 & 0 \\ 
3093 & 12.10 & 1.26 & 5844 & 0.03 & 0.9 & syn & 1.42 & 1.06 & 1.34 & 0.42 & 6.6 & 1.68 & 1 & 0 \\ 
3094 & 12.75 & 3.72 & 3783 & -0.28 & \nodata & emp & 0.50 & 0.49 & 0.49 & 4.05 & 12.0 & 5.60 & 1 & 1 \\ 
3096 & 11.91 & 1.18 & 5473 & -0.04 & 2.1 & syn & 1.66 & 0.97 & 1.64 & 0.22 & 10.9 & 1.10 & 1 & 1 \\ 
3097 & 10.65 & 2.08 & 5909 & -0.05 & 5.2 & syn & 1.62 & 1.11 & 1.60 & 0.27 & 6.2 & 2.16 & 1 & 1 \\ 
3100 & 12.04 & 1.04 & 5938 & 0.28 & 3.0 & syn & 1.68 & 1.30 & 1.67 & 0.27 & 3.6 & 1.01 & 1 & 0 \\ 
3102 & 13.10 & 2.02 & 4209 & 0.08 & \nodata & emp & 0.67 & 0.66 & 0.66 & 2.29 & 10.8 & 2.16 & 1 & 0 \\ 
3103 & 11.17 & 2.27 & 5898 & 0.30 & 3.4 & syn & 1.32 & 1.15 & 1.19 & 0.64 & 3.0 & 2.00 & 1 & 0 \\ 
3109 & 12.11 & 0.68 & 6237 & 0.09 & 17.3 & syn & 2.48 & 1.54 & 2.44 & 0.10 & 2.0 & 0.96 & 1 & 1 \\ 
3111 & 11.35 & 2.26 & 5950 & -0.06 & 2.5 & syn & 1.09 & 1.02 & 1.08 & 0.80 & 4.2 & 2.35 & 1 & 1 \\ 
3113 & 12.93 & 2.12 & 4751 & -0.36 & \nodata & emp & 0.64 & 0.66 & 0.64 & 2.45 & 8.5 & 2.05 & 1 & 0 \\ 
3114 & 10.96 & 1.18 & 6183 & 0.20 & 8.8 & syn & 2.43 & 1.56 & 2.40 & 0.11 & 2.0 & 1.59 & 1 & 1 \\ 
3117 & 11.51 & 2.54 & 5551 & 0.11 & 1.8 & syn & 0.91 & 0.95 & 0.91 & 1.24 & 3.5 & 2.53 & 1 & 0 \\ 
3122 & 10.82 & 1.31 & 6177 & 0.23 & 10.1 & syn & 2.29 & 1.53 & 2.28 & 0.13 & 2.1 & 1.60 & 1 & 1 \\ 
3125 & 11.73 & 1.44 & 6293 & -0.11 & 9.5 & syn & 1.38 & 1.18 & 1.37 & 0.46 & 3.0 & 1.67 & 1 & 1 \\ 
3128 & 11.90 & 0.91 & 6079 & -0.10 & 5.3 & syn & 2.07 & 1.24 & 2.04 & 0.14 & 4.0 & 1.13 & 1 & 1 \\ 
3130 & 11.73 & 3.45 & 4880 & -0.46 & 1.6 & syn & 0.67 & 0.67 & 0.65 & 2.34 & 9.5 & 3.61 & 1 & 1 \\ 
3132 & 11.24 & 1.03 & 6216 & 0.43 & 12.0 & syn & 2.42 & 1.66 & 2.39 & 0.12 & 1.6 & 1.32 & 1 & 0 \\ 
3136 & 13.56 & 1.33 & 4863 & -0.29 & 0.5 & syn & 0.75 & 0.70 & 0.70 & 2.01 & 11.7 & 1.49 & 1 & 1 \\ 
3140 & 12.78 & \nodata & 4132 & -0.19 & \nodata & emp & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
3145 & 13.36 & 1.71 & 4501 & -0.44 & \nodata & emp & 0.67 & 0.63 & 0.62 & 2.59 & 12.2 & 1.97 & 1 & 1 \\ 
3146 & 12.56 & 0.92 & 5693 & 0.23 & 2.3 & syn & 1.54 & 1.13 & 1.52 & 0.32 & 6.7 & 0.91 & 1 & 1 \\ 
3158 & 6.70 & 27.47 & 5002 & -0.43 & 0.5 & syn & 0.83 & 0.72 & 0.79 & 1.44 & 17.6 & 33.04 & 1 & 1 \\ 
3165 & 9.19 & 3.50 & 6255 & -0.18 & 7.8 & syn & 1.83 & 1.26 & 1.81 & 0.21 & 3.3 & 4.63 & 1 & 1 \\ 
3167 & 8.76 & 9.48 & 5554 & 0.02 & 3.4 & syn & 0.87 & 0.92 & 0.87 & 1.39 & 2.8 & 9.51 & 1 & 0 \\ 
3168 & 9.03 & 4.49 & 5792 & -0.16 & 2.7 & syn & 1.59 & 1.00 & 1.58 & 0.25 & 8.5 & 5.24 & 1 & 0 \\ 
3172 & 12.89 & \nodata & 6027 & -0.05 & 6.3 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
3179 & 10.63 & 3.73 & 5718 & 0.08 & 2.3 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
3180 & 9.62 & 1.90 & 6040 & 0.07 & 4.9 & syn & 2.83 & 1.48 & 2.79 & 0.07 & 2.4 & 2.67 & 1 & 0 \\ 
3184 & 9.79 & 3.50 & 5868 & 0.25 & 4.1 & syn & 1.41 & 1.18 & 1.41 & 0.41 & 4.7 & 3.38 & 1 & 0 \\ 
3190 & 10.96 & 2.47 & 6019 & -0.18 & 1.4 & syn & 1.17 & 1.00 & 1.17 & 0.63 & 5.9 & 2.68 & 1 & 1 \\ 
3193 & 14.69 & \nodata & 4933 & 0.07 & 3.8 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
3194 & 10.35 & 2.17 & 6391 & 0.21 & 6.9 & syn & 1.70 & 1.40 & 1.69 & 0.29 & 2.0 & 2.47 & 1 & 0 \\ 
3195 & 10.18 & 1.93 & 5876 & -0.44 & 3.8 & syn & 2.18 & 1.08 & 2.16 & 0.11 & 5.4 & 1.80 & 1 & 0 \\ 
3196 & 10.28 & 3.10 & 6120 & 0.00 & 3.6 & syn & 1.26 & 1.13 & 1.26 & 0.56 & 3.5 & 3.15 & 1 & 1 \\ 
3197 & 10.25 & 3.59 & 6202 & -0.08 & 7.4 & syn & 1.09 & 1.10 & 1.09 & 0.84 & 1.6 & 3.57 & 1 & 1 \\ 
3201 & 10.35 & 4.19 & 5753 & -0.42 & 0.9 & syn & 0.93 & 0.83 & 0.93 & 1.03 & 10.0 & 4.64 & 1 & 0 \\ 
3202 & 9.96 & 2.14 & 5242 & 0.02 & 3.2 & syn & 2.34 & 1.17 & 2.33 & 0.09 & 5.5 & 2.51 & 1 & 0 \\ 
3203 & 10.82 & 1.74 & 6550 & -0.14 & 16.3 & syn & 1.68 & 1.31 & 1.68 & 0.28 & 2.3 & 2.36 & 1 & 1 \\ 
3208 & 10.66 & 3.37 & 5858 & -0.12 & 2.5 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
3209 & 10.74 & 1.39 & 6408 & 0.09 & 27.4 & syn & 2.21 & 1.51 & 2.20 & 0.14 & 1.9 & 1.87 & 3 & 1 \\ 
3214 & 10.52 & \nodata & 5887 & -0.08 & 5.0 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
3215 & 10.40 & 4.39 & 5238 & 0.04 & 2.9 & syn & 0.91 & 0.84 & 0.91 & 1.11 & 12.6 & 1.72 & 1 & 0 \\ 
3218 & 10.71 & 3.05 & 6004 & 0.04 & 3.9 & syn & 1.05 & 1.07 & 1.05 & 0.92 & 1.9 & 3.00 & 1 & 0 \\ 
3220 & 10.97 & 1.67 & 6396 & 0.15 & 12.8 & syn & 1.66 & 1.37 & 1.65 & 0.30 & 2.1 & 2.03 & 1 & 1 \\ 
3224 & 10.46 & 4.71 & 5367 & 0.07 & 2.6 & syn & 0.81 & 0.89 & 0.82 & 1.59 & 2.4 & 4.48 & 1 & 1 \\ 
3225 & 10.50 & 4.42 & 5418 & 0.19 & 2.3 & syn & 0.84 & 0.93 & 0.86 & 1.48 & 2.1 & 4.13 & 1 & 0 \\ 
3227 & 10.77 & 2.73 & 5933 & 0.03 & 3.1 & syn & 1.17 & 1.06 & 1.16 & 0.67 & 4.6 & 2.72 & 1 & 0 \\ 
3232 & 10.80 & 3.39 & 5768 & 0.05 & 3.8 & syn & 0.94 & 0.99 & 0.94 & 1.19 & 2.1 & 3.31 & 1 & 1 \\ 
3233 & 10.89 & 3.11 & 5758 & 0.02 & 1.7 & syn & 0.97 & 0.98 & 0.97 & 1.07 & 3.5 & 3.07 & 1 & 0 \\ 
3234 & 11.02 & 1.71 & 6400 & -0.05 & 11.6 & syn & 1.60 & 1.28 & 1.58 & 0.32 & 2.5 & 2.38 & 1 & 0 \\ 
3236 & 11.05 & 1.85 & 6317 & 0.07 & 13.3 & syn & 1.45 & 1.27 & 1.43 & 0.42 & 2.2 & 2.01 & 1 & 0 \\ 
3237 & 10.81 & 3.15 & 5851 & 0.20 & 5.0 & syn & 1.00 & 1.07 & 1.00 & 1.05 & 1.4 & 3.05 & 1 & 1 \\ 
3239 & 10.75 & 3.77 & 5646 & 0.06 & 5.7 & syn & 0.88 & 0.95 & 0.89 & 1.36 & 1.9 & 3.69 & 1 & 0 \\ 
3240 & 10.53 & 1.35 & 6018 & 0.24 & 5.4 & syn & 2.62 & 1.60 & 2.58 & 0.09 & 2.0 & 1.61 & 1 & 0 \\ 
3244 & 10.18 & 0.69 & 4885 & -0.10 & 3.9 & syn & 6.87 & 1.42 & 6.82 & 0.00 & 2.5 & 0.85 & 1 & 0 \\ 
3245 & 11.11 & 2.00 & 6115 & -0.10 & 3.6 & syn & 1.33 & 1.10 & 1.32 & 0.47 & 4.5 & 2.30 & 1 & 1 \\ 
3246 & 10.20 & 6.60 & 4680 & 0.14 & \nodata & emp & 0.71 & 0.75 & 0.73 & 1.93 & 7.1 & 5.58 & 1 & 1 \\ 
3248 & 10.89 & 2.76 & 5735 & -0.02 & 1.5 & syn & 1.11 & 0.96 & 1.10 & 0.71 & 8.1 & 2.81 & 1 & 1 \\ 
3249 & 11.12 & 2.15 & 6003 & 0.03 & 4.0 & syn & 1.23 & 1.09 & 1.23 & 0.58 & 4.4 & 2.23 & 1 & 0 \\ 
3251 & 11.10 & 2.16 & 5921 & 0.09 & 3.8 & syn & 1.26 & 1.09 & 1.25 & 0.55 & 5.0 & 2.02 & 1 & 0 \\ 
3254 & 10.88 & 2.85 & 5590 & 0.32 & 2.7 & syn & 1.08 & 1.03 & 1.07 & 0.83 & 5.4 & 2.45 & 1 & 0 \\ 
3257 & 13.30 & 1.51 & 4370 & 0.23 & \nodata & emp & 0.79 & 0.73 & 0.72 & 1.94 & 12.9 & 1.71 & 1 & 0 \\ 
3263 & 12.73 & 2.31 & 4441 & -0.05 & \nodata & emp & 0.67 & 0.67 & 0.66 & 2.31 & 9.2 & 2.33 & 5 & 0 \\ 
3266 & 12.91 & 2.00 & 4377 & 0.12 & \nodata & emp & 0.71 & 0.70 & 0.69 & 2.11 & 10.8 & 2.10 & 1 & 1 \\ 
3277 & 11.63 & 1.03 & 5997 & -0.02 & 7.3 & syn & 2.08 & 1.25 & 2.06 & 0.14 & 4.1 & 1.22 & 1 & 1 \\ 
3278 & 12.98 & 1.32 & 5472 & 0.21 & 3.6 & syn & 0.91 & 0.96 & 0.91 & 1.26 & 3.3 & 1.31 & 1 & 0 \\ 
3282 & 12.92 & 2.82 & 3929 & -0.23 & \nodata & emp & 0.57 & 0.56 & 0.56 & 3.12 & 12.8 & 3.68 & 1 & 1 \\ 
3283 & 13.14 & 1.77 & 4734 & -0.03 & \nodata & emp & 0.69 & 0.72 & 0.70 & 2.04 & 7.4 & 1.51 & 1 & 1 \\ 
3286 & 12.68 & 2.72 & 4143 & -0.12 & \nodata & emp & 0.61 & 0.61 & 0.61 & 2.68 & 11.0 & 3.00 & 1 & 0 \\ 
3287 & 12.54 & 1.15 & 5891 & -0.10 & 3.0 & syn & 1.24 & 1.00 & 1.23 & 0.53 & 7.3 & 1.14 & 1 & 1 \\ 
3288 & 12.51 & 1.86 & 5440 & 0.08 & 2.3 & syn & 0.80 & 0.89 & 0.81 & 1.64 & 1.5 & 1.73 & 1 & 1 \\ 
3296 & 12.38 & 2.22 & 4673 & 0.13 & \nodata & emp & 0.78 & 0.76 & 0.75 & 1.76 & 11.2 & 2.06 & 1 & 1 \\ 
3298 & 13.36 & 1.83 & 4234 & -0.37 & \nodata & emp & 0.66 & 0.61 & 0.60 & 2.76 & 13.4 & 2.26 & 1 & 1 \\ 
3301 & 12.51 & 0.80 & 5755 & 0.27 & 2.9 & syn & 1.82 & 1.22 & 1.78 & 0.21 & 5.2 & 0.79 & 1 & 1 \\ 
3303 & 13.47 & 1.50 & 4850 & -0.24 & 2.3 & syn & 0.69 & 0.70 & 0.69 & 2.13 & 8.6 & 1.52 & 1 & 1 \\ 
3308 & 12.51 & 0.89 & 5890 & 0.03 & 3.1 & syn & 1.62 & 1.14 & 1.60 & 0.28 & 5.7 & 0.99 & 1 & 1 \\ 
3310 & 11.86 & 2.27 & 5444 & 0.21 & 0.3 & syn & 0.88 & 0.95 & 0.89 & 1.36 & 2.6 & 2.11 & 1 & 1 \\ 
3311 & 12.04 & 2.81 & 4531 & -0.04 & \nodata & emp & 0.74 & 0.70 & 0.69 & 2.06 & 11.2 & 3.02 & 1 & 0 \\ 
3313 & 12.60 & 2.11 & 4688 & 0.11 & \nodata & emp & 0.74 & 0.76 & 0.74 & 1.85 & 9.2 & 1.87 & 1 & 1 \\ 
3315 & 12.41 & 1.61 & 5617 & -0.41 & 0.2 & syn & 0.96 & 0.79 & 0.96 & 0.90 & 14.4 & 1.81 & 1 & 1 \\ 
3330 & 12.90 & 1.72 & 4718 & 0.07 & \nodata & emp & 0.80 & 0.76 & 0.75 & 1.73 & 11.7 & 1.65 & 1 & 1 \\ 
3334 & 11.84 & 2.84 & 4403 & 0.10 & \nodata & emp & 0.81 & 0.72 & 0.72 & 1.92 & 14.0 & 3.37 & 5 & 0 \\ 
3338 & 12.16 & 1.42 & 6197 & -0.16 & 2.1 & syn & 1.17 & 1.07 & 1.16 & 0.68 & 3.2 & 1.49 & 1 & 0 \\ 
3340 & 12.40 & 0.79 & 6114 & -0.09 & 6.5 & syn & 1.92 & 1.22 & 1.79 & 0.21 & 4.0 & 1.33 & 1 & 0 \\ 
3346 & 12.01 & 1.56 & 5946 & -0.01 & 2.6 & syn & 1.15 & 1.04 & 1.15 & 0.68 & 4.8 & 1.57 & 1 & 1 \\ 
3358 & 12.29 & 1.98 & 5395 & -0.08 & 2.6 & syn & 0.84 & 0.86 & 0.83 & 1.45 & 5.5 & 2.02 & 1 & 1 \\ 
3363 & 12.26 & 1.40 & 5704 & -0.06 & 1.0 & syn & 1.18 & 0.94 & 1.17 & 0.58 & 9.9 & 1.37 & 1 & 1 \\ 
3364 & 12.88 & 1.90 & 4632 & 0.09 & \nodata & emp & 0.73 & 0.74 & 0.72 & 1.92 & 9.2 & 1.70 & 1 & 0 \\ 
3370 & 12.60 & 2.20 & 4789 & 0.10 & \nodata & emp & 0.70 & 0.76 & 0.73 & 1.92 & 5.9 & 1.74 & 1 & 1 \\ 
3371 & 12.00 & 1.79 & 5413 & 0.00 & 1.8 & syn & 1.06 & 0.87 & 1.05 & 0.75 & 14.2 & 2.23 & 1 & 0 \\ 
3377 & 12.76 & \nodata & 4510 & 0.13 & \nodata & emp & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
3378 & 12.12 & 1.95 & 5580 & -0.41 & 0.0 & syn & 0.90 & 0.79 & 0.90 & 1.07 & 13.0 & 2.13 & 1 & 0 \\ 
3382 & 12.09 & 1.86 & 5426 & 0.20 & 0.9 & syn & 0.98 & 0.94 & 0.97 & 1.03 & 7.2 & 1.92 & 1 & 0 \\ 
3384 & 11.72 & 1.65 & 5956 & 0.05 & 3.9 & syn & 1.25 & 1.09 & 1.24 & 0.56 & 4.9 & 1.52 & 1 & 1 \\ 
3391 & 13.22 & 1.49 & 4327 & -0.22 & \nodata & emp & 0.84 & 0.66 & 0.66 & 2.25 & 14.6 & 2.13 & 1 & 0 \\ 
3398 & 12.29 & 1.01 & 6425 & 0.06 & 24.9 & syn & 1.51 & 1.31 & 1.49 & 0.38 & 2.1 & 1.16 & 3 & 1 \\ 
3403 & 11.64 & 1.13 & 5756 & 0.10 & 3.9 & syn & 1.91 & 1.18 & 1.90 & 0.17 & 5.7 & 1.22 & 1 & 1 \\ 
3412 & 12.16 & 3.04 & 4510 & -0.05 & \nodata & emp & 0.64 & 0.67 & 0.66 & 2.35 & 7.4 & 2.91 & 1 & 1 \\ 
3414 & 12.52 & 2.46 & 3910 & -0.16 & \nodata & emp & 0.71 & 0.62 & 0.64 & 2.38 & 15.6 & 4.37 & 1 & 0 \\ 
3419 & 11.74 & 1.05 & 6447 & -0.40 & 4.5 & syn & 1.88 & 1.20 & 1.86 & 0.18 & 3.6 & 1.02 & 1 & 0 \\ 
3421 & 12.65 & 0.78 & 6374 & 0.11 & 7.8 & syn & 1.63 & 1.34 & 1.62 & 0.31 & 2.3 & 0.96 & 1 & 0 \\ 
3422 & 11.67 & 2.03 & 5850 & 0.14 & 5.2 & syn & 1.05 & 1.06 & 1.04 & 0.93 & 2.6 & 2.09 & 1 & 0 \\ 
3425 & 11.51 & 1.10 & 6146 & 0.03 & 6.4 & syn & 2.06 & 1.36 & 2.03 & 0.16 & 2.8 & 1.45 & 1 & 1 \\ 
3436 & 11.46 & 3.25 & 5045 & 0.21 & 3.4 & syn & 0.78 & 0.85 & 0.81 & 1.56 & 5.8 & 3.10 & 1 & 1 \\ 
3438 & 12.36 & 1.36 & 6054 & -0.14 & 3.7 & syn & 1.12 & 1.03 & 1.11 & 0.75 & 4.2 & 1.43 & 1 & 1 \\ 
3439 & 12.91 & 0.69 & 6046 & -0.19 & 46.3 & syn & 1.76 & 1.12 & 1.72 & 0.21 & 5.4 & 0.17 & 3 & 1 \\ 
3451 & 12.71 & 1.20 & 6023 & 0.05 & 3.1 & syn & 1.08 & 1.09 & 1.07 & 0.87 & 2.0 & 1.18 & 1 & 0 \\ 
3456 & 11.41 & 2.04 & 5601 & -0.27 & 8.0 & syn & 1.19 & 0.84 & 1.18 & 0.50 & 15.2 & 2.98 & 1 & 0 \\ 
3465 & 11.39 & 3.14 & 5335 & 0.06 & 2.8 & syn & 0.80 & 0.88 & 0.81 & 1.64 & 2.3 & 2.99 & 1 & 0 \\ 
3469 & 12.47 & 1.16 & 5481 & 0.05 & 6.8 & syn & 1.32 & 0.93 & 1.31 & 0.41 & 13.4 & 1.79 & 1 & 1 \\ 
3473 & 11.82 & 2.94 & 5146 & 0.04 & 5.3 & syn & 0.73 & 0.83 & 0.78 & 1.70 & 4.0 & 2.75 & 1 & 1 \\ 
3474 & 12.62 & -2.97 & 5879 & -0.16 & 4.8 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
3478 & 11.18 & 4.06 & 4729 & 0.14 & \nodata & emp & 0.73 & 0.77 & 0.74 & 1.84 & 7.9 & 3.48 & 1 & 1 \\ 
3497 & 10.62 & 3.22 & 4685 & 0.10 & \nodata & emp & 1.22 & 0.81 & 0.87 & 1.20 & 18.7 & 4.71 & 1 & 0 \\ 
3500 & 11.83 & 0.94 & 6050 & 0.21 & 6.9 & syn & 2.07 & 1.42 & 2.04 & 0.16 & 2.7 & 1.04 & 1 & 1 \\ 
3503 & 12.48 & 1.15 & 6099 & -0.46 & 1.8 & syn & 1.25 & 0.94 & 1.24 & 0.49 & 7.8 & 1.53 & 1 & 0 \\ 
3541 & 12.31 & 0.87 & 6239 & -0.21 & 6.6 & syn & 1.75 & 1.22 & 1.73 & 0.23 & 3.6 & 1.23 & 1 & 0 \\ 
3545 & 13.36 & 1.20 & 4662 & -0.03 & 39.1 & syn & 0.94 & 0.77 & 0.83 & 1.33 & 18.0 & 1.54 & 5 & 0 \\ 
3546 & 12.19 & 2.95 & 4170 & 0.00 & \nodata & emp & 0.71 & 0.65 & 0.65 & 2.30 & 12.7 & 3.46 & 1 & 0 \\ 
3550 & 13.35 & 1.19 & 4760 & -0.03 & 37.0 & syn & 0.93 & 0.77 & 0.84 & 1.30 & 17.6 & 1.46 & 5 & 0 \\ 
3587 & 12.66 & \nodata & 5544 & 0.08 & 81.2 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 3 & 0 \\ 
3608 & 12.03 & 1.47 & 5863 & -0.07 & 2.1 & syn & 1.21 & 1.00 & 1.20 & 0.57 & 7.3 & 1.66 & 1 & 0 \\ 
3641 & 12.44 & 0.85 & 6167 & -0.09 & 3.2 & syn & 1.73 & 1.22 & 1.67 & 0.25 & 3.6 & 1.23 & 1 & 0 \\ 
3650 & 13.30 & 1.22 & 4628 & -0.29 & 9.5 & syn & 0.96 & 0.73 & 0.78 & 1.51 & 18.4 & 1.66 & 5 & 0 \\ 
3663 & 11.12 & 2.93 & 5729 & -0.00 & 2.0 & syn & 0.94 & 0.97 & 0.94 & 1.17 & 3.1 & 2.94 & 1 & 1 \\ 
3678 & 11.31 & 2.89 & 5501 & 0.18 & 1.5 & syn & 0.88 & 0.96 & 0.89 & 1.34 & 2.4 & 2.69 & 1 & 1 \\ 
3680 & 13.10 & 1.11 & 5814 & 0.23 & 2.3 & syn & 0.99 & 1.06 & 1.00 & 1.05 & 1.5 & 0.95 & 1 & 0 \\ 
3681 & 10.69 & 2.54 & 6247 & 0.17 & 8.1 & syn & 1.25 & 1.23 & 1.24 & 0.64 & 1.2 & 2.57 & 1 & 1 \\ 
3683 & 10.89 & 1.88 & 6321 & -0.04 & 10.7 & syn & 1.54 & 1.26 & 1.53 & 0.35 & 2.8 & 2.32 & 1 & 1 \\ 
3689 & 12.63 & 1.03 & 6002 & 0.03 & 4.0 & syn & 1.30 & 1.11 & 1.29 & 0.51 & 4.7 & 1.01 & 1 & 1 \\ 
3726 & 13.17 & 0.09 & 4921 & -0.28 & 11.1 & syn & 4.74 & 0.73 & 0.82 & 1.28 & 9.1 & 1.72 & 1 & 0 \\ 
3741 & 12.06 & 1.13 & 6296 & -0.36 & 33.6 & syn & 1.56 & 1.13 & 1.54 & 0.31 & 4.3 & 0.58 & 3 & 1 \\ 
3744 & 13.69 & 0.88 & 5304 & 0.05 & 29.6 & syn & 1.02 & 0.86 & 0.99 & 0.87 & 14.4 & 0.89 & 5 & 0 \\ 
3764 & 13.22 & 1.20 & 4574 & -0.68 & 143.1 & syn & 1.02 & 0.00 & 0.00 & 0.00 & 0.0 & 2.19 & 3 & 0 \\ 
3766 & 13.34 & 0.94 & 4989 & 0.21 & 80.4 & syn & 1.18 & 0.86 & 0.99 & 0.83 & 17.7 & 1.15 & 3 & 0 \\ 
3770 & 12.84 & 0.40 & 6087 & -0.05 & 6.4 & syn & 3.14 & 1.47 & 2.91 & 0.06 & 2.2 & 0.82 & 1 & 0 \\ 
3780 & 12.79 & 0.64 & 6324 & -0.24 & 8.6 & syn & 1.91 & 1.24 & 1.88 & 0.18 & 3.5 & 0.65 & 1 & 0 \\ 
3787 & 12.36 & 1.67 & 5716 & 0.14 & 1.1 & syn & 0.92 & 1.00 & 0.93 & 1.23 & 1.8 & 1.55 & 1 & 0 \\ 
3791 & 12.37 & 0.81 & 6069 & -0.01 & 5.1 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
3792 & 12.81 & 1.89 & 4321 & -0.02 & \nodata & emp & 0.79 & 0.69 & 0.69 & 2.08 & 14.4 & 2.35 & 5 & 0 \\ 
3794 & 13.32 & 1.67 & 4454 & 0.07 & \nodata & emp & 0.70 & 0.70 & 0.69 & 2.12 & 9.7 & 1.70 & 1 & 1 \\ 
3801 & 14.19 & 0.65 & 5563 & 0.30 & 3.0 & syn & 1.06 & 1.02 & 1.04 & 0.89 & 5.2 & 0.45 & 1 & 0 \\ 
3811 & 12.17 & 1.18 & 5762 & -0.18 & 4.4 & syn & 1.47 & 0.96 & 1.45 & 0.31 & 9.9 & 1.83 & 1 & 1 \\ 
3823 & 12.38 & 1.73 & 5657 & 0.11 & 1.5 & syn & 0.89 & 0.97 & 0.90 & 1.30 & 1.9 & 1.66 & 1 & 1 \\ 
3835 & 10.84 & 4.86 & 4990 & 0.03 & 4.9 & syn & 0.69 & 0.79 & 0.75 & 1.87 & 4.1 & 4.44 & 1 & 1 \\ 
3853 & 8.51 & 3.27 & 4873 & -0.08 & 3.7 & syn & 3.06 & 0.98 & 3.04 & 0.03 & 10.0 & 3.69 & 1 & 0 \\ 
3864 & 10.91 & 4.52 & 5033 & 0.09 & 4.5 & syn & 0.71 & 0.81 & 0.77 & 1.77 & 4.1 & 4.14 & 1 & 1 \\ 
3867 & 13.18 & 1.18 & 5571 & 0.15 & 1.5 & syn & 0.92 & 0.97 & 0.92 & 1.22 & 3.1 & 1.11 & 1 & 0 \\ 
3871 & 10.20 & 5.20 & 5184 & 0.08 & 3.3 & syn & 0.86 & 0.85 & 0.84 & 1.37 & 8.2 & 5.43 & 1 & 0 \\ 
3876 & 11.11 & 3.09 & 5700 & 0.11 & 10.0 & syn & 0.89 & 0.97 & 0.90 & 1.32 & 1.5 & 2.97 & 1 & 1 \\ 
3878 & 11.26 & 2.64 & 5854 & 0.13 & 3.2 & syn & 0.95 & 1.03 & 0.96 & 1.14 & 1.3 & 2.52 & 1 & 1 \\ 
3880 & 9.55 & 4.46 & 6317 & 0.10 & 14.4 & syn & 1.19 & 1.21 & 1.20 & 0.70 & 0.9 & 4.53 & 1 & 0 \\ 
3886 & 7.47 & \nodata & 4688 & 0.22 & 5.3 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
3889 & 12.10 & 1.43 & 5793 & 0.22 & 1.7 & syn & 1.21 & 1.09 & 1.20 & 0.62 & 5.1 & 1.34 & 1 & 0 \\ 
3890 & 10.89 & 0.59 & 4792 & -0.04 & \nodata & emp & 5.86 & 1.20 & 5.82 & 0.01 & 4.8 & 4.08 & 1 & 0 \\ 
3891 & 11.67 & 1.03 & 5089 & -0.08 & 2.7 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
3892 & 11.19 & 2.64 & 5673 & 0.30 & 2.4 & syn & 1.01 & 1.06 & 1.01 & 1.02 & 2.4 & 2.28 & 1 & 1 \\ 
3893 & 13.21 & 1.82 & 4412 & 0.03 & \nodata & emp & 0.68 & 0.69 & 0.67 & 2.22 & 9.6 & 1.86 & 1 & 1 \\ 
3907 & 11.18 & 1.75 & 6559 & -0.07 & 18.4 & syn & 1.44 & 1.28 & 1.43 & 0.43 & 1.8 & 2.15 & 1 & 0 \\ 
3908 & 10.45 & 1.99 & 5672 & 0.01 & 4.3 & syn & 1.93 & 1.12 & 1.91 & 0.16 & 6.5 & 2.00 & 1 & 0 \\ 
3913 & 13.46 & 0.75 & 5967 & 0.20 & 2.9 & syn & 1.22 & 1.14 & 1.21 & 0.63 & 3.1 & 0.73 & 1 & 0 \\ 
3925 & 12.30 & 2.07 & 5374 & 0.08 & 2.5 & syn & 0.80 & 0.88 & 0.81 & 1.63 & 2.0 & 1.96 & 1 & 1 \\ 
3928 & 11.77 & 1.52 & 6192 & -0.05 & 6.6 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
3936 & 11.29 & 3.65 & 5049 & 0.14 & 5.8 & syn & 0.75 & 0.83 & 0.79 & 1.66 & 5.0 & 3.44 & 1 & 1 \\ 
3943 & 11.33 & 1.64 & 6218 & -0.04 & 7.8 & syn & 1.48 & 1.21 & 1.47 & 0.37 & 3.3 & 1.98 & 1 & 1 \\ 
3946 & 11.93 & 1.06 & 6325 & -0.22 & 7.1 & syn & 1.73 & 1.24 & 1.71 & 0.24 & 3.2 & 1.47 & 1 & 1 \\ 
3970 & 11.80 & 2.62 & 4104 & 0.24 & \nodata & emp & 0.96 & 0.00 & 0.00 & 0.00 & 0.0 & 3.98 & 1 & 0 \\ 
3975 & 12.55 & 2.61 & 4282 & 0.00 & \nodata & emp & 0.65 & 0.65 & 0.65 & 2.41 & 9.9 & 2.69 & 1 & 1 \\ 
3980 & 13.08 & 0.85 & 5769 & 0.17 & 2.0 & syn & 1.31 & 1.08 & 1.29 & 0.49 & 6.5 & 0.96 & 1 & 0 \\ 
3991 & 11.41 & 3.11 & 5651 & -0.01 & 6.6 & syn & 0.78 & 0.90 & 0.83 & 1.58 & 1.2 & 2.76 & 1 & 0 \\ 
4002 & 13.15 & 1.43 & 5214 & 0.21 & 2.9 & syn & 0.80 & 0.89 & 0.82 & 1.61 & 2.7 & 1.33 & 1 & 0 \\ 
4004 & 11.11 & 3.07 & 5737 & -0.02 & 6.9 & syn & 0.89 & 0.95 & 0.90 & 1.31 & 2.1 & 3.05 & 1 & 1 \\ 
4005 & 12.92 & 1.35 & 5493 & 0.10 & 1.8 & syn & 0.92 & 0.93 & 0.91 & 1.22 & 4.7 & 1.31 & 1 & 0 \\ 
4011 & 11.14 & 2.06 & 5932 & 0.18 & 3.8 & syn & 1.29 & 1.14 & 1.28 & 0.53 & 4.2 & 1.99 & 1 & 0 \\ 
4014 & 12.35 & 1.42 & 5973 & 0.09 & 3.5 & syn & 1.07 & 1.08 & 1.07 & 0.88 & 2.1 & 1.32 & 1 & 1 \\ 
4016 & 11.52 & 4.11 & 4296 & 0.01 & \nodata & emp & 0.66 & 0.66 & 0.65 & 2.35 & 10.3 & 4.27 & 1 & 1 \\ 
4018 & 13.08 & 1.39 & 5486 & -0.01 & 1.8 & syn & 0.83 & 0.89 & 0.84 & 1.50 & 2.7 & 1.35 & 1 & 0 \\ 
4021 & 11.49 & \nodata & 6447 & 0.02 & 19.1 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
4022 & 11.89 & 0.97 & 5996 & -0.07 & 6.8 & syn & 1.96 & 1.20 & 1.94 & 0.16 & 4.6 & 1.20 & 1 & 1 \\ 
4024 & 11.93 & 2.42 & 5245 & -0.02 & 3.8 & syn & 0.83 & 0.84 & 0.83 & 1.47 & 6.9 & 2.47 & 1 & 1 \\ 
4032 & 10.99 & 2.53 & 5584 & 0.09 & 1.1 & syn & 1.17 & 0.96 & 1.16 & 0.60 & 10.4 & 2.62 & 1 & 1 \\ 
4036 & 11.90 & 3.01 & 4744 & 0.00 & \nodata & emp & 0.71 & 0.74 & 0.72 & 1.96 & 7.9 & 2.63 & 1 & 1 \\ 
4037 & 11.62 & 1.71 & 6265 & 0.01 & 7.3 & syn & 1.22 & 1.17 & 1.21 & 0.65 & 1.9 & 1.80 & 1 & 1 \\ 
4050 & 13.62 & 1.45 & 4521 & 0.02 & \nodata & emp & 0.70 & 0.70 & 0.69 & 2.12 & 9.1 & 1.46 & 1 & 0 \\ 
4051 & 13.14 & 1.39 & 5168 & 0.08 & 1.7 & syn & 0.84 & 0.85 & 0.83 & 1.45 & 7.2 & 1.39 & 1 & 1 \\ 
4053 & 11.44 & 2.36 & 6067 & -0.07 & 4.4 & syn & 0.99 & 1.04 & 0.99 & 1.06 & 1.4 & 2.34 & 1 & 1 \\ 
4054 & 12.74 & 1.74 & 5253 & 0.11 & 1.7 & syn & 0.79 & 0.87 & 0.80 & 1.67 & 2.4 & 1.63 & 1 & 0 \\ 
4060 & 12.29 & 1.10 & 5795 & 0.18 & 3.2 & syn & 1.46 & 1.13 & 1.44 & 0.37 & 5.9 & 1.07 & 1 & 0 \\ 
4062 & 12.76 & 0.94 & 6078 & 0.04 & 4.3 & syn & 1.35 & 1.15 & 1.34 & 0.47 & 3.9 & 0.92 & 1 & 0 \\ 
4066 & 12.20 & 1.17 & 6403 & 0.13 & 12.7 & syn & 1.33 & 1.29 & 1.32 & 0.55 & 1.2 & 1.24 & 1 & 0 \\ 
4067 & 12.82 & 1.13 & 6001 & 0.10 & 3.8 & syn & 1.09 & 1.10 & 1.09 & 0.85 & 2.1 & 1.06 & 1 & 1 \\ 
4069 & 12.49 & 2.40 & 4612 & 0.09 & \nodata & emp & 0.69 & 0.73 & 0.71 & 2.04 & 7.4 & 2.11 & 1 & 1 \\ 
4070 & 12.42 & 2.20 & 4926 & 0.07 & 1.9 & syn & 0.75 & 0.79 & 0.77 & 1.73 & 7.1 & 2.13 & 1 & 0 \\ 
4072 & 12.00 & 1.51 & 5872 & 0.14 & 2.7 & syn & 1.21 & 1.09 & 1.20 & 0.62 & 4.8 & 1.41 & 1 & 1 \\ 
4077 & 11.30 & 4.58 & 4199 & 0.05 & \nodata & emp & 0.67 & 0.65 & 0.65 & 2.31 & 11.3 & 5.00 & 1 & 0 \\ 
4087 & 12.12 & 3.35 & 3889 & -0.22 & \nodata & emp & 0.65 & 0.60 & 0.62 & 2.53 & 15.4 & 5.65 & 1 & 1 \\ 
4089 & 13.04 & 1.05 & 4839 & -0.12 & 29.3 & syn & 1.20 & 0.83 & 1.02 & 0.78 & 19.5 & 1.74 & 3 & 0 \\ 
4097 & 10.84 & 5.29 & 4341 & 0.13 & \nodata & emp & 0.69 & 0.70 & 0.68 & 2.16 & 10.3 & 5.47 & 1 & 1 \\ 
4098 & 11.79 & 2.86 & 4979 & -0.05 & 3.3 & syn & 0.80 & 0.77 & 0.77 & 1.67 & 9.3 & 2.94 & 1 & 0 \\ 
4103 & 12.88 & 1.32 & 5289 & -0.01 & 2.5 & syn & 0.98 & 0.84 & 0.96 & 0.92 & 15.0 & 1.61 & 1 & 0 \\ 
4109 & 12.37 & 2.23 & 4984 & 0.26 & 2.5 & syn & 0.76 & 0.84 & 0.80 & 1.64 & 5.0 & 2.00 & 1 & 1 \\ 
4121 & 13.81 & 1.08 & 5130 & -0.46 & 1.8 & syn & 0.79 & 0.71 & 0.75 & 1.66 & 14.7 & 1.23 & 1 & 0 \\ 
4123 & 12.10 & 0.75 & 6097 & 0.08 & 4.2 & syn & 2.31 & 1.39 & 2.26 & 0.12 & 2.8 & 0.67 & 1 & 1 \\ 
4129 & 11.58 & 3.05 & 5106 & 0.17 & 1.7 & syn & 0.77 & 0.85 & 0.81 & 1.57 & 5.1 & 2.83 & 1 & 1 \\ 
4132 & 12.80 & \nodata & 4077 & -0.28 & \nodata & emp & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
4134 & 13.70 & 1.40 & 4667 & -0.19 & \nodata & emp & 0.68 & 0.68 & 0.67 & 2.22 & 9.3 & 1.41 & 4 & 0 \\ 
4135 & 12.55 & 2.25 & 4631 & -0.35 & \nodata & emp & 0.72 & 0.66 & 0.66 & 2.23 & 12.9 & 2.58 & 1 & 0 \\ 
4136 & 12.42 & 0.82 & 5710 & 0.16 & 3.1 & syn & 1.85 & 1.16 & 1.83 & 0.19 & 6.2 & 0.87 & 1 & 1 \\ 
4144 & 12.97 & 1.21 & 5999 & -0.12 & 3.0 & syn & 0.97 & 1.00 & 0.97 & 1.10 & 1.9 & 1.13 & 1 & 0 \\ 
4146 & 11.66 & 3.09 & 5080 & 0.25 & 3.7 & syn & 0.74 & 0.86 & 0.81 & 1.63 & 3.7 & 2.78 & 1 & 1 \\ 
4156 & 12.25 & 1.02 & 5780 & 0.25 & 3.3 & syn & 1.61 & 1.21 & 1.59 & 0.30 & 5.0 & 0.94 & 1 & 1 \\ 
4157 & 11.47 & 1.81 & 6261 & 0.03 & 10.2 & syn & 1.22 & 1.18 & 1.22 & 0.65 & 1.8 & 1.88 & 1 & 1 \\ 
4159 & 12.63 & 1.65 & 5226 & 0.13 & 2.0 & syn & 0.88 & 0.87 & 0.87 & 1.30 & 8.1 & 1.62 & 1 & 0 \\ 
4160 & 11.87 & 2.01 & 5795 & 0.26 & 3.5 & syn & 0.95 & 1.05 & 0.97 & 1.15 & 1.1 & 1.85 & 1 & 1 \\ 
4184 & 11.37 & \nodata & 4911 & 0.02 & 5.0 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
4188 & 11.50 & 2.16 & 5991 & 0.14 & 4.2 & syn & 1.03 & 1.09 & 1.04 & 0.96 & 1.2 & 2.08 & 1 & 1 \\ 
4190 & 12.01 & 0.64 & 5691 & 0.33 & 3.0 & syn & 4.97 & 1.18 & 1.54 & 0.28 & 5.0 & 1.20 & 1 & 0 \\ 
4198 & 11.36 & 1.26 & 5952 & -0.48 & 6.0 & syn & 1.93 & 1.03 & 1.92 & 0.15 & 6.5 & 1.06 & 1 & 0 \\ 
4199 & 12.44 & 2.17 & 5118 & -0.13 & 0.9 & syn & 0.74 & 0.78 & 0.76 & 1.74 & 6.9 & 2.14 & 1 & 0 \\ 
4204 & 12.62 & 1.12 & 5884 & 0.17 & 3.3 & syn & 1.22 & 1.10 & 1.21 & 0.61 & 4.5 & 1.01 & 1 & 1 \\ 
4207 & 12.66 & 2.61 & 4162 & -0.02 & \nodata & emp & 0.64 & 0.63 & 0.63 & 2.46 & 10.9 & 2.83 & 1 & 1 \\ 
4208 & 13.04 & 1.73 & 4376 & 0.23 & \nodata & emp & 0.78 & 0.73 & 0.72 & 1.95 & 12.5 & 1.93 & 1 & 0 \\ 
4212 & 12.59 & 1.08 & 6215 & 0.14 & 6.6 & syn & 1.25 & 1.21 & 1.24 & 0.63 & 1.6 & 1.11 & 1 & 1 \\ 
4215 & 12.00 & 1.11 & 5427 & -0.25 & 2.0 & syn & 1.77 & 0.92 & 1.75 & 0.17 & 11.4 & 1.27 & 1 & 0 \\ 
4216 & 13.78 & \nodata & 4961 & 0.15 & 4.7 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
4222 & 12.04 & 1.51 & 5612 & -0.02 & 3.1 & syn & 1.25 & 0.93 & 1.23 & 0.49 & 11.6 & 2.12 & 1 & 1 \\ 
4226 & 11.20 & 1.39 & 5866 & 0.38 & 4.8 & syn & 1.92 & 1.38 & 1.90 & 0.20 & 3.2 & 1.26 & 1 & 0 \\ 
4230 & 12.37 & 1.08 & 5850 & -0.38 & 1.7 & syn & 1.43 & 0.92 & 1.42 & 0.32 & 10.4 & 1.29 & 1 & 1 \\ 
4235 & 12.05 & 1.20 & 6326 & 0.03 & 13.6 & syn & 1.40 & 1.25 & 1.40 & 0.45 & 2.3 & 1.30 & 1 & 1 \\ 
4238 & 12.77 & 1.86 & 4441 & 0.23 & \nodata & emp & 0.81 & 0.74 & 0.73 & 1.85 & 13.2 & 2.11 & 1 & 0 \\ 
4245 & 12.16 & 0.79 & 5995 & 0.20 & 5.9 & syn & 2.11 & 1.41 & 2.08 & 0.15 & 2.8 & 0.87 & 1 & 1 \\ 
4246 & 11.80 & 2.19 & 5713 & 0.28 & 6.4 & syn & 0.93 & 1.03 & 0.94 & 1.22 & 1.2 & 2.04 & 1 & 0 \\ 
4251 & 12.12 & 1.96 & 5548 & 0.07 & 1.8 & syn & 0.90 & 0.94 & 0.90 & 1.28 & 3.5 & 1.97 & 1 & 0 \\ 
4255 & 12.86 & 1.99 & 4689 & 0.12 & \nodata & emp & 0.70 & 0.75 & 0.72 & 1.97 & 6.6 & 1.65 & 1 & 1 \\ 
4257 & 11.64 & 0.89 & 5467 & 0.01 & 3.0 & syn & 2.53 & 1.29 & 2.51 & 0.08 & 3.7 & 1.07 & 1 & 0 \\ 
4266 & 13.25 & 1.55 & 5005 & -0.10 & 1.8 & syn & 0.74 & 0.76 & 0.75 & 1.77 & 8.1 & 1.47 & 1 & 0 \\ 
4269 & 11.14 & 0.99 & 4948 & 0.07 & 2.5 & syn & 3.01 & 1.18 & 3.00 & 0.04 & 5.5 & 1.08 & 1 & 0 \\ 
4273 & 11.31 & -1.25 & 6135 & 0.10 & 5.7 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
4276 & 11.25 & 1.02 & 6221 & 0.12 & 8.2 & syn & 2.46 & 1.54 & 2.42 & 0.11 & 2.0 & 1.32 & 1 & 1 \\ 
4287 & 10.04 & 4.64 & 6298 & -0.02 & 8.3 & syn & 0.96 & 1.13 & 1.09 & 0.85 & 0.9 & 3.56 & 1 & 0 \\ 
4288 & 11.03 & 2.05 & 5943 & 0.09 & 3.7 & syn & 1.37 & 1.13 & 1.36 & 0.44 & 5.0 & 2.02 & 1 & 1 \\ 
4289 & 12.53 & 2.37 & 4390 & 0.11 & \nodata & emp & 0.71 & 0.70 & 0.69 & 2.11 & 10.6 & 2.47 & 1 & 0 \\ 
4292 & 11.28 & 2.50 & 5532 & 0.05 & 1.9 & syn & 1.04 & 0.92 & 1.04 & 0.82 & 10.1 & 2.33 & 1 & 1 \\ 
4296 & 11.56 & 2.39 & 5677 & -0.46 & 0.8 & syn & 0.95 & 0.79 & 0.95 & 0.92 & 13.5 & 2.80 & 1 & 1 \\ 
4298 & 12.16 & 1.13 & 6118 & -0.38 & 2.9 & syn & 1.48 & 1.02 & 1.46 & 0.32 & 6.6 & 1.41 & 1 & 0 \\ 
4301 & 11.64 & 1.83 & 6266 & -0.14 & 5.0 & syn & 1.12 & 1.10 & 1.12 & 0.78 & 1.9 & 1.90 & 1 & 1 \\ 
4302 & 12.34 & 1.05 & 6094 & -0.13 & 5.5 & syn & 1.45 & 1.11 & 1.44 & 0.37 & 5.0 & 1.08 & 1 & 1 \\ 
4304 & 12.63 & 1.00 & 5860 & 0.08 & 3.5 & syn & 1.36 & 1.09 & 1.35 & 0.44 & 6.1 & 0.91 & 1 & 1 \\ 
4312 & 12.38 & 1.11 & 5706 & -0.19 & 1.1 & syn & 1.40 & 0.93 & 1.39 & 0.34 & 11.2 & 1.20 & 1 & 1 \\ 
4318 & 11.46 & 1.72 & 6493 & -0.02 & 18.1 & syn & 1.27 & 1.25 & 1.27 & 0.61 & 1.0 & 1.81 & 1 & 1 \\ 
4323 & 12.14 & 0.98 & 6294 & -0.06 & 11.0 & syn & 1.70 & 1.28 & 1.68 & 0.26 & 2.9 & 1.29 & 1 & 0 \\ 
4329 & 10.81 & 1.57 & 6276 & 0.12 & 7.9 & syn & 1.92 & 1.40 & 1.92 & 0.20 & 2.4 & 2.43 & 1 & 1 \\ 
4332 & 13.16 & 1.58 & 4750 & 0.12 & \nodata & emp & 0.76 & 0.77 & 0.75 & 1.77 & 9.2 & 1.38 & 1 & 0 \\ 
4334 & 13.62 & 1.49 & 4561 & -0.43 & \nodata & emp & 0.68 & 0.63 & 0.63 & 2.52 & 12.0 & 1.69 & 1 & 1 \\ 
4335 & 12.69 & 1.32 & 5753 & -0.31 & 0.2 & syn & 1.01 & 0.86 & 1.00 & 0.84 & 10.3 & 1.42 & 1 & 1 \\ 
4343 & 12.20 & 1.80 & 5876 & -0.40 & 3.4 & syn & 1.14 & 0.87 & 0.92 & 1.04 & 6.9 & 1.27 & 1 & 0 \\ 
4356 & 13.45 & 1.59 & 4599 & 0.10 & \nodata & emp & 0.68 & 0.73 & 0.70 & 2.09 & 6.7 & 1.38 & 1 & 1 \\ 
4366 & 13.73 & 1.10 & 5272 & -0.12 & 0.4 & syn & 0.79 & 0.82 & 0.79 & 1.61 & 5.9 & 1.08 & 1 & 0 \\ 
4367 & 12.69 & 0.88 & 6291 & -0.06 & 7.7 & syn & 1.46 & 1.22 & 1.44 & 0.40 & 2.9 & 0.98 & 1 & 1 \\ 
4368 & 11.54 & 0.98 & 5941 & 0.09 & 4.0 & syn & 2.30 & 1.32 & 2.27 & 0.11 & 3.5 & 1.18 & 1 & 0 \\ 
4372 & 13.16 & 1.68 & 4646 & 0.14 & \nodata & emp & 0.72 & 0.75 & 0.73 & 1.91 & 8.3 & 1.44 & 1 & 1 \\ 
4374 & 12.46 & 1.75 & 5417 & 0.05 & 1.3 & syn & 0.88 & 0.90 & 0.88 & 1.33 & 5.0 & 1.72 & 1 & 1 \\ 
4380 & 11.75 & 1.36 & 6248 & -0.13 & 9.2 & syn & 1.48 & 1.18 & 1.47 & 0.37 & 3.5 & 1.68 & 1 & 0 \\ 
4382 & 12.93 & 0.84 & 6217 & -0.12 & 10.0 & syn & 1.37 & 1.14 & 1.36 & 0.45 & 3.8 & 0.91 & 1 & 1 \\ 
4383 & 12.42 & 1.64 & 5782 & 0.07 & 2.7 & syn & 0.92 & 0.99 & 0.93 & 1.24 & 1.6 & 1.55 & 1 & 1 \\ 
4385 & 13.90 & 1.00 & 5158 & 0.15 & 1.3 & syn & 0.83 & 0.86 & 0.83 & 1.49 & 5.6 & 0.97 & 1 & 0 \\ 
4399 & 10.35 & 4.77 & 5502 & -0.05 & 1.7 & syn & 0.83 & 0.89 & 0.84 & 1.51 & 2.9 & 4.74 & 1 & 1 \\ 
4400 & 12.22 & 1.58 & 5809 & 0.05 & 2.1 & syn & 1.05 & 1.01 & 1.05 & 0.88 & 4.4 & 1.56 & 1 & 1 \\ 
4407 & 9.78 & 3.21 & 6486 & -0.13 & 7.5 & syn & 1.50 & 1.26 & 1.49 & 0.38 & 2.4 & 4.05 & 1 & 1 \\ 
4409 & 11.08 & 2.25 & 5921 & 0.23 & 3.8 & syn & 1.22 & 1.14 & 1.21 & 0.63 & 3.4 & 2.12 & 1 & 1 \\ 
4411 & 12.06 & 1.61 & 6119 & -0.14 & 4.2 & syn & 1.07 & 1.04 & 1.06 & 0.86 & 2.6 & 1.65 & 1 & 1 \\ 
4418 & 14.23 & 0.34 & 5840 & 0.23 & 1.2 & syn & 2.00 & 1.25 & 1.75 & 0.22 & 4.3 & 0.48 & 1 & 0 \\ 
4419 & 12.27 & 3.83 & 4005 & -0.42 & \nodata & emp & 0.56 & 0.54 & 0.53 & 3.52 & 12.9 & 4.81 & 1 & 1 \\ 
4421 & 11.41 & 1.73 & 5986 & 0.05 & 5.2 & syn & 1.37 & 1.13 & 1.36 & 0.44 & 4.8 & 1.66 & 1 & 0 \\ 
4423 & 11.87 & 1.00 & 6281 & -0.14 & 9.2 & syn & 1.87 & 1.29 & 1.85 & 0.20 & 3.0 & 1.33 & 1 & 0 \\ 
4426 & 12.24 & 0.86 & 6158 & 0.08 & 7.6 & syn & 1.86 & 1.33 & 1.84 & 0.21 & 3.0 & 0.96 & 1 & 0 \\ 
4427 & 12.50 & 3.64 & 3778 & 0.09 & \nodata & emp & 0.56 & 0.54 & 0.55 & 3.18 & 11.2 & 4.43 & 1 & 1 \\ 
4430 & 13.64 & 1.17 & 5105 & 0.10 & 2.2 & syn & 0.79 & 0.84 & 0.80 & 1.64 & 4.7 & 1.15 & 1 & 0 \\ 
4431 & 11.23 & 1.41 & 6233 & -0.16 & 9.7 & syn & 1.79 & 1.25 & 1.77 & 0.22 & 3.4 & 1.93 & 1 & 1 \\ 
4435 & 12.22 & 0.85 & 6191 & 0.13 & 8.8 & syn & 1.87 & 1.37 & 1.86 & 0.21 & 2.7 & 1.05 & 1 & 0 \\ 
4441 & 12.82 & 1.87 & 4770 & 0.07 & \nodata & emp & 0.75 & 0.76 & 0.75 & 1.81 & 8.9 & 1.66 & 1 & 0 \\ 
4443 & 12.56 & 0.89 & 6383 & -0.04 & 9.6 & syn & 1.51 & 1.26 & 1.50 & 0.37 & 2.5 & 1.06 & 1 & 0 \\ 
4444 & 12.85 & 2.80 & 4041 & -0.47 & \nodata & emp & 0.58 & 0.54 & 0.53 & 3.55 & 13.5 & 3.55 & 1 & 1 \\ 
4446 & 10.59 & 1.86 & 5088 & -0.28 & 2.8 & syn & 2.04 & 0.86 & 2.03 & 0.10 & 13.7 & 1.89 & 1 & 0 \\ 
4447 & 12.61 & 2.19 & 4720 & -0.03 & \nodata & emp & 0.70 & 0.73 & 0.71 & 2.00 & 8.3 & 1.92 & 1 & 1 \\ 
4452 & 12.25 & 1.12 & 5793 & -0.29 & 1.8 & syn & 1.48 & 0.94 & 1.46 & 0.30 & 10.2 & 1.32 & 1 & 1 \\ 
4457 & 12.44 & 1.19 & 6075 & -0.19 & 7.5 & syn & 1.23 & 1.03 & 1.21 & 0.57 & 5.4 & 1.25 & 1 & 0 \\ 
4464 & 12.44 & 2.89 & 4223 & -0.25 & \nodata & emp & 0.63 & 0.61 & 0.60 & 2.73 & 12.0 & 3.31 & 1 & 1 \\ 
4469 & 12.19 & 2.52 & 4793 & 0.04 & \nodata & emp & 0.74 & 0.76 & 0.74 & 1.83 & 8.6 & 2.20 & 1 & 0 \\ 
4473 & 12.22 & 0.80 & 5952 & 0.04 & 5.8 & syn & 2.09 & 1.25 & 2.04 & 0.14 & 4.2 & 1.00 & 1 & 0 \\ 
4480 & 12.36 & 1.40 & 5683 & 0.35 & 1.3 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
4482 & 11.35 & 1.94 & 6275 & -0.02 & 6.5 & syn & 1.23 & 1.16 & 1.22 & 0.64 & 2.1 & 2.03 & 1 & 0 \\ 
4493 & 12.87 & 1.47 & 4726 & -0.15 & \nodata & emp & 0.95 & 0.80 & 0.86 & 1.22 & 18.8 & 1.86 & 1 & 0 \\ 
4505 & 12.36 & 1.20 & 6121 & -0.09 & 5.7 & syn & 1.26 & 1.09 & 1.25 & 0.55 & 4.2 & 1.28 & 1 & 0 \\ 
4508 & 12.93 & 1.27 & 4559 & 0.04 & \nodata & emp & 1.12 & 0.75 & 0.76 & 1.66 & 16.4 & 1.96 & 1 & 0 \\ 
4509 & 13.11 & 1.97 & 4237 & -0.22 & \nodata & emp & 0.68 & 0.63 & 0.63 & 2.51 & 13.1 & 2.37 & 1 & 1 \\ 
4517 & 11.72 & 3.55 & 4733 & -0.28 & 94.6 & syn & 0.66 & 0.67 & 0.66 & 2.34 & 8.5 & 3.47 & 5 & 0 \\ 
4521 & 12.97 & 2.22 & 4150 & -0.02 & \nodata & emp & 0.65 & 0.63 & 0.64 & 2.43 & 11.4 & 2.48 & 1 & 0 \\ 
4546 & 12.02 & 1.37 & 5956 & 0.05 & 3.4 & syn & 1.30 & 1.10 & 1.29 & 0.50 & 5.1 & 1.38 & 1 & 0 \\ 
4552 & 12.86 & 1.85 & 4667 & 0.07 & \nodata & emp & 0.76 & 0.75 & 0.74 & 1.84 & 10.5 & 1.69 & 1 & 0 \\ 
4556 & 10.35 & 1.87 & 5458 & -0.09 & 3.4 & syn & 2.17 & 1.11 & 2.15 & 0.11 & 6.2 & 2.24 & 1 & 0 \\ 
4557 & 12.29 & 1.03 & 5930 & 0.00 & 3.8 & syn & 1.54 & 1.13 & 1.53 & 0.32 & 5.6 & 1.06 & 1 & 0 \\ 
4561 & 12.65 & 0.69 & 6009 & 0.01 & 6.4 & syn & 1.93 & 1.23 & 1.88 & 0.18 & 4.3 & 0.90 & 1 & 0 \\ 
4567 & 12.33 & 0.86 & 6417 & -0.08 & 10.4 & syn & 1.75 & 1.32 & 1.74 & 0.25 & 2.6 & 1.23 & 1 & 0 \\ 
4575 & 11.82 & 0.90 & 6199 & 0.02 & 5.9 & syn & 2.14 & 1.40 & 2.11 & 0.15 & 2.5 & 1.13 & 1 & 0 \\ 
4580 & 11.43 & \nodata & 5915 & -0.21 & 1.9 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
4581 & 12.09 & 1.49 & 5879 & 0.08 & 2.1 & syn & 1.17 & 1.06 & 1.17 & 0.66 & 5.0 & 1.46 & 1 & 0 \\ 
4582 & 10.22 & 4.48 & 5688 & -0.17 & 2.1 & syn & 0.93 & 0.90 & 0.92 & 1.13 & 6.2 & 4.64 & 1 & 0 \\ 
4585 & 12.23 & 0.90 & 6158 & -0.11 & 9.5 & syn & 1.76 & 1.24 & 1.75 & 0.23 & 3.6 & 1.18 & 1 & 0 \\ 
4588 & 11.91 & 0.92 & 6284 & -0.10 & 7.3 & syn & 1.98 & 1.33 & 1.96 & 0.17 & 2.7 & 1.39 & 1 & 0 \\ 
4594 & 11.88 & 4.60 & 3982 & -0.38 & \nodata & emp & 0.56 & 0.55 & 0.54 & 3.34 & 13.0 & 5.87 & 1 & 0 \\ 
4595 & 13.40 & 1.38 & 4884 & -0.10 & 1.6 & syn & 0.77 & 0.75 & 0.74 & 1.78 & 10.5 & 1.43 & 1 & 0 \\ 
4601 & 12.43 & 1.06 & 6234 & 0.23 & 8.0 & syn & 1.37 & 1.28 & 1.35 & 0.52 & 1.6 & 1.09 & 1 & 0 \\ 
4603 & 12.37 & 1.02 & 6257 & 0.22 & 8.1 & syn & 1.44 & 1.30 & 1.43 & 0.43 & 2.1 & 1.13 & 1 & 0 \\ 
4605 & 12.11 & 0.82 & 6037 & 0.03 & 4.4 & syn & 2.09 & 1.28 & 2.06 & 0.14 & 3.8 & 0.98 & 1 & 0 \\ 
4606 & 13.07 & 1.83 & 4710 & 0.07 & \nodata & emp & 0.68 & 0.74 & 0.71 & 2.01 & 6.5 & 1.51 & 1 & 0 \\ 
4613 & 12.26 & 2.05 & 5484 & -0.09 & 0.8 & syn & 0.81 & 0.87 & 0.82 & 1.59 & 2.8 & 2.00 & 1 & 1 \\ 
4614 & 12.48 & 1.07 & 6070 & 0.10 & 5.6 & syn & 1.34 & 1.17 & 1.32 & 0.49 & 3.5 & 1.09 & 1 & 0 \\ 
4617 & 12.32 & 1.14 & 5925 & -0.12 & 2.0 & syn & 1.37 & 1.03 & 1.36 & 0.41 & 7.2 & 1.22 & 1 & 1 \\ 
4633 & 12.31 & 0.98 & 5976 & 0.11 & 5.9 & syn & 1.60 & 1.22 & 1.59 & 0.30 & 4.2 & 1.06 & 1 & 0 \\ 
4634 & 12.25 & \nodata & 6070 & 0.14 & 3.2 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
4637 & 9.23 & 3.34 & 6259 & -0.18 & 5.3 & syn & 1.88 & 1.24 & 1.87 & 0.19 & 3.6 & 4.57 & 1 & 0 \\ 
4640 & 12.47 & 0.84 & 6396 & -0.06 & 10.7 & syn & 1.69 & 1.30 & 1.67 & 0.28 & 2.6 & 1.10 & 1 & 0 \\ 
4647 & 11.77 & 0.86 & 5167 & 0.25 & 3.0 & syn & 2.52 & 1.32 & 2.52 & 0.08 & 4.0 & 1.07 & 1 & 0 \\ 
4650 & 13.23 & 1.96 & 4255 & -0.26 & \nodata & emp & 0.65 & 0.62 & 0.61 & 2.68 & 12.1 & 2.27 & 1 & 0 \\ 
4651 & 12.13 & 1.84 & 5726 & 0.05 & 2.7 & syn & 0.94 & 0.98 & 0.94 & 1.16 & 2.7 & 1.85 & 1 & 0 \\ 
4653 & 12.26 & 1.11 & 6167 & 0.02 & 7.6 & syn & 1.43 & 1.20 & 1.41 & 0.42 & 3.4 & 1.20 & 1 & 0 \\ 
4657 & 11.42 & 2.74 & 5363 & -0.02 & 0.4 & syn & 0.90 & 0.86 & 0.90 & 1.18 & 9.4 & 2.91 & 1 & 0 \\ 
4659 & 12.12 & 1.94 & 5632 & -0.00 & 1.4 & syn & 0.90 & 0.94 & 0.90 & 1.29 & 3.2 & 1.90 & 1 & 0 \\ 
4663 & 11.09 & 1.44 & 5545 & 0.31 & 3.6 & syn & 1.97 & 1.20 & 1.95 & 0.16 & 6.0 & 1.50 & 1 & 0 \\ 
4665 & 12.15 & 1.18 & 5672 & 0.01 & 2.3 & syn & 1.47 & 1.00 & 1.45 & 0.32 & 9.6 & 1.12 & 1 & 0 \\ 
4672 & 13.64 & 1.40 & 4796 & -0.16 & \nodata & emp & 0.69 & 0.71 & 0.69 & 2.09 & 8.3 & 1.18 & 1 & 0 \\ 
4674 & 12.03 & 1.54 & 5744 & 0.22 & 1.4 & syn & 1.17 & 1.06 & 1.17 & 0.66 & 5.6 & 1.51 & 1 & 0 \\ 
4686 & 10.67 & 1.76 & 5704 & 0.34 & 3.8 & syn & 1.92 & 1.24 & 1.90 & 0.18 & 5.1 & 1.84 & 1 & 0 \\ 
4693 & 11.86 & 1.39 & 5712 & -0.24 & 1.4 & syn & 1.43 & 0.92 & 1.42 & 0.32 & 11.4 & 1.61 & 1 & 0 \\ 
4699 & 11.62 & 1.73 & 6152 & 0.07 & 4.9 & syn & 1.21 & 1.16 & 1.20 & 0.66 & 2.2 & 1.74 & 1 & 0 \\ 
4706 & 12.20 & \nodata & 5969 & -0.27 & 2.5 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
4715 & 12.54 & 0.71 & 6142 & -0.08 & 8.3 & syn & 1.99 & 1.24 & 1.95 & 0.17 & 3.8 & 0.91 & 1 & 0 \\ 
4716 & 10.98 & 2.06 & 6066 & 0.08 & 4.7 & syn & 1.38 & 1.17 & 1.37 & 0.45 & 3.8 & 2.19 & 1 & 0 \\ 
4717 & 13.89 & 0.85 & 5664 & -0.27 & 0.3 & syn & 0.93 & 0.85 & 0.91 & 1.09 & 8.5 & 0.90 & 1 & 0 \\ 
4721 & 13.74 & 1.35 & 4685 & -0.12 & \nodata & emp & 0.69 & 0.70 & 0.69 & 2.13 & 8.8 & 1.32 & 1 & 0 \\ 
4725 & 11.19 & 4.04 & 4698 & -0.06 & \nodata & emp & 0.74 & 0.73 & 0.72 & 1.93 & 10.5 & 3.91 & 1 & 1 \\ 
4735 & 12.70 & 2.01 & 4907 & -0.12 & 0.4 & syn & 0.73 & 0.74 & 0.73 & 1.89 & 8.6 & 2.04 & 1 & 0 \\ 
4742 & 12.49 & 2.76 & 4427 & -0.59 & \nodata & emp & 0.63 & 0.59 & 0.58 & 2.97 & 13.1 & 3.19 & 1 & 1 \\ 
4744 & 12.27 & 1.12 & 5760 & 0.27 & 3.1 & syn & 1.44 & 1.15 & 1.43 & 0.39 & 5.7 & 1.03 & 1 & 0 \\ 
4745 & 13.81 & 1.27 & 4693 & 0.08 & \nodata & emp & 0.70 & 0.74 & 0.72 & 1.96 & 7.5 & 1.09 & 1 & 0 \\ 
4746 & 12.27 & 1.69 & 4944 & 0.08 & 4.6 & syn & 1.12 & 0.80 & 0.83 & 1.34 & 14.1 & 2.27 & 1 & 0 \\ 
4762 & 13.21 & 1.92 & 4366 & -0.22 & \nodata & emp & 0.65 & 0.64 & 0.63 & 2.53 & 11.0 & 2.10 & 1 & 0 \\ 
4763 & 12.52 & 0.79 & 5676 & 0.15 & 3.6 & syn & 1.84 & 1.15 & 1.81 & 0.19 & 6.5 & 0.85 & 1 & 0 \\ 
4765 & 12.10 & 1.28 & 6227 & 0.15 & 6.8 & syn & 1.30 & 1.23 & 1.30 & 0.55 & 2.0 & 1.33 & 1 & 0 \\ 
4771 & 12.72 & 0.92 & 6339 & -0.05 & 10.6 & syn & 1.35 & 1.20 & 1.34 & 0.49 & 2.5 & 1.05 & 1 & 0 \\ 
4773 & 12.04 & 0.86 & 6107 & -0.28 & 6.2 & syn & 2.10 & 1.19 & 2.08 & 0.13 & 4.2 & 1.08 & 1 & 0 \\ 
4774 & 12.04 & 2.36 & 5249 & 0.02 & 1.5 & syn & 0.80 & 0.85 & 0.81 & 1.60 & 4.2 & 2.30 & 1 & 1 \\ 
4775 & 11.07 & 1.40 & 5160 & 0.44 & 2.9 & syn & 2.12 & 1.21 & 2.11 & 0.13 & 6.4 & 1.18 & 1 & 0 \\ 
4778 & 11.67 & 1.42 & 5645 & -0.24 & 1.6 & syn & 1.53 & 0.92 & 1.51 & 0.26 & 11.5 & 1.71 & 1 & 0 \\ 
4784 & 13.02 & 1.95 & 4356 & 0.03 & \nodata & emp & 0.70 & 0.68 & 0.67 & 2.21 & 10.9 & 2.06 & 1 & 0 \\ 
4792 & 12.83 & 1.25 & 5911 & 0.07 & 2.7 & syn & 0.99 & 1.04 & 0.99 & 1.05 & 1.7 & 1.17 & 1 & 0 \\ 
4808 & 12.51 & 3.14 & 3850 & 0.44 & \nodata & emp & 0.63 & 0.60 & 0.62 & 2.44 & 9.6 & 3.27 & 1 & 0 \\ 
4809 & 12.87 & 1.61 & 4172 & -0.02 & \nodata & emp & 0.95 & 0.00 & 0.00 & 0.00 & 0.0 & 2.60 & 5 & 0 \\ 
4811 & 12.14 & 0.87 & 5555 & 0.05 & 2.7 & syn & 2.02 & 1.13 & 2.00 & 0.14 & 6.4 & 0.99 & 1 & 0 \\ 
4822 & 12.05 & 1.09 & 5801 & -0.02 & 2.6 & syn & 1.64 & 1.08 & 1.62 & 0.25 & 7.3 & 1.14 & 1 & 0 \\ 
4829 & 12.80 & 1.00 & 6042 & -0.05 & 3.1 & syn & 1.24 & 1.08 & 1.23 & 0.57 & 4.6 & 0.96 & 1 & 0 \\ 
4833 & 12.10 & 1.17 & 5714 & 0.01 & 2.3 & syn & 1.51 & 1.03 & 1.49 & 0.31 & 8.7 & 1.19 & 1 & 0 \\ 
4834 & 10.96 & 1.29 & 5012 & 0.40 & 3.1 & syn & 2.48 & 1.29 & 2.48 & 0.08 & 4.8 & 1.23 & 1 & 0 \\ 
4838 & 12.47 & 2.52 & 4260 & 0.15 & \nodata & emp & 0.70 & 0.69 & 0.68 & 2.17 & 11.4 & 2.72 & 1 & 0 \\ 
4839 & 12.03 & 1.26 & 6115 & -0.09 & 3.3 & syn & 1.43 & 1.13 & 1.41 & 0.39 & 4.5 & 1.33 & 1 & 0 \\ 
4841 & 13.67 & 1.37 & 4716 & 0.03 & \nodata & emp & 0.71 & 0.74 & 0.72 & 1.96 & 8.0 & 1.19 & 1 & 0 \\ 
4848 & 13.00 & 2.10 & 4073 & 0.20 & \nodata & emp & 0.69 & 0.64 & 0.67 & 2.12 & 12.5 & 2.40 & 1 & 0 \\ 
4850 & 12.53 & 1.57 & 5605 & 0.08 & 1.4 & syn & 0.93 & 0.96 & 0.93 & 1.19 & 3.6 & 1.50 & 1 & 0 \\ 
4859 & 13.28 & 1.69 & 4583 & -0.06 & \nodata & emp & 0.69 & 0.70 & 0.69 & 2.14 & 9.2 & 1.71 & 1 & 0 \\ 
4862 & 13.06 & 2.02 & 4260 & -0.14 & \nodata & emp & 0.67 & 0.64 & 0.64 & 2.45 & 12.2 & 2.31 & 1 & 0 \\ 
4864 & 11.66 & 0.94 & 5763 & -0.23 & 2.9 & syn & 2.31 & 1.17 & 2.29 & 0.10 & 4.6 & 1.33 & 1 & 0 \\ 
4875 & 12.64 & 3.37 & 3781 & 0.02 & \nodata & emp & 0.57 & 0.55 & 0.56 & 3.11 & 11.9 & 4.41 & 1 & 0 \\ 
4881 & 12.39 & 1.04 & 6280 & -0.02 & 9.4 & syn & 1.40 & 1.21 & 1.39 & 0.45 & 2.7 & 1.12 & 1 & 0 \\ 
4887 & 11.55 & 1.02 & 5846 & 0.02 & 4.8 & syn & 2.22 & 1.25 & 2.19 & 0.12 & 4.2 & 1.18 & 1 & 0 \\ 
4892 & 12.58 & 0.59 & 5568 & -0.37 & 2.6 & syn & 2.46 & 1.12 & 2.44 & 0.08 & 4.9 & 0.84 & 1 & 0 \\ 
4898 & 14.14 & 0.53 & 5799 & -0.12 & 0.3 & syn & 1.31 & 0.96 & 1.26 & 0.47 & 9.2 & 0.56 & 1 & 0 \\ 
4902 & 12.83 & 0.27 & 4822 & 0.19 & 3.6 & syn & 5.22 & 1.37 & 5.04 & 0.01 & 3.4 & 0.32 & 1 & 0 \\ 
4907 & 12.38 & 1.24 & 5961 & 0.05 & 2.9 & syn & 1.22 & 1.08 & 1.21 & 0.60 & 4.6 & 1.21 & 1 & 0 \\ 
4926 & 13.29 & 1.64 & 4683 & -0.03 & \nodata & emp & 0.71 & 0.72 & 0.71 & 2.03 & 8.6 & 1.48 & 1 & 0 \\ 
4928 & 12.31 & 3.89 & 3640 & 0.27 & \nodata & emp & 0.57 & 0.55 & 0.56 & 3.04 & 11.6 & 5.05 & 1 & 1 \\ 
4941 & 14.42 & 0.29 & 5067 & -0.17 & 4.5 & syn & 2.35 & 0.93 & 2.22 & 0.08 & 11.1 & 0.34 & 1 & 0 \\ 
4961 & 12.96 & 1.71 & 4587 & 0.15 & \nodata & emp & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
4977 & 13.05 & 1.47 & 4414 & 0.04 & \nodata & emp & 0.91 & 0.76 & 0.78 & 1.56 & 18.4 & 1.98 & 1 & 0 \\ 
4978 & 13.51 & 1.09 & 5550 & 0.18 & 1.8 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
5018 & 13.53 & 1.00 & 5485 & 0.39 & 1.5 & syn & 0.93 & 1.01 & 0.94 & 1.19 & 2.4 & 0.87 & 1 & 0 \\ 
5021 & 13.58 & 0.93 & 5814 & 0.13 & 1.0 & syn & 0.96 & 1.03 & 0.97 & 1.10 & 1.7 & 0.88 & 1 & 0 \\ 
5039 & 13.81 & 1.38 & 4744 & 0.04 & \nodata & emp & 0.65 & 0.73 & 0.70 & 2.09 & 5.3 & 1.09 & 1 & 0 \\ 
5048 & 11.20 & 0.68 & 4922 & 0.07 & 3.0 & syn & 4.32 & 1.32 & 4.30 & 0.02 & 3.6 & 0.76 & 1 & 0 \\ 
5057 & 10.35 & 0.89 & 5006 & 0.01 & 3.0 & syn & 4.85 & 1.44 & 4.85 & 0.01 & 2.5 & 1.07 & 1 & 0 \\ 
5084 & 13.92 & 0.46 & 5576 & 0.23 & 1.9 & syn & 1.72 & 1.10 & 1.62 & 0.25 & 7.9 & 0.46 & 1 & 0 \\ 
5085 & 14.19 & 0.79 & 5659 & -0.05 & 0.7 & syn & 0.87 & 0.92 & 0.88 & 1.32 & 3.1 & 0.74 & 1 & 0 \\ 
5107 & 11.39 & 0.39 & 4935 & -0.13 & 3.7 & syn & 7.00 & 1.48 & 6.92 & 0.00 & 2.1 & 0.49 & 1 & 0 \\ 
5119 & 10.35 & 0.66 & 4947 & 0.03 & 3.9 & syn & 6.83 & 1.58 & 6.71 & 0.01 & 1.9 & 0.87 & 1 & 0 \\ 
5124 & 13.97 & 0.96 & 5302 & 0.03 & 0.8 & syn & 0.81 & 0.86 & 0.82 & 1.53 & 4.1 & 0.83 & 1 & 0 \\ 
5135 & 13.60 & 0.82 & 5197 & 0.06 & 3.0 & syn & 1.14 & 0.86 & 1.10 & 0.63 & 17.8 & 1.12 & 1 & 0 \\ 
5155 & 13.85 & 0.67 & 5728 & -0.01 & 1.3 & syn & 1.19 & 0.97 & 1.15 & 0.61 & 8.7 & 0.64 & 1 & 0 \\ 
5159 & 13.33 & 0.84 & 6124 & 0.14 & 4.4 & syn & 1.17 & 1.16 & 1.16 & 0.73 & 1.6 & 0.83 & 1 & 0 \\ 
5192 & 12.68 & 2.00 & 4916 & 0.01 & 2.4 & syn & 0.74 & 0.77 & 0.75 & 1.78 & 7.4 & 1.97 & 1 & 0 \\ 
5198 & 13.88 & 0.99 & 5386 & 0.06 & 0.8 & syn & 0.81 & 0.89 & 0.83 & 1.54 & 2.8 & 0.94 & 1 & 0 \\ 
5216 & 13.78 & 0.91 & 5603 & -0.01 & 0.8 & syn & 0.91 & 0.93 & 0.91 & 1.22 & 4.2 & 0.91 & 1 & 0 \\ 
5236 & 11.72 & 1.95 & 6100 & -0.19 & 3.0 & syn & 1.04 & 1.02 & 1.04 & 0.91 & 2.9 & 2.03 & 1 & 0 \\ 
5241 & 13.55 & 0.54 & 6104 & -0.27 & 2.7 & syn & 1.66 & 1.09 & 1.60 & 0.26 & 5.6 & 0.67 & 1 & 0 \\ 
5247 & 13.30 & 0.64 & 5946 & 0.11 & 2.9 & syn & 1.53 & 1.18 & 1.52 & 0.33 & 4.6 & 0.63 & 1 & 0 \\ 
5269 & 13.59 & 1.23 & 5374 & -0.01 & 1.6 & syn & 0.75 & 0.86 & 0.81 & 1.62 & 2.9 & 1.11 & 1 & 0 \\ 
5278 & 13.94 & 0.82 & 5495 & 0.08 & 71.6 & syn & 0.96 & 0.93 & 0.94 & 1.09 & 6.4 & 0.87 & 1 & 0 \\ 
5284 & 12.93 & 0.92 & 5665 & 0.40 & 1.6 & syn & 1.31 & 1.12 & 1.30 & 0.51 & 5.9 & 0.77 & 1 & 0 \\ 
5290 & 14.08 & 0.84 & 5516 & 0.08 & 0.9 & syn & 0.86 & 0.93 & 0.88 & 1.37 & 2.9 & 0.74 & 1 & 0 \\ 
5324 & 11.62 & 0.60 & 4970 & -0.12 & 3.5 & syn & 3.97 & 1.19 & 3.94 & 0.02 & 4.4 & 0.61 & 1 & 0 \\ 
5341 & 11.24 & 2.29 & 6320 & 0.09 & 17.9 & syn & 1.09 & 1.15 & 1.10 & 0.86 & 0.5 & 2.19 & 3 & 1 \\ 
5375 & 11.60 & 0.42 & 5019 & -0.19 & 5.4 & syn & 5.91 & 1.44 & 5.83 & 0.01 & 2.2 & 0.69 & 1 & 0 \\ 
5379 & 10.48 & 0.95 & 5047 & 0.02 & 3.3 & syn & 4.21 & 1.42 & 4.23 & 0.02 & 2.6 & 1.04 & 1 & 0 \\ 
5380 & 13.91 & 0.87 & 5580 & -0.20 & 0.0 & syn & 0.90 & 0.86 & 0.88 & 1.22 & 7.4 & 0.92 & 1 & 0 \\ 
5387 & 11.86 & 3.57 & 4152 & 0.13 & \nodata & emp & 0.67 & 0.65 & 0.66 & 2.20 & 11.1 & 3.88 & 1 & 0 \\ 
5393 & 11.09 & 0.61 & 4810 & 0.01 & 3.6 & syn & 5.19 & 1.21 & 5.14 & 0.01 & 4.8 & 0.66 & 1 & 0 \\ 
5423 & 13.42 & 0.79 & 5724 & 0.34 & 2.5 & syn & 1.22 & 1.10 & 1.21 & 0.61 & 5.0 & 0.67 & 1 & 0 \\ 
5475 & 11.66 & 1.42 & 5948 & -0.07 & 3.1 & syn & 1.49 & 1.08 & 1.48 & 0.33 & 6.2 & 1.49 & 1 & 1 \\ 
5499 & 13.26 & 1.19 & 4884 & -0.18 & 3.8 & syn & 0.95 & 0.77 & 0.88 & 1.12 & 18.3 & 1.57 & 1 & 0 \\ 
5546 & 13.49 & 0.82 & 6232 & -0.04 & 5.0 & syn & 1.10 & 1.12 & 1.10 & 0.83 & 1.3 & 0.82 & 1 & 0 \\ 
5567 & 13.14 & 0.53 & 5581 & 0.16 & 3.4 & syn & 2.10 & 1.20 & 2.05 & 0.14 & 5.5 & 0.81 & 1 & 0 \\ 
5579 & 13.38 & 1.65 & 4764 & -0.19 & \nodata & emp & 0.66 & 0.69 & 0.67 & 2.25 & 7.2 & 1.40 & 1 & 0 \\ 
5592 & 13.52 & 0.68 & 6124 & -0.01 & 5.7 & syn & 1.32 & 1.14 & 1.30 & 0.51 & 3.6 & 0.72 & 1 & 0 \\ 
5597 & 11.76 & 2.54 & 5056 & 0.45 & 3.1 & syn & 0.86 & 0.91 & 0.86 & 1.40 & 5.5 & 2.03 & 1 & 1 \\ 
5612 & 13.97 & 0.84 & 5199 & 0.03 & 0.5 & syn & 0.95 & 0.83 & 0.91 & 1.07 & 14.1 & 0.95 & 1 & 0 \\ 
5613 & 13.78 & 0.92 & 5559 & 0.16 & 49.0 & syn & 0.90 & 0.96 & 0.91 & 1.26 & 2.8 & 0.71 & 1 & 0 \\ 
5622 & 13.89 & 0.96 & 5241 & 0.06 & 0.7 & syn & 0.84 & 0.86 & 0.84 & 1.42 & 6.5 & 0.92 & 1 & 0 \\ 
5625 & 13.88 & 0.17 & 4867 & -0.23 & 3.1 & syn & 4.92 & 1.00 & 4.39 & 0.01 & 7.9 & 0.24 & 1 & 0 \\ 
5626 & 13.94 & 0.64 & 5990 & -0.00 & 2.3 & syn & 1.16 & 1.06 & 1.14 & 0.70 & 3.9 & 0.60 & 1 & 0 \\ 
5628 & 13.40 & 1.72 & 4523 & -0.32 & \nodata & emp & 0.65 & 0.64 & 0.63 & 2.55 & 10.3 & 1.81 & 1 & 0 \\ 
5645 & 14.22 & 0.85 & 5457 & -0.03 & 0.5 & syn & 0.81 & 0.88 & 0.83 & 1.51 & 3.2 & 0.79 & 1 & 0 \\ 
5653 & 13.16 & 1.81 & 4769 & -0.03 & \nodata & emp & 0.67 & 0.72 & 0.70 & 2.10 & 6.0 & 1.49 & 1 & 0 \\ 
5663 & 11.79 & 1.69 & 6026 & 0.09 & 4.0 & syn & 1.16 & 1.11 & 1.15 & 0.72 & 2.7 & 1.66 & 1 & 1 \\ 
5683 & 12.43 & 1.76 & 5236 & -0.65 & 42.4 & syn & 0.91 & 0.72 & 0.87 & 1.11 & 18.4 & 0.91 & 5 & 0 \\ 
5689 & 13.45 & 1.47 & 4512 & 0.11 & \nodata & emp & 0.74 & 0.73 & 0.71 & 1.97 & 10.6 & 1.54 & 1 & 0 \\ 
5692 & 11.18 & 5.22 & 3967 & 0.01 & \nodata & emp & 0.65 & 0.62 & 0.63 & 2.39 & 13.5 & 6.75 & 1 & 1 \\ 
5702 & 13.94 & 0.87 & 5828 & 0.04 & 2.8 & syn & 0.86 & 0.97 & 0.90 & 1.32 & 1.2 & 0.79 & 1 & 0 \\ 
5704 & 11.41 & 3.40 & 4912 & -0.31 & 1.3 & syn & 0.77 & 0.71 & 0.71 & 1.90 & 12.8 & 3.77 & 1 & 0 \\ 
5706 & 14.23 & 0.54 & 5758 & 0.20 & 1.2 & syn & 1.24 & 1.07 & 1.20 & 0.60 & 5.7 & 0.52 & 1 & 0 \\ 
5708 & 10.90 & 1.88 & 5662 & 0.11 & 7.2 & syn & 1.64 & 1.07 & 1.62 & 0.25 & 8.1 & 2.23 & 1 & 0 \\ 
5782 & 9.38 & 1.83 & 5032 & 0.10 & 2.9 & syn & 3.59 & 1.38 & 3.60 & 0.03 & 3.0 & 2.19 & 1 & 0 \\ 
5790 & 13.31 & 1.47 & 4739 & 0.14 & \nodata & emp & 0.76 & 0.77 & 0.75 & 1.77 & 9.1 & 1.28 & 1 & 0 \\ 
5792 & 12.55 & \nodata & 4724 & -0.03 & \nodata & emp & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
5798 & 13.64 & 1.33 & 4969 & 0.03 & 1.5 & syn & 0.71 & 0.79 & 0.75 & 1.82 & 5.1 & 1.21 & 1 & 0 \\ 
5826 & 13.10 & 2.53 & 4021 & -0.46 & \nodata & emp & 0.58 & 0.54 & 0.53 & 3.57 & 13.4 & 3.25 & 4 & 0 \\ 
5833 & 11.67 & 1.44 & 6007 & -0.09 & 4.2 & syn & 1.44 & 1.09 & 1.42 & 0.37 & 5.6 & 1.48 & 1 & 0 \\ 
5837 & 13.74 & 0.77 & 5732 & 0.11 & 2.2 & syn & 1.08 & 1.01 & 1.06 & 0.83 & 5.2 & 0.75 & 1 & 0 \\ 
5850 & 13.30 & 0.96 & 5623 & 0.09 & 1.8 & syn & 1.08 & 0.96 & 1.06 & 0.80 & 7.8 & 1.05 & 1 & 0 \\ 
5852 & 13.97 & 0.48 & 5654 & 0.01 & 0.9 & syn & 1.58 & 1.02 & 1.53 & 0.27 & 9.2 & 0.51 & 1 & 0 \\ 
5855 & 13.53 & 0.95 & 5708 & 0.14 & 1.3 & syn & 0.96 & 1.01 & 0.96 & 1.11 & 2.5 & 0.92 & 1 & 0 \\ 
5869 & 13.21 & -0.24 & 4768 & -0.25 & 3.3 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
5877 & 13.96 & 0.95 & 5523 & 0.06 & 0.4 & syn & 0.80 & 0.91 & 0.84 & 1.53 & 1.8 & 0.86 & 1 & 0 \\ 
5888 & 13.73 & 1.19 & 5175 & -0.08 & 0.9 & syn & 0.74 & 0.80 & 0.77 & 1.71 & 5.4 & 1.12 & 1 & 0 \\ 
5900 & 11.94 & 1.29 & 6295 & -0.11 & 12.9 & syn & 1.39 & 1.18 & 1.38 & 0.45 & 3.1 & 1.18 & 1 & 0 \\ 
5909 & 13.68 & 1.38 & 4607 & 0.12 & \nodata & emp & 0.71 & 0.74 & 0.71 & 1.99 & 7.9 & 1.18 & 1 & 0 \\ 
5924 & 13.56 & 0.74 & 5090 & 0.03 & 2.2 & syn & 1.79 & 0.83 & 0.84 & 1.10 & 13.4 & 1.22 & 1 & 0 \\ 
5929 & 13.09 & 1.10 & 5504 & -0.07 & 1.3 & syn & 1.04 & 0.87 & 1.03 & 0.78 & 12.7 & 1.08 & 1 & 0 \\ 
5932 & 14.07 & 0.34 & 5421 & -0.18 & 1.2 & syn & 2.21 & 1.05 & 2.10 & 0.11 & 7.1 & 0.53 & 1 & 0 \\ 
5935 & 13.57 & 1.41 & 4741 & 0.06 & \nodata & emp & 0.71 & 0.75 & 0.73 & 1.93 & 7.4 & 1.19 & 1 & 0 \\ 
5949 & 11.82 & 1.94 & 5806 & -0.23 & 0.6 & syn & 1.03 & 0.90 & 1.02 & 0.85 & 8.2 & 2.09 & 1 & 0 \\ 
5953 & 13.51 & 1.15 & 5097 & 0.33 & 1.7 & syn & 0.85 & 0.89 & 0.85 & 1.43 & 5.6 & 1.08 & 1 & 0 \\ 
5965 & 13.57 & 1.58 & 4582 & -0.40 & \nodata & emp & 0.65 & 0.63 & 0.62 & 2.58 & 10.7 & 1.68 & 1 & 0 \\ 
5971 & 11.44 & 2.51 & 4740 & -0.42 & 6.7 & syn & 1.05 & 0.00 & 0.00 & 0.00 & 0.0 & 4.34 & 4 & 0 \\ 
5974 & 11.20 & 3.98 & 4707 & 0.10 & \nodata & emp & 0.74 & 0.76 & 0.74 & 1.85 & 8.9 & 3.54 & 1 & 0 \\ 
6102 & 9.83 & 1.62 & 6323 & -0.13 & 11.8 & syn & 2.96 & 1.49 & 2.93 & 0.06 & 2.0 & 1.14 & 1 & 0 \\ 
6130 & 12.73 & 1.89 & 4634 & -0.77 & 116.9 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 5 & 0 \\ 
6166 & 12.07 & 2.44 & 5144 & 0.18 & 3.0 & syn & 0.78 & 0.86 & 0.82 & 1.54 & 4.9 & 2.32 & 1 & 1 \\ 
6186 & 11.64 & 2.95 & 4939 & 0.10 & 9.3 & syn & 0.80 & 0.80 & 0.80 & 1.56 & 9.6 & 3.01 & 1 & 1 \\ 
6195 & 12.97 & 1.80 & 4728 & 0.13 & 71.9 & syn & 0.73 & 0.77 & 0.74 & 1.85 & 7.9 & 0.83 & 3 & 0 \\ 
6202 & 10.11 & 3.07 & 5739 & -0.42 & 2.1 & syn & 1.42 & 0.87 & 1.41 & 0.30 & 12.5 & 3.81 & 1 & 0 \\ 
6246 & 10.46 & 3.40 & 6057 & 0.13 & 15.4 & syn & 1.05 & 1.11 & 1.06 & 0.92 & 1.1 & 3.31 & 1 & 1 \\ 
6299 & 12.22 & 1.89 & 5536 & 0.14 & 1.5 & syn & 0.90 & 0.96 & 0.90 & 1.31 & 2.7 & 1.82 & 1 & 1 \\ 
6384 & 14.22 & 0.71 & 5816 & 0.21 & 1.1 & syn & 0.96 & 1.06 & 1.01 & 1.00 & 1.9 & 0.62 & 1 & 0 \\ 
6401 & 12.44 & 0.65 & 6520 & -0.20 & 64.1 & syn & 2.20 & 1.39 & 2.15 & 0.14 & 2.2 & 0.69 & 3 & 1 \\ 
6425 & 12.63 & 0.93 & 5756 & 0.08 & 0.8 & syn & 1.48 & 1.07 & 1.46 & 0.34 & 7.6 & 0.98 & 1 & 0 \\ 
6676 & 12.78 & 0.56 & 6489 & -0.19 & 26.5 & syn & 2.16 & 1.39 & 2.12 & 0.14 & 2.3 & 0.86 & 1 & 0 \\ 
6734 & 13.59 & 0.98 & 5434 & 0.40 & 2.1 & syn & 0.93 & 1.00 & 0.94 & 1.20 & 2.8 & 0.93 & 1 & 0 \\ 
6745 & 13.95 & 0.49 & 6538 & 0.13 & 6.8 & syn & 1.44 & 1.34 & 1.41 & 0.46 & 1.2 & 0.54 & 1 & 0 \\ 
6759 & 13.15 & 0.63 & 5504 & 0.36 & 2.5 & syn & 1.76 & 1.13 & 1.72 & 0.22 & 7.6 & 0.61 & 1 & 0 \\ 
6786 & 14.14 & 0.71 & 5805 & -0.02 & 1.6 & syn & 0.98 & 0.98 & 0.97 & 1.05 & 3.3 & 0.73 & 1 & 0 \\ 
6860 & 10.69 & 5.81 & 4307 & 0.15 & \nodata & emp & 0.68 & 0.69 & 0.68 & 2.20 & 10.0 & 5.95 & 1 & 1 \\ 
6863 & 12.03 & 7.86 & 3395 & -0.19 & \nodata & emp & 0.37 & 0.35 & 0.37 & 6.84 & 10.7 & 16.39 & 1 & 0 \\ 
6883 & 13.36 & 1.10 & 5471 & 0.05 & 1.8 & syn & 0.92 & 0.91 & 0.91 & 1.17 & 6.2 & 0.95 & 1 & 0 \\ 
6927 & 12.71 & 1.99 & 4929 & 0.13 & 1.9 & syn & 0.73 & 0.80 & 0.76 & 1.78 & 5.3 & 1.85 & 1 & 0 \\ 
6971 & 12.57 & 2.33 & 4874 & -0.20 & 1.7 & syn & 0.68 & 0.71 & 0.69 & 2.14 & 6.9 & 2.28 & 1 & 0 \\ 
6981 & 13.11 & 0.52 & 5942 & -0.37 & 3.9 & syn & 2.08 & 1.10 & 2.04 & 0.13 & 5.4 & 1.04 & 1 & 0 \\ 
7016 & 11.85 & 1.84 & 5775 & 0.24 & 1.6 & syn & 1.07 & 1.08 & 1.07 & 0.88 & 2.9 & 1.66 & 1 & 0 \\ 
7040 & 13.43 & 0.63 & 6137 & -0.39 & 7.8 & syn & 1.50 & 1.03 & 1.47 & 0.32 & 6.4 & 0.58 & 1 & 0 \\ 
7073 & 11.77 & 1.40 & 6135 & 0.01 & 6.5 & syn & 1.40 & 1.18 & 1.39 & 0.43 & 3.6 & 1.53 & 1 & 1 \\ 
7136 & 13.89 & 0.88 & 5522 & 0.34 & 1.2 & syn & 0.90 & 1.00 & 0.93 & 1.25 & 2.0 & 0.73 & 1 & 0 \\ 
7179 & 11.16 & 2.52 & 5726 & 0.03 & 1.7 & syn & 1.08 & 0.97 & 1.07 & 0.78 & 7.0 & 2.35 & 1 & 0 \\ 
7223 & 12.79 & 1.02 & 5549 & -0.37 & 3.0 & syn & 1.33 & 0.82 & 1.30 & 0.36 & 16.5 & 1.73 & 1 & 0 \\ 
7235 & 13.02 & 0.93 & 5418 & -0.02 & 0.8 & syn & 2.05 & 0.88 & 1.02 & 0.71 & 12.6 & 1.35 & 1 & 0 \\ 
7345 & 13.53 & 0.86 & 5700 & -0.05 & 1.8 & syn & 1.06 & 0.94 & 1.05 & 0.80 & 8.2 & 0.93 & 1 & 0 \\ 
7375 & 11.89 & 3.22 & 4063 & -0.04 & \nodata & emp & 0.72 & 0.65 & 0.66 & 2.23 & 14.9 & 4.49 & 1 & 1 \\ 
7566 & 13.42 & 0.75 & 5727 & 0.23 & 2.5 & syn & 1.32 & 1.09 & 1.30 & 0.49 & 6.5 & 0.69 & 1 & 0 \\ 
7587 & 9.98 & 4.52 & 5763 & 0.03 & 2.9 & syn & 1.04 & 0.99 & 1.03 & 0.90 & 5.0 & 4.76 & 1 & 0 \\ 
7599 & 13.90 & 0.78 & 5792 & 0.24 & 2.2 & syn & 0.98 & 1.06 & 1.01 & 1.03 & 1.7 & 0.75 & 1 & 0 \\ 
7605 & 13.29 & \nodata & 5942 & -0.07 & 3.9 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 1 & 0 \\ 
7923 & 10.48 & 4.82 & 5016 & -0.34 & 1.2 & syn & 0.83 & 0.73 & 0.80 & 1.42 & 17.1 & 5.64 & 1 & 1 \\ 
8061 & 7.38 & 15.23 & 5983 & 0.03 & 10.9 & syn & 0.98 & 1.04 & 0.99 & 1.08 & 1.3 & 14.98 & 1 & 0 \\ 
\nodata & 9.59 & 8.06 & 5067 & 0.00 & 2.0 & syn & 0.74 & 0.80 & 0.77 & 1.73 & 5.4 & 7.73 & 1 & 0 \\ 
\nodata & 12.94 & 0.87 & 5639 & 0.14 & 2.5 & syn & 1.39 & 1.03 & 1.36 & 0.40 & 9.1 & 1.18 & 1 & 0 \\ 
\nodata & 14.49 & 0.62 & 5709 & -0.36 & 0.6 & syn & 0.97 & 0.84 & 0.93 & 1.00 & 9.9 & 0.68 & 1 & 0 \\ 
\nodata & 13.48 & 1.01 & 5566 & -0.10 & 0.6 & syn & 0.94 & 0.89 & 0.93 & 1.08 & 8.0 & 1.00 & 1 & 0 \\ 

==> val_fitd.tex <==
\newcommand{\fitd}[1]{%%
\IfEqCase{#1}{%
{sn-m-R0}{2.49 \pm 0.02}%
{sn-m-alpha-mass}{0.25 \pm 0.03}%
{sn-m-alpha-met}{0.00 \pm 0.00}%
{sn-m-alpha-age}{0.00 \pm 0.00}%
{se-m-R0}{1.35 \pm 0.02}%
{se-m-alpha-mass}{0.03 \pm 0.03}%
{se-m-alpha-met}{0.00 \pm 0.00}%
{se-m-alpha-age}{0.00 \pm 0.00}%
{sn-mm-R0}{2.49 \pm 0.12}%
{sn-mm-alpha-mass}{0.25 \pm 0.04}%
{sn-mm-alpha-met}{-0.00 \pm 0.02}%
{sn-mm-alpha-age}{0.00 \pm 0.00}%
{se-mm-R0}{1.35 \pm 0.11}%
{se-mm-alpha-mass}{0.03 \pm 0.03}%
{se-mm-alpha-met}{-0.00 \pm 0.02}%
{se-mm-alpha-age}{0.00 \pm 0.00}%
{sn-mma-R0}{2.51 \pm 0.20}%
{sn-mma-alpha-mass}{0.26 \pm 0.11}%
{sn-mma-alpha-met}{-0.04 \pm 0.03}%
{sn-mma-alpha-age}{-0.01 \pm 0.03}%
{se-mma-R0}{1.36 \pm 0.16}%
{se-mma-alpha-mass}{0.10 \pm 0.11}%
{se-mma-alpha-met}{0.02 \pm 0.03}%
{se-mma-alpha-age}{0.02 \pm 0.02}%
}[XX]%
}
